Efficient Monitoring of Hyperproperties using Prefix Trees

Hyperproperties, such as non-interference and observational determinism, relate multiple computation traces with each other and are thus not monitorable by tools that consider computations in isolation. We present the monitoring approach implemented in the latest version of RVHyper, a runtime verification tool for hyperproperties. The input to the tool are specifications given in the temporal logic HyperLTL, which extends linear-time temporal logic (LTL) with trace quantifiers and trace variables. RVHyper processes execution traces sequentially until a violation of the specification is detected. In this case, a counter example, in the form of a set of traces, is returned. RVHyper employs a range of optimizations: a preprocessing analysis of the specification and a procedure that minimizes the traces that need to be stored during the monitoring process. In this article, we introduce a novel trace storage technique that arranges the traces in a tree-like structure to exploit partially equal traces. We evaluate RVhyper on existing benchmarks on secure information-flow control, error correcting codes and symmetry in hardware designs. As an example application outside of security, we show how RVHyper can be used to detect spurious dependencies in hardware designs.

==> encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> old/commands.tex <==

% Common math
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{{\langle #1 \rangle}}
\newcommand{\card}[1]{{|#1|}}
\newcommand{\ldot}{\mathpunct{.}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\dom}{\mathrm{dom}}

% Languages
\newcommand{\good}{\mathit{good}}
\newcommand{\bad}{\mathit{bad}}
\newcommand{\winning}{\mathit{winning}}
\newcommand{\losing}{\mathit{losing}}
\newcommand{\hlang}{\mathcal{H}}

% Complexity classes
\newcommand{\pspace}{\textsc{PSpace}}

% Logics
\newcommand{\ltl}{\text{LTL}}
\newcommand{\hyperltl}{\text{HyperLTL}}
\newcommand{\secltl}{\text{SecLTL}}


\newcommand{\lang}{\mathcal{L}}
\newcommand{\ap}{\text{AP}}
\renewcommand{\models}{\vDash}
\newcommand{\nmodels}{\nvDash}
\newcommand{\traces}{\mathit{TR}}

% Traces
\newcommand{\pref}{\preceq}
\newcommand{\tracebox}[1]{\framebox[4.5ex][l]{#1}}
\newcommand{\pctracebox}[1]{\framebox[4.5ex][l]{#1}}

% LTL
\newcommand{\U}{\Until}
\newcommand{\X}{\Next}
\newcommand{\G}{\Globally}
\newcommand{\F}{\Eventually}
\newcommand{\R}{\Release}
\newcommand{\W}{\WUntil}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

% HyperLTL
\newcommand{\pathassign}{\Pi}
\newcommand{\pathvars}{\mathcal{V}}
\newcommand{\pathassignfin}{\Pi_\mathit{fin}}

% Monitoring
\newcommand{\monitor}{\mathcal{M}}
\newcommand{\tool}{\text{RVHyper}}

% Tools
\newcommand{\eahyper}{\text{EAHyper}}

% TODOs and Marking
\newcommand{\todo}[1]{\marginpar{TODO}\textcolor{red}{#1}}
%\newcommand{\tbchecked}[1]{\marginpar{To be checked}\textcolor{blue}{#1}}

\newcommand{\ninfluences}{\not\leadsto}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> old/encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> old/encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> old/encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> old/encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> old/enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> old/enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> old/introduction.tex <==
%===============================================================================
\section{Introduction}
\label{sec:intro}
%===============================================================================

\emph{Hyperproperties}~\cite{journals/jcs/ClarksonS10} are widely studied in (but not limited to) the context of secure information-flow control. They generalize trace properties in that they not only check the correctness of \emph{individual} computation traces in isolation, but relate \emph{multiple} computation traces to each other.
%Hyperproperties are widely studied in the context of information-flow control.
%Information-flow policies cannot be monitored with standard runtime verification tools
Examples include information-flow policies, such as observational determinism~\cite{journals/jcs/McLean92,conf/sp/Roscoe95,conf/csfw/ZdancewicM03}, (quantitative) noninterference~\cite{journals/jcs/McLean92,DBLP:conf/fossacs/Smith09,DBLP:conf/esorics/YasuokaT10} as well as symmetry~\cite{conf/cav/FinkbeinerRS15} and spurious dependencies in hardware designs~\cite{conf/tacas/FinkbeinerHST18}, error correcting codes~\cite{conf/cav/FinkbeinerRS15}, and anti-doping of automotive software~\cite{conf/esop/DArgenioBBFH17}.
%The application of hyperproperties 

In this article, we present the monitoring approach implemented in the latest version of $\tool$, an automata-based monitoring tool for hyperproperties~\cite{journals/fmsd/FinkbeinerH19}.
In dynamic verification of hyperproperties, efficient and light-weight monitoring techniques are instrumented in systems, which are usually far beyond the scope of static verification approaches. By doing so, countermeasures are enacted before, for example, irreparable information leaks happen.
%
A runtime verification tool for hyperproperties is in particular useful if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
$\tool$ also supports the verification workflow by providing a method to test and develop specifications: Specifications can be checked on sample traces without the need for a complete model.
Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning.

%However, standard runtime verification tools~\todo{cite} that only consider computations in isolation, can, in general, not monitor such properties.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The input of $\tool$ is given in the temporal logic $\hyperltl$~\cite{conf/post/ClarksonFKMRS14}, which expresses temporal hyperproperties, by extending linear-time temporal logic with \emph{explicit} trace quantification (see~\cite{conf/lics/CoenenFHH19} for a recent study of hyperlogics).
HyperLTL has been used extensively to specify hyperproperties of practical interest (e.g~\cite{conf/cav/FinkbeinerRS15,journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18,conf/cav/FinkbeinerHT18,conf/cav/FinkbeinerHLST18,conf/esop/DArgenioBBFH17}).
For example, observational determinism is expressed as the following formula:
$$
\forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
$$
stating that every trace pair $\pi,\pi'$ has to agree on the output as long as they agree on the inputs as well.
%$\hyperltl$ has been used to specify a variety of information-flow and security properties~\todo{cite}.
When detecting a violation, $\tool$ outputs a counter example, which is a set of computations that does not satisfy the input formula.
%Examples include classical properties like non-interference and observational determinism, as well as quantitative information-flow properties, symmetries in hardware designs, and formally verified error correcting codes~\cite{conf/cav/FinkbeinerRS15}.

Efficient model checking, synthesis and satisfiability checking tools for HyperLTL already exist~\cite{conf/cav/FinkbeinerRS15,conf/cav/FinkbeinerHT18,conf/concur/FinkbeinerH16,DBLP:conf/atva/FinkbeinerHH18,conf/cav/FinkbeinerHS17,conf/cav/FinkbeinerHLST18}. Implementing an efficient runtime verification tool for HyperLTL specifications is, despite recent theoretical progress~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17,conf/csfw/BonakdarpourF18,conf/isola/BonakdarpourSS18,conf/tacas/HahnST19,journals/fmsd/FinkbeinerH19} difficult:
%
%This is because monitoring hyperproperties is difficult:
In principle, the monitor not only needs to process every observed trace, but must also \emph{store} every trace observed so far, so that future traces can be compared with the traces seen so far.
%On the other hand, a runtime verification tool for hyperproperties is certainly useful, in particular if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
%Furthermore, monitoring hyperproperties can be used to simulation plays a significant role in designing specifications and, for example, hardware.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The previous version of $\tool$ tackles this challenging problem by implementing two optimizations~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}: a \emph{specification analysis} to detect exploitable properties of a hyperproperty, such as \emph{symmetry} and a \emph{trace analysis}, which detects all redundant traces that can be omitted during the monitoring process. The trace analysis, which is based on a language inclusion check, can, however, only analyze and prune \emph{entire} traces.
For example, consider the traces $t_1 = \{a\}\{a\}\{\}$ and $t_2 = \{a\}\{\}\{a\}$ of length $3$ and the HyperLTL formula $\forall \pi. \forall \pi'. \G ( a_\pi \rightarrow \neg b_{\pi'} )$. Neither $t_1$ nor $t_2$ is dominated by the other trace, in the sense of the trace analysis, i.e., that one of the traces poses strictly less requirements on future traces~\cite{journals/fmsd/FinkbeinerH19}.
The traces, however, are equal on the first position.
% storage optimization technique that arranges the traces in a tree-like structure.
%This leaves room for optimization, which we address in this article.
This provides an opportunity for optimization, which our new approach exploits.
We introduce a novel trace storage technique (that also has massive impact on the running time), such that $\tool$ can also handle \emph{partially equal} traces by storing them in a tree structure.

We evaluate $\tool$ on existing benchmarks such as classical information-flow security by checking for violations of noninterference or monitoring error-resistant encoder. $\hyperltl$ is, however, not limited to security policies. As an example of such an application beyond security, we show how $\tool$ can be used to detect spurious dependencies in hardware designs.

\paragraph{Structure of this Article.}

The remainder of this article is structured as follows.
We begin by giving preliminaries on $\hyperltl$, its finite trace semantics and notation in Section~\ref{sec:prelims}. In Section~\ref{sec:rvhyper}, we present automata-based monitoring approach implemented in $\tool$, before discussing optimizations in Section~\ref{sec:opt} that make the monitoring feasible in practice. In Section~\ref{sec:eval}, we evaluate $\tool$ with a focus on the novel storage optimization technique using our tree data structure.%: we show $\tool$s performance on a benchmark

This is a revised and extended version of a paper that appeared at TACAS~2018~\cite{conf/tacas/FinkbeinerHST18}.
Our contribution and extension compared to~\cite{conf/tacas/FinkbeinerHST18} is the inclusion of a new trace storage optimization technique presented in Sec.~\ref{sec:trie} and an extended evaluation in Sec.~\ref{sec:eval}.

\paragraph{Related Work.}

The temporal logic $\hyperltl$ was introduced to model check security properties of reactive systems~\cite{conf/post/ClarksonFKMRS14,conf/cav/FinkbeinerRS15}.
For one of its predecessors, $\secltl$~\cite{conf/vmcai/DimitrovaFKRS12}, there has been a proposal for a white box monitoring approach~\cite{conf/isola/DimitrovaFR12} based on alternating automata.
The problem of monitoring $\hyperltl$ has been considered before~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17}.
Agrawal and Bonakdarpour~\cite{conf/csfw/AgrawalB16} were the first to study the monitoring problem of HyperLTL for the sequential model. They gave a syntactic characterization of monitorable $\hyperltl$ formulas. They present a first monitoring algorithm based on a progression logic expressing trace interdependencies and the composition of an LTL$_3$ monitor.
A first constraint-based approach has been outlined in~\cite{conf/tacas/BrettSB17}, which works for a subclass of HyperLTL specifications. The idea is to identify a set of propositions of interest and store corresponding constraints.
A constraint-based algorithm for the complete fragment of $\forall^2$ HyperLTL formulas has been proposed in~\cite{conf/tacas/HahnST19}. The algorithms rewrites a HyperLTL formula and an incoming event into a constraint composed of a plain LTL requirement as well as a HyperLTL requirement.
An constraint system is built incrementally: the HyperLTL part is encoded with variables, which will be incrementally defined with more incoming events of a trace.
Like with our monitoring algorithm, they do not have access to the implementation (black box), but in contrast to our work, they do not provide witnessing traces as a monitor verdict.

In~\cite{conf/csfw/BonakdarpourF18}, the authors study the complexity of monitoring hyperproperties. They show that the form and size of the input, as well as the formula have a significant impact on the feasibility of the monitoring process. They differentiate between several input forms and study their complexity: a set of linear traces, tree-shaped Kripke structures, and acyclic Kripke structures. For acyclic structures and alternation-free HyperLTL formulas, the problems complexity gets as low as NC.
In~\cite{conf/isola/BonakdarpourSS18}, the authors discuss examples where static analysis can be combined with runtime verification techniques to monitor HyperLTL formulas beyond the alternation-free fragment. They discuss the challenges in monitoring formulas beyond this fragment and lay the foundations towards a general method.

For certain information flow policies, like non-interference and some extensions, dynamic enforcement mechanisms have been proposed.
Techniques for the enforcement of information flow policies include tracking dependencies at the hardware level~\cite{conf/asplos/SuhLZD04}, language-based monitors~\cite{journals/jsac/SabelfeldM03,conf/csfw/AskarovS09,conf/pldi/AustinF10,conf/csfw/VanhoefGDPR14,conf/post/BichhawatRGH14}, and abstraction-based dependency tracking~\cite{conf/asian/GuernicBJS06,conf/essos/KovacsS12,conf/csfw/ChudnovKN14}.
Secure multi-execution~\cite{conf/sp/DevrieseP10} is a technique that can enforce non-interference by executing a program multiple times in different security levels.
% and by using special rules for I/O operations.
To enforce non-interference, the inputs are replaced by default values whenever a program tries to read from a higher security level.
%In this article, we are concerned with the monitorability of hyperproperties expressed in $\hyperltl$, which is able to formalize security properties beyond non-interference.

==> old/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> old/mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> old/mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> old/mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> old/mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> old/mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> old/preliminaries.tex <==
%===============================================================================
\section{Preliminaries}
%===============================================================================
\label{sec:prelims}
Let $\mathit{AP}$ be a finite set of \emph{atomic propositions} and let $\Sigma = 2^\mathit{AP}$ be the corresponding \emph{alphabet}.
An infinite \emph{trace} $t \in  \Sigma^\omega$ is an infinite sequence over the alphabet.
A subset $T \subseteq \Sigma^\omega$ is called a \emph{trace property}. A \emph{hyperproperty} $H \subseteq 2^{(\Sigma^\omega)}$ is a generalization of a trace property.
A finite trace $t \in \Sigma^+$ is a finite sequence over $\Sigma$.
In the case of finite traces, $|t|$ denotes the length of a trace.
%Depending on the context, we refer to either $(2^\mathit{AP})^\omega$ or $(2^\mathit{AP})^+$ as the alphabet $\Sigma^\omega$ or $\Sigma^+$.
We use the following notation to access and manipulate traces:
Let $t$ be a trace and $i$ be a natural number.
$t[i]$ denotes the $i$-th element of $t$.
Therefore, $t[0]$ represents the first element of the trace.
Let $j$ be natural number. If $j \geq i$ and $i\leq|t|$, then
$t[i,j]$ denotes the sequence $t[i] t[i+1] \cdots t[min(j,|t|-1)]$. Otherwise it denotes the empty trace $\epsilon$.
$t[i\rangle$ denotes the suffix of $t$ starting at position $i$.
For two finite traces $s$ and $t$, we denote their concatenation by $s \cdot t$.

%\subsection{LTL}
%\paragraph{Syntax.} Linear-time Temporal Logic (LTL)~\cite{} combines the usual Boolean connectives with temporal modalities.
%\begin{alignat*}{3}
%\varphi \coloneqq ~ a ~ | ~ \neg \varphi ~ | ~ \varphi \vee \varphi ~ | ~ \LTLnext \varphi ~ | ~ \varphi \LTLuntil \varphi
%\end{alignat*}
%where $a \in \mathit{AP}$ is an atomic proposition. We use the standard derived operators \emph{eventually} $\LTLdiamond \varphi \equiv \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \equiv \neg \LTLdiamond \neg \varphi$, \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \equiv (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \varphi_1 \LTLweakuntil (\varphi_1 \wedge \varphi_2)$.
%\paragraph{Semantics.} Let $a \in \mathit{AP}$ and $t \in \Sigma^\omega$. The semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\vDash_{LTL} a \quad &&\text{iff } a \in t[0] \\
%t &\vDash_{LTL} \psi_1 \vee \psi_2 \quad &&\text{iff } t \vDash \psi_1 \vee t \models_{LTL} \psi_2\\
%t &\vDash_{LTL} \neg \psi \quad &&\text{iff } t \not \models_{LTL} \psi\\
%t &\models_{LTL} \LTLnext \psi \quad &&\text{iff } t[1\rangle \models_{LTL} \psi\\
%t &\vDash_{LTL} \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; t[i\rangle \models_{LTL} \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \models_{LTL}\psi_1
%\end{alignat*}
%\paragraph{Finite trace Semantics.} Let $a \in \mathit{AP}$ and let $t \in \Sigma^+$ be a finite trace. The finite trace semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\modelsltlfin a \quad &&\text{iff } a \in t[0] \\
%t &\modelsltlfin \psi_1 \lor \psi_2 \quad &&\text{iff } t \modelsltlfin \psi_1 \text{ or } t \modelsltlfin \psi_2\\
%t &\modelsltlfin \neg \psi \quad &&\text{iff } t \not \modelsltlfin \psi\\
%t &\modelsltlfin \LTLnext \psi \quad &&\text{iff } |t| > 1 \text{ and } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \LTLweaknext \psi \quad &&\text{iff } |t| = 1 \text{ or } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \modelsltlfin \psi_1\\
%t &\modelsltlfin \psi_1 \LTLrelease \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_1\\
%& &&\text{ and for all } 0 \leq j \leq i \text{ we have } t[j\rangle \modelsltlfin \psi_2\\
%& &&\text{ or for all } 0 \leq i < |t| \text{ we have } t[i\rangle \modelsltlfin \psi_2\\
%\end{alignat*}~\todo{finite trace semantics bauen die wir brauchen}


%-------------------------------------------------------------------------------
%\subsection{HyperLTL}
%-------------------------------------------------------------------------------

\paragraph{HyperLTL Syntax.}\label{thltl:syntax}
HyperLTL~\cite{conf/post/ClarksonFKMRS14} extends LTL with trace variables and trace quantifiers.
Let $\mathcal{V}$ be a finite set of trace variables.
The syntax of HyperLTL is given by the grammar
%\begin{figure}[h!]
\begin{alignat*}{3}
  \varphi  &{}\coloneqq ~ \forall \pi . \; \varphi \mid \exists \pi . \; \varphi \mid \psi  \\
  \psi &{}\coloneqq ~ a_{\pi} \mid \psi \wedge \psi \mid \neg \psi \mid \LTLnext \psi  \mid \psi \; \LTLuntil \;  \psi \enspace ,
\end{alignat*}
where $a \in \mathit{AP}$ is an atomic proposition and $\pi \in \mathcal{V}$ is a trace variable.
Atomic propositions are indexed by trace variables. The explicit trace quantification enables us to express properties like ``on all traces $\varphi$ must hold'', expressed by $\forall \pi \ldot \varphi$. Dually, we can express ``there exists a trace such that $\varphi$ holds'', expressed by $\exists \pi \ldot \varphi$.
We use the standard derived operators \emph{release} $\varphi \LTLrelease \psi \coloneqq \neg(\neg \varphi \LTLuntil \neg\psi)$, \emph{eventually} $\LTLdiamond \varphi \coloneqq \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \coloneqq \neg \LTLdiamond \neg \varphi$, and \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \coloneqq (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$.
As we use the finite trace semantics, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to false.
To enable duality in the finite trace setting, we additionally use the \emph{weak} next operator $\LTLweaknext \varphi$ which evaluates to true if a trace ends before the satisfaction of $\varphi$ can be determined and is defined as $\LTLweaknext \varphi \coloneqq \neg \LTLnext \neg \varphi$.
%$\LTLuntil$ denotes the \emph{until}-operator, $\LTLrelease$ the \emph{release}-operator, and we distinguish between a weak and a strong next operator, where $\LTLweaknext \varphi$ denotes the \emph{weak} version, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to true. In contrast, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator.
%$\LTLdiamond$ means that $\varphi$ holds eventually in the future, $\LTLsquare$ means that $\varphi$ holds globally, and $\LTLweakuntil$ is the \emph{weak} version of the \emph{until} operator.
%We call a HyperLTL formula alternation-free, if either all trace variables are universally quantified or all trace variables are existentially quantified.
%, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \neg (\neg\varphi_1 \LTLuntil \neg \varphi_2)$.
We call $\psi$ of a HyperLTL formula $\vec{Q}. \psi$, with an arbitrary quantifier prefix $\vec{Q}$, the \emph{body} of the formula. A HyperLTL formula $\vec{Q}. \psi$ is in the \emph{alternation-free fragment} if either $\vec{Q}$ consists solely of universal quantifiers or solely of existential quantifiers.
%We also call the $\forall^n$ fragment and $\exists^n$ fragment, with $n$ being a natural number, as the respective alternation-free fragments.
We also denote the respective alternation-free fragments as the $\forall^n$ fragment and the $\exists^n$ fragment, with $n$ being the number of quantifiers in the prefix.

%\paragraph{Semantics}\label{thltl:sem}
%%Similar to \HLTL{}, \THLTL{} defines the semantics over a set $T$ of traces.
%A HyperLTL formula can express hyperproperties.
%A trace set $T$ satisfies the hyperproperty $H$ if $T \in H$.
%The semantics of HyperLTL is formally defined over a trace assignment, which is a partial mapping $\Pi: \mathcal{V} \to T$ from trace variables to  traces.
%We write $\Pi[\pi \mapsto t]$ for the updated trace assignment, where $\pi \text{ is mapped to } t$.
%$\Pi[i\rangle$ denotes the trace assignment that is equal to $\Pi(\pi)[i\rangle$ for all $\pi \in \dom(\Pi)$.
%We write the trace set $T$ as subscript since the satisfaction depends on the trace mapping.
%%For the sake of decidability, we assume that $x < y$.
%The satisfaction of a HyperLTL formula $\varphi$ over a trace assignment $\Pi$ and a set of traces $T$, denoted by $\Pi \models_T \varphi$, is defined as follows:
%\begin{alignat*}{2}
%\Pi &\vDash_T a_{\pi} \quad &&\text{iff } a \in \Pi(\pi)[0] \\
%\Pi &\vDash_T \psi_1 \wedge \psi_2 \quad &&\text{iff } \Pi \vDash_T \psi_1 \wedge \Pi \vDash_T \psi_2\\
%\Pi &\vDash_T \neg \psi \quad &&\text{iff } \Pi \nvDash_T \psi\\
%\Pi &\vDash_T \forall \pi. \; \psi \quad &&\text{iff } \forall t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\vDash_T \exists \pi. \; \psi \quad &&\text{iff } \exists t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\models_T \LTLnext \psi \quad &&\text{iff } \Pi[1\rangle \models_T \psi\\
%\Pi &\vDash_T \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; \Pi[i\rangle \models_T \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } \Pi[j\rangle \models_T \psi_1
%\end{alignat*}
%We say a trace set T satisfies a HyperLTL formula $\varphi$ if $\emptyset \models_T \varphi$.
%If unambiguously deducible from the context, we omit $T$ and just write $\models$ instead of $\models_T$.

\paragraph{Finite Trace Semantics.}
We recap the finite trace semantics for HyperLTL~\cite{conf/tacas/BrettSB17} which is itself based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029}.
% and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029} and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a HyperLTL formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
%Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^+$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i\rangle$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i\rangle$ for all $\pi \in \dom(\pathassignfin)$.
By slight abuse of notation, we write $t \in \pathassignfin$ to access traces $t$ in the image of $\pathassignfin$.
%
The satisfaction of a HyperLTL formula $\varphi$ over a finite trace assignment $\pathassignfin$ and a set of finite traces $T$, denoted by $\pathassignfin \models_T \varphi$, is defined as follows:%~\todo{define min t in Pi fin}:
\begin{equation*}
\begin{array}{ll}
    \pathassignfin \models_T a_\pi         \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
    \pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
    \pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
    \pathassignfin \models_T \LTLnext \varphi          & \text{if } \forall t \in \pathassignfin \ldot |t|>1 \text{ and } \pathassignfin[1\rangle \models_T \varphi \\
%    \pathassignfin \models_T \LTLweaknext \varphi      & \text{if } \pathassignfin \models_T \LTLnext \varphi \\
%    & \text{or } \exists t \in \pathassignfin \text{ with } |t| \leq 1 \\
    \pathassignfin \models_T \varphi\LTLuntil\psi      & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \psi \\
    &~\hspace{1ex} \land \forall j < i \ldot \pathassignfin[j\rangle \models_T \varphi \\
%    \pathassignfin \models_T \varphi\LTLrelease\psi    & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \varphi \land \forall j \leq i \ldot \pathassignfin[j\rangle \models_T \psi \\
%   & \text{or } \forall j \leq \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[j\rangle \models_T \varphi\\
    \pathassignfin \models_T \exists \pi \ldot \varphi & \text{if } \exists t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi \\
    \pathassignfin \models_T \forall \pi \ldot \varphi & \text{if } \forall t \in T \text{ holds that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%\subsection{$\forall^2 \hyperltl$}
%As our constraint based monitoring approach will only be concerned with $\forall^2 \hyperltl$ formulas, we introduce special notation, which will help us down the road.
%\begin{definition}
%
The hyperproperty represented by a $\hyperltl$ formula $\varphi$, denoted by $\hlang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%Due to duality of $\LTLuntil$/$\LTLrelease$, $\LTLnext$/$\LTLweaknext$, $\exists$/$\forall$, and the standard Boolean operators, every HyperLTL formula $\varphi$ can be transformed into negation normal form~(NNF), i.e., for every $\varphi$ there is some $\psi$ in negation normal form such that for all $\pathassignfin$ and $T$ it holds that $\pathassignfin \models_T \varphi$ if, and only if, $\pathassignfin \models_T \psi$.
%
%The standard LTL semantic, written $t \modelsltlfin \varphi$, for some LTL formula $\varphi$ is equal to $\set{ \pi \mapsto t }_\mathit{fin} \models_\emptyset \varphi'$, where $\varphi'$ is derived from $\varphi$ by replacing every proposition $p \in \mathit{AP}$ by $p_\pi$.


==> old/runtime-verification.tex <==
%===============================================================================
\section{Runtime Verification of Hyperproperties with $\tool$}
%===============================================================================
\label{sec:rvhyper}
%Since Hyperproperties relate multiple system executions to each other, $\tool$ necessarily processes (and stores) multiple runs of a system.
%For example, previous recorded sessions in a dating app or recorded daily behavior of a smart home.
%Monitoring a system against hyperproperties, such as information-flow policies, is essential if a user suspects that private information might be inferred from notwithstanding behavior of a single system run. For example, \emph{observational determinism} is a general information-flow policy that can be monitored with $\tool$. It states that low-security outputs may not depend on high-security inputs.
In this section, we present an overview over $\tool$, before describing the implementation setup, present the monitoring algorithm, and discuss our optimization techniques.

The input of $\tool$ is given as a universally quantified HyperLTL formula and, in addition, the observed behavior of the system under consideration.
The observed behavior is represented as a trace set $T$, where each $t \in T$ represents a previously observed execution of the system to monitor.
%
$\tool$ can therefore detect violations of every monitorable $k$-safety hyperproperty (see~\cite{journals/fmsd/FinkbeinerH19} for an extensive study of monitorability of hyperproperties).
If $\tool$ detects that the system violates the hyperproperty, it outputs a counter example, i.e, a $k$-ary tuple of traces, where $k$ is the number of quantifiers in the HyperLTL formula.
%that make the monitoring of hyperproperties (despite its theoretical unbounded memory consumption) feasible in practice.
%\subsection{Specification}
%The input specification of $\tool$ is given in $\hyperltl$, which is a temporal logic for specifying hyperproperties.
%It extends $\ltl$ by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
%The set of trace variables is $\pathvars$.
%Formulas in $\hyperltl$ are given by the grammar
%\begin{align*}
%\varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
%\psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
%\end{align*}
%where $a \in \ap$ and $\pi \in \pathvars$.
%%
%%The formal semantics is given in Appendix~\ref{appendix:hyperltl}.
%The finite trace semantics for $\hyperltl$ is based on the finite trace semantics of LTL.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
%Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
%$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
%\[
%t[i,j] = \begin{cases}
%\epsilon & \text{if } i \geq |t|\\
%t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
%\end{cases}
%\]
%\begin{equation*}
%\begin{array}{ll}
%\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
%\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
%\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
%\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
%\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
%\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
%\end{array}
%\end{equation*}
%For example, above mentioned observational determinism can be formalized as the HyperLTL formula
%$\forall \pi \ldot \forall \pi' \ldot (O_\pi = O_{\pi'}) \WUntil (I_\pi \not = I_{\pi'})$, where $\WUntil$ is the weak version of $\Until$.
%
%While earlier work on $\hyperltl$~\cite{conf/cav/FinkbeinerRS15} has focused on model checking, recently runtime verification methods have been proposed as a complementation~\cite{conf/csfw/AgrawalB16,conf/rv/FinkbeinerHST17}.
%$\tool$ also supports the verification workflow by providing a method to test and develop $\hyperltl$ specifications: Specifications can be checked on sample traces without the need for a complete model.
%Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning~\todo{passt hier nicht?}.

\subsection{Implementation Details}
$\tool$\footnote{The implementation is available at \url{https://react.uni-saarland.de/tools/rvhyper/}.} is written in C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}.
It uses \emph{spot}~\cite{duret.16.atva2} for building the deterministic monitor automata and the \emph{Buddy} BDD library for handling symbolic constraints.
We use the $\hyperltl$ satisfiability solver $\eahyper$~\cite{conf/cav/FinkbeinerHS17,conf/concur/FinkbeinerH16} to determine whether the input formula is reflexive, symmetric, or transitive.
Depending on those results, we omit redundant tuples in the monitoring algorithm.

%-------------------------------------------------------------------------------
\subsection{Online Monitoring Algorithm}
%-------------------------------------------------------------------------------

For the online algorithm, we use standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.
Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0, F)$ is a tuple of
a finite alphabet $\Sigma = 2^{(\ap \times \pathvars)}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \hookrightarrow Q$,
a designated initial state $q_0 \in Q$, and
a set of accepting states $F \subseteq Q$.
The instantiated automaton runs in parallel over traces in $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
\delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted, if there is a run on $\monitor$ that ends in an accepting state.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over trace variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}  \label{ex:obsdet-monitor}
  As an example formula, consider again the observational determinism formula introduced in the introduction:
  \begin{equation*}
    \forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
  \end{equation*}
  The corresponding monitor template is depicted in Fig.~\ref{fig:monitor-template}.
\end{example}
\begin{figure}[t]
	\centering
 \begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.9]
 \node[state,initial,initial text=,accepting] (init) {$q_0$};
 \node[state,below left=1.3 and 1.5 of init,accepting] (accepting) {$q_\top$};
 \node[state,black!50,below right=1.3 and 1.5 of init] (rejecting) {$q_\bot$};
 
 \draw (init) edge[loop right] node[swap] {$o_\pi = o_{\pi'} \land i_\pi = i_{\pi'}$} ()
       (init) edge node {$i_\pi \neq i_{\pi'}$} (accepting)
       (init) edge[black!50] node[near end] {$o_\pi \neq o_{\pi'} \land i_\pi = i_{\pi'}$} (rejecting)
       (accepting) edge[loop right] node {$\top$} (accepting)
       (rejecting) edge[loop right,black!50] node {$\top$} (rejecting)
 ;
 \end{tikzpicture}
	\caption{Visualization of a monitor template corresponding to the formula given in Example~\ref{ex:obsdet-monitor}. We use a symbolic representation of the transition function $\delta$. For illustration reasons, we depict a sink rejecting state $q_\bot$.}
	\label{fig:monitor-template}
\end{figure}

%\paragraph{Online Algorithm.}~\todo{adept arbitarily formulas}
The algorithm for monitoring $\hyperltl$ formulas when traces are given sequentially to the monitor is presented in Algorithm~\ref{alg:algorithms-sequential}.
%The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, the algorithm accepts new traces and afterwards proceeds with the pace of the incoming stream.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever the current trace $t$ progresses, we progress every tuple $(t_1,\ldots,t_n)$ that contains $t$ with one of the following outcomes:
\begin{enumerate}
  \item One of the traces $t_1,\ldots,t_n$ may have ended, thus, we check if the monitor is in an accepting state and report a violation if this is not the case.
  \item There is a successor state in the monitor, thus we update $S$.
  \item There is no successor state, hence, we report a violation.
\end{enumerate}
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $\vec{t} \in (T \cup \set{t})^n$ containing the new trace $t$.%~\todo{explain notion of instantiation?}
			\begin{algorithm*}[t]
				\SetKwInOut{Input}{input}
				\SetKwInOut{Output}{output}
				\SetAlgoLined
				%\KwResult{Write here the result }
				\Input{$\forall^n$ HyperLTL formula $\varphi$}
				\Output{satisfied or $n$-ary tuple witnessing violation}
				\BlankLine
				$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
				$T \gets \emptyset$\;
				$S: T^n \rightarrow Q$ \quad // initially empty\;
				$t$  \quad // container for the subsequently incoming event traces
				\BlankLine
				\While{there is a new event trace}{
                  $t \gets \epsilon$ \quad // initialize empty trace\;
                  \For(init $S$ for every new tuple $\vec{t}$){$\vec{t} \in ((T \cup \set{t})^n \setminus T^n)$}{
    				$S(\vec{t}) \gets q_0$\;
    			  }
                  \While{$p \in \Sigma$ is a new input event}{
						$t' \gets t~p$ \quad // append $p$ to $t$\;
                        \For(// progress every state in $S$) {$( (t_1,\ldots,t_n), q) \in S$ where $t \in \{t_1,\ldots,t_n\}$}{
                            \uIf(// some trace ended){$\exists t^* \in \{t_1,\ldots,t_n\} \ldot \card{t^*} < \card{t}$}{
                             \eIf {$q \in F$} {
                              remove $(t_1,\ldots,t_n)$ from $S$\;
                              \textbf{continue}\;
                             } { \Return violation and witnessing tuple $(t_1,\ldots,t_n)$\;}
                          }
                          $\vec{t} \gets (t_1,\ldots,t_n)$, where $t_i$ is replaced with $t'$, for each $t_i = t$\;
                          \uIf {$\delta(q, \bigcup_{i=1}^n \bigcup_{a \in \vec{t}(i)[\card{t'}-1]} \set{ (a, \pi_i) }) = q'$} {
        				     $S(\vec{t}) \gets q'$\;
        				  }
        				  \Else{
        				    \Return violation and witnessing tuple $\vec{t}$\;
        				  }
        				}
						$t \gets t'$ \quad // re-assign $t$\;
				  } 
				  $T \gets T \cup \set{t}$\; \quad //add $t$ to already seen traces
				}
				\Return satisfied\;
				\BlankLine
	\caption{Online monitoring algorithm for $\forall^n \hyperltl$: The algorithm subsequently reads event traces and monitors them against already seen traces. Already seen traces are stored in $T$ before continuing with a new event trace.}
	\label{alg:algorithms-sequential}
			\end{algorithm*}

\begin{example} \label{ex:obsdet-algorithm}
  We continue \autoref{ex:obsdet-monitor} by showing how the algorithm progresses on the given formula.
  Assume for the sake of readability that we have a single input proposition $i$ and a single output proposition $o$.
  Furthermore, assume that we have already seen the trace $t_0 = \set{i}\set{i,o}\set{o}$, that is, $T = \set{t_0}$ and $S(t_0,t_0) = q_0$.
  We now show how the algorithm continues with a fresh trace $t_1$.
  In lines 6--8 we add the pairs $(t_0,t_1)$, $(t_0,t_1)$, and $(t_1,t_1)$ with the initial state $q_0$ to $S$.
  Let $p = \set{i}$ be the first input proposition, thus, $t_1 = \set{i}$.
  Since $t_0[0] = t_1[0]$, the monitor remains in $q_0$ for every tuple.
  Let $p = \set{i}$ be the next input proposition, thus, $t_1 = \set{i}\set{i}$.
  Consider the tuple $(t_0,t_1)$.
  As $t_0[1]$ and $t_1[1]$ are equal with respect to $i$ but differ in $o$, the monitor progresses to the rejecting state $q_\bot$ and the algorithm terminates by reporting the violation.
  If, the previous input proposition is $p = \set{}$, both tuples, $(t_0,t_1)$ and $(t_1,t_0)$ would progress to the accepting sink state $q_\top$ as the input proposition is different to $t_0[1]$.
  Assume two more inputs, e.g., $t_1 = \set{i}\set{i}\set{}\set{}$, then the pairs $(t_0,t_0)$, $(t_0,t_1)$, and $(t_1,t_0)$ are removed from $S$ as $t_1$ is strict longer than $t_0$.
\end{example}


\section{Optimizations}
\label{sec:opt}
In this section, we present three optimizations implemented in $\tool$, which, as we will see in the evaluation section, are necessary to make the automata-based monitoring approach feasible in practice. We begin by explaining a \emph{specification analysis}, which is a preprocessing step that exploits properties of the specification to reduce the algorithmic workload. In the subsequent section, we show how $\tool$ tackles the problem of potentially unbounded memory consumption: We recap the \emph{trace analysis}, which was so far the only storage optimization implemented in $\tool$. We then provide a novel storage optimization technique based on prefix-trees, so-called \emph{tries}, to exploit partial equality of the given traces, which the trace analysis neglected so far.
%-------------------------------------------------------------------------------
\subsection{Decreasing Running Time}
%-------------------------------------------------------------------------------

In the example execution in \autoref{ex:obsdet-algorithm} we have seen that the algorithm had to do more work than necessary to monitor observational determinism.
For example, a tuple $(t,t)$ for some trace $t$ cannot violate observational determinism as the traces are equal.
Further, from the pairs $(t,t')$ and $(t',t)$ for some traces $t$ and $t'$, we only need to check one of them as a violation in one of them implies the violation in the other pair.
We can automatically check for such conditions and, thus, omit unnecessary work.

$\tool$ utilizes the HyperLTL satisfiability solver EAHyper~\cite{conf/concur/FinkbeinerH16,conf/cav/FinkbeinerHS17} for its \emph{specification analysis}, which is a preprocessing step that analyzes the HyperLTL formula under consideration.
EAHyper can detect whether a formula is (1) \emph{symmetric}, i.e., we halve the number of instantiated monitors, (2) \emph{transitive}, i.e, we reduce the number of instantiated monitors to two, or (3) \emph{reflexive}, i.e., we can omit the self comparison of traces.

\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:symmetry}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	%Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_n \ldot \psi$, where $\psi$ is an $\ltl$ formula over trace variables $\{\pi_1, \dots, \pi_n\}$.
	%For an assignment $\pathassign$ and an permutation $\sigma : \Pi \to \Pi$, we define $\pathassign \circ \sigma$, such that $(\pathassign \circ \sigma)(\pi) = \pathassign(\sigma(\pi))$ for every $\pi \in \Pi$.
	We say $\varphi$ is invariant under trace variable permutation $\sigma : \pathvars \to \pathvars$, if for any set of traces $T \subseteq \Sigma^{\omega}$ and any assignment $\pathassign : \pathvars \to T$, $(\emptyset, \pathassign, 0) \models \psi \Leftrightarrow (\emptyset, \pathassign \circ \sigma, 0) \models \psi$.
	We say $\varphi$ is symmetric, if it is invariant under every trace variable permutation in $\pathvars$.
\end{definition}
Symmetry is particular interesting since many information flow policies satisfy this property. Consider, for example, observational determinism: 
$
\forall \pi\ldot \forall \pi'\ldot (o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'}).
$ %\todo{different notation than in \autoref{ex:obsdet-algorithm} and intro.}
$\tool$ detects symmetry by translating this formula to a formula that is unsatisfiable if there exists no set of traces for which every trace pair violates the symmetry condition:
$
\exists \pi\ldot \exists \pi'\ldot \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big) \nleftrightarrow \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big)
$.
If the resulting formula turns out to be unsatisfiable, $\tool$ omits the symmetric instantiations of the monitor automaton.
%, which turns out to be, especially in combination with $\tool$s \emph{trace analysis}, a major optimization in practice~\cite{conf/rv/FinkbeinerHST17}.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:transitivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\set{\pi_1, \pi_2}$.
	Let $T = \set{t_1, t_2, t_3} \in \Sigma^{\omega}$ be a three-elemented set of traces.
	We define the assignment $\pathassign_{i,j} : \pathvars \to \Sigma^{\omega}$ by $\pathassign_{i,j} \coloneqq \{\pi_1 \mapsto t_i, \pi_2 \mapsto t_j\}$.
	We say $\varphi$ is transitive, if for all three-elemented sets $T$ it holds that $(\emptyset, \pathassign_{1,2}, 0) \models \psi \wedge (\emptyset, \pathassign_{2,3}, 0) \models \psi \rightarrow (\emptyset, \pathassign_{1,3}, 0) \models \psi$.
\end{definition}
While symmetric HyperLTL formulas allow us to prune half of the monitor instances, transitivity of a HyperLTL formula has an even larger impact on the required memory. Equality, i.e, $\forall \pi. \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$, for example, is transitive and symmetric and allows us to reduce the number of monitor instances to one, since we can check equality against any reference trace.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:reflexivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	We say $\varphi$ is reflexive, if for any trace $t \in \Sigma^{\omega}$ and the corresponding assignment $\pathassign : \pathvars \to \{t\}$, $(\emptyset, \pathassign, 0) \models \psi$.
\end{definition}
Lastly, if a formula is reflexive, $\tool$ omits the composition of a trace with itself during the monitoring process.
%Both $\hyperltl$ formulas considered in this section, $\mathit{ObsDet}$ and $\mathit{EQ}$, are reflexive.
For example, equality and observational determinism have reflexive HyperLTL formulas.

\begin{example}
  Consider again the observational determinism formula from \autoref{ex:obsdet-monitor}.
  We have seen that this formula is both, reflexive and symmetric, thus, we can omit those instances in the algorithm.  
\end{example}


%-------------------------------------------------------------------------------
\subsection{Optimizing Trace Storage}
\label{sec:trie}
%-------------------------------------------------------------------------------

The main obstacle in monitoring hyperproperties is the potentially unbounded space consumption.
So far, RVHyper employed a \emph{trace analysis} technique to detect redundant traces, with respect to a given HyperLTL formula, i.e., traces that can be safely discarded without losing any information and without losing the ability to return a counter example.

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given a HyperLTL formula $\varphi$, a trace set $T$ and an arbitrary $t \in \traces$, we say that $t$ is $(T,\varphi)$-redundant if $T$ is a model of $\varphi$ if and only if $T \cup \set{t}$ is a model of $\varphi$ as well, formally
	\begin{equation*}
	\forall T' \supseteq T \ldot T' \in \hlang(\varphi) \Leftrightarrow T' \cup \{t\} \in \hlang(\varphi) \enspace.
	\end{equation*}
\end{definition}

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given $t,t' \in \Sigma^\omega$, we say $t$ \emph{dominates} $t'$ with respect to $\varphi$ (or simply $t$ \emph{dominates} $t'$ if it is clear from the context) if $t'$ is ($\{t\},\varphi$)-redundant.
\end{definition}

\begin{example}
  For observational determinism, a trace $t$ is dominated by a trace $t'$ if $\card{t} < \card{t'}$ and both traces agree on the input propositions.
\end{example}


This is efficiently implemented in $\tool$ (cf. Algorithm~\ref{alg:traceopti}) and is guaranteed to catch all redundant traces.
In our experiments~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.

The trace analysis, as it is based on a language inclusion check of the entire traces, cannot handle \emph{partial redundancy}, for example, in the case that traces have redundant prefix requirements.
This leaves room for optimization, which we address by implementing a so-called \emph{trie} data structure for managing the storage of incoming traces.

\begin{algorithm}
	%\label{alg_minimization}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\hyperltl$ formula $\varphi$, redundancy free trace set $T$, fresh trace $t$}
	\Output{redundancy free set of traces $T_\mathit{min} \subseteq T \cup \set{t}$}
	%\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}
	\BlankLine
	\ForEach{$t' \in T$}{
		\If{ $t'$ dominates $t$ }
		{
			\Return $T$\;
		}
	}
	\ForEach{$t' \in T$}{
		\If{$t$ dominates $t'$}
		{
			$T \coloneqq T \setminus \set{t'}$\;
		}
	}
	\Return $T \cup \set{t}$\;
	%\BlankLine
	\caption{Trace analysis algorithm to minimize trace storage.}
	\label{alg:traceopti}
\end{algorithm}



%In our experiments~\cite{conf/rv/FinkbeinerHST17,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.
%Ideally one wants to avoid this overhead when monitoring a trace that shares some prefixes with already seen traces.
%We implemented this idea with a so-called \emph{trie} data structure.
Tries, also known as prefix trees, describe a tree data structure, which can represent a set of words over an alphabet in a compact manner.
The root of a trie is identified with the empty word $\epsilon$, additionally each node can have several child nodes, each of which corresponds to a unique letter getting appended to the representing word of the parent node. So the set of words of a trie is identified with the set of words the leaf nodes represent.

\begin{definition}
A trie is a four tuple $(\Sigma, \Tau, \longrightarrow, \tau_0)$ consisting of
\begin{itemize}
    \item a finite alphabet $\Sigma$,
    \item a non-empty set of states $\Tau$,
    \item a transition function $\longrightarrow: \Tau \times \Sigma \rightarrow \Tau$,
    \item and a designated initial state $\tau_0 \in \Tau$ called the root.
    \end{itemize}
\end{definition}
Instead of $((\tau,a),\tau') \in \longrightarrow$ we will write $\tau \overset{a}{\longrightarrow} \tau'$ in the following.
For a trie to be of valid form we restrict $\longrightarrow$ such that, $\forall \tau,\tau' \in \Tau. |\{\tau \overset{a}{\longrightarrow} \tau'| a \in \Sigma\}| \leq 1$.

%Additionally to our analysis phases it would be helpful if we could use some insights from trace analysis 


%As mentioned before, storing the incoming traces succinctly is a major concern in monitoring hyperproperties.
In our case the alphabet would be the set of propositions used in the specification, and the word built by the trie represents the traces. %build from it are what we call traces.
%Tries provide a 
Instead of storing each trace individually, we store all of them in one trie structure, branching only in case of deviation. This means equal prefixes only have to be stored once.
Besides the obvious benefits for memory, we also can make use of the maintained trie data structure to improve the runtime of our monitoring algorithms. As traces with same prefixes end up corresponding to the same path in the trie, we only have to instantiate the monitor automaton as much as the trie contains branches.
%O(size branches) times.
\begin{example}
	Consider the following traces of length $6$ over the alphabet $2^{\{i,o\}}$:
	\begin{itemize}
		\item
		$t_1: \{\set{i},\set{i,o},\set{i},\set{i},\set{i},\set{i,o} \}$
		\item
		$t_2: \{\set{i}, \set{i,o}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_3: \{\set{i}, \set{i}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_4: \{\set{i}, \set{i}, \set{}, \set{} , \set{}, \set{}\}$
	\end{itemize}
After processing the traces sequentially, the resulting trie looks as follows:

\vspace{1ex}

\begin{tikzpicture}[sibling distance=7em, level distance = 30pt,
every node/.style = {shape=circle,
	draw, align=center, minimum size = 0.9cm, inner sep = 0pt},
level 1/.style = {sibling distance = 10em},
level 2/.style = {sibling distance = 5em},
level 5/.style = {sibling distance = 5em}]
\node {$\{i\}$}
child { node {$\{i\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} } } } } 
	child { node {$\{ \}$}  
		child { node {$\{ \}$} 
			child { node {$\{ \}$}
				child { node {$\{ \}$} } } } } }
child { node {$\{i,o\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} }
				child { node {$\{i,o\}$} } } } } };
\end{tikzpicture}
\end{example}

\subsection{Trie-based Monitoring Algorithm}

We depict a trie-based offline monitoring algorithm in Fig.~\ref{alg:trie-offline}.
For the sake of readability, we assume that there are as many traces as universal quantifier, that we progress through all traces in parallel, and that all traces have the same length.
This is merely a simplification in the presentation, one can build the trie in a sequential fashion for online monitoring by a slight modification of the presented algorithm.

Without using tries our monitoring algorithm was based on instantiating the deterministic monitor template $\monitor_\varphi$ with tuples of traces. Now we instantiate $\monitor_\varphi$ with tuples of tries. Initially we only have to create the single instance having the the root of our trie.

\begin{comment}
	\begin{algorithm*}
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
		$S: \Tau^n \rightarrow Q$, \quad $E: \Tau^n \rightarrow \Sigma$\;
		$\tau_0 \coloneqq $\texttt{ new\_trie()}\;
		%$\mathbf{i} \coloneqq \underbrace{(\tau_0,\ldots,\tau_0)}{n \text{times}}$\;
		%$I \coloneqq \{\mathbf{i}\}$\;
		\BlankLine
		$i_0 \in \{ \tau_0 \}^n$\;
		$S(i_0) = q_0$\;
		\While{there is a new trace}{
			$I \leftarrow \{i_0\}$\;
			$\tau \leftarrow \tau_0$\;
			\While{$p \in \Sigma$ is a new event}{
				$\tau' \leftarrow$ \texttt{add\_child($\tau,p$)} //\texttt{assert($E(\tau')==p$)}\;
				$I_n \leftarrow \emptyset$\;
				\ForEach{$i \in I$}{
					$I' \leftarrow \{i' \mid i(j) \rightarrow i'(j), a \in \Sigma, 1 \leq j \leq n\}$\;
					$I' \leftarrow \{i' \in I' \mid \exists k. i'(k) = \tau'\}$\;
					\ForEach{$i' \in I'$}{
						\uIf{$\delta(S(i), \cup_{j=1}^n \cup_{a\in E(i'(j))} \{(a,\pi_j)\}) = q$}{
							$S(i') = q$\;
						}
						\Else{
							\Return(\texttt{rooted\_seq($i'(1)$)}, \ldots, \texttt{rooted\_seq($i'(n)$)})\;
						}
					}
				}
			}
		}
		%\While{$\mathbf{p} \leftarrow$ new elements (in a forward fashion)}{
		%	\For{$1 \leq j \leq n$}{
		%		$\mathbf{i}(j) \leftarrow $\texttt{add\_value($\mathbf{i}(j)$, $j$, $\mathbf{p}(j)$)}\;
		%	}
		%	$I \leftarrow \bigcup_{\mathbf{i} \in I} \{(i'_1,\ldots, i'_n)| \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n\}$\;
		%	\ForEach{$\mathbf{i} \in I$}{
		%		%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
		%		progress every state in $S$ according to $\delta$\;
		%		\If{violation in $M_\varphi$}{
		%			$t \coloneqq ($\texttt{rooted\_sequence($i(1)$)}$,\ldots,$\texttt{rooted\_sequence($i(n)$)}$)$\;
		%			\Return witnessing tuple $t^n$\;
		%		}
		%	}
		%}
		%\Return satisfied\;
		%\BlankLine
	\caption{Online algorithm using trie data structure.}
	\label{alg:trie-online-parallel}
	\end{algorithm*}
\end{comment}
	\begin{algorithm*}[t]
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\\
		$S: \Tau^n \rightarrow Q$\\
		$\tau_0 \coloneqq $\texttt{new\_trie()}\\
		$\mathbf{i} \coloneqq (\tau_0,\ldots,\tau_0) \in \Tau^n$\\
		$I \coloneqq \{\mathbf{i}\}$  \quad // set of not-yet terminated branches\\
		\BlankLine
		\While{$\mathbf{p} \leftarrow$ new event (in $\Sigma^n$)}{
			\For{$1 \leq j \leq n$}{
				$\mathbf{i}(j) \leftarrow $\texttt{add\_child($\mathbf{i}(j)$, $\mathbf{p}(j)$)} \quad // add child with value $\vec{p}(j)$ to $\vec{i}(j)$ if needed \\
			}
			// update set of active branches\\
			$I \leftarrow \bigcup_{\mathbf{i} \in I} \set{ (i'_1,\ldots, i'_n) \mid \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n }$\\
			\ForEach{$\mathbf{i} \in I$}{
				%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
				progress every state in $S$ according to $\delta$\;
				\If{violation in $\monitor_\varphi$}{
				    // return sequence from root to $\vec{i}$\\
					$t \gets ($\texttt{rooted\_sequence($\vec{i}(1)$)}$,\ldots,$\texttt{rooted\_sequence($\vec{i}(n)$)}$)$\\
					\Return witnessing tuple $t^n$\\
				}
			}
		}
		\Return satisfied if $\forall \vec{i} \in I \ldots S(\vec{i}) \in F$ else violation\\
		\BlankLine
	\caption{Offline algorithm using trie data structure.}
	\label{alg:trie-offline}
\end{algorithm*}

The trie-based algorithm has much in common with its previously discussed trace-based counterpart. Initially, we have to build the deterministic monitor automaton $\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F)$.
We instantiate the monitor with a fresh trie root $\tau_0$.
A mapping from trie instantiations to a state in $\monitor_\varphi$ $S: \Tau^n \rightarrow Q$, stores the current state of every active branch of the trie, stored in the set $I$.
For each of the incoming traces, we provide an entry in a tuple of tries $\mathbf{\tau}$, each entry gets initialized to $\tau_0$.
During the run of our algorithm these entries will get updated such that they always correspond to the word built by the traces up to this point.
For as long as there are traces left, which have not yet ended, and we have not yet detected a violation, we will proceed updating the entries in $\vec{i}$ as follows.
Having entry $\tau$ and the correspond trace sequence proceeds with $a$, if $\exists \tau' \in \Tau. \tau \overset{a}{\longrightarrow} \tau'$, we update the entry to $\tau'$ otherwise we create such a child node of $\tau$ (\texttt{add\_child} in line 8).
Creating a new node in the trie always occurs, if the prefix of the incoming trace starts to differ from already seen prefixes.
After having moved on step in our traces sequences, we have to reflect this step in our trie structure, in order for the trie-instantiated automata to correctly monitor the new propositions.
As a trie node can branch to multiple child nodes, each monitor instantiation will get replaced by the set of instantiations, where all possible child combinations of the different assigned tries are existent (update of $I$ in line 11).
Afterwards, we update $S$ in the same way as in Algorithm~\ref{alg:traceopti}, thus, we omit algorithmic details here.
%This can be efficiently implemented as we essential fork the monitor instantiation for the different branches in the trie.
%After this preprocessing we are able to update our mapping $S$ according to $\delta$.
If a violation is detected here, that is there is no transition in the monitor corresponding to $\vec{i}$, we will return the corresponding counter example as a tuple of traces, as those can get reconstructed by stepping upwards in the tries of $\vec{i}$.
%Note that the sequential algorithm is derived from the parallel one by progressing one trace at a time and additionally when forking the monitor instantiations, only those new instantiation have to be kept, which contain the (single) trie in $\mathbf{\tau}$ at least once. 
If the traces end, we check if every open branch $\vec{i} \in I$ is in an accepting state.

%\subsection{Tries and Trace Analysis in Combination}
%\todo{TODO}


==> old/submission 2/commands.tex <==

% Common math
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{{\langle #1 \rangle}}
\newcommand{\card}[1]{{|#1|}}
\newcommand{\ldot}{\mathpunct{.}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\dom}{\mathrm{dom}}

% Languages
\newcommand{\good}{\mathit{good}}
\newcommand{\bad}{\mathit{bad}}
\newcommand{\winning}{\mathit{winning}}
\newcommand{\losing}{\mathit{losing}}
\newcommand{\hlang}{\mathcal{H}}

% Complexity classes
\newcommand{\pspace}{\textsc{PSpace}}

% Logics
\newcommand{\ltl}{\text{LTL}}
\newcommand{\hyperltl}{\text{HyperLTL}}
\newcommand{\secltl}{\text{SecLTL}}


\newcommand{\lang}{\mathcal{L}}
\newcommand{\ap}{\text{AP}}
\renewcommand{\models}{\vDash}
\newcommand{\nmodels}{\nvDash}
\newcommand{\traces}{\mathit{TR}}

% Traces
\newcommand{\pref}{\preceq}
\newcommand{\tracebox}[1]{\framebox[4.5ex][l]{#1}}
\newcommand{\pctracebox}[1]{\framebox[4.5ex][l]{#1}}

% LTL
\newcommand{\U}{\Until}
\newcommand{\X}{\Next}
\newcommand{\G}{\Globally}
\newcommand{\F}{\Eventually}
\newcommand{\R}{\Release}
\newcommand{\W}{\WUntil}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

% HyperLTL
\newcommand{\pathassign}{\Pi}
\newcommand{\pathvars}{\mathcal{V}}
\newcommand{\pathassignfin}{\Pi_\mathit{fin}}

% Monitoring
\newcommand{\monitor}{\mathcal{M}}
\newcommand{\tool}{\text{RVHyper}}

% Tools
\newcommand{\eahyper}{\text{EAHyper}}

% TODOs and Marking
\newcommand{\todo}[1]{\marginpar{TODO}\textcolor{red}{#1}}
%\newcommand{\tbchecked}[1]{\marginpar{To be checked}\textcolor{blue}{#1}}

\newcommand{\ninfluences}{\not\leadsto}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> old/submission 2/encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> old/submission 2/encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> old/submission 2/encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> old/submission 2/encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> old/submission 2/enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> old/submission 2/enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> old/submission 2/introduction.tex <==
%===============================================================================
\section{Introduction}
\label{sec:intro}
%===============================================================================

\emph{Hyperproperties}~\cite{journals/jcs/ClarksonS10} are widely studied in (but not limited to) the context of secure information-flow control. They generalize trace properties in that they not only check the correctness of \emph{individual} computation traces in isolation, but relate \emph{multiple} computation traces to each other.
%Hyperproperties are widely studied in the context of information-flow control.
%Information-flow policies cannot be monitored with standard runtime verification tools
Examples include information-flow policies, such as observational determinism~\cite{journals/jcs/McLean92,conf/sp/Roscoe95,conf/csfw/ZdancewicM03}, (quantitative) noninterference~\cite{journals/jcs/McLean92,DBLP:conf/fossacs/Smith09,DBLP:conf/esorics/YasuokaT10} as well as symmetry~\cite{conf/cav/FinkbeinerRS15} and spurious dependencies in hardware designs~\cite{conf/tacas/FinkbeinerHST18}, error correcting codes~\cite{conf/cav/FinkbeinerRS15}, and anti-doping of automotive software~\cite{conf/esop/DArgenioBBFH17}.
%The application of hyperproperties 

In this article, we present the monitoring approach implemented in the latest version of $\tool$, an automata-based monitoring tool for hyperproperties~\cite{journals/fmsd/FinkbeinerH19}.
In dynamic verification of hyperproperties, efficient and light-weight monitoring techniques are instrumented in systems, which are usually far beyond the scope of static verification approaches. By doing so, countermeasures are enacted before, for example, irreparable information leaks happen.
%
A runtime verification tool for hyperproperties is in particular useful if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
$\tool$ also supports the verification workflow by providing a method to test and develop specifications: Specifications can be checked on sample traces without the need for a complete model.
Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning.

%However, standard runtime verification tools~\todo{cite} that only consider computations in isolation, can, in general, not monitor such properties.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The input of $\tool$ is given in the temporal logic $\hyperltl$~\cite{conf/post/ClarksonFKMRS14}, which expresses temporal hyperproperties, by extending linear-time temporal logic with \emph{explicit} trace quantification (see~\cite{conf/lics/CoenenFHH19} for a recent study of hyperlogics).
HyperLTL has been used extensively to specify hyperproperties of practical interest (e.g~\cite{conf/cav/FinkbeinerRS15,journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18,conf/cav/FinkbeinerHT18,conf/cav/FinkbeinerHLST18,conf/esop/DArgenioBBFH17}).
For example, observational determinism is expressed as the following formula:
$$
\forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
$$
stating that every trace pair $\pi,\pi'$ has to agree on the output as long as they agree on the inputs as well.
%$\hyperltl$ has been used to specify a variety of information-flow and security properties~\todo{cite}.
When detecting a violation, $\tool$ outputs a counter example, which is a set of computations that does not satisfy the input formula.
%Examples include classical properties like non-interference and observational determinism, as well as quantitative information-flow properties, symmetries in hardware designs, and formally verified error correcting codes~\cite{conf/cav/FinkbeinerRS15}.

Efficient model checking, synthesis and satisfiability checking tools for HyperLTL already exist~\cite{conf/cav/FinkbeinerRS15,conf/cav/FinkbeinerHT18,conf/concur/FinkbeinerH16,DBLP:conf/atva/FinkbeinerHH18,conf/cav/FinkbeinerHS17,conf/cav/FinkbeinerHLST18}. Implementing an efficient runtime verification tool for HyperLTL specifications is, despite recent theoretical progress~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17,conf/csfw/BonakdarpourF18,conf/isola/BonakdarpourSS18,conf/tacas/HahnST19,journals/fmsd/FinkbeinerH19} difficult:
%
%This is because monitoring hyperproperties is difficult:
In principle, the monitor not only needs to process every observed trace, but must also \emph{store} every trace observed so far, so that future traces can be compared with the traces seen so far.
%On the other hand, a runtime verification tool for hyperproperties is certainly useful, in particular if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
%Furthermore, monitoring hyperproperties can be used to simulation plays a significant role in designing specifications and, for example, hardware.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The previous version of $\tool$ tackles this challenging problem by implementing two optimizations~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}: a \emph{specification analysis} to detect exploitable properties of a hyperproperty, such as \emph{symmetry} and a \emph{trace analysis}, which detects all redundant traces that can be omitted during the monitoring process. The trace analysis, which is based on a language inclusion check, can, however, only analyze and prune \emph{entire} traces.
For example, consider the traces $t_1 = \{a\}\{a\}\{\}$ and $t_2 = \{a\}\{\}\{a\}$ of length $3$ and the HyperLTL formula $\forall \pi. \forall \pi'. \G ( a_\pi \rightarrow \neg b_{\pi'} )$. Neither $t_1$ nor $t_2$ is dominated by the other trace, in the sense of the trace analysis, i.e., that one of the traces poses strictly less requirements on future traces~\cite{journals/fmsd/FinkbeinerH19}.
The traces, however, are equal on the first position.
% storage optimization technique that arranges the traces in a tree-like structure.
%This leaves room for optimization, which we address in this article.
This provides an opportunity for optimization, which our new approach exploits.
We introduce a novel trace storage technique (that also has massive impact on the running time), such that $\tool$ can also handle \emph{partially equal} traces by storing them in a tree structure.

We evaluate $\tool$ on existing benchmarks such as classical information-flow security by checking for violations of noninterference or monitoring error-resistant encoder. $\hyperltl$ is, however, not limited to security policies. As an example of such an application beyond security, we show how $\tool$ can be used to detect spurious dependencies in hardware designs.

\paragraph{Structure of this Article.}

The remainder of this article is structured as follows.
We begin by giving preliminaries on $\hyperltl$, its finite trace semantics and notation in Section~\ref{sec:prelims}. In Section~\ref{sec:rvhyper}, we present automata-based monitoring approach implemented in $\tool$, before discussing optimizations in Section~\ref{sec:opt} that make the monitoring feasible in practice. In Section~\ref{sec:eval}, we evaluate $\tool$ with a focus on the novel storage optimization technique using our tree data structure.%: we show $\tool$s performance on a benchmark

This is a revised and extended version of a paper that appeared at TACAS~2018~\cite{conf/tacas/FinkbeinerHST18}.
Our contribution and extension compared to~\cite{conf/tacas/FinkbeinerHST18} is the inclusion of a new trace storage optimization technique presented in Sec.~\ref{sec:trie} and an extended evaluation in Sec.~\ref{sec:eval}.

\paragraph{Related Work.}

The temporal logic $\hyperltl$ was introduced to model check security properties of reactive systems~\cite{conf/post/ClarksonFKMRS14,conf/cav/FinkbeinerRS15}.
For one of its predecessors, $\secltl$~\cite{conf/vmcai/DimitrovaFKRS12}, there has been a proposal for a white box monitoring approach~\cite{conf/isola/DimitrovaFR12} based on alternating automata.
The problem of monitoring $\hyperltl$ has been considered before~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17}.
Agrawal and Bonakdarpour~\cite{conf/csfw/AgrawalB16} were the first to study the monitoring problem of HyperLTL for the sequential model. They gave a syntactic characterization of monitorable $\hyperltl$ formulas. They present a first monitoring algorithm based on a progression logic expressing trace interdependencies and the composition of an LTL$_3$ monitor.
A first constraint-based approach has been outlined in~\cite{conf/tacas/BrettSB17}, which works for a subclass of HyperLTL specifications. The idea is to identify a set of propositions of interest and store corresponding constraints.
A constraint-based algorithm for the complete fragment of $\forall^2$ HyperLTL formulas has been proposed in~\cite{conf/tacas/HahnST19}. The algorithms rewrites a HyperLTL formula and an incoming event into a constraint composed of a plain LTL requirement as well as a HyperLTL requirement.
An constraint system is built incrementally: the HyperLTL part is encoded with variables, which will be incrementally defined with more incoming events of a trace.
Like with our monitoring algorithm, they do not have access to the implementation (black box), but in contrast to our work, they do not provide witnessing traces as a monitor verdict.

In~\cite{conf/csfw/BonakdarpourF18}, the authors study the complexity of monitoring hyperproperties. They show that the form and size of the input, as well as the formula have a significant impact on the feasibility of the monitoring process. They differentiate between several input forms and study their complexity: a set of linear traces, tree-shaped Kripke structures, and acyclic Kripke structures. For acyclic structures and alternation-free HyperLTL formulas, the problems complexity gets as low as NC.
In~\cite{conf/isola/BonakdarpourSS18}, the authors discuss examples where static analysis can be combined with runtime verification techniques to monitor HyperLTL formulas beyond the alternation-free fragment. They discuss the challenges in monitoring formulas beyond this fragment and lay the foundations towards a general method.

For certain information flow policies, like non-interference and some extensions, dynamic enforcement mechanisms have been proposed.
Techniques for the enforcement of information flow policies include tracking dependencies at the hardware level~\cite{conf/asplos/SuhLZD04}, language-based monitors~\cite{journals/jsac/SabelfeldM03,conf/csfw/AskarovS09,conf/pldi/AustinF10,conf/csfw/VanhoefGDPR14,conf/post/BichhawatRGH14}, and abstraction-based dependency tracking~\cite{conf/asian/GuernicBJS06,conf/essos/KovacsS12,conf/csfw/ChudnovKN14}.
Secure multi-execution~\cite{conf/sp/DevrieseP10} is a technique that can enforce non-interference by executing a program multiple times in different security levels.
% and by using special rules for I/O operations.
To enforce non-interference, the inputs are replaced by default values whenever a program tries to read from a higher security level.
%In this article, we are concerned with the monitorability of hyperproperties expressed in $\hyperltl$, which is able to formalize security properties beyond non-interference.

==> old/submission 2/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/submission 2/mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> old/submission 2/mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> old/submission 2/mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> old/submission 2/mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> old/submission 2/mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> old/submission 2/mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> old/submission 2/preliminaries.tex <==
%===============================================================================
\section{Preliminaries}
%===============================================================================
\label{sec:prelims}
Let $\mathit{AP}$ be a finite set of \emph{atomic propositions} and let $\Sigma = 2^\mathit{AP}$ be the corresponding \emph{alphabet}.
An infinite \emph{trace} $t \in  \Sigma^\omega$ is an infinite sequence over the alphabet.
A subset $T \subseteq \Sigma^\omega$ is called a \emph{trace property}. A \emph{hyperproperty} $H \subseteq 2^{(\Sigma^\omega)}$ is a generalization of a trace property.
A finite trace $t \in \Sigma^+$ is a finite sequence over $\Sigma$.
In the case of finite traces, $|t|$ denotes the length of a trace.
%Depending on the context, we refer to either $(2^\mathit{AP})^\omega$ or $(2^\mathit{AP})^+$ as the alphabet $\Sigma^\omega$ or $\Sigma^+$.
We use the following notation to access and manipulate traces:
Let $t$ be a trace and $i$ be a natural number.
$t[i]$ denotes the $i$-th element of $t$.
Therefore, $t[0]$ represents the first element of the trace.
Let $j$ be natural number. If $j \geq i$ and $i\leq|t|$, then
$t[i,j]$ denotes the sequence $t[i] t[i+1] \cdots t[min(j,|t|-1)]$. Otherwise it denotes the empty trace $\epsilon$.
$t[i\rangle$ denotes the suffix of $t$ starting at position $i$.
For two finite traces $s$ and $t$, we denote their concatenation by $s \cdot t$.

%\subsection{LTL}
%\paragraph{Syntax.} Linear-time Temporal Logic (LTL)~\cite{} combines the usual Boolean connectives with temporal modalities.
%\begin{alignat*}{3}
%\varphi \coloneqq ~ a ~ | ~ \neg \varphi ~ | ~ \varphi \vee \varphi ~ | ~ \LTLnext \varphi ~ | ~ \varphi \LTLuntil \varphi
%\end{alignat*}
%where $a \in \mathit{AP}$ is an atomic proposition. We use the standard derived operators \emph{eventually} $\LTLdiamond \varphi \equiv \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \equiv \neg \LTLdiamond \neg \varphi$, \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \equiv (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \varphi_1 \LTLweakuntil (\varphi_1 \wedge \varphi_2)$.
%\paragraph{Semantics.} Let $a \in \mathit{AP}$ and $t \in \Sigma^\omega$. The semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\vDash_{LTL} a \quad &&\text{iff } a \in t[0] \\
%t &\vDash_{LTL} \psi_1 \vee \psi_2 \quad &&\text{iff } t \vDash \psi_1 \vee t \models_{LTL} \psi_2\\
%t &\vDash_{LTL} \neg \psi \quad &&\text{iff } t \not \models_{LTL} \psi\\
%t &\models_{LTL} \LTLnext \psi \quad &&\text{iff } t[1\rangle \models_{LTL} \psi\\
%t &\vDash_{LTL} \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; t[i\rangle \models_{LTL} \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \models_{LTL}\psi_1
%\end{alignat*}
%\paragraph{Finite trace Semantics.} Let $a \in \mathit{AP}$ and let $t \in \Sigma^+$ be a finite trace. The finite trace semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\modelsltlfin a \quad &&\text{iff } a \in t[0] \\
%t &\modelsltlfin \psi_1 \lor \psi_2 \quad &&\text{iff } t \modelsltlfin \psi_1 \text{ or } t \modelsltlfin \psi_2\\
%t &\modelsltlfin \neg \psi \quad &&\text{iff } t \not \modelsltlfin \psi\\
%t &\modelsltlfin \LTLnext \psi \quad &&\text{iff } |t| > 1 \text{ and } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \LTLweaknext \psi \quad &&\text{iff } |t| = 1 \text{ or } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \modelsltlfin \psi_1\\
%t &\modelsltlfin \psi_1 \LTLrelease \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_1\\
%& &&\text{ and for all } 0 \leq j \leq i \text{ we have } t[j\rangle \modelsltlfin \psi_2\\
%& &&\text{ or for all } 0 \leq i < |t| \text{ we have } t[i\rangle \modelsltlfin \psi_2\\
%\end{alignat*}~\todo{finite trace semantics bauen die wir brauchen}


%-------------------------------------------------------------------------------
%\subsection{HyperLTL}
%-------------------------------------------------------------------------------

\paragraph{HyperLTL Syntax.}\label{thltl:syntax}
HyperLTL~\cite{conf/post/ClarksonFKMRS14} extends LTL with trace variables and trace quantifiers.
Let $\mathcal{V}$ be a finite set of trace variables.
The syntax of HyperLTL is given by the grammar
%\begin{figure}[h!]
\begin{alignat*}{3}
  \varphi  &{}\coloneqq ~ \forall \pi . \; \varphi \mid \exists \pi . \; \varphi \mid \psi  \\
  \psi &{}\coloneqq ~ a_{\pi} \mid \psi \wedge \psi \mid \neg \psi \mid \LTLnext \psi  \mid \psi \; \LTLuntil \;  \psi \enspace ,
\end{alignat*}
where $a \in \mathit{AP}$ is an atomic proposition and $\pi \in \mathcal{V}$ is a trace variable.
Atomic propositions are indexed by trace variables. The explicit trace quantification enables us to express properties like ``on all traces $\varphi$ must hold'', expressed by $\forall \pi \ldot \varphi$. Dually, we can express ``there exists a trace such that $\varphi$ holds'', expressed by $\exists \pi \ldot \varphi$.
We use the standard derived operators \emph{release} $\varphi \LTLrelease \psi \coloneqq \neg(\neg \varphi \LTLuntil \neg\psi)$, \emph{eventually} $\LTLdiamond \varphi \coloneqq \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \coloneqq \neg \LTLdiamond \neg \varphi$, and \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \coloneqq (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$.
As we use the finite trace semantics, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to false.
To enable duality in the finite trace setting, we additionally use the \emph{weak} next operator $\LTLweaknext \varphi$ which evaluates to true if a trace ends before the satisfaction of $\varphi$ can be determined and is defined as $\LTLweaknext \varphi \coloneqq \neg \LTLnext \neg \varphi$.
%$\LTLuntil$ denotes the \emph{until}-operator, $\LTLrelease$ the \emph{release}-operator, and we distinguish between a weak and a strong next operator, where $\LTLweaknext \varphi$ denotes the \emph{weak} version, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to true. In contrast, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator.
%$\LTLdiamond$ means that $\varphi$ holds eventually in the future, $\LTLsquare$ means that $\varphi$ holds globally, and $\LTLweakuntil$ is the \emph{weak} version of the \emph{until} operator.
%We call a HyperLTL formula alternation-free, if either all trace variables are universally quantified or all trace variables are existentially quantified.
%, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \neg (\neg\varphi_1 \LTLuntil \neg \varphi_2)$.
We call $\psi$ of a HyperLTL formula $\vec{Q}. \psi$, with an arbitrary quantifier prefix $\vec{Q}$, the \emph{body} of the formula. A HyperLTL formula $\vec{Q}. \psi$ is in the \emph{alternation-free fragment} if either $\vec{Q}$ consists solely of universal quantifiers or solely of existential quantifiers.
%We also call the $\forall^n$ fragment and $\exists^n$ fragment, with $n$ being a natural number, as the respective alternation-free fragments.
We also denote the respective alternation-free fragments as the $\forall^n$ fragment and the $\exists^n$ fragment, with $n$ being the number of quantifiers in the prefix.

%\paragraph{Semantics}\label{thltl:sem}
%%Similar to \HLTL{}, \THLTL{} defines the semantics over a set $T$ of traces.
%A HyperLTL formula can express hyperproperties.
%A trace set $T$ satisfies the hyperproperty $H$ if $T \in H$.
%The semantics of HyperLTL is formally defined over a trace assignment, which is a partial mapping $\Pi: \mathcal{V} \to T$ from trace variables to  traces.
%We write $\Pi[\pi \mapsto t]$ for the updated trace assignment, where $\pi \text{ is mapped to } t$.
%$\Pi[i\rangle$ denotes the trace assignment that is equal to $\Pi(\pi)[i\rangle$ for all $\pi \in \dom(\Pi)$.
%We write the trace set $T$ as subscript since the satisfaction depends on the trace mapping.
%%For the sake of decidability, we assume that $x < y$.
%The satisfaction of a HyperLTL formula $\varphi$ over a trace assignment $\Pi$ and a set of traces $T$, denoted by $\Pi \models_T \varphi$, is defined as follows:
%\begin{alignat*}{2}
%\Pi &\vDash_T a_{\pi} \quad &&\text{iff } a \in \Pi(\pi)[0] \\
%\Pi &\vDash_T \psi_1 \wedge \psi_2 \quad &&\text{iff } \Pi \vDash_T \psi_1 \wedge \Pi \vDash_T \psi_2\\
%\Pi &\vDash_T \neg \psi \quad &&\text{iff } \Pi \nvDash_T \psi\\
%\Pi &\vDash_T \forall \pi. \; \psi \quad &&\text{iff } \forall t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\vDash_T \exists \pi. \; \psi \quad &&\text{iff } \exists t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\models_T \LTLnext \psi \quad &&\text{iff } \Pi[1\rangle \models_T \psi\\
%\Pi &\vDash_T \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; \Pi[i\rangle \models_T \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } \Pi[j\rangle \models_T \psi_1
%\end{alignat*}
%We say a trace set T satisfies a HyperLTL formula $\varphi$ if $\emptyset \models_T \varphi$.
%If unambiguously deducible from the context, we omit $T$ and just write $\models$ instead of $\models_T$.

\paragraph{Finite Trace Semantics.}
We recap the finite trace semantics for HyperLTL~\cite{conf/tacas/BrettSB17} which is itself based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029}.
% and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029} and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a HyperLTL formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
%Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^+$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i\rangle$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i\rangle$ for all $\pi \in \dom(\pathassignfin)$.
By slight abuse of notation, we write $t \in \pathassignfin$ to access traces $t$ in the image of $\pathassignfin$.
%
The satisfaction of a HyperLTL formula $\varphi$ over a finite trace assignment $\pathassignfin$ and a set of finite traces $T$, denoted by $\pathassignfin \models_T \varphi$, is defined as follows:%~\todo{define min t in Pi fin}:
\begin{equation*}
\begin{array}{ll}
    \pathassignfin \models_T a_\pi         \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
    \pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
    \pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
    \pathassignfin \models_T \LTLnext \varphi          & \text{if } \forall t \in \pathassignfin \ldot |t|>1 \text{ and } \pathassignfin[1\rangle \models_T \varphi \\
%    \pathassignfin \models_T \LTLweaknext \varphi      & \text{if } \pathassignfin \models_T \LTLnext \varphi \\
%    & \text{or } \exists t \in \pathassignfin \text{ with } |t| \leq 1 \\
    \pathassignfin \models_T \varphi\LTLuntil\psi      & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \psi \\
    &~\hspace{1ex} \land \forall j < i \ldot \pathassignfin[j\rangle \models_T \varphi \\
%    \pathassignfin \models_T \varphi\LTLrelease\psi    & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \varphi \land \forall j \leq i \ldot \pathassignfin[j\rangle \models_T \psi \\
%   & \text{or } \forall j \leq \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[j\rangle \models_T \varphi\\
    \pathassignfin \models_T \exists \pi \ldot \varphi & \text{if } \exists t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi \\
    \pathassignfin \models_T \forall \pi \ldot \varphi & \text{if } \forall t \in T \text{ holds that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%\subsection{$\forall^2 \hyperltl$}
%As our constraint based monitoring approach will only be concerned with $\forall^2 \hyperltl$ formulas, we introduce special notation, which will help us down the road.
%\begin{definition}
%
The hyperproperty represented by a $\hyperltl$ formula $\varphi$, denoted by $\hlang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%Due to duality of $\LTLuntil$/$\LTLrelease$, $\LTLnext$/$\LTLweaknext$, $\exists$/$\forall$, and the standard Boolean operators, every HyperLTL formula $\varphi$ can be transformed into negation normal form~(NNF), i.e., for every $\varphi$ there is some $\psi$ in negation normal form such that for all $\pathassignfin$ and $T$ it holds that $\pathassignfin \models_T \varphi$ if, and only if, $\pathassignfin \models_T \psi$.
%
%The standard LTL semantic, written $t \modelsltlfin \varphi$, for some LTL formula $\varphi$ is equal to $\set{ \pi \mapsto t }_\mathit{fin} \models_\emptyset \varphi'$, where $\varphi'$ is derived from $\varphi$ by replacing every proposition $p \in \mathit{AP}$ by $p_\pi$.


==> old/submission 2/runtime-verification.tex <==
%===============================================================================
\section{Runtime Verification of Hyperproperties with $\tool$}
%===============================================================================
\label{sec:rvhyper}
%Since Hyperproperties relate multiple system executions to each other, $\tool$ necessarily processes (and stores) multiple runs of a system.
%For example, previous recorded sessions in a dating app or recorded daily behavior of a smart home.
%Monitoring a system against hyperproperties, such as information-flow policies, is essential if a user suspects that private information might be inferred from notwithstanding behavior of a single system run. For example, \emph{observational determinism} is a general information-flow policy that can be monitored with $\tool$. It states that low-security outputs may not depend on high-security inputs.
In this section, we present an overview over $\tool$, before describing the implementation setup, present the monitoring algorithm, and discuss our optimization techniques.

The input of $\tool$ is given as a universally quantified HyperLTL formula and, in addition, the observed behavior of the system under consideration.
The observed behavior is represented as a trace set $T$, where each $t \in T$ represents a previously observed execution of the system to monitor.
%
$\tool$ can therefore detect violations of every monitorable $k$-safety hyperproperty (see~\cite{journals/fmsd/FinkbeinerH19} for an extensive study of monitorability of hyperproperties).
If $\tool$ detects that the system violates the hyperproperty, it outputs a counter example, i.e, a $k$-ary tuple of traces, where $k$ is the number of quantifiers in the HyperLTL formula.
%that make the monitoring of hyperproperties (despite its theoretical unbounded memory consumption) feasible in practice.
%\subsection{Specification}
%The input specification of $\tool$ is given in $\hyperltl$, which is a temporal logic for specifying hyperproperties.
%It extends $\ltl$ by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
%The set of trace variables is $\pathvars$.
%Formulas in $\hyperltl$ are given by the grammar
%\begin{align*}
%\varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
%\psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
%\end{align*}
%where $a \in \ap$ and $\pi \in \pathvars$.
%%
%%The formal semantics is given in Appendix~\ref{appendix:hyperltl}.
%The finite trace semantics for $\hyperltl$ is based on the finite trace semantics of LTL.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
%Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
%$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
%\[
%t[i,j] = \begin{cases}
%\epsilon & \text{if } i \geq |t|\\
%t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
%\end{cases}
%\]
%\begin{equation*}
%\begin{array}{ll}
%\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
%\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
%\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
%\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
%\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
%\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
%\end{array}
%\end{equation*}
%For example, above mentioned observational determinism can be formalized as the HyperLTL formula
%$\forall \pi \ldot \forall \pi' \ldot (O_\pi = O_{\pi'}) \WUntil (I_\pi \not = I_{\pi'})$, where $\WUntil$ is the weak version of $\Until$.
%
%While earlier work on $\hyperltl$~\cite{conf/cav/FinkbeinerRS15} has focused on model checking, recently runtime verification methods have been proposed as a complementation~\cite{conf/csfw/AgrawalB16,conf/rv/FinkbeinerHST17}.
%$\tool$ also supports the verification workflow by providing a method to test and develop $\hyperltl$ specifications: Specifications can be checked on sample traces without the need for a complete model.
%Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning~\todo{passt hier nicht?}.

\subsection{Implementation Details}
$\tool$\footnote{The implementation is available at \url{https://react.uni-saarland.de/tools/rvhyper/}.} is written in C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}.
It uses \emph{spot}~\cite{duret.16.atva2} for building the deterministic monitor automata and the \emph{Buddy} BDD library for handling symbolic constraints.
We use the $\hyperltl$ satisfiability solver $\eahyper$~\cite{conf/cav/FinkbeinerHS17,conf/concur/FinkbeinerH16} to determine whether the input formula is reflexive, symmetric, or transitive.
Depending on those results, we omit redundant tuples in the monitoring algorithm.

%-------------------------------------------------------------------------------
\subsection{Online Monitoring Algorithm}
%-------------------------------------------------------------------------------

For the online algorithm, we use standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.
Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0, F)$ is a tuple of
a finite alphabet $\Sigma = 2^{(\ap \times \pathvars)}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \hookrightarrow Q$,
a designated initial state $q_0 \in Q$, and
a set of accepting states $F \subseteq Q$.
The instantiated automaton runs in parallel over traces in $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
\delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted, if there is a run on $\monitor$ that ends in an accepting state.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over trace variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}  \label{ex:obsdet-monitor}
  As an example formula, consider again the observational determinism formula introduced in the introduction:
  \begin{equation*}
    \forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
  \end{equation*}
  The corresponding monitor template is depicted in Fig.~\ref{fig:monitor-template}.
\end{example}
\begin{figure}[t]
	\centering
 \begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.9]
 \node[state,initial,initial text=,accepting] (init) {$q_0$};
 \node[state,below left=1.3 and 1.5 of init,accepting] (accepting) {$q_\top$};
 \node[state,black!50,below right=1.3 and 1.5 of init] (rejecting) {$q_\bot$};
 
 \draw (init) edge[loop right] node[swap] {$o_\pi = o_{\pi'} \land i_\pi = i_{\pi'}$} ()
       (init) edge node {$i_\pi \neq i_{\pi'}$} (accepting)
       (init) edge[black!50] node[near end] {$o_\pi \neq o_{\pi'} \land i_\pi = i_{\pi'}$} (rejecting)
       (accepting) edge[loop right] node {$\top$} (accepting)
       (rejecting) edge[loop right,black!50] node {$\top$} (rejecting)
 ;
 \end{tikzpicture}
	\caption{Visualization of a monitor template corresponding to the formula given in Example~\ref{ex:obsdet-monitor}. We use a symbolic representation of the transition function $\delta$. For illustration reasons, we depict a sink rejecting state $q_\bot$.}
	\label{fig:monitor-template}
\end{figure}

%\paragraph{Online Algorithm.}~\todo{adept arbitarily formulas}
The algorithm for monitoring $\hyperltl$ formulas when traces are given sequentially to the monitor is presented in Algorithm~\ref{alg:algorithms-sequential}.
%The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, the algorithm accepts new traces and afterwards proceeds with the pace of the incoming stream.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever the current trace $t$ progresses, we progress every tuple $(t_1,\ldots,t_n)$ that contains $t$ with one of the following outcomes:
\begin{enumerate}
  \item One of the traces $t_1,\ldots,t_n$ may have ended, thus, we check if the monitor is in an accepting state and report a violation if this is not the case.
  \item There is a successor state in the monitor, thus we update $S$.
  \item There is no successor state, hence, we report a violation.
\end{enumerate}
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $\vec{t} \in (T \cup \set{t})^n$ containing the new trace $t$.%~\todo{explain notion of instantiation?}
			\begin{algorithm*}[t]
				\SetKwInOut{Input}{input}
				\SetKwInOut{Output}{output}
				\SetAlgoLined
				%\KwResult{Write here the result }
				\Input{$\forall^n$ HyperLTL formula $\varphi$}
				\Output{satisfied or $n$-ary tuple witnessing violation}
				\BlankLine
				$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
				$T \gets \emptyset$\;
				$S: T^n \rightarrow Q$ \quad // initially empty\;
				$t$  \quad // container for the subsequently incoming event traces
				\BlankLine
				\While{there is a new event trace}{
                  $t \gets \epsilon$ \quad // initialize empty trace\;
                  \For(init $S$ for every new tuple $\vec{t}$){$\vec{t} \in ((T \cup \set{t})^n \setminus T^n)$}{
    				$S(\vec{t}) \gets q_0$\;
    			  }
                  \While{$p \in \Sigma$ is a new input event}{
						$t' \gets t~p$ \quad // append $p$ to $t$\;
                        \For(// progress every state in $S$) {$( (t_1,\ldots,t_n), q) \in S$ where $t \in \{t_1,\ldots,t_n\}$}{
                            \uIf(// some trace ended){$\exists t^* \in \{t_1,\ldots,t_n\} \ldot \card{t^*} < \card{t}$}{
                             \eIf {$q \in F$} {
                              remove $(t_1,\ldots,t_n)$ from $S$\;
                              \textbf{continue}\;
                             } { \Return violation and witnessing tuple $(t_1,\ldots,t_n)$\;}
                          }
                          $\vec{t} \gets (t_1,\ldots,t_n)$, where $t_i$ is replaced with $t'$, for each $t_i = t$\;
                          \uIf {$\delta(q, \bigcup_{i=1}^n \bigcup_{a \in \vec{t}(i)[\card{t'}-1]} \set{ (a, \pi_i) }) = q'$} {
        				     $S(\vec{t}) \gets q'$\;
        				  }
        				  \Else{
        				    \Return violation and witnessing tuple $\vec{t}$\;
        				  }
        				}
						$t \gets t'$ \quad // re-assign $t$\;
				  } 
				  $T \gets T \cup \set{t}$\; \quad //add $t$ to already seen traces
				}
				\Return satisfied\;
				\BlankLine
	\caption{Online monitoring algorithm for $\forall^n \hyperltl$: The algorithm subsequently reads event traces and monitors them against already seen traces. Already seen traces are stored in $T$ before continuing with a new event trace.}
	\label{alg:algorithms-sequential}
			\end{algorithm*}

\begin{example} \label{ex:obsdet-algorithm}
  We continue \autoref{ex:obsdet-monitor} by showing how the algorithm progresses on the given formula.
  Assume for the sake of readability that we have a single input proposition $i$ and a single output proposition $o$.
  Furthermore, assume that we have already seen the trace $t_0 = \set{i}\set{i,o}\set{o}$, that is, $T = \set{t_0}$ and $S(t_0,t_0) = q_0$.
  We now show how the algorithm continues with a fresh trace $t_1$.
  In lines 6--8 we add the pairs $(t_0,t_1)$, $(t_0,t_1)$, and $(t_1,t_1)$ with the initial state $q_0$ to $S$.
  Let $p = \set{i}$ be the first input proposition, thus, $t_1 = \set{i}$.
  Since $t_0[0] = t_1[0]$, the monitor remains in $q_0$ for every tuple.
  Let $p = \set{i}$ be the next input proposition, thus, $t_1 = \set{i}\set{i}$.
  Consider the tuple $(t_0,t_1)$.
  As $t_0[1]$ and $t_1[1]$ are equal with respect to $i$ but differ in $o$, the monitor progresses to the rejecting state $q_\bot$ and the algorithm terminates by reporting the violation.
  If, the previous input proposition is $p = \set{}$, both tuples, $(t_0,t_1)$ and $(t_1,t_0)$ would progress to the accepting sink state $q_\top$ as the input proposition is different to $t_0[1]$.
  Assume two more inputs, e.g., $t_1 = \set{i}\set{i}\set{}\set{}$, then the pairs $(t_0,t_0)$, $(t_0,t_1)$, and $(t_1,t_0)$ are removed from $S$ as $t_1$ is strict longer than $t_0$.
\end{example}


\section{Optimizations}
\label{sec:opt}
In this section, we present three optimizations implemented in $\tool$, which, as we will see in the evaluation section, are necessary to make the automata-based monitoring approach feasible in practice. We begin by explaining a \emph{specification analysis}, which is a preprocessing step that exploits properties of the specification to reduce the algorithmic workload. In the subsequent section, we show how $\tool$ tackles the problem of potentially unbounded memory consumption: We recap the \emph{trace analysis}, which was so far the only storage optimization implemented in $\tool$. We then provide a novel storage optimization technique based on prefix-trees, so-called \emph{tries}, to exploit partial equality of the given traces, which the trace analysis neglected so far.
%-------------------------------------------------------------------------------
\subsection{Decreasing Running Time}
%-------------------------------------------------------------------------------

In the example execution in \autoref{ex:obsdet-algorithm} we have seen that the algorithm had to do more work than necessary to monitor observational determinism.
For example, a tuple $(t,t)$ for some trace $t$ cannot violate observational determinism as the traces are equal.
Further, from the pairs $(t,t')$ and $(t',t)$ for some traces $t$ and $t'$, we only need to check one of them as a violation in one of them implies the violation in the other pair.
We can automatically check for such conditions and, thus, omit unnecessary work.

$\tool$ utilizes the HyperLTL satisfiability solver EAHyper~\cite{conf/concur/FinkbeinerH16,conf/cav/FinkbeinerHS17} for its \emph{specification analysis}, which is a preprocessing step that analyzes the HyperLTL formula under consideration.
EAHyper can detect whether a formula is (1) \emph{symmetric}, i.e., we halve the number of instantiated monitors, (2) \emph{transitive}, i.e, we reduce the number of instantiated monitors to two, or (3) \emph{reflexive}, i.e., we can omit the self comparison of traces.

\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:symmetry}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	%Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_n \ldot \psi$, where $\psi$ is an $\ltl$ formula over trace variables $\{\pi_1, \dots, \pi_n\}$.
	%For an assignment $\pathassign$ and an permutation $\sigma : \Pi \to \Pi$, we define $\pathassign \circ \sigma$, such that $(\pathassign \circ \sigma)(\pi) = \pathassign(\sigma(\pi))$ for every $\pi \in \Pi$.
	We say $\varphi$ is invariant under trace variable permutation $\sigma : \pathvars \to \pathvars$, if for any set of traces $T \subseteq \Sigma^{\omega}$ and any assignment $\pathassign : \pathvars \to T$, $(\emptyset, \pathassign, 0) \models \psi \Leftrightarrow (\emptyset, \pathassign \circ \sigma, 0) \models \psi$.
	We say $\varphi$ is symmetric, if it is invariant under every trace variable permutation in $\pathvars$.
\end{definition}
Symmetry is particular interesting since many information flow policies satisfy this property. Consider, for example, observational determinism: 
$
\forall \pi\ldot \forall \pi'\ldot (o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'}).
$ %\todo{different notation than in \autoref{ex:obsdet-algorithm} and intro.}
$\tool$ detects symmetry by translating this formula to a formula that is unsatisfiable if there exists no set of traces for which every trace pair violates the symmetry condition:
$
\exists \pi\ldot \exists \pi'\ldot \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big) \nleftrightarrow \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big)
$.
If the resulting formula turns out to be unsatisfiable, $\tool$ omits the symmetric instantiations of the monitor automaton.
%, which turns out to be, especially in combination with $\tool$s \emph{trace analysis}, a major optimization in practice~\cite{conf/rv/FinkbeinerHST17}.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:transitivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\set{\pi_1, \pi_2}$.
	Let $T = \set{t_1, t_2, t_3} \in \Sigma^{\omega}$ be a three-elemented set of traces.
	We define the assignment $\pathassign_{i,j} : \pathvars \to \Sigma^{\omega}$ by $\pathassign_{i,j} \coloneqq \{\pi_1 \mapsto t_i, \pi_2 \mapsto t_j\}$.
	We say $\varphi$ is transitive, if for all three-elemented sets $T$ it holds that $(\emptyset, \pathassign_{1,2}, 0) \models \psi \wedge (\emptyset, \pathassign_{2,3}, 0) \models \psi \rightarrow (\emptyset, \pathassign_{1,3}, 0) \models \psi$.
\end{definition}
While symmetric HyperLTL formulas allow us to prune half of the monitor instances, transitivity of a HyperLTL formula has an even larger impact on the required memory. Equality, i.e, $\forall \pi. \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$, for example, is transitive and symmetric and allows us to reduce the number of monitor instances to one, since we can check equality against any reference trace.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:reflexivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	We say $\varphi$ is reflexive, if for any trace $t \in \Sigma^{\omega}$ and the corresponding assignment $\pathassign : \pathvars \to \{t\}$, $(\emptyset, \pathassign, 0) \models \psi$.
\end{definition}
Lastly, if a formula is reflexive, $\tool$ omits the composition of a trace with itself during the monitoring process.
%Both $\hyperltl$ formulas considered in this section, $\mathit{ObsDet}$ and $\mathit{EQ}$, are reflexive.
For example, equality and observational determinism have reflexive HyperLTL formulas.

\begin{example}
  Consider again the observational determinism formula from \autoref{ex:obsdet-monitor}.
  We have seen that this formula is both, reflexive and symmetric, thus, we can omit those instances in the algorithm.  
\end{example}


%-------------------------------------------------------------------------------
\subsection{Optimizing Trace Storage}
\label{sec:trie}
%-------------------------------------------------------------------------------

The main obstacle in monitoring hyperproperties is the potentially unbounded space consumption.
So far, RVHyper employed a \emph{trace analysis} technique to detect redundant traces, with respect to a given HyperLTL formula, i.e., traces that can be safely discarded without losing any information and without losing the ability to return a counter example.

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given a HyperLTL formula $\varphi$, a trace set $T$ and an arbitrary $t \in \traces$, we say that $t$ is $(T,\varphi)$-redundant if $T$ is a model of $\varphi$ if and only if $T \cup \set{t}$ is a model of $\varphi$ as well, formally
	\begin{equation*}
	\forall T' \supseteq T \ldot T' \in \hlang(\varphi) \Leftrightarrow T' \cup \{t\} \in \hlang(\varphi) \enspace.
	\end{equation*}
\end{definition}

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given $t,t' \in \Sigma^\omega$, we say $t$ \emph{dominates} $t'$ with respect to $\varphi$ (or simply $t$ \emph{dominates} $t'$ if it is clear from the context) if $t'$ is ($\{t\},\varphi$)-redundant.
\end{definition}

\begin{example}
  For observational determinism, a trace $t$ is dominated by a trace $t'$ if $\card{t} < \card{t'}$ and both traces agree on the input propositions.
\end{example}


This is efficiently implemented in $\tool$ (cf. Algorithm~\ref{alg:traceopti}) and is guaranteed to catch all redundant traces.
In our experiments~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.

The trace analysis, as it is based on a language inclusion check of the entire traces, cannot handle \emph{partial redundancy}, for example, in the case that traces have redundant prefix requirements.
This leaves room for optimization, which we address by implementing a so-called \emph{trie} data structure for managing the storage of incoming traces.

\begin{algorithm}
	%\label{alg_minimization}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\hyperltl$ formula $\varphi$, redundancy free trace set $T$, fresh trace $t$}
	\Output{redundancy free set of traces $T_\mathit{min} \subseteq T \cup \set{t}$}
	%\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}
	\BlankLine
	\ForEach{$t' \in T$}{
		\If{ $t'$ dominates $t$ }
		{
			\Return $T$\;
		}
	}
	\ForEach{$t' \in T$}{
		\If{$t$ dominates $t'$}
		{
			$T \coloneqq T \setminus \set{t'}$\;
		}
	}
	\Return $T \cup \set{t}$\;
	%\BlankLine
	\caption{Trace analysis algorithm to minimize trace storage.}
	\label{alg:traceopti}
\end{algorithm}



%In our experiments~\cite{conf/rv/FinkbeinerHST17,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.
%Ideally one wants to avoid this overhead when monitoring a trace that shares some prefixes with already seen traces.
%We implemented this idea with a so-called \emph{trie} data structure.
Tries, also known as prefix trees, describe a tree data structure, which can represent a set of words over an alphabet in a compact manner.
The root of a trie is identified with the empty word $\epsilon$, additionally each node can have several child nodes, each of which corresponds to a unique letter getting appended to the representing word of the parent node. So the set of words of a trie is identified with the set of words the leaf nodes represent.

\begin{definition}
A trie is a four tuple $(\Sigma, \Tau, \longrightarrow, \tau_0)$ consisting of
\begin{itemize}
    \item a finite alphabet $\Sigma$,
    \item a non-empty set of states $\Tau$,
    \item a transition function $\longrightarrow: \Tau \times \Sigma \rightarrow \Tau$,
    \item and a designated initial state $\tau_0 \in \Tau$ called the root.
    \end{itemize}
\end{definition}
Instead of $((\tau,a),\tau') \in \longrightarrow$ we will write $\tau \overset{a}{\longrightarrow} \tau'$ in the following.
For a trie to be of valid form we restrict $\longrightarrow$ such that, $\forall \tau,\tau' \in \Tau. |\{\tau \overset{a}{\longrightarrow} \tau'| a \in \Sigma\}| \leq 1$.

%Additionally to our analysis phases it would be helpful if we could use some insights from trace analysis 


%As mentioned before, storing the incoming traces succinctly is a major concern in monitoring hyperproperties.
In our case the alphabet would be the set of propositions used in the specification, and the word built by the trie represents the traces. %build from it are what we call traces.
%Tries provide a 
Instead of storing each trace individually, we store all of them in one trie structure, branching only in case of deviation. This means equal prefixes only have to be stored once.
Besides the obvious benefits for memory, we also can make use of the maintained trie data structure to improve the runtime of our monitoring algorithms. As traces with same prefixes end up corresponding to the same path in the trie, we only have to instantiate the monitor automaton as much as the trie contains branches.
%O(size branches) times.
\begin{example}
	Consider the following traces of length $6$ over the alphabet $2^{\{i,o\}}$:
	\begin{itemize}
		\item
		$t_1: \{\set{i},\set{i,o},\set{i},\set{i},\set{i},\set{i,o} \}$
		\item
		$t_2: \{\set{i}, \set{i,o}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_3: \{\set{i}, \set{i}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_4: \{\set{i}, \set{i}, \set{}, \set{} , \set{}, \set{}\}$
	\end{itemize}
After processing the traces sequentially, the resulting trie looks as follows:

\vspace{1ex}

\begin{tikzpicture}[sibling distance=7em, level distance = 30pt,
every node/.style = {shape=circle,
	draw, align=center, minimum size = 0.9cm, inner sep = 0pt},
level 1/.style = {sibling distance = 10em},
level 2/.style = {sibling distance = 5em},
level 5/.style = {sibling distance = 5em}]
\node {$\{i\}$}
child { node {$\{i\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} } } } } 
	child { node {$\{ \}$}  
		child { node {$\{ \}$} 
			child { node {$\{ \}$}
				child { node {$\{ \}$} } } } } }
child { node {$\{i,o\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} }
				child { node {$\{i,o\}$} } } } } };
\end{tikzpicture}
\end{example}

\subsection{Trie-based Monitoring Algorithm}

We depict a trie-based offline monitoring algorithm in Fig.~\ref{alg:trie-offline}.
For the sake of readability, we assume that there are as many traces as universal quantifier, that we progress through all traces in parallel, and that all traces have the same length.
This is merely a simplification in the presentation, one can build the trie in a sequential fashion for online monitoring by a slight modification of the presented algorithm.

Without using tries our monitoring algorithm was based on instantiating the deterministic monitor template $\monitor_\varphi$ with tuples of traces. Now we instantiate $\monitor_\varphi$ with tuples of tries. Initially we only have to create the single instance having the the root of our trie.

\begin{comment}
	\begin{algorithm*}
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
		$S: \Tau^n \rightarrow Q$, \quad $E: \Tau^n \rightarrow \Sigma$\;
		$\tau_0 \coloneqq $\texttt{ new\_trie()}\;
		%$\mathbf{i} \coloneqq \underbrace{(\tau_0,\ldots,\tau_0)}{n \text{times}}$\;
		%$I \coloneqq \{\mathbf{i}\}$\;
		\BlankLine
		$i_0 \in \{ \tau_0 \}^n$\;
		$S(i_0) = q_0$\;
		\While{there is a new trace}{
			$I \leftarrow \{i_0\}$\;
			$\tau \leftarrow \tau_0$\;
			\While{$p \in \Sigma$ is a new event}{
				$\tau' \leftarrow$ \texttt{add\_child($\tau,p$)} //\texttt{assert($E(\tau')==p$)}\;
				$I_n \leftarrow \emptyset$\;
				\ForEach{$i \in I$}{
					$I' \leftarrow \{i' \mid i(j) \rightarrow i'(j), a \in \Sigma, 1 \leq j \leq n\}$\;
					$I' \leftarrow \{i' \in I' \mid \exists k. i'(k) = \tau'\}$\;
					\ForEach{$i' \in I'$}{
						\uIf{$\delta(S(i), \cup_{j=1}^n \cup_{a\in E(i'(j))} \{(a,\pi_j)\}) = q$}{
							$S(i') = q$\;
						}
						\Else{
							\Return(\texttt{rooted\_seq($i'(1)$)}, \ldots, \texttt{rooted\_seq($i'(n)$)})\;
						}
					}
				}
			}
		}
		%\While{$\mathbf{p} \leftarrow$ new elements (in a forward fashion)}{
		%	\For{$1 \leq j \leq n$}{
		%		$\mathbf{i}(j) \leftarrow $\texttt{add\_value($\mathbf{i}(j)$, $j$, $\mathbf{p}(j)$)}\;
		%	}
		%	$I \leftarrow \bigcup_{\mathbf{i} \in I} \{(i'_1,\ldots, i'_n)| \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n\}$\;
		%	\ForEach{$\mathbf{i} \in I$}{
		%		%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
		%		progress every state in $S$ according to $\delta$\;
		%		\If{violation in $M_\varphi$}{
		%			$t \coloneqq ($\texttt{rooted\_sequence($i(1)$)}$,\ldots,$\texttt{rooted\_sequence($i(n)$)}$)$\;
		%			\Return witnessing tuple $t^n$\;
		%		}
		%	}
		%}
		%\Return satisfied\;
		%\BlankLine
	\caption{Online algorithm using trie data structure.}
	\label{alg:trie-online-parallel}
	\end{algorithm*}
\end{comment}
	\begin{algorithm*}[t]
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\\
		$S: \Tau^n \rightarrow Q$\\
		$\tau_0 \coloneqq $\texttt{new\_trie()}\\
		$\mathbf{i} \coloneqq (\tau_0,\ldots,\tau_0) \in \Tau^n$\\
		$I \coloneqq \{\mathbf{i}\}$  \quad // set of not-yet terminated branches\\
		\BlankLine
		\While{$\mathbf{p} \leftarrow$ new event (in $\Sigma^n$)}{
			\For{$1 \leq j \leq n$}{
				$\mathbf{i}(j) \leftarrow $\texttt{add\_child($\mathbf{i}(j)$, $\mathbf{p}(j)$)} \quad // add child with value $\vec{p}(j)$ to $\vec{i}(j)$ if needed \\
			}
			// update set of active branches\\
			$I \leftarrow \bigcup_{\mathbf{i} \in I} \set{ (i'_1,\ldots, i'_n) \mid \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n }$\\
			\ForEach{$\mathbf{i} \in I$}{
				%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
				progress every state in $S$ according to $\delta$\;
				\If{violation in $\monitor_\varphi$}{
				    // return sequence from root to $\vec{i}$\\
					$t \gets ($\texttt{rooted\_sequence($\vec{i}(1)$)}$,\ldots,$\texttt{rooted\_sequence($\vec{i}(n)$)}$)$\\
					\Return witnessing tuple $t^n$\\
				}
			}
		}
		\Return satisfied if $\forall \vec{i} \in I \ldots S(\vec{i}) \in F$ else violation\\
		\BlankLine
	\caption{Offline algorithm using trie data structure.}
	\label{alg:trie-offline}
\end{algorithm*}

The trie-based algorithm has much in common with its previously discussed trace-based counterpart. Initially, we have to build the deterministic monitor automaton $\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F)$.
We instantiate the monitor with a fresh trie root $\tau_0$.
A mapping from trie instantiations to a state in $\monitor_\varphi$ $S: \Tau^n \rightarrow Q$, stores the current state of every active branch of the trie, stored in the set $I$.
For each of the incoming traces, we provide an entry in a tuple of tries $\mathbf{\tau}$, each entry gets initialized to $\tau_0$.
During the run of our algorithm these entries will get updated such that they always correspond to the word built by the traces up to this point.
For as long as there are traces left, which have not yet ended, and we have not yet detected a violation, we will proceed updating the entries in $\vec{i}$ as follows.
Having entry $\tau$ and the correspond trace sequence proceeds with $a$, if $\exists \tau' \in \Tau. \tau \overset{a}{\longrightarrow} \tau'$, we update the entry to $\tau'$ otherwise we create such a child node of $\tau$ (\texttt{add\_child} in line 8).
Creating a new node in the trie always occurs, if the prefix of the incoming trace starts to differ from already seen prefixes.
After having moved on step in our traces sequences, we have to reflect this step in our trie structure, in order for the trie-instantiated automata to correctly monitor the new propositions.
As a trie node can branch to multiple child nodes, each monitor instantiation will get replaced by the set of instantiations, where all possible child combinations of the different assigned tries are existent (update of $I$ in line 11).
Afterwards, we update $S$ in the same way as in Algorithm~\ref{alg:traceopti}, thus, we omit algorithmic details here.
%This can be efficiently implemented as we essential fork the monitor instantiation for the different branches in the trie.
%After this preprocessing we are able to update our mapping $S$ according to $\delta$.
If a violation is detected here, that is there is no transition in the monitor corresponding to $\vec{i}$, we will return the corresponding counter example as a tuple of traces, as those can get reconstructed by stepping upwards in the tries of $\vec{i}$.
%Note that the sequential algorithm is derived from the parallel one by progressing one trace at a time and additionally when forking the monitor instantiations, only those new instantiation have to be kept, which contain the (single) trie in $\mathbf{\tau}$ at least once. 
If the traces end, we check if every open branch $\vec{i} \in I$ is in an accepting state.

%\subsection{Tries and Trace Analysis in Combination}
%\todo{TODO}


==> old/submission 2/tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> old/submission 2/tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/submission 3/commands.tex <==

% Common math
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{{\langle #1 \rangle}}
\newcommand{\card}[1]{{|#1|}}
\newcommand{\ldot}{\mathpunct{.}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\dom}{\mathrm{dom}}

% Languages
\newcommand{\good}{\mathit{good}}
\newcommand{\bad}{\mathit{bad}}
\newcommand{\winning}{\mathit{winning}}
\newcommand{\losing}{\mathit{losing}}
\newcommand{\hlang}{\mathcal{H}}

% Complexity classes
\newcommand{\pspace}{\textsc{PSpace}}

% Logics
\newcommand{\ltl}{\text{LTL}}
\newcommand{\hyperltl}{\text{HyperLTL}}
\newcommand{\secltl}{\text{SecLTL}}


\newcommand{\lang}{\mathcal{L}}
\newcommand{\ap}{\text{AP}}
\renewcommand{\models}{\vDash}
\newcommand{\nmodels}{\nvDash}
\newcommand{\traces}{\mathit{TR}}

% Traces
\newcommand{\pref}{\preceq}
\newcommand{\tracebox}[1]{\framebox[4.5ex][l]{#1}}
\newcommand{\pctracebox}[1]{\framebox[4.5ex][l]{#1}}

% LTL
\newcommand{\U}{\Until}
\newcommand{\X}{\Next}
\newcommand{\G}{\Globally}
\newcommand{\F}{\Eventually}
\newcommand{\R}{\Release}
\newcommand{\W}{\WUntil}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

% HyperLTL
\newcommand{\pathassign}{\Pi}
\newcommand{\pathvars}{\mathcal{V}}
\newcommand{\pathassignfin}{\Pi_\mathit{fin}}

% Monitoring
\newcommand{\monitor}{\mathcal{M}}
\newcommand{\tool}{\text{RVHyper}}

% Tools
\newcommand{\eahyper}{\text{EAHyper}}

% TODOs and Marking
\newcommand{\todo}[1]{\marginpar{TODO}\textcolor{red}{#1}}
%\newcommand{\tbchecked}[1]{\marginpar{To be checked}\textcolor{blue}{#1}}

\newcommand{\ninfluences}{\not\leadsto}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> old/submission 3/encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> old/submission 3/encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> old/submission 3/encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> old/submission 3/encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> old/submission 3/enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> old/submission 3/enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> old/submission 3/introduction.tex <==
%===============================================================================
\section{Introduction}
\label{sec:intro}
%===============================================================================

\emph{Hyperproperties}~\cite{journals/jcs/ClarksonS10} are widely studied in (but not limited to) the context of secure information-flow control. They generalize trace properties in that they not only check the correctness of \emph{individual} computation traces in isolation, but relate \emph{multiple} computation traces to each other.
%Hyperproperties are widely studied in the context of information-flow control.
%Information-flow policies cannot be monitored with standard runtime verification tools
Examples include information-flow policies, such as observational determinism~\cite{journals/jcs/McLean92,conf/sp/Roscoe95,conf/csfw/ZdancewicM03}, (quantitative) noninterference~\cite{journals/jcs/McLean92,DBLP:conf/fossacs/Smith09,DBLP:conf/esorics/YasuokaT10} as well as symmetry~\cite{conf/cav/FinkbeinerRS15} and spurious dependencies in hardware designs~\cite{conf/tacas/FinkbeinerHST18}, error correcting codes~\cite{conf/cav/FinkbeinerRS15}, and anti-doping of automotive software~\cite{conf/esop/DArgenioBBFH17}.
%The application of hyperproperties 

In this article, we present the monitoring approach implemented in the latest version of $\tool$, an automata-based monitoring tool for hyperproperties~\cite{journals/fmsd/FinkbeinerH19}.
In dynamic verification of hyperproperties, efficient and light-weight monitoring techniques are instrumented in systems, which are usually far beyond the scope of static verification approaches. By doing so, countermeasures are enacted before, for example, irreparable information leaks happen.
%
A runtime verification tool for hyperproperties is in particular useful if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
$\tool$ also supports the verification workflow by providing a method to test and develop specifications: Specifications can be checked on sample traces without the need for a complete model.
Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning.

%However, standard runtime verification tools~\todo{cite} that only consider computations in isolation, can, in general, not monitor such properties.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The input of $\tool$ is given in the temporal logic $\hyperltl$~\cite{conf/post/ClarksonFKMRS14}, which expresses temporal hyperproperties, by extending linear-time temporal logic with \emph{explicit} trace quantification (see~\cite{conf/lics/CoenenFHH19} for a recent study of hyperlogics).
HyperLTL has been used extensively to specify hyperproperties of practical interest (e.g~\cite{conf/cav/FinkbeinerRS15,journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18,conf/cav/FinkbeinerHT18,conf/cav/FinkbeinerHLST18,conf/esop/DArgenioBBFH17}).
For example, observational determinism is expressed as the following formula:
$$
\forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
$$
stating that every trace pair $\pi,\pi'$ has to agree on the output as long as they agree on the inputs as well.
%$\hyperltl$ has been used to specify a variety of information-flow and security properties~\todo{cite}.
When detecting a violation, $\tool$ outputs a counter example, which is a set of computations that does not satisfy the input formula.
%Examples include classical properties like non-interference and observational determinism, as well as quantitative information-flow properties, symmetries in hardware designs, and formally verified error correcting codes~\cite{conf/cav/FinkbeinerRS15}.

Efficient model checking, synthesis and satisfiability checking tools for HyperLTL already exist~\cite{conf/cav/FinkbeinerRS15,conf/cav/FinkbeinerHT18,conf/concur/FinkbeinerH16,DBLP:conf/atva/FinkbeinerHH18,conf/cav/FinkbeinerHS17,conf/cav/FinkbeinerHLST18}. Implementing an efficient runtime verification tool for HyperLTL specifications is, despite recent theoretical progress~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17,conf/csfw/BonakdarpourF18,conf/isola/BonakdarpourSS18,conf/tacas/HahnST19,journals/fmsd/FinkbeinerH19} difficult:
%
%This is because monitoring hyperproperties is difficult:
In principle, the monitor not only needs to process every observed trace, but must also \emph{store} every trace observed so far, so that future traces can be compared with the traces seen so far.
%On the other hand, a runtime verification tool for hyperproperties is certainly useful, in particular if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
%Furthermore, monitoring hyperproperties can be used to simulation plays a significant role in designing specifications and, for example, hardware.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The previous version of $\tool$ tackles this challenging problem by implementing two optimizations~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}: a \emph{specification analysis} to detect exploitable properties of a hyperproperty, such as \emph{symmetry} and a \emph{trace analysis}, which detects all redundant traces that can be omitted during the monitoring process. The trace analysis, which is based on a language inclusion check, can, however, only analyze and prune \emph{entire} traces.
For example, consider the traces $t_1 = \{a\}\{a\}\{\}$ and $t_2 = \{a\}\{\}\{a\}$ of length $3$ and the HyperLTL formula $\forall \pi. \forall \pi'. \G ( a_\pi \rightarrow \neg b_{\pi'} )$. Neither $t_1$ nor $t_2$ is dominated by the other trace, in the sense of the trace analysis, i.e., that one of the traces poses strictly less requirements on future traces~\cite{journals/fmsd/FinkbeinerH19}.
The traces, however, are equal on the first position.
% storage optimization technique that arranges the traces in a tree-like structure.
%This leaves room for optimization, which we address in this article.
This provides an opportunity for optimization, which our new approach exploits.
We introduce a novel trace storage technique (that also has massive impact on the running time), such that $\tool$ can also handle \emph{partially equal} traces by storing them in a tree structure.

We evaluate $\tool$ on existing benchmarks such as classical information-flow security by checking for violations of noninterference or monitoring error-resistant encoder. $\hyperltl$ is, however, not limited to security policies. As an example of such an application beyond security, we show how $\tool$ can be used to detect spurious dependencies in hardware designs.

\paragraph{Structure of this Article.}

The remainder of this article is structured as follows.
We begin by giving preliminaries on $\hyperltl$, its finite trace semantics and notation in Section~\ref{sec:prelims}. In Section~\ref{sec:rvhyper}, we present automata-based monitoring approach implemented in $\tool$, before discussing optimizations in Section~\ref{sec:opt} that make the monitoring feasible in practice. In Section~\ref{sec:eval}, we evaluate $\tool$ with a focus on the novel storage optimization technique using our tree data structure.%: we show $\tool$s performance on a benchmark

This is a revised and extended version of a paper that appeared at TACAS~2018~\cite{conf/tacas/FinkbeinerHST18}.
Our contribution and extension compared to~\cite{conf/tacas/FinkbeinerHST18} is the inclusion of a new trace storage optimization technique presented in Sec.~\ref{sec:trie} and an extended evaluation in Sec.~\ref{sec:eval}.

\paragraph{Related Work.}

The temporal logic $\hyperltl$ was introduced to model check security properties of reactive systems~\cite{conf/post/ClarksonFKMRS14,conf/cav/FinkbeinerRS15}.
For one of its predecessors, $\secltl$~\cite{conf/vmcai/DimitrovaFKRS12}, there has been a proposal for a white box monitoring approach~\cite{conf/isola/DimitrovaFR12} based on alternating automata.
The problem of monitoring $\hyperltl$ has been considered before~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17}.
Agrawal and Bonakdarpour~\cite{conf/csfw/AgrawalB16} were the first to study the monitoring problem of HyperLTL for the sequential model. They gave a syntactic characterization of monitorable $\hyperltl$ formulas. They present a first monitoring algorithm based on a progression logic expressing trace interdependencies and the composition of an LTL$_3$ monitor.
A first constraint-based approach has been outlined in~\cite{conf/tacas/BrettSB17}, which works for a subclass of HyperLTL specifications. The idea is to identify a set of propositions of interest and store corresponding constraints.
A constraint-based algorithm for the complete fragment of $\forall^2$ HyperLTL formulas has been proposed in~\cite{conf/tacas/HahnST19}. The algorithms rewrites a HyperLTL formula and an incoming event into a constraint composed of a plain LTL requirement as well as a HyperLTL requirement.
An constraint system is built incrementally: the HyperLTL part is encoded with variables, which will be incrementally defined with more incoming events of a trace.
Like with our monitoring algorithm, they do not have access to the implementation (black box), but in contrast to our work, they do not provide witnessing traces as a monitor verdict.

In~\cite{conf/csfw/BonakdarpourF18}, the authors study the complexity of monitoring hyperproperties. They show that the form and size of the input, as well as the formula have a significant impact on the feasibility of the monitoring process. They differentiate between several input forms and study their complexity: a set of linear traces, tree-shaped Kripke structures, and acyclic Kripke structures. For acyclic structures and alternation-free HyperLTL formulas, the problems complexity gets as low as NC.
In~\cite{conf/isola/BonakdarpourSS18}, the authors discuss examples where static analysis can be combined with runtime verification techniques to monitor HyperLTL formulas beyond the alternation-free fragment. They discuss the challenges in monitoring formulas beyond this fragment and lay the foundations towards a general method.

For certain information flow policies, like non-interference and some extensions, dynamic enforcement mechanisms have been proposed.
Techniques for the enforcement of information flow policies include tracking dependencies at the hardware level~\cite{conf/asplos/SuhLZD04}, language-based monitors~\cite{journals/jsac/SabelfeldM03,conf/csfw/AskarovS09,conf/pldi/AustinF10,conf/csfw/VanhoefGDPR14,conf/post/BichhawatRGH14}, and abstraction-based dependency tracking~\cite{conf/asian/GuernicBJS06,conf/essos/KovacsS12,conf/csfw/ChudnovKN14}.
Secure multi-execution~\cite{conf/sp/DevrieseP10} is a technique that can enforce non-interference by executing a program multiple times in different security levels.
% and by using special rules for I/O operations.
To enforce non-interference, the inputs are replaced by default values whenever a program tries to read from a higher security level.
%In this article, we are concerned with the monitorability of hyperproperties expressed in $\hyperltl$, which is able to formalize security properties beyond non-interference.

==> old/submission 3/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/submission 3/mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> old/submission 3/mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> old/submission 3/mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> old/submission 3/mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> old/submission 3/mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> old/submission 3/mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> old/submission 3/preliminaries.tex <==
%===============================================================================
\section{Preliminaries}
%===============================================================================
\label{sec:prelims}
Let $\mathit{AP}$ be a finite set of \emph{atomic propositions} and let $\Sigma = 2^\mathit{AP}$ be the corresponding \emph{alphabet}.
An infinite \emph{trace} $t \in  \Sigma^\omega$ is an infinite sequence over the alphabet.
A subset $T \subseteq \Sigma^\omega$ is called a \emph{trace property}. A \emph{hyperproperty} $H \subseteq 2^{(\Sigma^\omega)}$ is a generalization of a trace property.
A finite trace $t \in \Sigma^+$ is a finite sequence over $\Sigma$.
In the case of finite traces, $|t|$ denotes the length of a trace.
%Depending on the context, we refer to either $(2^\mathit{AP})^\omega$ or $(2^\mathit{AP})^+$ as the alphabet $\Sigma^\omega$ or $\Sigma^+$.
We use the following notation to access and manipulate traces:
Let $t$ be a trace and $i$ be a natural number.
$t[i]$ denotes the $i$-th element of $t$.
Therefore, $t[0]$ represents the first element of the trace.
Let $j$ be natural number. If $j \geq i$ and $i\leq|t|$, then
$t[i,j]$ denotes the sequence $t[i] t[i+1] \cdots t[min(j,|t|-1)]$. Otherwise it denotes the empty trace $\epsilon$.
$t[i\rangle$ denotes the suffix of $t$ starting at position $i$.
For two finite traces $s$ and $t$, we denote their concatenation by $s \cdot t$.

%\subsection{LTL}
%\paragraph{Syntax.} Linear-time Temporal Logic (LTL)~\cite{} combines the usual Boolean connectives with temporal modalities.
%\begin{alignat*}{3}
%\varphi \coloneqq ~ a ~ | ~ \neg \varphi ~ | ~ \varphi \vee \varphi ~ | ~ \LTLnext \varphi ~ | ~ \varphi \LTLuntil \varphi
%\end{alignat*}
%where $a \in \mathit{AP}$ is an atomic proposition. We use the standard derived operators \emph{eventually} $\LTLdiamond \varphi \equiv \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \equiv \neg \LTLdiamond \neg \varphi$, \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \equiv (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \varphi_1 \LTLweakuntil (\varphi_1 \wedge \varphi_2)$.
%\paragraph{Semantics.} Let $a \in \mathit{AP}$ and $t \in \Sigma^\omega$. The semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\vDash_{LTL} a \quad &&\text{iff } a \in t[0] \\
%t &\vDash_{LTL} \psi_1 \vee \psi_2 \quad &&\text{iff } t \vDash \psi_1 \vee t \models_{LTL} \psi_2\\
%t &\vDash_{LTL} \neg \psi \quad &&\text{iff } t \not \models_{LTL} \psi\\
%t &\models_{LTL} \LTLnext \psi \quad &&\text{iff } t[1\rangle \models_{LTL} \psi\\
%t &\vDash_{LTL} \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; t[i\rangle \models_{LTL} \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \models_{LTL}\psi_1
%\end{alignat*}
%\paragraph{Finite trace Semantics.} Let $a \in \mathit{AP}$ and let $t \in \Sigma^+$ be a finite trace. The finite trace semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\modelsltlfin a \quad &&\text{iff } a \in t[0] \\
%t &\modelsltlfin \psi_1 \lor \psi_2 \quad &&\text{iff } t \modelsltlfin \psi_1 \text{ or } t \modelsltlfin \psi_2\\
%t &\modelsltlfin \neg \psi \quad &&\text{iff } t \not \modelsltlfin \psi\\
%t &\modelsltlfin \LTLnext \psi \quad &&\text{iff } |t| > 1 \text{ and } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \LTLweaknext \psi \quad &&\text{iff } |t| = 1 \text{ or } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \modelsltlfin \psi_1\\
%t &\modelsltlfin \psi_1 \LTLrelease \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_1\\
%& &&\text{ and for all } 0 \leq j \leq i \text{ we have } t[j\rangle \modelsltlfin \psi_2\\
%& &&\text{ or for all } 0 \leq i < |t| \text{ we have } t[i\rangle \modelsltlfin \psi_2\\
%\end{alignat*}~\todo{finite trace semantics bauen die wir brauchen}


%-------------------------------------------------------------------------------
%\subsection{HyperLTL}
%-------------------------------------------------------------------------------

\paragraph{HyperLTL Syntax.}\label{thltl:syntax}
HyperLTL~\cite{conf/post/ClarksonFKMRS14} extends LTL with trace variables and trace quantifiers.
Let $\mathcal{V}$ be a finite set of trace variables.
The syntax of HyperLTL is given by the grammar
%\begin{figure}[h!]
\begin{alignat*}{3}
  \varphi  &{}\coloneqq ~ \forall \pi . \; \varphi \mid \exists \pi . \; \varphi \mid \psi  \\
  \psi &{}\coloneqq ~ a_{\pi} \mid \psi \wedge \psi \mid \neg \psi \mid \LTLnext \psi  \mid \psi \; \LTLuntil \;  \psi \enspace ,
\end{alignat*}
where $a \in \mathit{AP}$ is an atomic proposition and $\pi \in \mathcal{V}$ is a trace variable.
Atomic propositions are indexed by trace variables. The explicit trace quantification enables us to express properties like ``on all traces $\varphi$ must hold'', expressed by $\forall \pi \ldot \varphi$. Dually, we can express ``there exists a trace such that $\varphi$ holds'', expressed by $\exists \pi \ldot \varphi$.
We use the standard derived operators \emph{release} $\varphi \LTLrelease \psi \coloneqq \neg(\neg \varphi \LTLuntil \neg\psi)$, \emph{eventually} $\LTLdiamond \varphi \coloneqq \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \coloneqq \neg \LTLdiamond \neg \varphi$, and \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \coloneqq (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$.
As we use the finite trace semantics, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to false.
To enable duality in the finite trace setting, we additionally use the \emph{weak} next operator $\LTLweaknext \varphi$ which evaluates to true if a trace ends before the satisfaction of $\varphi$ can be determined and is defined as $\LTLweaknext \varphi \coloneqq \neg \LTLnext \neg \varphi$.
%$\LTLuntil$ denotes the \emph{until}-operator, $\LTLrelease$ the \emph{release}-operator, and we distinguish between a weak and a strong next operator, where $\LTLweaknext \varphi$ denotes the \emph{weak} version, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to true. In contrast, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator.
%$\LTLdiamond$ means that $\varphi$ holds eventually in the future, $\LTLsquare$ means that $\varphi$ holds globally, and $\LTLweakuntil$ is the \emph{weak} version of the \emph{until} operator.
%We call a HyperLTL formula alternation-free, if either all trace variables are universally quantified or all trace variables are existentially quantified.
%, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \neg (\neg\varphi_1 \LTLuntil \neg \varphi_2)$.
We call $\psi$ of a HyperLTL formula $\vec{Q}. \psi$, with an arbitrary quantifier prefix $\vec{Q}$, the \emph{body} of the formula. A HyperLTL formula $\vec{Q}. \psi$ is in the \emph{alternation-free fragment} if either $\vec{Q}$ consists solely of universal quantifiers or solely of existential quantifiers.
%We also call the $\forall^n$ fragment and $\exists^n$ fragment, with $n$ being a natural number, as the respective alternation-free fragments.
We also denote the respective alternation-free fragments as the $\forall^n$ fragment and the $\exists^n$ fragment, with $n$ being the number of quantifiers in the prefix.

%\paragraph{Semantics}\label{thltl:sem}
%%Similar to \HLTL{}, \THLTL{} defines the semantics over a set $T$ of traces.
%A HyperLTL formula can express hyperproperties.
%A trace set $T$ satisfies the hyperproperty $H$ if $T \in H$.
%The semantics of HyperLTL is formally defined over a trace assignment, which is a partial mapping $\Pi: \mathcal{V} \to T$ from trace variables to  traces.
%We write $\Pi[\pi \mapsto t]$ for the updated trace assignment, where $\pi \text{ is mapped to } t$.
%$\Pi[i\rangle$ denotes the trace assignment that is equal to $\Pi(\pi)[i\rangle$ for all $\pi \in \dom(\Pi)$.
%We write the trace set $T$ as subscript since the satisfaction depends on the trace mapping.
%%For the sake of decidability, we assume that $x < y$.
%The satisfaction of a HyperLTL formula $\varphi$ over a trace assignment $\Pi$ and a set of traces $T$, denoted by $\Pi \models_T \varphi$, is defined as follows:
%\begin{alignat*}{2}
%\Pi &\vDash_T a_{\pi} \quad &&\text{iff } a \in \Pi(\pi)[0] \\
%\Pi &\vDash_T \psi_1 \wedge \psi_2 \quad &&\text{iff } \Pi \vDash_T \psi_1 \wedge \Pi \vDash_T \psi_2\\
%\Pi &\vDash_T \neg \psi \quad &&\text{iff } \Pi \nvDash_T \psi\\
%\Pi &\vDash_T \forall \pi. \; \psi \quad &&\text{iff } \forall t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\vDash_T \exists \pi. \; \psi \quad &&\text{iff } \exists t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\models_T \LTLnext \psi \quad &&\text{iff } \Pi[1\rangle \models_T \psi\\
%\Pi &\vDash_T \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; \Pi[i\rangle \models_T \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } \Pi[j\rangle \models_T \psi_1
%\end{alignat*}
%We say a trace set T satisfies a HyperLTL formula $\varphi$ if $\emptyset \models_T \varphi$.
%If unambiguously deducible from the context, we omit $T$ and just write $\models$ instead of $\models_T$.

\paragraph{Finite Trace Semantics.}
We recap the finite trace semantics for HyperLTL~\cite{conf/tacas/BrettSB17} which is itself based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029}.
% and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029} and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a HyperLTL formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
%Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^+$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i\rangle$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i\rangle$ for all $\pi \in \dom(\pathassignfin)$.
By slight abuse of notation, we write $t \in \pathassignfin$ to access traces $t$ in the image of $\pathassignfin$.
%
The satisfaction of a HyperLTL formula $\varphi$ over a finite trace assignment $\pathassignfin$ and a set of finite traces $T$, denoted by $\pathassignfin \models_T \varphi$, is defined as follows:%~\todo{define min t in Pi fin}:
\begin{equation*}
\begin{array}{ll}
    \pathassignfin \models_T a_\pi         \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
    \pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
    \pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
    \pathassignfin \models_T \LTLnext \varphi          & \text{if } \forall t \in \pathassignfin \ldot |t|>1 \text{ and } \pathassignfin[1\rangle \models_T \varphi \\
%    \pathassignfin \models_T \LTLweaknext \varphi      & \text{if } \pathassignfin \models_T \LTLnext \varphi \\
%    & \text{or } \exists t \in \pathassignfin \text{ with } |t| \leq 1 \\
    \pathassignfin \models_T \varphi\LTLuntil\psi      & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \psi \\
    &~\hspace{1ex} \land \forall j < i \ldot \pathassignfin[j\rangle \models_T \varphi \\
%    \pathassignfin \models_T \varphi\LTLrelease\psi    & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \varphi \land \forall j \leq i \ldot \pathassignfin[j\rangle \models_T \psi \\
%   & \text{or } \forall j \leq \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[j\rangle \models_T \varphi\\
    \pathassignfin \models_T \exists \pi \ldot \varphi & \text{if } \exists t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi \\
    \pathassignfin \models_T \forall \pi \ldot \varphi & \text{if } \forall t \in T \text{ holds that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%\subsection{$\forall^2 \hyperltl$}
%As our constraint based monitoring approach will only be concerned with $\forall^2 \hyperltl$ formulas, we introduce special notation, which will help us down the road.
%\begin{definition}
%
The hyperproperty represented by a $\hyperltl$ formula $\varphi$, denoted by $\hlang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%Due to duality of $\LTLuntil$/$\LTLrelease$, $\LTLnext$/$\LTLweaknext$, $\exists$/$\forall$, and the standard Boolean operators, every HyperLTL formula $\varphi$ can be transformed into negation normal form~(NNF), i.e., for every $\varphi$ there is some $\psi$ in negation normal form such that for all $\pathassignfin$ and $T$ it holds that $\pathassignfin \models_T \varphi$ if, and only if, $\pathassignfin \models_T \psi$.
%
%The standard LTL semantic, written $t \modelsltlfin \varphi$, for some LTL formula $\varphi$ is equal to $\set{ \pi \mapsto t }_\mathit{fin} \models_\emptyset \varphi'$, where $\varphi'$ is derived from $\varphi$ by replacing every proposition $p \in \mathit{AP}$ by $p_\pi$.


==> old/submission 3/runtime-verification.tex <==
%===============================================================================
\section{Runtime Verification of Hyperproperties with $\tool$}
%===============================================================================
\label{sec:rvhyper}
%Since Hyperproperties relate multiple system executions to each other, $\tool$ necessarily processes (and stores) multiple runs of a system.
%For example, previous recorded sessions in a dating app or recorded daily behavior of a smart home.
%Monitoring a system against hyperproperties, such as information-flow policies, is essential if a user suspects that private information might be inferred from notwithstanding behavior of a single system run. For example, \emph{observational determinism} is a general information-flow policy that can be monitored with $\tool$. It states that low-security outputs may not depend on high-security inputs.
In this section, we present an overview over $\tool$, before describing the implementation setup, present the monitoring algorithm, and discuss our optimization techniques.

The input of $\tool$ is given as a universally quantified HyperLTL formula and, in addition, the observed behavior of the system under consideration.
The observed behavior is represented as a trace set $T$, where each $t \in T$ represents a previously observed execution of the system to monitor.
%
$\tool$ can therefore detect violations of every monitorable $k$-safety hyperproperty (see~\cite{journals/fmsd/FinkbeinerH19} for an extensive study of monitorability of hyperproperties).
If $\tool$ detects that the system violates the hyperproperty, it outputs a counter example, i.e, a $k$-ary tuple of traces, where $k$ is the number of quantifiers in the HyperLTL formula.
%that make the monitoring of hyperproperties (despite its theoretical unbounded memory consumption) feasible in practice.
%\subsection{Specification}
%The input specification of $\tool$ is given in $\hyperltl$, which is a temporal logic for specifying hyperproperties.
%It extends $\ltl$ by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
%The set of trace variables is $\pathvars$.
%Formulas in $\hyperltl$ are given by the grammar
%\begin{align*}
%\varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
%\psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
%\end{align*}
%where $a \in \ap$ and $\pi \in \pathvars$.
%%
%%The formal semantics is given in Appendix~\ref{appendix:hyperltl}.
%The finite trace semantics for $\hyperltl$ is based on the finite trace semantics of LTL.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
%Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
%$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
%\[
%t[i,j] = \begin{cases}
%\epsilon & \text{if } i \geq |t|\\
%t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
%\end{cases}
%\]
%\begin{equation*}
%\begin{array}{ll}
%\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
%\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
%\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
%\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
%\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
%\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
%\end{array}
%\end{equation*}
%For example, above mentioned observational determinism can be formalized as the HyperLTL formula
%$\forall \pi \ldot \forall \pi' \ldot (O_\pi = O_{\pi'}) \WUntil (I_\pi \not = I_{\pi'})$, where $\WUntil$ is the weak version of $\Until$.
%
%While earlier work on $\hyperltl$~\cite{conf/cav/FinkbeinerRS15} has focused on model checking, recently runtime verification methods have been proposed as a complementation~\cite{conf/csfw/AgrawalB16,conf/rv/FinkbeinerHST17}.
%$\tool$ also supports the verification workflow by providing a method to test and develop $\hyperltl$ specifications: Specifications can be checked on sample traces without the need for a complete model.
%Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning~\todo{passt hier nicht?}.

\subsection{Implementation Details}
$\tool$\footnote{The implementation is available at \url{https://react.uni-saarland.de/tools/rvhyper/}.} is written in C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}.
It uses \emph{spot}~\cite{duret.16.atva2} for building the deterministic monitor automata and the \emph{Buddy} BDD library for handling symbolic constraints.
We use the $\hyperltl$ satisfiability solver $\eahyper$~\cite{conf/cav/FinkbeinerHS17,conf/concur/FinkbeinerH16} to determine whether the input formula is reflexive, symmetric, or transitive.
Depending on those results, we omit redundant tuples in the monitoring algorithm.

%-------------------------------------------------------------------------------
\subsection{Online Monitoring Algorithm}
%-------------------------------------------------------------------------------

For the online algorithm, we use standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.
Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0, F)$ is a tuple of
a finite alphabet $\Sigma = 2^{(\ap \times \pathvars)}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \hookrightarrow Q$,
a designated initial state $q_0 \in Q$, and
a set of accepting states $F \subseteq Q$.
The instantiated automaton runs in parallel over traces in $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
\delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted, if there is a run on $\monitor$ that ends in an accepting state.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over trace variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}  \label{ex:obsdet-monitor}
  As an example formula, consider again the observational determinism formula introduced in the introduction:
  \begin{equation*}
    \forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
  \end{equation*}
  The corresponding monitor template is depicted in Fig.~\ref{fig:monitor-template}.
\end{example}
\begin{figure}[t]
	\centering
 \begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.9]
 \node[state,initial,initial text=,accepting] (init) {$q_0$};
 \node[state,below left=1.3 and 1.5 of init,accepting] (accepting) {$q_\top$};
 \node[state,black!50,below right=1.3 and 1.5 of init] (rejecting) {$q_\bot$};
 
 \draw (init) edge[loop right] node[swap] {$o_\pi = o_{\pi'} \land i_\pi = i_{\pi'}$} ()
       (init) edge node {$i_\pi \neq i_{\pi'}$} (accepting)
       (init) edge[black!50] node[near end] {$o_\pi \neq o_{\pi'} \land i_\pi = i_{\pi'}$} (rejecting)
       (accepting) edge[loop right] node {$\top$} (accepting)
       (rejecting) edge[loop right,black!50] node {$\top$} (rejecting)
 ;
 \end{tikzpicture}
	\caption{Visualization of a monitor template corresponding to the formula given in Example~\ref{ex:obsdet-monitor}. We use a symbolic representation of the transition function $\delta$. For illustration reasons, we depict a sink rejecting state $q_\bot$.}
	\label{fig:monitor-template}
\end{figure}

%\paragraph{Online Algorithm.}~\todo{adept arbitarily formulas}
The algorithm for monitoring $\hyperltl$ formulas when traces are given sequentially to the monitor is presented in Algorithm~\ref{alg:algorithms-sequential}.
%The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, the algorithm accepts new traces and afterwards proceeds with the pace of the incoming stream.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever the current trace $t$ progresses, we progress every tuple $(t_1,\ldots,t_n)$ that contains $t$ with one of the following outcomes:
\begin{enumerate}
  \item One of the traces $t_1,\ldots,t_n$ may have ended, thus, we check if the monitor is in an accepting state and report a violation if this is not the case.
  \item There is a successor state in the monitor, thus we update $S$.
  \item There is no successor state, hence, we report a violation.
\end{enumerate}
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $\vec{t} \in (T \cup \set{t})^n$ containing the new trace $t$.%~\todo{explain notion of instantiation?}
			\begin{algorithm*}[t]
				\SetKwInOut{Input}{input}
				\SetKwInOut{Output}{output}
				\SetAlgoLined
				%\KwResult{Write here the result }
				\Input{$\forall^n$ HyperLTL formula $\varphi$}
				\Output{satisfied or $n$-ary tuple witnessing violation}
				\BlankLine
				$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
				$T \gets \emptyset$\;
				$S: T^n \rightarrow Q$ \quad // initially empty\;
				$t$  \quad // container for the subsequently incoming event traces
				\BlankLine
				\While{there is a new event trace}{
                  $t \gets \epsilon$ \quad // initialize empty trace\;
                  \For(init $S$ for every new tuple $\vec{t}$){$\vec{t} \in ((T \cup \set{t})^n \setminus T^n)$}{
    				$S(\vec{t}) \gets q_0$\;
    			  }
                  \While{$p \in \Sigma$ is a new input event}{
						$t' \gets t~p$ \quad // append $p$ to $t$\;
                        \For(// progress every state in $S$) {$( (t_1,\ldots,t_n), q) \in S$ where $t \in \{t_1,\ldots,t_n\}$}{
                            \uIf(// some trace ended){$\exists t^* \in \{t_1,\ldots,t_n\} \ldot \card{t^*} < \card{t}$}{
                             \eIf {$q \in F$} {
                              remove $(t_1,\ldots,t_n)$ from $S$\;
                              \textbf{continue}\;
                             } { \Return violation and witnessing tuple $(t_1,\ldots,t_n)$\;}
                          }
                          $\vec{t} \gets (t_1,\ldots,t_n)$, where $t_i$ is replaced with $t'$, for each $t_i = t$\;
                          \uIf {$\delta(q, \bigcup_{i=1}^n \bigcup_{a \in \vec{t}(i)[\card{t'}-1]} \set{ (a, \pi_i) }) = q'$} {
        				     $S(\vec{t}) \gets q'$\;
        				  }
        				  \Else{
        				    \Return violation and witnessing tuple $\vec{t}$\;
        				  }
        				}
						$t \gets t'$ \quad // re-assign $t$\;
				  } 
				  $T \gets T \cup \set{t}$\; \quad //add $t$ to already seen traces
				}
				\Return satisfied\;
				\BlankLine
	\caption{Online monitoring algorithm for $\forall^n \hyperltl$: The algorithm subsequently reads event traces and monitors them against already seen traces. Already seen traces are stored in $T$ before continuing with a new event trace.}
	\label{alg:algorithms-sequential}
			\end{algorithm*}

\begin{example} \label{ex:obsdet-algorithm}
  We continue \autoref{ex:obsdet-monitor} by showing how the algorithm progresses on the given formula.
  Assume for the sake of readability that we have a single input proposition $i$ and a single output proposition $o$.
  Furthermore, assume that we have already seen the trace $t_0 = \set{i}\set{i,o}\set{o}$, that is, $T = \set{t_0}$ and $S(t_0,t_0) = q_0$.
  We now show how the algorithm continues with a fresh trace $t_1$.
  In lines 6--8 we add the pairs $(t_0,t_1)$, $(t_0,t_1)$, and $(t_1,t_1)$ with the initial state $q_0$ to $S$.
  Let $p = \set{i}$ be the first input proposition, thus, $t_1 = \set{i}$.
  Since $t_0[0] = t_1[0]$, the monitor remains in $q_0$ for every tuple.
  Let $p = \set{i}$ be the next input proposition, thus, $t_1 = \set{i}\set{i}$.
  Consider the tuple $(t_0,t_1)$.
  As $t_0[1]$ and $t_1[1]$ are equal with respect to $i$ but differ in $o$, the monitor progresses to the rejecting state $q_\bot$ and the algorithm terminates by reporting the violation.
  If, the previous input proposition is $p = \set{}$, both tuples, $(t_0,t_1)$ and $(t_1,t_0)$ would progress to the accepting sink state $q_\top$ as the input proposition is different to $t_0[1]$.
  Assume two more inputs, e.g., $t_1 = \set{i}\set{i}\set{}\set{}$, then the pairs $(t_0,t_0)$, $(t_0,t_1)$, and $(t_1,t_0)$ are removed from $S$ as $t_1$ is strict longer than $t_0$.
\end{example}


\section{Optimizations}
\label{sec:opt}
In this section, we present three optimizations implemented in $\tool$, which, as we will see in the evaluation section, are necessary to make the automata-based monitoring approach feasible in practice. We begin by explaining a \emph{specification analysis}, which is a preprocessing step that exploits properties of the specification to reduce the algorithmic workload. In the subsequent section, we show how $\tool$ tackles the problem of potentially unbounded memory consumption: We recap the \emph{trace analysis}, which was so far the only storage optimization implemented in $\tool$. We then provide a novel storage optimization technique based on prefix-trees, so-called \emph{tries}, to exploit partial equality of the given traces, which the trace analysis neglected so far.
%-------------------------------------------------------------------------------
\subsection{Decreasing Running Time}
%-------------------------------------------------------------------------------

In the example execution in \autoref{ex:obsdet-algorithm} we have seen that the algorithm had to do more work than necessary to monitor observational determinism.
For example, a tuple $(t,t)$ for some trace $t$ cannot violate observational determinism as the traces are equal.
Further, from the pairs $(t,t')$ and $(t',t)$ for some traces $t$ and $t'$, we only need to check one of them as a violation in one of them implies the violation in the other pair.
We can automatically check for such conditions and, thus, omit unnecessary work.

$\tool$ utilizes the HyperLTL satisfiability solver EAHyper~\cite{conf/concur/FinkbeinerH16,conf/cav/FinkbeinerHS17} for its \emph{specification analysis}, which is a preprocessing step that analyzes the HyperLTL formula under consideration.
EAHyper can detect whether a formula is (1) \emph{symmetric}, i.e., we halve the number of instantiated monitors, (2) \emph{transitive}, i.e, we reduce the number of instantiated monitors to two, or (3) \emph{reflexive}, i.e., we can omit the self comparison of traces.

\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:symmetry}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	%Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_n \ldot \psi$, where $\psi$ is an $\ltl$ formula over trace variables $\{\pi_1, \dots, \pi_n\}$.
	%For an assignment $\pathassign$ and an permutation $\sigma : \Pi \to \Pi$, we define $\pathassign \circ \sigma$, such that $(\pathassign \circ \sigma)(\pi) = \pathassign(\sigma(\pi))$ for every $\pi \in \Pi$.
	We say $\varphi$ is invariant under trace variable permutation $\sigma : \pathvars \to \pathvars$, if for any set of traces $T \subseteq \Sigma^{\omega}$ and any assignment $\pathassign : \pathvars \to T$, $(\emptyset, \pathassign, 0) \models \psi \Leftrightarrow (\emptyset, \pathassign \circ \sigma, 0) \models \psi$.
	We say $\varphi$ is symmetric, if it is invariant under every trace variable permutation in $\pathvars$.
\end{definition}
Symmetry is particular interesting since many information flow policies satisfy this property. Consider, for example, observational determinism: 
$
\forall \pi\ldot \forall \pi'\ldot (o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'}).
$ %\todo{different notation than in \autoref{ex:obsdet-algorithm} and intro.}
$\tool$ detects symmetry by translating this formula to a formula that is unsatisfiable if there exists no set of traces for which every trace pair violates the symmetry condition:
$
\exists \pi\ldot \exists \pi'\ldot \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big) \nleftrightarrow \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big)
$.
If the resulting formula turns out to be unsatisfiable, $\tool$ omits the symmetric instantiations of the monitor automaton.
%, which turns out to be, especially in combination with $\tool$s \emph{trace analysis}, a major optimization in practice~\cite{conf/rv/FinkbeinerHST17}.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:transitivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\set{\pi_1, \pi_2}$.
	Let $T = \set{t_1, t_2, t_3} \in \Sigma^{\omega}$ be a three-elemented set of traces.
	We define the assignment $\pathassign_{i,j} : \pathvars \to \Sigma^{\omega}$ by $\pathassign_{i,j} \coloneqq \{\pi_1 \mapsto t_i, \pi_2 \mapsto t_j\}$.
	We say $\varphi$ is transitive, if for all three-elemented sets $T$ it holds that $(\emptyset, \pathassign_{1,2}, 0) \models \psi \wedge (\emptyset, \pathassign_{2,3}, 0) \models \psi \rightarrow (\emptyset, \pathassign_{1,3}, 0) \models \psi$.
\end{definition}
While symmetric HyperLTL formulas allow us to prune half of the monitor instances, transitivity of a HyperLTL formula has an even larger impact on the required memory. Equality, i.e, $\forall \pi. \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$, for example, is transitive and symmetric and allows us to reduce the number of monitor instances to one, since we can check equality against any reference trace.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:reflexivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	We say $\varphi$ is reflexive, if for any trace $t \in \Sigma^{\omega}$ and the corresponding assignment $\pathassign : \pathvars \to \{t\}$, $(\emptyset, \pathassign, 0) \models \psi$.
\end{definition}
Lastly, if a formula is reflexive, $\tool$ omits the composition of a trace with itself during the monitoring process.
%Both $\hyperltl$ formulas considered in this section, $\mathit{ObsDet}$ and $\mathit{EQ}$, are reflexive.
For example, equality and observational determinism have reflexive HyperLTL formulas.

\begin{example}
  Consider again the observational determinism formula from \autoref{ex:obsdet-monitor}.
  We have seen that this formula is both, reflexive and symmetric, thus, we can omit those instances in the algorithm.  
\end{example}


%-------------------------------------------------------------------------------
\subsection{Optimizing Trace Storage}
\label{sec:trie}
%-------------------------------------------------------------------------------

The main obstacle in monitoring hyperproperties is the potentially unbounded space consumption.
So far, RVHyper employed a \emph{trace analysis} technique to detect redundant traces, with respect to a given HyperLTL formula, i.e., traces that can be safely discarded without losing any information and without losing the ability to return a counter example.

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given a HyperLTL formula $\varphi$, a trace set $T$ and an arbitrary $t \in \traces$, we say that $t$ is $(T,\varphi)$-redundant if $T$ is a model of $\varphi$ if and only if $T \cup \set{t}$ is a model of $\varphi$ as well, formally
	\begin{equation*}
	\forall T' \supseteq T \ldot T' \in \hlang(\varphi) \Leftrightarrow T' \cup \{t\} \in \hlang(\varphi) \enspace.
	\end{equation*}
\end{definition}

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given $t,t' \in \Sigma^\omega$, we say $t$ \emph{dominates} $t'$ with respect to $\varphi$ (or simply $t$ \emph{dominates} $t'$ if it is clear from the context) if $t'$ is ($\{t\},\varphi$)-redundant.
\end{definition}

\begin{example}
  For observational determinism, a trace $t$ is dominated by a trace $t'$ if $\card{t} < \card{t'}$ and both traces agree on the input propositions.
\end{example}


This is efficiently implemented in $\tool$ (cf. Algorithm~\ref{alg:traceopti}) and is guaranteed to catch all redundant traces.
In our experiments~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.

The trace analysis, as it is based on a language inclusion check of the entire traces, cannot handle \emph{partial redundancy}, for example, in the case that traces have redundant prefix requirements.
This leaves room for optimization, which we address by implementing a so-called \emph{trie} data structure for managing the storage of incoming traces.

\begin{algorithm}
	%\label{alg_minimization}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\hyperltl$ formula $\varphi$, redundancy free trace set $T$, fresh trace $t$}
	\Output{redundancy free set of traces $T_\mathit{min} \subseteq T \cup \set{t}$}
	%\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}
	\BlankLine
	\ForEach{$t' \in T$}{
		\If{ $t'$ dominates $t$ }
		{
			\Return $T$\;
		}
	}
	\ForEach{$t' \in T$}{
		\If{$t$ dominates $t'$}
		{
			$T \coloneqq T \setminus \set{t'}$\;
		}
	}
	\Return $T \cup \set{t}$\;
	%\BlankLine
	\caption{Trace analysis algorithm to minimize trace storage.}
	\label{alg:traceopti}
\end{algorithm}



%In our experiments~\cite{conf/rv/FinkbeinerHST17,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.
%Ideally one wants to avoid this overhead when monitoring a trace that shares some prefixes with already seen traces.
%We implemented this idea with a so-called \emph{trie} data structure.
Tries, also known as prefix trees, describe a tree data structure, which can represent a set of words over an alphabet in a compact manner.
The root of a trie is identified with the empty word $\epsilon$, additionally each node can have several child nodes, each of which corresponds to a unique letter getting appended to the representing word of the parent node. So the set of words of a trie is identified with the set of words the leaf nodes represent.

\begin{definition}
A trie is a four tuple $(\Sigma, \Tau, \longrightarrow, \tau_0)$ consisting of
\begin{itemize}
    \item a finite alphabet $\Sigma$,
    \item a non-empty set of states $\Tau$,
    \item a transition function $\longrightarrow: \Tau \times \Sigma \rightarrow \Tau$,
    \item and a designated initial state $\tau_0 \in \Tau$ called the root.
    \end{itemize}
\end{definition}
Instead of $((\tau,a),\tau') \in \longrightarrow$ we will write $\tau \overset{a}{\longrightarrow} \tau'$ in the following.
For a trie to be of valid form we restrict $\longrightarrow$ such that, $\forall \tau,\tau' \in \Tau. |\{\tau \overset{a}{\longrightarrow} \tau'| a \in \Sigma\}| \leq 1$.

%Additionally to our analysis phases it would be helpful if we could use some insights from trace analysis 


%As mentioned before, storing the incoming traces succinctly is a major concern in monitoring hyperproperties.
In our case the alphabet would be the set of propositions used in the specification, and the word built by the trie represents the traces. %build from it are what we call traces.
%Tries provide a 
Instead of storing each trace individually, we store all of them in one trie structure, branching only in case of deviation. This means equal prefixes only have to be stored once.
Besides the obvious benefits for memory, we also can make use of the maintained trie data structure to improve the runtime of our monitoring algorithms. As traces with same prefixes end up corresponding to the same path in the trie, we only have to instantiate the monitor automaton as much as the trie contains branches.
%O(size branches) times.
\begin{example}
	Consider the following traces of length $6$ over the alphabet $2^{\{i,o\}}$:
	\begin{itemize}
		\item
		$t_1: \{\set{i},\set{i,o},\set{i},\set{i},\set{i},\set{i,o} \}$
		\item
		$t_2: \{\set{i}, \set{i,o}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_3: \{\set{i}, \set{i}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_4: \{\set{i}, \set{i}, \set{}, \set{} , \set{}, \set{}\}$
	\end{itemize}
After processing the traces sequentially, the resulting trie looks as follows:

\vspace{1ex}

\begin{tikzpicture}[sibling distance=7em, level distance = 30pt,
every node/.style = {shape=circle,
	draw, align=center, minimum size = 0.9cm, inner sep = 0pt},
level 1/.style = {sibling distance = 10em},
level 2/.style = {sibling distance = 5em},
level 5/.style = {sibling distance = 5em}]
\node {$\{i\}$}
child { node {$\{i\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} } } } } 
	child { node {$\{ \}$}  
		child { node {$\{ \}$} 
			child { node {$\{ \}$}
				child { node {$\{ \}$} } } } } }
child { node {$\{i,o\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} }
				child { node {$\{i,o\}$} } } } } };
\end{tikzpicture}
\end{example}

\subsection{Trie-based Monitoring Algorithm}

We depict a trie-based offline monitoring algorithm in Fig.~\ref{alg:trie-offline}.
For the sake of readability, we assume that there are as many traces as universal quantifier, that we progress through all traces in parallel, and that all traces have the same length.
This is merely a simplification in the presentation, one can build the trie in a sequential fashion for online monitoring by a slight modification of the presented algorithm.

Without using tries our monitoring algorithm was based on instantiating the deterministic monitor template $\monitor_\varphi$ with tuples of traces. Now we instantiate $\monitor_\varphi$ with tuples of tries. Initially we only have to create the single instance having the the root of our trie.

\begin{comment}
	\begin{algorithm*}
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
		$S: \Tau^n \rightarrow Q$, \quad $E: \Tau^n \rightarrow \Sigma$\;
		$\tau_0 \coloneqq $\texttt{ new\_trie()}\;
		%$\mathbf{i} \coloneqq \underbrace{(\tau_0,\ldots,\tau_0)}{n \text{times}}$\;
		%$I \coloneqq \{\mathbf{i}\}$\;
		\BlankLine
		$i_0 \in \{ \tau_0 \}^n$\;
		$S(i_0) = q_0$\;
		\While{there is a new trace}{
			$I \leftarrow \{i_0\}$\;
			$\tau \leftarrow \tau_0$\;
			\While{$p \in \Sigma$ is a new event}{
				$\tau' \leftarrow$ \texttt{add\_child($\tau,p$)} //\texttt{assert($E(\tau')==p$)}\;
				$I_n \leftarrow \emptyset$\;
				\ForEach{$i \in I$}{
					$I' \leftarrow \{i' \mid i(j) \rightarrow i'(j), a \in \Sigma, 1 \leq j \leq n\}$\;
					$I' \leftarrow \{i' \in I' \mid \exists k. i'(k) = \tau'\}$\;
					\ForEach{$i' \in I'$}{
						\uIf{$\delta(S(i), \cup_{j=1}^n \cup_{a\in E(i'(j))} \{(a,\pi_j)\}) = q$}{
							$S(i') = q$\;
						}
						\Else{
							\Return(\texttt{rooted\_seq($i'(1)$)}, \ldots, \texttt{rooted\_seq($i'(n)$)})\;
						}
					}
				}
			}
		}
		%\While{$\mathbf{p} \leftarrow$ new elements (in a forward fashion)}{
		%	\For{$1 \leq j \leq n$}{
		%		$\mathbf{i}(j) \leftarrow $\texttt{add\_value($\mathbf{i}(j)$, $j$, $\mathbf{p}(j)$)}\;
		%	}
		%	$I \leftarrow \bigcup_{\mathbf{i} \in I} \{(i'_1,\ldots, i'_n)| \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n\}$\;
		%	\ForEach{$\mathbf{i} \in I$}{
		%		%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
		%		progress every state in $S$ according to $\delta$\;
		%		\If{violation in $M_\varphi$}{
		%			$t \coloneqq ($\texttt{rooted\_sequence($i(1)$)}$,\ldots,$\texttt{rooted\_sequence($i(n)$)}$)$\;
		%			\Return witnessing tuple $t^n$\;
		%		}
		%	}
		%}
		%\Return satisfied\;
		%\BlankLine
	\caption{Online algorithm using trie data structure.}
	\label{alg:trie-online-parallel}
	\end{algorithm*}
\end{comment}
	\begin{algorithm*}[t]
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\\
		$S: \Tau^n \rightarrow Q$\\
		$\tau_0 \coloneqq $\texttt{new\_trie()}\\
		$\mathbf{i} \coloneqq (\tau_0,\ldots,\tau_0) \in \Tau^n$\\
		$I \coloneqq \{\mathbf{i}\}$  \quad // set of not-yet terminated branches\\
		\BlankLine
		\While{$\mathbf{p} \leftarrow$ new event (in $\Sigma^n$)}{
			\For{$1 \leq j \leq n$}{
				$\mathbf{i}(j) \leftarrow $\texttt{add\_child($\mathbf{i}(j)$, $\mathbf{p}(j)$)} \quad // add child with value $\vec{p}(j)$ to $\vec{i}(j)$ if needed \\
			}
			// update set of active branches\\
			$I \leftarrow \bigcup_{\mathbf{i} \in I} \set{ (i'_1,\ldots, i'_n) \mid \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n }$\\
			\ForEach{$\mathbf{i} \in I$}{
				%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
				progress every state in $S$ according to $\delta$\;
				\If{violation in $\monitor_\varphi$}{
				    // return sequence from root to $\vec{i}$\\
					$t \gets ($\texttt{rooted\_sequence($\vec{i}(1)$)}$,\ldots,$\texttt{rooted\_sequence($\vec{i}(n)$)}$)$\\
					\Return witnessing tuple $t^n$\\
				}
			}
		}
		\Return satisfied if $\forall \vec{i} \in I \ldots S(\vec{i}) \in F$ else violation\\
		\BlankLine
	\caption{Offline algorithm using trie data structure.}
	\label{alg:trie-offline}
\end{algorithm*}

The trie-based algorithm has much in common with its previously discussed trace-based counterpart. Initially, we have to build the deterministic monitor automaton $\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F)$.
We instantiate the monitor with a fresh trie root $\tau_0$.
A mapping from trie instantiations to a state in $\monitor_\varphi$ $S: \Tau^n \rightarrow Q$, stores the current state of every active branch of the trie, stored in the set $I$.
For each of the incoming traces, we provide an entry in a tuple of tries $\mathbf{\tau}$, each entry gets initialized to $\tau_0$.
During the run of our algorithm these entries will get updated such that they always correspond to the word built by the traces up to this point.
For as long as there are traces left, which have not yet ended, and we have not yet detected a violation, we will proceed updating the entries in $\vec{i}$ as follows.
Having entry $\tau$ and the correspond trace sequence proceeds with $a$, if $\exists \tau' \in \Tau. \tau \overset{a}{\longrightarrow} \tau'$, we update the entry to $\tau'$ otherwise we create such a child node of $\tau$ (\texttt{add\_child} in line 8).
Creating a new node in the trie always occurs, if the prefix of the incoming trace starts to differ from already seen prefixes.
After having moved on step in our traces sequences, we have to reflect this step in our trie structure, in order for the trie-instantiated automata to correctly monitor the new propositions.
As a trie node can branch to multiple child nodes, each monitor instantiation will get replaced by the set of instantiations, where all possible child combinations of the different assigned tries are existent (update of $I$ in line 11).
Afterwards, we update $S$ in the same way as in Algorithm~\ref{alg:traceopti}, thus, we omit algorithmic details here.
%This can be efficiently implemented as we essential fork the monitor instantiation for the different branches in the trie.
%After this preprocessing we are able to update our mapping $S$ according to $\delta$.
If a violation is detected here, that is there is no transition in the monitor corresponding to $\vec{i}$, we will return the corresponding counter example as a tuple of traces, as those can get reconstructed by stepping upwards in the tries of $\vec{i}$.
%Note that the sequential algorithm is derived from the parallel one by progressing one trace at a time and additionally when forking the monitor instantiations, only those new instantiation have to be kept, which contain the (single) trie in $\mathbf{\tau}$ at least once. 
If the traces end, we check if every open branch $\vec{i} \in I$ is in an accepting state.

%\subsection{Tries and Trace Analysis in Combination}
%\todo{TODO}


==> old/submission 3/tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> old/submission 3/tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/submission/commands.tex <==

% Common math
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{{\langle #1 \rangle}}
\newcommand{\card}[1]{{|#1|}}
\newcommand{\ldot}{\mathpunct{.}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\dom}{\mathrm{dom}}

% Languages
\newcommand{\good}{\mathit{good}}
\newcommand{\bad}{\mathit{bad}}
\newcommand{\winning}{\mathit{winning}}
\newcommand{\losing}{\mathit{losing}}
\newcommand{\hlang}{\mathcal{H}}

% Complexity classes
\newcommand{\pspace}{\textsc{PSpace}}

% Logics
\newcommand{\ltl}{\text{LTL}}
\newcommand{\hyperltl}{\text{HyperLTL}}
\newcommand{\secltl}{\text{SecLTL}}


\newcommand{\lang}{\mathcal{L}}
\newcommand{\ap}{\text{AP}}
\renewcommand{\models}{\vDash}
\newcommand{\nmodels}{\nvDash}
\newcommand{\traces}{\mathit{TR}}

% Traces
\newcommand{\pref}{\preceq}
\newcommand{\tracebox}[1]{\framebox[4.5ex][l]{#1}}
\newcommand{\pctracebox}[1]{\framebox[4.5ex][l]{#1}}

% LTL
\newcommand{\U}{\Until}
\newcommand{\X}{\Next}
\newcommand{\G}{\Globally}
\newcommand{\F}{\Eventually}
\newcommand{\R}{\Release}
\newcommand{\W}{\WUntil}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

% HyperLTL
\newcommand{\pathassign}{\Pi}
\newcommand{\pathvars}{\mathcal{V}}
\newcommand{\pathassignfin}{\Pi_\mathit{fin}}

% Monitoring
\newcommand{\monitor}{\mathcal{M}}
\newcommand{\tool}{\text{RVHyper}}

% Tools
\newcommand{\eahyper}{\text{EAHyper}}

% TODOs and Marking
\newcommand{\todo}[1]{\marginpar{TODO}\textcolor{red}{#1}}
%\newcommand{\tbchecked}[1]{\marginpar{To be checked}\textcolor{blue}{#1}}

\newcommand{\ninfluences}{\not\leadsto}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> old/submission/encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> old/submission/encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> old/submission/encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> old/submission/encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> old/submission/enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> old/submission/enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> old/submission/introduction.tex <==
%===============================================================================
\section{Introduction}
\label{sec:intro}
%===============================================================================

\emph{Hyperproperties}~\cite{journals/jcs/ClarksonS10} are widely studied in (but not limited to) the context of secure information-flow control. They generalize trace properties in that they not only check the correctness of \emph{individual} computation traces in isolation, but relate \emph{multiple} computation traces to each other.
%Hyperproperties are widely studied in the context of information-flow control.
%Information-flow policies cannot be monitored with standard runtime verification tools
Examples include information-flow policies, such as observational determinism~\cite{journals/jcs/McLean92,conf/sp/Roscoe95,conf/csfw/ZdancewicM03}, (quantitative) noninterference~\cite{journals/jcs/McLean92,DBLP:conf/fossacs/Smith09,DBLP:conf/esorics/YasuokaT10} as well as symmetry~\cite{conf/cav/FinkbeinerRS15} and spurious dependencies in hardware designs~\cite{conf/tacas/FinkbeinerHST18}, error correcting codes~\cite{conf/cav/FinkbeinerRS15}, and anti-doping of automotive software~\cite{conf/esop/DArgenioBBFH17}.
%The application of hyperproperties 

In this article, we present the monitoring approach implemented in the latest version of $\tool$, an automata-based monitoring tool for hyperproperties~\cite{journals/fmsd/FinkbeinerH19}.
In dynamic verification of hyperproperties, efficient and light-weight monitoring techniques are instrumented in systems, which are usually far beyond the scope of static verification approaches. By doing so, countermeasures are enacted before, for example, irreparable information leaks happen.
%
A runtime verification tool for hyperproperties is in particular useful if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
$\tool$ also supports the verification workflow by providing a method to test and develop specifications: Specifications can be checked on sample traces without the need for a complete model.
Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning.

%However, standard runtime verification tools~\todo{cite} that only consider computations in isolation, can, in general, not monitor such properties.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The input of $\tool$ is given in the temporal logic $\hyperltl$~\cite{conf/post/ClarksonFKMRS14}, which expresses temporal hyperproperties, by extending linear-time temporal logic with \emph{explicit} trace quantification (see~\cite{conf/lics/CoenenFHH19} for a recent study of hyperlogics).
HyperLTL has been used extensively to specify hyperproperties of practical interest (e.g~\cite{conf/cav/FinkbeinerRS15,journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18,conf/cav/FinkbeinerHT18,conf/cav/FinkbeinerHLST18,conf/esop/DArgenioBBFH17}).
For example, observational determinism is expressed as the following formula:
$$
\forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
$$
stating that every trace pair $\pi,\pi'$ has to agree on the output as long as they agree on the inputs as well.
%$\hyperltl$ has been used to specify a variety of information-flow and security properties~\todo{cite}.
When detecting a violation, $\tool$ outputs a counter example, which is a set of computations that does not satisfy the input formula.
%Examples include classical properties like non-interference and observational determinism, as well as quantitative information-flow properties, symmetries in hardware designs, and formally verified error correcting codes~\cite{conf/cav/FinkbeinerRS15}.

Efficient model checking, synthesis and satisfiability checking tools for HyperLTL already exist~\cite{conf/cav/FinkbeinerRS15,conf/cav/FinkbeinerHT18,conf/concur/FinkbeinerH16,DBLP:conf/atva/FinkbeinerHH18,conf/cav/FinkbeinerHS17,conf/cav/FinkbeinerHLST18}. Implementing an efficient runtime verification tool for HyperLTL specifications is, despite recent theoretical progress~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17,conf/csfw/BonakdarpourF18,conf/isola/BonakdarpourSS18,conf/tacas/HahnST19,journals/fmsd/FinkbeinerH19} difficult:
%
%This is because monitoring hyperproperties is difficult:
In principle, the monitor not only needs to process every observed trace, but must also \emph{store} every trace observed so far, so that future traces can be compared with the traces seen so far.
%On the other hand, a runtime verification tool for hyperproperties is certainly useful, in particular if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
%Furthermore, monitoring hyperproperties can be used to simulation plays a significant role in designing specifications and, for example, hardware.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The previous version of $\tool$ tackles this challenging problem by implementing two optimizations~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}: a \emph{specification analysis} to detect exploitable properties of a hyperproperty, such as \emph{symmetry} and a \emph{trace analysis}, which detects all redundant traces that can be omitted during the monitoring process. The trace analysis, which is based on a language inclusion check, can, however, only analyze and prune \emph{entire} traces.
For example, consider the traces $t_1 = \{a\}\{a\}\{\}$ and $t_2 = \{a\}\{\}\{a\}$ of length $3$ and the HyperLTL formula $\forall \pi. \forall \pi'. \G ( a_\pi \rightarrow \neg b_{\pi'} )$. Neither $t_1$ nor $t_2$ is dominated by the other trace, in the sense of the trace analysis, i.e., that one of the traces poses strictly less requirements on future traces~\cite{journals/fmsd/FinkbeinerH19}.
The traces, however, are equal on the first position.
% storage optimization technique that arranges the traces in a tree-like structure.
%This leaves room for optimization, which we address in this article.
This provides an opportunity for optimization, which our new approach exploits.
We introduce a novel trace storage technique (that also has massive impact on the running time), such that $\tool$ can also handle \emph{partially equal} traces by storing them in a tree structure.

We evaluate $\tool$ on existing benchmarks such as classical information-flow security by checking for violations of noninterference or monitoring error-resistant encoder. $\hyperltl$ is, however, not limited to security policies. As an example of such an application beyond security, we show how $\tool$ can be used to detect spurious dependencies in hardware designs.

\paragraph{Structure of this Article.}

The remainder of this article is structured as follows.
We begin by giving preliminaries on $\hyperltl$, its finite trace semantics and notation in Section~\ref{sec:prelims}. In Section~\ref{sec:rvhyper}, we present automata-based monitoring approach implemented in $\tool$, before discussing optimizations in Section~\ref{sec:opt} that make the monitoring feasible in practice. In Section~\ref{sec:eval}, we evaluate $\tool$ with a focus on the novel storage optimization technique using our tree data structure.%: we show $\tool$s performance on a benchmark

This is a revised and extended version of a paper that appeared at TACAS~2018~\cite{conf/tacas/FinkbeinerHST18}.
Our contribution and extension compared to~\cite{conf/tacas/FinkbeinerHST18} is the inclusion of a new trace storage optimization technique presented in Sec.~\ref{sec:trie} and an extended evaluation in Sec.~\ref{sec:eval}.

\paragraph{Related Work.}

The temporal logic $\hyperltl$ was introduced to model check security properties of reactive systems~\cite{conf/post/ClarksonFKMRS14,conf/cav/FinkbeinerRS15}.
For one of its predecessors, $\secltl$~\cite{conf/vmcai/DimitrovaFKRS12}, there has been a proposal for a white box monitoring approach~\cite{conf/isola/DimitrovaFR12} based on alternating automata.
The problem of monitoring $\hyperltl$ has been considered before~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17}.
Agrawal and Bonakdarpour~\cite{conf/csfw/AgrawalB16} were the first to study the monitoring problem of HyperLTL for the sequential model. They gave a syntactic characterization of monitorable $\hyperltl$ formulas. They present a first monitoring algorithm based on a progression logic expressing trace interdependencies and the composition of an LTL$_3$ monitor.
A first constraint-based approach has been outlined in~\cite{conf/tacas/BrettSB17}, which works for a subclass of HyperLTL specifications. The idea is to identify a set of propositions of interest and store corresponding constraints.
A constraint-based algorithm for the complete fragment of $\forall^2$ HyperLTL formulas has been proposed in~\cite{conf/tacas/HahnST19}. The algorithms rewrites a HyperLTL formula and an incoming event into a constraint composed of a plain LTL requirement as well as a HyperLTL requirement.
An constraint system is built incrementally: the HyperLTL part is encoded with variables, which will be incrementally defined with more incoming events of a trace.
Like with our monitoring algorithm, they do not have access to the implementation (black box), but in contrast to our work, they do not provide witnessing traces as a monitor verdict.

In~\cite{conf/csfw/BonakdarpourF18}, the authors study the complexity of monitoring hyperproperties. They show that the form and size of the input, as well as the formula have a significant impact on the feasibility of the monitoring process. They differentiate between several input forms and study their complexity: a set of linear traces, tree-shaped Kripke structures, and acyclic Kripke structures. For acyclic structures and alternation-free HyperLTL formulas, the problems complexity gets as low as NC.
In~\cite{conf/isola/BonakdarpourSS18}, the authors discuss examples where static analysis can be combined with runtime verification techniques to monitor HyperLTL formulas beyond the alternation-free fragment. They discuss the challenges in monitoring formulas beyond this fragment and lay the foundations towards a general method.

For certain information flow policies, like non-interference and some extensions, dynamic enforcement mechanisms have been proposed.
Techniques for the enforcement of information flow policies include tracking dependencies at the hardware level~\cite{conf/asplos/SuhLZD04}, language-based monitors~\cite{journals/jsac/SabelfeldM03,conf/csfw/AskarovS09,conf/pldi/AustinF10,conf/csfw/VanhoefGDPR14,conf/post/BichhawatRGH14}, and abstraction-based dependency tracking~\cite{conf/asian/GuernicBJS06,conf/essos/KovacsS12,conf/csfw/ChudnovKN14}.
Secure multi-execution~\cite{conf/sp/DevrieseP10} is a technique that can enforce non-interference by executing a program multiple times in different security levels.
% and by using special rules for I/O operations.
To enforce non-interference, the inputs are replaced by default values whenever a program tries to read from a higher security level.
%In this article, we are concerned with the monitorability of hyperproperties expressed in $\hyperltl$, which is able to formalize security properties beyond non-interference.

==> old/submission/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/submission/mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> old/submission/mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> old/submission/mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> old/submission/mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> old/submission/mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> old/submission/mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> old/submission/preliminaries.tex <==
%===============================================================================
\section{Preliminaries}
%===============================================================================
\label{sec:prelims}
Let $\mathit{AP}$ be a finite set of \emph{atomic propositions} and let $\Sigma = 2^\mathit{AP}$ be the corresponding \emph{alphabet}.
An infinite \emph{trace} $t \in  \Sigma^\omega$ is an infinite sequence over the alphabet.
A subset $T \subseteq \Sigma^\omega$ is called a \emph{trace property}. A \emph{hyperproperty} $H \subseteq 2^{(\Sigma^\omega)}$ is a generalization of a trace property.
A finite trace $t \in \Sigma^+$ is a finite sequence over $\Sigma$.
In the case of finite traces, $|t|$ denotes the length of a trace.
%Depending on the context, we refer to either $(2^\mathit{AP})^\omega$ or $(2^\mathit{AP})^+$ as the alphabet $\Sigma^\omega$ or $\Sigma^+$.
We use the following notation to access and manipulate traces:
Let $t$ be a trace and $i$ be a natural number.
$t[i]$ denotes the $i$-th element of $t$.
Therefore, $t[0]$ represents the first element of the trace.
Let $j$ be natural number. If $j \geq i$ and $i\leq|t|$, then
$t[i,j]$ denotes the sequence $t[i] t[i+1] \cdots t[min(j,|t|-1)]$. Otherwise it denotes the empty trace $\epsilon$.
$t[i\rangle$ denotes the suffix of $t$ starting at position $i$.
For two finite traces $s$ and $t$, we denote their concatenation by $s \cdot t$.

%\subsection{LTL}
%\paragraph{Syntax.} Linear-time Temporal Logic (LTL)~\cite{} combines the usual Boolean connectives with temporal modalities.
%\begin{alignat*}{3}
%\varphi \coloneqq ~ a ~ | ~ \neg \varphi ~ | ~ \varphi \vee \varphi ~ | ~ \LTLnext \varphi ~ | ~ \varphi \LTLuntil \varphi
%\end{alignat*}
%where $a \in \mathit{AP}$ is an atomic proposition. We use the standard derived operators \emph{eventually} $\LTLdiamond \varphi \equiv \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \equiv \neg \LTLdiamond \neg \varphi$, \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \equiv (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \varphi_1 \LTLweakuntil (\varphi_1 \wedge \varphi_2)$.
%\paragraph{Semantics.} Let $a \in \mathit{AP}$ and $t \in \Sigma^\omega$. The semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\vDash_{LTL} a \quad &&\text{iff } a \in t[0] \\
%t &\vDash_{LTL} \psi_1 \vee \psi_2 \quad &&\text{iff } t \vDash \psi_1 \vee t \models_{LTL} \psi_2\\
%t &\vDash_{LTL} \neg \psi \quad &&\text{iff } t \not \models_{LTL} \psi\\
%t &\models_{LTL} \LTLnext \psi \quad &&\text{iff } t[1\rangle \models_{LTL} \psi\\
%t &\vDash_{LTL} \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; t[i\rangle \models_{LTL} \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \models_{LTL}\psi_1
%\end{alignat*}
%\paragraph{Finite trace Semantics.} Let $a \in \mathit{AP}$ and let $t \in \Sigma^+$ be a finite trace. The finite trace semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\modelsltlfin a \quad &&\text{iff } a \in t[0] \\
%t &\modelsltlfin \psi_1 \lor \psi_2 \quad &&\text{iff } t \modelsltlfin \psi_1 \text{ or } t \modelsltlfin \psi_2\\
%t &\modelsltlfin \neg \psi \quad &&\text{iff } t \not \modelsltlfin \psi\\
%t &\modelsltlfin \LTLnext \psi \quad &&\text{iff } |t| > 1 \text{ and } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \LTLweaknext \psi \quad &&\text{iff } |t| = 1 \text{ or } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \modelsltlfin \psi_1\\
%t &\modelsltlfin \psi_1 \LTLrelease \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_1\\
%& &&\text{ and for all } 0 \leq j \leq i \text{ we have } t[j\rangle \modelsltlfin \psi_2\\
%& &&\text{ or for all } 0 \leq i < |t| \text{ we have } t[i\rangle \modelsltlfin \psi_2\\
%\end{alignat*}~\todo{finite trace semantics bauen die wir brauchen}


%-------------------------------------------------------------------------------
%\subsection{HyperLTL}
%-------------------------------------------------------------------------------

\paragraph{HyperLTL Syntax.}\label{thltl:syntax}
HyperLTL~\cite{conf/post/ClarksonFKMRS14} extends LTL with trace variables and trace quantifiers.
Let $\mathcal{V}$ be a finite set of trace variables.
The syntax of HyperLTL is given by the grammar
%\begin{figure}[h!]
\begin{alignat*}{3}
  \varphi  &{}\coloneqq ~ \forall \pi . \; \varphi \mid \exists \pi . \; \varphi \mid \psi  \\
  \psi &{}\coloneqq ~ a_{\pi} \mid \psi \wedge \psi \mid \neg \psi \mid \LTLnext \psi  \mid \psi \; \LTLuntil \;  \psi \enspace ,
\end{alignat*}
where $a \in \mathit{AP}$ is an atomic proposition and $\pi \in \mathcal{V}$ is a trace variable.
Atomic propositions are indexed by trace variables. The explicit trace quantification enables us to express properties like ``on all traces $\varphi$ must hold'', expressed by $\forall \pi \ldot \varphi$. Dually, we can express ``there exists a trace such that $\varphi$ holds'', expressed by $\exists \pi \ldot \varphi$.
We use the standard derived operators \emph{release} $\varphi \LTLrelease \psi \coloneqq \neg(\neg \varphi \LTLuntil \neg\psi)$, \emph{eventually} $\LTLdiamond \varphi \coloneqq \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \coloneqq \neg \LTLdiamond \neg \varphi$, and \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \coloneqq (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$.
As we use the finite trace semantics, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to false.
To enable duality in the finite trace setting, we additionally use the \emph{weak} next operator $\LTLweaknext \varphi$ which evaluates to true if a trace ends before the satisfaction of $\varphi$ can be determined and is defined as $\LTLweaknext \varphi \coloneqq \neg \LTLnext \neg \varphi$.
%$\LTLuntil$ denotes the \emph{until}-operator, $\LTLrelease$ the \emph{release}-operator, and we distinguish between a weak and a strong next operator, where $\LTLweaknext \varphi$ denotes the \emph{weak} version, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to true. In contrast, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator.
%$\LTLdiamond$ means that $\varphi$ holds eventually in the future, $\LTLsquare$ means that $\varphi$ holds globally, and $\LTLweakuntil$ is the \emph{weak} version of the \emph{until} operator.
%We call a HyperLTL formula alternation-free, if either all trace variables are universally quantified or all trace variables are existentially quantified.
%, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \neg (\neg\varphi_1 \LTLuntil \neg \varphi_2)$.
We call $\psi$ of a HyperLTL formula $\vec{Q}. \psi$, with an arbitrary quantifier prefix $\vec{Q}$, the \emph{body} of the formula. A HyperLTL formula $\vec{Q}. \psi$ is in the \emph{alternation-free fragment} if either $\vec{Q}$ consists solely of universal quantifiers or solely of existential quantifiers.
%We also call the $\forall^n$ fragment and $\exists^n$ fragment, with $n$ being a natural number, as the respective alternation-free fragments.
We also denote the respective alternation-free fragments as the $\forall^n$ fragment and the $\exists^n$ fragment, with $n$ being the number of quantifiers in the prefix.

%\paragraph{Semantics}\label{thltl:sem}
%%Similar to \HLTL{}, \THLTL{} defines the semantics over a set $T$ of traces.
%A HyperLTL formula can express hyperproperties.
%A trace set $T$ satisfies the hyperproperty $H$ if $T \in H$.
%The semantics of HyperLTL is formally defined over a trace assignment, which is a partial mapping $\Pi: \mathcal{V} \to T$ from trace variables to  traces.
%We write $\Pi[\pi \mapsto t]$ for the updated trace assignment, where $\pi \text{ is mapped to } t$.
%$\Pi[i\rangle$ denotes the trace assignment that is equal to $\Pi(\pi)[i\rangle$ for all $\pi \in \dom(\Pi)$.
%We write the trace set $T$ as subscript since the satisfaction depends on the trace mapping.
%%For the sake of decidability, we assume that $x < y$.
%The satisfaction of a HyperLTL formula $\varphi$ over a trace assignment $\Pi$ and a set of traces $T$, denoted by $\Pi \models_T \varphi$, is defined as follows:
%\begin{alignat*}{2}
%\Pi &\vDash_T a_{\pi} \quad &&\text{iff } a \in \Pi(\pi)[0] \\
%\Pi &\vDash_T \psi_1 \wedge \psi_2 \quad &&\text{iff } \Pi \vDash_T \psi_1 \wedge \Pi \vDash_T \psi_2\\
%\Pi &\vDash_T \neg \psi \quad &&\text{iff } \Pi \nvDash_T \psi\\
%\Pi &\vDash_T \forall \pi. \; \psi \quad &&\text{iff } \forall t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\vDash_T \exists \pi. \; \psi \quad &&\text{iff } \exists t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\models_T \LTLnext \psi \quad &&\text{iff } \Pi[1\rangle \models_T \psi\\
%\Pi &\vDash_T \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; \Pi[i\rangle \models_T \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } \Pi[j\rangle \models_T \psi_1
%\end{alignat*}
%We say a trace set T satisfies a HyperLTL formula $\varphi$ if $\emptyset \models_T \varphi$.
%If unambiguously deducible from the context, we omit $T$ and just write $\models$ instead of $\models_T$.

\paragraph{Finite Trace Semantics.}
We recap the finite trace semantics for HyperLTL~\cite{conf/tacas/BrettSB17} which is itself based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029}.
% and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029} and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a HyperLTL formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
%Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^+$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i\rangle$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i\rangle$ for all $\pi \in \dom(\pathassignfin)$.
By slight abuse of notation, we write $t \in \pathassignfin$ to access traces $t$ in the image of $\pathassignfin$.
%
The satisfaction of a HyperLTL formula $\varphi$ over a finite trace assignment $\pathassignfin$ and a set of finite traces $T$, denoted by $\pathassignfin \models_T \varphi$, is defined as follows:%~\todo{define min t in Pi fin}:
\begin{equation*}
\begin{array}{ll}
    \pathassignfin \models_T a_\pi         \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
    \pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
    \pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
    \pathassignfin \models_T \LTLnext \varphi          & \text{if } \forall t \in \pathassignfin \ldot |t|>1 \text{ and } \pathassignfin[1\rangle \models_T \varphi \\
%    \pathassignfin \models_T \LTLweaknext \varphi      & \text{if } \pathassignfin \models_T \LTLnext \varphi \\
%    & \text{or } \exists t \in \pathassignfin \text{ with } |t| \leq 1 \\
    \pathassignfin \models_T \varphi\LTLuntil\psi      & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \psi \\
    &~\hspace{1ex} \land \forall j < i \ldot \pathassignfin[j\rangle \models_T \varphi \\
%    \pathassignfin \models_T \varphi\LTLrelease\psi    & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \varphi \land \forall j \leq i \ldot \pathassignfin[j\rangle \models_T \psi \\
%   & \text{or } \forall j \leq \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[j\rangle \models_T \varphi\\
    \pathassignfin \models_T \exists \pi \ldot \varphi & \text{if } \exists t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi \\
    \pathassignfin \models_T \forall \pi \ldot \varphi & \text{if } \forall t \in T \text{ holds that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%\subsection{$\forall^2 \hyperltl$}
%As our constraint based monitoring approach will only be concerned with $\forall^2 \hyperltl$ formulas, we introduce special notation, which will help us down the road.
%\begin{definition}
%
The hyperproperty represented by a $\hyperltl$ formula $\varphi$, denoted by $\hlang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%Due to duality of $\LTLuntil$/$\LTLrelease$, $\LTLnext$/$\LTLweaknext$, $\exists$/$\forall$, and the standard Boolean operators, every HyperLTL formula $\varphi$ can be transformed into negation normal form~(NNF), i.e., for every $\varphi$ there is some $\psi$ in negation normal form such that for all $\pathassignfin$ and $T$ it holds that $\pathassignfin \models_T \varphi$ if, and only if, $\pathassignfin \models_T \psi$.
%
%The standard LTL semantic, written $t \modelsltlfin \varphi$, for some LTL formula $\varphi$ is equal to $\set{ \pi \mapsto t }_\mathit{fin} \models_\emptyset \varphi'$, where $\varphi'$ is derived from $\varphi$ by replacing every proposition $p \in \mathit{AP}$ by $p_\pi$.


==> old/submission/runtime-verification.tex <==
%===============================================================================
\section{Runtime Verification of Hyperproperties with $\tool$}
%===============================================================================
\label{sec:rvhyper}
%Since Hyperproperties relate multiple system executions to each other, $\tool$ necessarily processes (and stores) multiple runs of a system.
%For example, previous recorded sessions in a dating app or recorded daily behavior of a smart home.
%Monitoring a system against hyperproperties, such as information-flow policies, is essential if a user suspects that private information might be inferred from notwithstanding behavior of a single system run. For example, \emph{observational determinism} is a general information-flow policy that can be monitored with $\tool$. It states that low-security outputs may not depend on high-security inputs.
In this section, we present an overview over $\tool$, before describing the implementation setup, present the monitoring algorithm, and discuss our optimization techniques.

The input of $\tool$ is given as a universally quantified HyperLTL formula and, in addition, the observed behavior of the system under consideration.
The observed behavior is represented as a trace set $T$, where each $t \in T$ represents a previously observed execution of the system to monitor.
%
$\tool$ can therefore detect violations of every monitorable $k$-safety hyperproperty (see~\cite{journals/fmsd/FinkbeinerH19} for an extensive study of monitorability of hyperproperties).
If $\tool$ detects that the system violates the hyperproperty, it outputs a counter example, i.e, a $k$-ary tuple of traces, where $k$ is the number of quantifiers in the HyperLTL formula.
%that make the monitoring of hyperproperties (despite its theoretical unbounded memory consumption) feasible in practice.
%\subsection{Specification}
%The input specification of $\tool$ is given in $\hyperltl$, which is a temporal logic for specifying hyperproperties.
%It extends $\ltl$ by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
%The set of trace variables is $\pathvars$.
%Formulas in $\hyperltl$ are given by the grammar
%\begin{align*}
%\varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
%\psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
%\end{align*}
%where $a \in \ap$ and $\pi \in \pathvars$.
%%
%%The formal semantics is given in Appendix~\ref{appendix:hyperltl}.
%The finite trace semantics for $\hyperltl$ is based on the finite trace semantics of LTL.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
%Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
%$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
%\[
%t[i,j] = \begin{cases}
%\epsilon & \text{if } i \geq |t|\\
%t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
%\end{cases}
%\]
%\begin{equation*}
%\begin{array}{ll}
%\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
%\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
%\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
%\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
%\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
%\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
%\end{array}
%\end{equation*}
%For example, above mentioned observational determinism can be formalized as the HyperLTL formula
%$\forall \pi \ldot \forall \pi' \ldot (O_\pi = O_{\pi'}) \WUntil (I_\pi \not = I_{\pi'})$, where $\WUntil$ is the weak version of $\Until$.
%
%While earlier work on $\hyperltl$~\cite{conf/cav/FinkbeinerRS15} has focused on model checking, recently runtime verification methods have been proposed as a complementation~\cite{conf/csfw/AgrawalB16,conf/rv/FinkbeinerHST17}.
%$\tool$ also supports the verification workflow by providing a method to test and develop $\hyperltl$ specifications: Specifications can be checked on sample traces without the need for a complete model.
%Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning~\todo{passt hier nicht?}.

\subsection{Implementation Details}
$\tool$\footnote{The implementation is available at \url{https://react.uni-saarland.de/tools/rvhyper/}.} is written in C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}.
It uses \emph{spot}~\cite{duret.16.atva2} for building the deterministic monitor automata and the \emph{Buddy} BDD library for handling symbolic constraints.
We use the $\hyperltl$ satisfiability solver $\eahyper$~\cite{conf/cav/FinkbeinerHS17,conf/concur/FinkbeinerH16} to determine whether the input formula is reflexive, symmetric, or transitive.
Depending on those results, we omit redundant tuples in the monitoring algorithm.

%-------------------------------------------------------------------------------
\subsection{Online Monitoring Algorithm}
%-------------------------------------------------------------------------------

For the online algorithm, we use standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.
Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0, F)$ is a tuple of
a finite alphabet $\Sigma = 2^{(\ap \times \pathvars)}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \hookrightarrow Q$,
a designated initial state $q_0 \in Q$, and
a set of accepting states $F \subseteq Q$.
The instantiated automaton runs in parallel over traces in $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
\delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted, if there is a run on $\monitor$ that ends in an accepting state.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over trace variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}  \label{ex:obsdet-monitor}
  As an example formula, consider again the observational determinism formula introduced in the introduction:
  \begin{equation*}
    \forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
  \end{equation*}
  The corresponding monitor template is depicted in Fig.~\ref{fig:monitor-template}.
\end{example}
\begin{figure}[t]
	\centering
 \begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.9]
 \node[state,initial,initial text=,accepting] (init) {$q_0$};
 \node[state,below left=1.3 and 1.5 of init,accepting] (accepting) {$q_\top$};
 \node[state,black!50,below right=1.3 and 1.5 of init] (rejecting) {$q_\bot$};
 
 \draw (init) edge[loop right] node[swap] {$o_\pi = o_{\pi'} \land i_\pi = i_{\pi'}$} ()
       (init) edge node {$i_\pi \neq i_{\pi'}$} (accepting)
       (init) edge[black!50] node[near end] {$o_\pi \neq o_{\pi'} \land i_\pi = i_{\pi'}$} (rejecting)
       (accepting) edge[loop right] node {$\top$} (accepting)
       (rejecting) edge[loop right,black!50] node {$\top$} (rejecting)
 ;
 \end{tikzpicture}
	\caption{Visualization of a monitor template corresponding to the formula given in Example~\ref{ex:obsdet-monitor}. We use a symbolic representation of the transition function $\delta$. For illustration reasons, we depict a sink rejecting state $q_\bot$.}
	\label{fig:monitor-template}
\end{figure}

%\paragraph{Online Algorithm.}~\todo{adept arbitarily formulas}
The algorithm for monitoring $\hyperltl$ formulas when traces are given sequentially to the monitor is presented in Algorithm~\ref{alg:algorithms-sequential}.
%The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, the algorithm accepts new traces and afterwards proceeds with the pace of the incoming stream.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever the current trace $t$ progresses, we progress every tuple $(t_1,\ldots,t_n)$ that contains $t$ with one of the following outcomes:
\begin{enumerate}
  \item One of the traces $t_1,\ldots,t_n$ may have ended, thus, we check if the monitor is in an accepting state and report a violation if this is not the case.
  \item There is a successor state in the monitor, thus we update $S$.
  \item There is no successor state, hence, we report a violation.
\end{enumerate}
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $\vec{t} \in (T \cup \set{t})^n$ containing the new trace $t$.%~\todo{explain notion of instantiation?}
			\begin{algorithm*}[t]
				\SetKwInOut{Input}{input}
				\SetKwInOut{Output}{output}
				\SetAlgoLined
				%\KwResult{Write here the result }
				\Input{$\forall^n$ HyperLTL formula $\varphi$}
				\Output{satisfied or $n$-ary tuple witnessing violation}
				\BlankLine
				$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
				$T \gets \emptyset$\;
				$S: T^n \rightarrow Q$ \quad // initially empty\;
				$t$  \quad // container for the subsequently incoming event traces
				\BlankLine
				\While{there is a new event trace}{
                  $t \gets \epsilon$ \quad // initialize empty trace\;
                  \For(init $S$ for every new tuple $\vec{t}$){$\vec{t} \in ((T \cup \set{t})^n \setminus T^n)$}{
    				$S(\vec{t}) \gets q_0$\;
    			  }
                  \While{$p \in \Sigma$ is a new input event}{
						$t' \gets t~p$ \quad // append $p$ to $t$\;
                        \For(// progress every state in $S$) {$( (t_1,\ldots,t_n), q) \in S$ where $t \in \{t_1,\ldots,t_n\}$}{
                            \uIf(// some trace ended){$\exists t^* \in \{t_1,\ldots,t_n\} \ldot \card{t^*} < \card{t}$}{
                             \eIf {$q \in F$} {
                              remove $(t_1,\ldots,t_n)$ from $S$\;
                              \textbf{continue}\;
                             } { \Return violation and witnessing tuple $(t_1,\ldots,t_n)$\;}
                          }
                          $\vec{t} \gets (t_1,\ldots,t_n)$, where $t_i$ is replaced with $t'$, for each $t_i = t$\;
                          \uIf {$\delta(q, \bigcup_{i=1}^n \bigcup_{a \in \vec{t}(i)[\card{t'}-1]} \set{ (a, \pi_i) }) = q'$} {
        				     $S(\vec{t}) \gets q'$\;
        				  }
        				  \Else{
        				    \Return violation and witnessing tuple $\vec{t}$\;
        				  }
        				}
						$t \gets t'$ \quad // re-assign $t$\;
				  } 
				  $T \gets T \cup \set{t}$\; \quad //add $t$ to already seen traces
				}
				\Return satisfied\;
				\BlankLine
	\caption{Online monitoring algorithm for $\forall^n \hyperltl$: The algorithm subsequently reads event traces and monitors them against already seen traces. Already seen traces are stored in $T$ before continuing with a new event trace.}
	\label{alg:algorithms-sequential}
			\end{algorithm*}

\begin{example} \label{ex:obsdet-algorithm}
  We continue \autoref{ex:obsdet-monitor} by showing how the algorithm progresses on the given formula.
  Assume for the sake of readability that we have a single input proposition $i$ and a single output proposition $o$.
  Furthermore, assume that we have already seen the trace $t_0 = \set{i}\set{i,o}\set{o}$, that is, $T = \set{t_0}$ and $S(t_0,t_0) = q_0$.
  We now show how the algorithm continues with a fresh trace $t_1$.
  In lines 6--8 we add the pairs $(t_0,t_1)$, $(t_0,t_1)$, and $(t_1,t_1)$ with the initial state $q_0$ to $S$.
  Let $p = \set{i}$ be the first input proposition, thus, $t_1 = \set{i}$.
  Since $t_0[0] = t_1[0]$, the monitor remains in $q_0$ for every tuple.
  Let $p = \set{i}$ be the next input proposition, thus, $t_1 = \set{i}\set{i}$.
  Consider the tuple $(t_0,t_1)$.
  As $t_0[1]$ and $t_1[1]$ are equal with respect to $i$ but differ in $o$, the monitor progresses to the rejecting state $q_\bot$ and the algorithm terminates by reporting the violation.
  If, the previous input proposition is $p = \set{}$, both tuples, $(t_0,t_1)$ and $(t_1,t_0)$ would progress to the accepting sink state $q_\top$ as the input proposition is different to $t_0[1]$.
  Assume two more inputs, e.g., $t_1 = \set{i}\set{i}\set{}\set{}$, then the pairs $(t_0,t_0)$, $(t_0,t_1)$, and $(t_1,t_0)$ are removed from $S$ as $t_1$ is strict longer than $t_0$.
\end{example}


\section{Optimizations}
\label{sec:opt}
In this section, we present three optimizations implemented in $\tool$, which, as we will see in the evaluation section, are necessary to make the automata-based monitoring approach feasible in practice. We begin by explaining a \emph{specification analysis}, which is a preprocessing step that exploits properties of the specification to reduce the algorithmic workload. In the subsequent section, we show how $\tool$ tackles the problem of potentially unbounded memory consumption: We recap the \emph{trace analysis}, which was so far the only storage optimization implemented in $\tool$. We then provide a novel storage optimization technique based on prefix-trees, so-called \emph{tries}, to exploit partial equality of the given traces, which the trace analysis neglected so far.
%-------------------------------------------------------------------------------
\subsection{Decreasing Running Time}
%-------------------------------------------------------------------------------

In the example execution in \autoref{ex:obsdet-algorithm} we have seen that the algorithm had to do more work than necessary to monitor observational determinism.
For example, a tuple $(t,t)$ for some trace $t$ cannot violate observational determinism as the traces are equal.
Further, from the pairs $(t,t')$ and $(t',t)$ for some traces $t$ and $t'$, we only need to check one of them as a violation in one of them implies the violation in the other pair.
We can automatically check for such conditions and, thus, omit unnecessary work.

$\tool$ utilizes the HyperLTL satisfiability solver EAHyper~\cite{conf/concur/FinkbeinerH16,conf/cav/FinkbeinerHS17} for its \emph{specification analysis}, which is a preprocessing step that analyzes the HyperLTL formula under consideration.
EAHyper can detect whether a formula is (1) \emph{symmetric}, i.e., we halve the number of instantiated monitors, (2) \emph{transitive}, i.e, we reduce the number of instantiated monitors to two, or (3) \emph{reflexive}, i.e., we can omit the self comparison of traces.

\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:symmetry}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	%Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_n \ldot \psi$, where $\psi$ is an $\ltl$ formula over trace variables $\{\pi_1, \dots, \pi_n\}$.
	%For an assignment $\pathassign$ and an permutation $\sigma : \Pi \to \Pi$, we define $\pathassign \circ \sigma$, such that $(\pathassign \circ \sigma)(\pi) = \pathassign(\sigma(\pi))$ for every $\pi \in \Pi$.
	We say $\varphi$ is invariant under trace variable permutation $\sigma : \pathvars \to \pathvars$, if for any set of traces $T \subseteq \Sigma^{\omega}$ and any assignment $\pathassign : \pathvars \to T$, $(\emptyset, \pathassign, 0) \models \psi \Leftrightarrow (\emptyset, \pathassign \circ \sigma, 0) \models \psi$.
	We say $\varphi$ is symmetric, if it is invariant under every trace variable permutation in $\pathvars$.
\end{definition}
Symmetry is particular interesting since many information flow policies satisfy this property. Consider, for example, observational determinism: 
$
\forall \pi\ldot \forall \pi'\ldot (o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'}).
$ %\todo{different notation than in \autoref{ex:obsdet-algorithm} and intro.}
$\tool$ detects symmetry by translating this formula to a formula that is unsatisfiable if there exists no set of traces for which every trace pair violates the symmetry condition:
$
\exists \pi\ldot \exists \pi'\ldot \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big) \nleftrightarrow \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big)
$.
If the resulting formula turns out to be unsatisfiable, $\tool$ omits the symmetric instantiations of the monitor automaton.
%, which turns out to be, especially in combination with $\tool$s \emph{trace analysis}, a major optimization in practice~\cite{conf/rv/FinkbeinerHST17}.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:transitivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\set{\pi_1, \pi_2}$.
	Let $T = \set{t_1, t_2, t_3} \in \Sigma^{\omega}$ be a three-elemented set of traces.
	We define the assignment $\pathassign_{i,j} : \pathvars \to \Sigma^{\omega}$ by $\pathassign_{i,j} \coloneqq \{\pi_1 \mapsto t_i, \pi_2 \mapsto t_j\}$.
	We say $\varphi$ is transitive, if for all three-elemented sets $T$ it holds that $(\emptyset, \pathassign_{1,2}, 0) \models \psi \wedge (\emptyset, \pathassign_{2,3}, 0) \models \psi \rightarrow (\emptyset, \pathassign_{1,3}, 0) \models \psi$.
\end{definition}
While symmetric HyperLTL formulas allow us to prune half of the monitor instances, transitivity of a HyperLTL formula has an even larger impact on the required memory. Equality, i.e, $\forall \pi. \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$, for example, is transitive and symmetric and allows us to reduce the number of monitor instances to one, since we can check equality against any reference trace.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:reflexivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	We say $\varphi$ is reflexive, if for any trace $t \in \Sigma^{\omega}$ and the corresponding assignment $\pathassign : \pathvars \to \{t\}$, $(\emptyset, \pathassign, 0) \models \psi$.
\end{definition}
Lastly, if a formula is reflexive, $\tool$ omits the composition of a trace with itself during the monitoring process.
%Both $\hyperltl$ formulas considered in this section, $\mathit{ObsDet}$ and $\mathit{EQ}$, are reflexive.
For example, equality and observational determinism have reflexive HyperLTL formulas.

\begin{example}
  Consider again the observational determinism formula from \autoref{ex:obsdet-monitor}.
  We have seen that this formula is both, reflexive and symmetric, thus, we can omit those instances in the algorithm.  
\end{example}


%-------------------------------------------------------------------------------
\subsection{Optimizing Trace Storage}
\label{sec:trie}
%-------------------------------------------------------------------------------

The main obstacle in monitoring hyperproperties is the potentially unbounded space consumption.
So far, RVHyper employed a \emph{trace analysis} technique to detect redundant traces, with respect to a given HyperLTL formula, i.e., traces that can be safely discarded without losing any information and without losing the ability to return a counter example.

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given a HyperLTL formula $\varphi$, a trace set $T$ and an arbitrary $t \in \traces$, we say that $t$ is $(T,\varphi)$-redundant if $T$ is a model of $\varphi$ if and only if $T \cup \set{t}$ is a model of $\varphi$ as well, formally
	\begin{equation*}
	\forall T' \supseteq T \ldot T' \in \hlang(\varphi) \Leftrightarrow T' \cup \{t\} \in \hlang(\varphi) \enspace.
	\end{equation*}
\end{definition}

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given $t,t' \in \Sigma^\omega$, we say $t$ \emph{dominates} $t'$ with respect to $\varphi$ (or simply $t$ \emph{dominates} $t'$ if it is clear from the context) if $t'$ is ($\{t\},\varphi$)-redundant.
\end{definition}

\begin{example}
  For observational determinism, a trace $t$ is dominated by a trace $t'$ if $\card{t} < \card{t'}$ and both traces agree on the input propositions.
\end{example}


This is efficiently implemented in $\tool$ (cf. Algorithm~\ref{alg:traceopti}) and is guaranteed to catch all redundant traces.
In our experiments~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.

The trace analysis, as it is based on a language inclusion check of the entire traces, cannot handle \emph{partial redundancy}, for example, in the case that traces have redundant prefix requirements.
This leaves room for optimization, which we address by implementing a so-called \emph{trie} data structure for managing the storage of incoming traces.

\begin{algorithm}
	%\label{alg_minimization}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\hyperltl$ formula $\varphi$, redundancy free trace set $T$, fresh trace $t$}
	\Output{redundancy free set of traces $T_\mathit{min} \subseteq T \cup \set{t}$}
	%\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}
	\BlankLine
	\ForEach{$t' \in T$}{
		\If{ $t'$ dominates $t$ }
		{
			\Return $T$\;
		}
	}
	\ForEach{$t' \in T$}{
		\If{$t$ dominates $t'$}
		{
			$T \coloneqq T \setminus \set{t'}$\;
		}
	}
	\Return $T \cup \set{t}$\;
	%\BlankLine
	\caption{Trace analysis algorithm to minimize trace storage.}
	\label{alg:traceopti}
\end{algorithm}



%In our experiments~\cite{conf/rv/FinkbeinerHST17,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.
%Ideally one wants to avoid this overhead when monitoring a trace that shares some prefixes with already seen traces.
%We implemented this idea with a so-called \emph{trie} data structure.
Tries, also known as prefix trees, describe a tree data structure, which can represent a set of words over an alphabet in a compact manner.
The root of a trie is identified with the empty word $\epsilon$, additionally each node can have several child nodes, each of which corresponds to a unique letter getting appended to the representing word of the parent node. So the set of words of a trie is identified with the set of words the leaf nodes represent.

\begin{definition}
A trie is a four tuple $(\Sigma, \Tau, \longrightarrow, \tau_0)$ consisting of
\begin{itemize}
    \item a finite alphabet $\Sigma$,
    \item a non-empty set of states $\Tau$,
    \item a transition function $\longrightarrow: \Tau \times \Sigma \rightarrow \Tau$,
    \item and a designated initial state $\tau_0 \in \Tau$ called the root.
    \end{itemize}
\end{definition}
Instead of $((\tau,a),\tau') \in \longrightarrow$ we will write $\tau \overset{a}{\longrightarrow} \tau'$ in the following.
For a trie to be of valid form we restrict $\longrightarrow$ such that, $\forall \tau,\tau' \in \Tau. |\{\tau \overset{a}{\longrightarrow} \tau'| a \in \Sigma\}| \leq 1$.

%Additionally to our analysis phases it would be helpful if we could use some insights from trace analysis 


%As mentioned before, storing the incoming traces succinctly is a major concern in monitoring hyperproperties.
In our case the alphabet would be the set of propositions used in the specification, and the word built by the trie represents the traces. %build from it are what we call traces.
%Tries provide a 
Instead of storing each trace individually, we store all of them in one trie structure, branching only in case of deviation. This means equal prefixes only have to be stored once.
Besides the obvious benefits for memory, we also can make use of the maintained trie data structure to improve the runtime of our monitoring algorithms. As traces with same prefixes end up corresponding to the same path in the trie, we only have to instantiate the monitor automaton as much as the trie contains branches.
%O(size branches) times.
\begin{example}
	Consider the following traces of length $6$ over the alphabet $2^{\{i,o\}}$:
	\begin{itemize}
		\item
		$t_1: \{\set{i},\set{i,o},\set{i},\set{i},\set{i},\set{i,o} \}$
		\item
		$t_2: \{\set{i}, \set{i,o}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_3: \{\set{i}, \set{i}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_4: \{\set{i}, \set{i}, \set{}, \set{} , \set{}, \set{}\}$
	\end{itemize}
After processing the traces sequentially, the resulting trie looks as follows:

\vspace{1ex}

\begin{tikzpicture}[sibling distance=7em, level distance = 30pt,
every node/.style = {shape=circle,
	draw, align=center, minimum size = 0.9cm, inner sep = 0pt},
level 1/.style = {sibling distance = 10em},
level 2/.style = {sibling distance = 5em},
level 5/.style = {sibling distance = 5em}]
\node {$\{i\}$}
child { node {$\{i\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} } } } } 
	child { node {$\{ \}$}  
		child { node {$\{ \}$} 
			child { node {$\{ \}$}
				child { node {$\{ \}$} } } } } }
child { node {$\{i,o\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} }
				child { node {$\{i,o\}$} } } } } };
\end{tikzpicture}
\end{example}

\subsection{Trie-based Monitoring Algorithm}

We depict a trie-based offline monitoring algorithm in Fig.~\ref{alg:trie-offline}.
For the sake of readability, we assume that there are as many traces as universal quantifier, that we progress through all traces in parallel, and that all traces have the same length.
This is merely a simplification in the presentation, one can build the trie in a sequential fashion for online monitoring by a slight modification of the presented algorithm.

Without using tries our monitoring algorithm was based on instantiating the deterministic monitor template $\monitor_\varphi$ with tuples of traces. Now we instantiate $\monitor_\varphi$ with tuples of tries. Initially we only have to create the single instance having the the root of our trie.

\begin{comment}
	\begin{algorithm*}
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
		$S: \Tau^n \rightarrow Q$, \quad $E: \Tau^n \rightarrow \Sigma$\;
		$\tau_0 \coloneqq $\texttt{ new\_trie()}\;
		%$\mathbf{i} \coloneqq \underbrace{(\tau_0,\ldots,\tau_0)}{n \text{times}}$\;
		%$I \coloneqq \{\mathbf{i}\}$\;
		\BlankLine
		$i_0 \in \{ \tau_0 \}^n$\;
		$S(i_0) = q_0$\;
		\While{there is a new trace}{
			$I \leftarrow \{i_0\}$\;
			$\tau \leftarrow \tau_0$\;
			\While{$p \in \Sigma$ is a new event}{
				$\tau' \leftarrow$ \texttt{add\_child($\tau,p$)} //\texttt{assert($E(\tau')==p$)}\;
				$I_n \leftarrow \emptyset$\;
				\ForEach{$i \in I$}{
					$I' \leftarrow \{i' \mid i(j) \rightarrow i'(j), a \in \Sigma, 1 \leq j \leq n\}$\;
					$I' \leftarrow \{i' \in I' \mid \exists k. i'(k) = \tau'\}$\;
					\ForEach{$i' \in I'$}{
						\uIf{$\delta(S(i), \cup_{j=1}^n \cup_{a\in E(i'(j))} \{(a,\pi_j)\}) = q$}{
							$S(i') = q$\;
						}
						\Else{
							\Return(\texttt{rooted\_seq($i'(1)$)}, \ldots, \texttt{rooted\_seq($i'(n)$)})\;
						}
					}
				}
			}
		}
		%\While{$\mathbf{p} \leftarrow$ new elements (in a forward fashion)}{
		%	\For{$1 \leq j \leq n$}{
		%		$\mathbf{i}(j) \leftarrow $\texttt{add\_value($\mathbf{i}(j)$, $j$, $\mathbf{p}(j)$)}\;
		%	}
		%	$I \leftarrow \bigcup_{\mathbf{i} \in I} \{(i'_1,\ldots, i'_n)| \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n\}$\;
		%	\ForEach{$\mathbf{i} \in I$}{
		%		%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
		%		progress every state in $S$ according to $\delta$\;
		%		\If{violation in $M_\varphi$}{
		%			$t \coloneqq ($\texttt{rooted\_sequence($i(1)$)}$,\ldots,$\texttt{rooted\_sequence($i(n)$)}$)$\;
		%			\Return witnessing tuple $t^n$\;
		%		}
		%	}
		%}
		%\Return satisfied\;
		%\BlankLine
	\caption{Online algorithm using trie data structure.}
	\label{alg:trie-online-parallel}
	\end{algorithm*}
\end{comment}
	\begin{algorithm*}[t]
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\\
		$S: \Tau^n \rightarrow Q$\\
		$\tau_0 \coloneqq $\texttt{new\_trie()}\\
		$\mathbf{i} \coloneqq (\tau_0,\ldots,\tau_0) \in \Tau^n$\\
		$I \coloneqq \{\mathbf{i}\}$  \quad // set of not-yet terminated branches\\
		\BlankLine
		\While{$\mathbf{p} \leftarrow$ new event (in $\Sigma^n$)}{
			\For{$1 \leq j \leq n$}{
				$\mathbf{i}(j) \leftarrow $\texttt{add\_child($\mathbf{i}(j)$, $\mathbf{p}(j)$)} \quad // add child with value $\vec{p}(j)$ to $\vec{i}(j)$ if needed \\
			}
			// update set of active branches\\
			$I \leftarrow \bigcup_{\mathbf{i} \in I} \set{ (i'_1,\ldots, i'_n) \mid \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n }$\\
			\ForEach{$\mathbf{i} \in I$}{
				%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
				progress every state in $S$ according to $\delta$\;
				\If{violation in $\monitor_\varphi$}{
				    // return sequence from root to $\vec{i}$\\
					$t \gets ($\texttt{rooted\_sequence($\vec{i}(1)$)}$,\ldots,$\texttt{rooted\_sequence($\vec{i}(n)$)}$)$\\
					\Return witnessing tuple $t^n$\\
				}
			}
		}
		\Return satisfied if $\forall \vec{i} \in I \ldots S(\vec{i}) \in F$ else violation\\
		\BlankLine
	\caption{Offline algorithm using trie data structure.}
	\label{alg:trie-offline}
\end{algorithm*}

The trie-based algorithm has much in common with its previously discussed trace-based counterpart. Initially, we have to build the deterministic monitor automaton $\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F)$.
We instantiate the monitor with a fresh trie root $\tau_0$.
A mapping from trie instantiations to a state in $\monitor_\varphi$ $S: \Tau^n \rightarrow Q$, stores the current state of every active branch of the trie, stored in the set $I$.
For each of the incoming traces, we provide an entry in a tuple of tries $\mathbf{\tau}$, each entry gets initialized to $\tau_0$.
During the run of our algorithm these entries will get updated such that they always correspond to the word built by the traces up to this point.
For as long as there are traces left, which have not yet ended, and we have not yet detected a violation, we will proceed updating the entries in $\vec{i}$ as follows.
Having entry $\tau$ and the correspond trace sequence proceeds with $a$, if $\exists \tau' \in \Tau. \tau \overset{a}{\longrightarrow} \tau'$, we update the entry to $\tau'$ otherwise we create such a child node of $\tau$ (\texttt{add\_child} in line 8).
Creating a new node in the trie always occurs, if the prefix of the incoming trace starts to differ from already seen prefixes.
After having moved on step in our traces sequences, we have to reflect this step in our trie structure, in order for the trie-instantiated automata to correctly monitor the new propositions.
As a trie node can branch to multiple child nodes, each monitor instantiation will get replaced by the set of instantiations, where all possible child combinations of the different assigned tries are existent (update of $I$ in line 11).
Afterwards, we update $S$ in the same way as in Algorithm~\ref{alg:traceopti}, thus, we omit algorithmic details here.
%This can be efficiently implemented as we essential fork the monitor instantiation for the different branches in the trie.
%After this preprocessing we are able to update our mapping $S$ according to $\delta$.
If a violation is detected here, that is there is no transition in the monitor corresponding to $\vec{i}$, we will return the corresponding counter example as a tuple of traces, as those can get reconstructed by stepping upwards in the tries of $\vec{i}$.
%Note that the sequential algorithm is derived from the parallel one by progressing one trace at a time and additionally when forking the monitor instantiations, only those new instantiation have to be kept, which contain the (single) trie in $\mathbf{\tau}$ at least once. 
If the traces end, we check if every open branch $\vec{i} \in I$ is in an accepting state.

%\subsection{Tries and Trace Analysis in Combination}
%\todo{TODO}


==> old/submission/tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> old/submission/tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> old/tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> old/tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> sub_final/commands.tex <==

% Common math
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{{\langle #1 \rangle}}
\newcommand{\card}[1]{{|#1|}}
\newcommand{\ldot}{\mathpunct{.}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\dom}{\mathrm{dom}}

% Languages
\newcommand{\good}{\mathit{good}}
\newcommand{\bad}{\mathit{bad}}
\newcommand{\winning}{\mathit{winning}}
\newcommand{\losing}{\mathit{losing}}
\newcommand{\hlang}{\mathcal{H}}

% Complexity classes
\newcommand{\pspace}{\textsc{PSpace}}

% Logics
\newcommand{\ltl}{\text{LTL}}
\newcommand{\hyperltl}{\text{HyperLTL}}
\newcommand{\secltl}{\text{SecLTL}}


\newcommand{\lang}{\mathcal{L}}
\newcommand{\ap}{\text{AP}}
\renewcommand{\models}{\vDash}
\newcommand{\nmodels}{\nvDash}
\newcommand{\traces}{\mathit{TR}}

% Traces
\newcommand{\pref}{\preceq}
\newcommand{\tracebox}[1]{\framebox[4.5ex][l]{#1}}
\newcommand{\pctracebox}[1]{\framebox[4.5ex][l]{#1}}

% LTL
\newcommand{\U}{\Until}
\newcommand{\X}{\Next}
\newcommand{\G}{\Globally}
\newcommand{\F}{\Eventually}
\newcommand{\R}{\Release}
\newcommand{\W}{\WUntil}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

% HyperLTL
\newcommand{\pathassign}{\Pi}
\newcommand{\pathvars}{\mathcal{V}}
\newcommand{\pathassignfin}{\Pi_\mathit{fin}}

% Monitoring
\newcommand{\monitor}{\mathcal{M}}
\newcommand{\tool}{\text{RVHyper}}

% Tools
\newcommand{\eahyper}{\text{EAHyper}}

% TODOs and Marking
\newcommand{\todo}[1]{\marginpar{TODO}\textcolor{red}{#1}}
%\newcommand{\tbchecked}[1]{\marginpar{To be checked}\textcolor{blue}{#1}}

\newcommand{\ninfluences}{\not\leadsto}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> sub_final/encboth.tex <==
n	millisec
1	1
2	2
3	4
4	5
5	7
6	8
7	9
8	11
9	12
10	13
11	15
12	16
13	18
14	21
15	24
16	28
17	30
18	32
19	35
20	38
21	41
22	43
23	47
24	50
25	55
26	59
27	62
28	64
29	67
30	69
31	72
32	76
33	79
34	82
35	85
36	90
37	96
38	100
39	103
40	107
41	113
42	116
43	120
44	123
45	128
46	131
47	135
48	139
49	143
50	149
51	155
52	158
53	162
54	168
55	173
56	177
57	183
58	190
59	198
60	204
61	208
62	214
63	220
64	226
65	234
66	240
67	250
68	259
69	264
70	270
71	275
72	280
73	290
74	295
75	299
76	305
77	311
78	317
79	322
80	328
81	333
82	343
83	351
84	358
85	365
86	371
87	378
88	384
89	390
90	396
91	402
92	410
93	415
94	424
95	431
96	437
97	452
98	458
99	466
100	479
101	485
102	492
103	501
104	508
105	517
106	527
107	536
108	545
109	557
110	570
111	585
112	594
113	602
114	610
115	625
116	632
117	641
118	648
119	658
120	668
121	676
122	691
123	701
124	712
125	720
126	731
127	741
128	749
129	769
130	778
131	789
132	798
133	808
134	818
135	829
136	841
137	851
138	868
139	878
140	887
141	897
142	906
143	919
144	932
145	943
146	953
147	963
148	981
149	990
150	1001
151	1012
152	1021
153	1037
154	1060
155	1070
156	1091
157	1101
158	1112
159	1123
160	1133
161	1145
162	1165
163	1177
164	1187
165	1196
166	1209
167	1221
168	1247
169	1257
170	1269
171	1291
172	1303
173	1314
174	1327
175	1342
176	1354
177	1365
178	1376
179	1388
180	1400
181	1411
182	1423
183	1436
184	1457
185	1480
186	1498
187	1509
188	1521
189	1534
190	1555
191	1566
192	1580
193	1592
194	1604
195	1617
196	1632
197	1649
198	1660
199	1675
200	1694
201	1706
202	1719
203	1736
204	1756
205	1768
206	1785
207	1797
208	1813
209	1826
210	1842
211	1854
212	1866
213	1878
214	1890
215	1901
216	1913
217	1926
218	1940
219	1951
220	1966
221	1978
222	2001
223	2013
224	2027
225	2044
226	2066
227	2078
228	2090
229	2104
230	2128
231	2143
232	2167
233	2181
234	2196
235	2209
236	2221
237	2252
238	2277
239	2294
240	2308
241	2326
242	2345
243	2359
244	2373
245	2387
246	2401
247	2414
248	2438
249	2451
250	2465
251	2478
252	2492
253	2522
254	2547
255	2561
256	2574
257	2588
258	2601
259	2614
260	2630
261	2645
262	2658
263	2672
264	2686
265	2701
266	2715
267	2736
268	2751
269	2765
270	2778
271	2796
272	2818
273	2841
274	2859
275	2878
276	2907
277	2929
278	2943
279	2959
280	2981
281	3002
282	3022
283	3045
284	3063
285	3078
286	3093
287	3109
288	3127
289	3155
290	3171
291	3186
292	3201
293	3216
294	3241
295	3272
296	3300
297	3321
298	3335
299	3352
300	3368
301	3384
302	3399
303	3438
304	3464
305	3487
306	3510
307	3527
308	3543
309	3563
310	3578
311	3594
312	3619
313	3637
314	3653
315	3667
316	3681
317	3697
318	3712
319	3727
320	3743
321	3758
322	3772
323	3787
324	3801
325	3816
326	3834
327	3850
328	3866
329	3883
330	3898
331	3914
332	3931
333	3948
334	3964
335	3982
336	3997
337	4021
338	4038
339	4054
340	4069
341	4084
342	4100
343	4118
344	4135
345	4156
346	4171
347	4186
348	4202
349	4217
350	4238
351	4254
352	4270
353	4285
354	4301
355	4316
356	4333
357	4348
358	4363
359	4380
360	4396
361	4422
362	4449
363	4465
364	4480
365	4501
366	4517
367	4538
368	4558
369	4574
370	4591
371	4612
372	4635
373	4656
374	4682
375	4698
376	4714
377	4732
378	4750
379	4766
380	4790
381	4807
382	4823
383	4843
384	4859
385	4879
386	4907
387	4936
388	4961
389	4987
390	5005
391	5024
392	5044
393	5062
394	5079
395	5109
396	5128
397	5148
398	5169
399	5187
400	5220
401	5241
402	5283
403	5301
404	5319
405	5345
406	5364
407	5386
408	5407
409	5430
410	5451
411	5472
412	5493
413	5520
414	5555
415	5590
416	5616
417	5645
418	5664
419	5683
420	5701
421	5721
422	5781
423	5803
424	5821
425	5847
426	5871
427	5892
428	5918
429	5948
430	5967
431	5989
432	6017
433	6040
434	6058
435	6076
436	6095
437	6117
438	6138
439	6156
440	6174
441	6192
442	6212
443	6232
444	6252
445	6270
446	6291
447	6308
448	6325
449	6361
450	6379
451	6397
452	6416
453	6435
454	6456
455	6476
456	6495
457	6517
458	6539
459	6559
460	6578
461	6600
462	6618
463	6640
464	6658
465	6686
466	6705
467	6723
468	6754
469	6773
470	6793
471	6829
472	6851
473	6877
474	6897
475	6917
476	6941
477	6960
478	6980
479	7000
480	7020
481	7041
482	7060
483	7084
484	7102
485	7122
486	7148
487	7167
488	7186
489	7205
490	7228
491	7251
492	7270
493	7289
494	7311
495	7332
496	7352
497	7376
498	7399
499	7418
500	7439
501	7458
502	7483
503	7506
504	7525
505	7548
506	7567
507	7588
508	7608
509	7645
510	7666
511	7685
512	7704
513	7725
514	7749
515	7768
516	7787
517	7808
518	7827
519	7850
520	7870
521	7889
522	7919
523	7939
524	7959
525	7979
526	7998
527	8017
528	8047
529	8070
530	8089
531	8114
532	8134
533	8163
534	8187
535	8207
536	8226
537	8248
538	8269
539	8301
540	8321
541	8342
542	8365
543	8389
544	8414
545	8437
546	8458
547	8478
548	8497
549	8517
550	8549
551	8575
552	8596
553	8616
554	8643
555	8663
556	8687
557	8709
558	8731
559	8753
560	8774
561	8794
562	8816
563	8839
564	8861
565	8886
566	8906
567	8927
568	8950
569	8971
570	8992
571	9012
572	9042
573	9063
574	9084
575	9108
576	9128
577	9153
578	9176
579	9214
580	9235
581	9259
582	9280
583	9300
584	9321
585	9344
586	9373
587	9394
588	9418
589	9447
590	9468
591	9489
592	9510
593	9546
594	9567
595	9589
596	9611
597	9631
598	9655
599	9676
600	9697
601	9718
602	9740
603	9763
604	9790
605	9812
606	9837
607	9861
608	9897
609	9918
610	9944
611	9966
612	9995
613	10017
614	10044
615	10065
616	10086
617	10107
618	10129
619	10153
620	10175
621	10196
622	10217
623	10240
624	10266
625	10295
626	10318
627	10344
628	10367
629	10392
630	10414
631	10438
632	10465
633	10488
634	10512
635	10538
636	10564
637	10587
638	10613
639	10638
640	10665
641	10686
642	10707
643	10729
644	10753
645	10776
646	10798
647	10819
648	10850
649	10874
650	10898
651	10921
652	10949
653	10974
654	10998
655	11022
656	11048
657	11073
658	11095
659	11119
660	11148
661	11171
662	11195
663	11218
664	11243
665	11268
666	11291
667	11313
668	11336
669	11363
670	11385
671	11408
672	11430
673	11456
674	11478
675	11500
676	11525
677	11551
678	11573
679	11597
680	11622
681	11653
682	11676
683	11701
684	11725
685	11750
686	11778
687	11801
688	11823
689	11850
690	11872
691	11894
692	11915
693	11938
694	11961
695	11983
696	12006
697	12048
698	12072
699	12097
700	12119
701	12145
702	12169
703	12192
704	12215
705	12251
706	12274
707	12297
708	12325
709	12350
710	12373
711	12395
712	12420
713	12443
714	12467
715	12493
716	12516
717	12539
718	12564
719	12589
720	12611
721	12635
722	12659
723	12694
724	12717
725	12741
726	12766
727	12796
728	12818
729	12847
730	12882
731	12911
732	12935
733	12959
734	12982
735	13006
736	13029
737	13053
738	13079
739	13104
740	13129
741	13155
742	13179
743	13203
744	13253
745	13281
746	13307
747	13331
748	13355
749	13390
750	13412
751	13435
752	13460
753	13483
754	13507
755	13530
756	13556
757	13584
758	13614
759	13638
760	13664
761	13704
762	13728
763	13762
764	13787
765	13814
766	13838
767	13867
768	13891
769	13917
770	13944
771	13969
772	14001
773	14033
774	14072
775	14098
776	14143
777	14181
778	14204
779	14229
780	14257
781	14281
782	14305
783	14329
784	14357
785	14388
786	14413
787	14460
788	14483
789	14507
790	14534
791	14564
792	14594
793	14617
794	14641
795	14667
796	14691
797	14716
798	14740
799	14770
800	14795
801	14819
802	14844
803	14876
804	14906
805	14931
806	14961
807	14987
808	15011
809	15043
810	15077
811	15102
812	15129
813	15157
814	15188
815	15218
816	15243
817	15269
818	15294
819	15319
820	15346
821	15373
822	15398
823	15422
824	15447
825	15476
826	15501
827	15532
828	15560
829	15589
830	15614
831	15643
832	15670
833	15695
834	15720
835	15746
836	15773
837	15801
838	15827
839	15853
840	15878
841	15924
842	15949
843	15975
844	16002
845	16027
846	16053
847	16078
848	16109
849	16134
850	16162
851	16187
852	16213
853	16247
854	16276
855	16302
856	16328
857	16356
858	16392
859	16418
860	16444
861	16473
862	16500
863	16526
864	16553
865	16582
866	16608
867	16636
868	16664
869	16690
870	16720
871	16747
872	16776
873	16803
874	16830
875	16859
876	16892
877	16920
878	16946
879	16974
880	17022
881	17050
882	17078
883	17106
884	17134
885	17163
886	17189
887	17215
888	17241
889	17269
890	17295
891	17321
892	17348
893	17381
894	17407
895	17436
896	17466
897	17492
898	17519
899	17544
900	17578
901	17604
902	17631
903	17664
904	17690
905	17716
906	17752
907	17779
908	17806
909	17834
910	17861
911	17886
912	17912
913	17939
914	17966
915	17994
916	18021
917	18047
918	18095
919	18122
920	18150
921	18176
922	18204
923	18230
924	18259
925	18286
926	18312
927	18338
928	18368
929	18394
930	18421
931	18451
932	18478
933	18506
934	18533
935	18562
936	18589
937	18636
938	18664
939	18695
940	18722
941	18754
942	18782
943	18811
944	18845
945	18876
946	18903
947	18930
948	18959
949	18985
950	19012
951	19042
952	19068
953	19095
954	19122
955	19157
956	19191
957	19219
958	19247
959	19279
960	19306
961	19337
962	19366
963	19415
964	19448
965	19475
966	19503
967	19536
968	19571
969	19601
970	19629
971	19659
972	19695
973	19723
974	19752
975	19781
976	19809
977	19841
978	19877
979	19907
980	19936
981	19963
982	19996
983	20023
984	20051
985	20078
986	20120
987	20148
988	20179
989	20207
990	20238
991	20267
992	20319
993	20351
994	20381
995	20425
996	20455
997	20487
998	20516
999	20548
1000	20603
1001	20638
1002	20671
1003	20700
1004	20732
1005	20763
1006	20794
1007	20847
1008	20875
1009	20905
1010	20934
1011	20967
1012	20996
1013	21029
1014	21062
1015	21090
1016	21120
1017	21153
1018	21182
1019	21212
1020	21242
1021	21271
1022	21299
1023	21328
1024	21382
1025	21414
1026	21444
1027	21473
1028	21501
1029	21530
1030	21568
1031	21598
1032	21633
1033	21664
1034	21693
1035	21721
1036	21753
1037	21781
1038	21834
1039	21867
1040	21898
1041	21930
1042	21964
1043	21993
1044	22026
1045	22059
1046	22093
1047	22121
1048	22153
1049	22185
1050	22214
1051	22243
1052	22274
1053	22304
1054	22333
1055	22363
1056	22392
1057	22421
1058	22454
1059	22485
1060	22515
1061	22548
1062	22579
1063	22610
1064	22639
1065	22671
1066	22705
1067	22738
1068	22769
1069	22806
1070	22854
1071	22884
1072	22914
1073	22943
1074	22972
1075	23001
1076	23030
1077	23063
1078	23092
1079	23124
1080	23154
1081	23190
1082	23221
1083	23261
1084	23294
1085	23330
1086	23366
1087	23417
1088	23448
1089	23483
1090	23513
1091	23546
1092	23580
1093	23612
1094	23649
1095	23686
1096	23716
1097	23746
1098	23781
1099	23811
1100	23840
1101	23875
1102	23904
1103	23938
1104	23968
1105	24001
1106	24030
1107	24062
1108	24092
1109	24122
1110	24156
1111	24189
1112	24219
1113	24248
1114	24285
1115	24315
1116	24351
1117	24382
1118	24418
1119	24454
1120	24507
1121	24538
1122	24587
1123	24634
1124	24670
1125	24702
1126	24733
1127	24765
1128	24798
1129	24854
1130	24887
1131	24918
1132	24951
1133	24986
1134	25019
1135	25054
1136	25090
1137	25123
1138	25157
1139	25191
1140	25222
1141	25252
1142	25284
1143	25316
1144	25350
1145	25384
1146	25415
1147	25445
1148	25478
1149	25537
1150	25573
1151	25609
1152	25640
1153	25673
1154	25705
1155	25736
1156	25768
1157	25799
1158	25831
1159	25861
1160	25894
1161	25935
1162	25969
1163	26000
1164	26031
1165	26063
1166	26098
1167	26133
1168	26176
1169	26207
1170	26238
1171	26278
1172	26313
1173	26348
1174	26383
1175	26418
1176	26451
1177	26488
1178	26521
1179	26555
1180	26620
1181	26654
1182	26691
1183	26747
1184	26783
1185	26815
1186	26846
1187	26881
1188	26929
1189	26960
1190	26996
1191	27030
1192	27062
1193	27098
1194	27129
1195	27161
1196	27195
1197	27231
1198	27266
1199	27300
1200	27332
1201	27363
1202	27398
1203	27430
1204	27473
1205	27509
1206	27542
1207	27580
1208	27613
1209	27645
1210	27681
1211	27714
1212	27747
1213	27785
1214	27819
1215	27851
1216	27894
1217	27928
1218	27961
1219	27998
1220	28032
1221	28065
1222	28127
1223	28172
1224	28207
1225	28239
1226	28274
1227	28308
1228	28343
1229	28379
1230	28444
1231	28485
1232	28519
1233	28554
1234	28596
1235	28639
1236	28672
1237	28707
1238	28740
1239	28774
1240	28808
1241	28846
1242	28897
1243	28931
1244	28967
1245	29005
1246	29038
1247	29070
1248	29110
1249	29146
1250	29186
1251	29222
1252	29257
1253	29298
1254	29338
1255	29374
1256	29412
1257	29451
1258	29493
1259	29529
1260	29564
1261	29619
1262	29655
1263	29693
1264	29733
1265	29767
1266	29807
1267	29845
1268	29882
1269	29918
1270	29952
1271	29987
1272	30022
1273	30055
1274	30094
1275	30128
1276	30176
1277	30215
1278	30252
1279	30292
1280	30333
1281	30373
1282	30412
1283	30455
1284	30493
1285	30530
1286	30565
1287	30608
1288	30642
1289	30678
1290	30716
1291	30775
1292	30816
1293	30856
1294	30901
1295	30939
1296	30978
1297	31018
1298	31057
1299	31096
1300	31131
1301	31167
1302	31206
1303	31240
1304	31275
1305	31314
1306	31349
1307	31385
1308	31424
1309	31465
1310	31503
1311	31537
1312	31573
1313	31610
1314	31655
1315	31693
1316	31730
1317	31765
1318	31804
1319	31838
1320	31873
1321	31909
1322	31968
1323	32008
1324	32043
1325	32078
1326	32119
1327	32154
1328	32189
1329	32227
1330	32262
1331	32298
1332	32337
1333	32405
1334	32440
1335	32481
1336	32519
1337	32555
1338	32592
1339	32630
1340	32666
1341	32704
1342	32764
1343	32810
1344	32849
1345	32884
1346	32921
1347	32958
1348	32994
1349	33031
1350	33080
1351	33159
1352	33197
1353	33233
1354	33305
1355	33344
1356	33383
1357	33427
1358	33467
1359	33506
1360	33560
1361	33625
1362	33661
1363	33701
1364	33748
1365	33822
1366	33862
1367	33904
1368	33943
1369	33983
1370	34030
1371	34069
1372	34112
1373	34151
1374	34194
1375	34239
1376	34279
1377	34323
1378	34363
1379	34406
1380	34444
1381	34483
1382	34526
1383	34565
1384	34606
1385	34645
1386	34682
1387	34751
1388	34787
1389	34825
1390	34863
1391	34932
1392	34968
1393	35007
1394	35048
1395	35086
1396	35125
1397	35170
1398	35212
1399	35253
1400	35290
1401	35328
1402	35366
1403	35402
1404	35445
1405	35485
1406	35528
1407	35570
1408	35614
1409	35657
1410	35697
1411	35738
1412	35777
1413	35821
1414	35861
1415	35900
1416	35941
1417	35982
1418	36024
1419	36091
1420	36133
1421	36188
1422	36228
1423	36271
1424	36313
1425	36353
1426	36393
1427	36435
1428	36474
1429	36516
1430	36558
1431	36603
1432	36643
1433	36681
1434	36727
1435	36770
1436	36812
1437	36849
1438	36887
1439	36932
1440	36970
1441	37008
1442	37046
1443	37084
1444	37124
1445	37162
1446	37199
1447	37240
1448	37278
1449	37320
1450	37358
1451	37401
1452	37440
1453	37482
1454	37522
1455	37564
1456	37604
1457	37645
1458	37705
1459	37747
1460	37787
1461	37830
1462	37875
1463	37917
1464	37955
1465	37996
1466	38038
1467	38077
1468	38129
1469	38170
1470	38210
1471	38253
1472	38293
1473	38333
1474	38374
1475	38416
1476	38461
1477	38501
1478	38548
1479	38588
1480	38628
1481	38669
1482	38707
1483	38746
1484	38783
1485	38823
1486	38862
1487	38900
1488	38941
1489	38979
1490	39020
1491	39059
1492	39097
1493	39138
1494	39178
1495	39247
1496	39290
1497	39330
1498	39370
1499	39409
1500	39485
1501	39561
1502	39601
1503	39649
1504	39689
1505	39735
1506	39774
1507	39817
1508	39859
1509	39900
1510	39940
1511	39983
1512	40025
1513	40067
1514	40107
1515	40153
1516	40192
1517	40237
1518	40280
1519	40320
1520	40359
1521	40399
1522	40440
1523	40480
1524	40522
1525	40566
1526	40604
1527	40655
1528	40694
1529	40764
1530	40804
1531	40848
1532	40924
1533	40986
1534	41028
1535	41067
1536	41108
1537	41151
1538	41194
1539	41236
1540	41276
1541	41316
1542	41358
1543	41397
1544	41440
1545	41480
1546	41519
1547	41561
1548	41609
1549	41653
1550	41694
1551	41734
1552	41774
1553	41813
1554	41856
1555	41931
1556	41972
1557	42019
1558	42071
1559	42114
1560	42161
1561	42207
1562	42274
1563	42317
1564	42362
1565	42405
1566	42448
1567	42491
1568	42539
1569	42591
1570	42637
1571	42677
1572	42719
1573	42779
1574	42859
1575	42902
1576	42945
1577	42987
1578	43028
1579	43071
1580	43147
1581	43191
1582	43233
1583	43290
1584	43338
1585	43392
1586	43434
1587	43481
1588	43526
1589	43567
1590	43608
1591	43658
1592	43698
1593	43741
1594	43781
1595	43824
1596	43865
1597	43906
1598	43949
1599	43998
1600	44045
1601	44089
1602	44133
1603	44173
1604	44250
1605	44292
1606	44341
1607	44385
1608	44428
1609	44472
1610	44512
1611	44559
1612	44603
1613	44651
1614	44701
1615	44748
1616	44793
1617	44845
1618	44902
1619	45025
1620	45167
1621	45258
1622	45303
1623	45349
1624	45392
1625	45441
1626	45485
1627	45534
1628	45600
1629	45648
1630	45693
1631	45745
1632	45789
1633	45836
1634	45881
1635	45927
1636	45974
1637	46018
1638	46067
1639	46109
1640	46156
1641	46197
1642	46243
1643	46286
1644	46331
1645	46373
1646	46418
1647	46463
1648	46504
1649	46550
1650	46591
1651	46637
1652	46678
1653	46723
1654	46766
1655	46813
1656	46860
1657	46902
1658	46983
1659	47037
1660	47094
1661	47141
1662	47190
1663	47241
1664	47285
1665	47332
1666	47378
1667	47436
1668	47482
1669	47532
1670	47574
1671	47616
1672	47661
1673	47703
1674	47753
1675	47795
1676	47841
1677	47885
1678	47927
1679	47971
1680	48014
1681	48068
1682	48110
1683	48164
1684	48211
1685	48270
1686	48314
1687	48377
1688	48419
1689	48464
1690	48514
1691	48563
1692	48610
1693	48658
1694	48701
1695	48748
1696	48793
1697	48839
1698	48889
1699	48936
1700	48980
1701	49023
1702	49072
1703	49122
1704	49170
1705	49250
1706	49405
1707	49491
1708	49543
1709	49587
1710	49636
1711	49680
1712	49729
1713	49777
1714	49830
1715	49878
1716	49922
1717	49968
1718	50011
1719	50088
1720	50138
1721	50183
1722	50231
1723	50276
1724	50325
1725	50375
1726	50419
1727	50475
1728	50527
1729	50576
1730	50626
1731	50671
1732	50718
1733	50772
1734	50820
1735	50866
1736	50917
1737	50963
1738	51006
1739	51052
1740	51096
1741	51144
1742	51187
1743	51240
1744	51283
1745	51331
1746	51380
1747	51431
1748	51481
1749	51531
1750	51574
1751	51624
1752	51670
1753	51719
1754	51767
1755	51813
1756	51861
1757	51907
1758	51955
1759	51998
1760	52049
1761	52094
1762	52141
1763	52184
1764	52232
1765	52279
1766	52327
1767	52370
1768	52418
1769	52462
1770	52515
1771	52562
1772	52609
1773	52715
1774	52770
1775	52816
1776	52862
1777	52907
1778	52949
1779	53030
1780	53080
1781	53127
1782	53172
1783	53214
1784	53263
1785	53314
1786	53367
1787	53413
1788	53458
1789	53503
1790	53553
1791	53598
1792	53652
1793	53701
1794	53760
1795	53804
1796	53850
1797	53894
1798	53976
1799	54053
1800	54100
1801	54147
1802	54195
1803	54251
1804	54298
1805	54351
1806	54399
1807	54448
1808	54494
1809	54543
1810	54588
1811	54637
1812	54683
1813	54732
1814	54776
1815	54821
1816	54867
1817	54911
1818	54958
1819	55002
1820	55052
1821	55100
1822	55147
1823	55192
1824	55242
1825	55288
1826	55339
1827	55388
1828	55434
1829	55479
1830	55524
1831	55571
1832	55620
1833	55670
1834	55713
1835	55759
1836	55805
1837	55851
1838	55895
1839	55948
1840	55992
1841	56040
1842	56087
1843	56133
1844	56176
1845	56221
1846	56270
1847	56348
1848	56433
1849	56478
1850	56524
1851	56572
1852	56616
1853	56671
1854	56716
1855	56763
1856	56808
1857	56856
1858	56900
1859	56951
1860	57001
1861	57049
1862	57099
1863	57145
1864	57191
1865	57239
1866	57286
1867	57338
1868	57390
1869	57443
1870	57490
1871	57536
1872	57582
1873	57627
1874	57683
1875	57729
1876	57777
1877	57822
1878	57869
1879	57917
1880	57965
1881	58015
1882	58069
1883	58119
1884	58168
1885	58219
1886	58266
1887	58315
1888	58363
1889	58412
1890	58463
1891	58512
1892	58562
1893	58615
1894	58673
1895	58728
1896	58790
1897	58847
1898	58908
1899	58960
1900	59030
1901	59094
1902	59141
1903	59192
1904	59238
1905	59288
1906	59345
1907	59401
1908	59458
1909	59520
1910	59583
1911	59634
1912	59690
1913	59744
1914	59797
1915	59844
1916	59893
1917	59939
1918	59988
1919	60032
1920	60083
1921	60130
1922	60180
1923	60239
1924	60292
1925	60338
1926	60387
1927	60434
1928	60483
1929	60540
1930	60588
1931	60633
1932	60686
1933	60732
1934	60779
1935	60826
1936	60874
1937	60919
1938	61002
1939	61048
1940	61098
1941	61160
1942	61208
1943	61255
1944	61304
1945	61350
1946	61401
1947	61446
1948	61496
1949	61545
1950	61594
1951	61639
1952	61690
1953	61736
1954	61786
1955	61831
1956	61881
1957	61929
1958	61977
1959	62053
1960	62107
1961	62154
1962	62203
1963	62249
1964	62302
1965	62347
1966	62396
1967	62444
1968	62494
1969	62547
1970	62624
1971	62680
1972	62734
1973	62820
1974	62872
1975	62929
1976	62980
1977	63047
1978	63113
1979	63173
1980	63247
1981	63300
1982	63347
1983	63403
1984	63450
1985	63500
1986	63547
1987	63599
1988	63648
1989	63706
1990	63757
1991	63810
1992	63865
1993	63921
1994	63971
1995	64030
1996	64090
1997	64146
1998	64207
1999	64256
2000	64308


==> sub_final/encnaive.tex <==
n	millisec
1	0
2	1
3	2
4	3
5	6
6	9
7	13
8	20
9	27
10	32
11	37
12	43
13	48
14	54
15	59
16	66
17	72
18	79
19	86
20	95
21	103
22	112
23	125
24	135
25	145
26	159
27	169
28	181
29	192
30	203
31	219
32	233
33	246
34	259
35	273
36	287
37	302
38	317
39	335
40	352
41	368
42	384
43	401
44	421
45	439
46	457
47	475
48	494
49	513
50	535
51	555
52	576
53	597
54	621
55	642
56	664
57	687
58	712
59	739
60	762
61	788
62	817
63	844
64	872
65	899
66	929
67	956
68	985
69	1016
70	1045
71	1075
72	1104
73	1138
74	1171
75	1202
76	1234
77	1268
78	1301
79	1336
80	1371
81	1405
82	1441
83	1473
84	1507
85	1545
86	1580
87	1619
88	1657
89	1694
90	1740
91	1777
92	1816
93	1856
94	1896
95	1936
96	1975
97	2019
98	2060
99	2101
100	2144
101	2184
102	2228
103	2269
104	2313
105	2355
106	2399
107	2447
108	2491
109	2538
110	2586
111	2635
112	2685
113	2735
114	2785
115	2839
116	2887
117	2941
118	2993
119	3048
120	3099
121	3158
122	3215
123	3268
124	3328
125	3390
126	3450
127	3504
128	3562
129	3619
130	3674
131	3734
132	3788
133	3845
134	3898
135	3956
136	4011
137	4069
138	4128
139	4184
140	4245
141	4303
142	4363
143	4423
144	4482
145	4543
146	4603
147	4665
148	4729
149	4790
150	4857
151	4921
152	4983
153	5049
154	5113
155	5179
156	5248
157	5315
158	5388
159	5455
160	5524
161	5589
162	5656
163	5728
164	5793
165	5862
166	5930
167	6001
168	6082
169	6157
170	6232
171	6303
172	6374
173	6445
174	6520
175	6592
176	6674
177	6778
178	6854
179	6933
180	7012
181	7094
182	7172
183	7249
184	7327
185	7406
186	7488
187	7570
188	7649
189	7731
190	7813
191	7895
192	7976
193	8058
194	8142
195	8231
196	8326
197	8427
198	8515
199	8602
200	8692
201	8790
202	8886
203	8978
204	9065
205	9157
206	9245
207	9333
208	9418
209	9506
210	9595
211	9689
212	9784
213	9879
214	9976
215	10068
216	10167
217	10264
218	10360
219	10458
220	10554
221	10654
222	10749
223	10843
224	10933
225	11025
226	11119
227	11216
228	11316
229	11419
230	11520
231	11620
232	11721
233	11819
234	11920
235	12018
236	12118
237	12221
238	12321
239	12425
240	12524
241	12626
242	12730
243	12833
244	12935
245	13042
246	13144
247	13249
248	13354
249	13460
250	13568
251	13674
252	13782
253	13893
254	14008
255	14122
256	14248
257	14367
258	14479
259	14592
260	14705
261	14813
262	14922
263	15033
264	15144
265	15269
266	15390
267	15511
268	15630
269	15750
270	15873
271	15996
272	16119
273	16245
274	16369
275	16495
276	16622
277	16746
278	16873
279	17002
280	17128
281	17255
282	17383
283	17509
284	17634
285	17761
286	17892
287	18020
288	18146
289	18275
290	18424
291	18555
292	18692
293	18857
294	18990
295	19119
296	19248
297	19377
298	19503
299	19631
300	19757
301	19888
302	20019
303	20157
304	20297
305	20433
306	20562
307	20696
308	20837
309	20980
310	21110
311	21242
312	21372
313	21507
314	21637
315	21779
316	21914
317	22050
318	22190
319	22330
320	22472
321	22613
322	22756
323	22898
324	23036
325	23191
326	23332
327	23478
328	23623
329	23774
330	23924
331	24072
332	24224
333	24367
334	24513
335	24668
336	24822
337	24972
338	25127
339	25283
340	25444
341	25603
342	25759
343	25915
344	26070
345	26230
346	26387
347	26546
348	26709
349	26869
350	27029
351	27185
352	27342
353	27514
354	27680
355	27841
356	27998
357	28167
358	28343
359	28515
360	28688
361	28876
362	29032
363	29188
364	29345
365	29514
366	29681
367	29849
368	30019
369	30178
370	30339
371	30503
372	30675
373	30848
374	31019
375	31183
376	31350
377	31520
378	31688
379	31856
380	32024
381	32190
382	32356
383	32527
384	32697
385	32862
386	33031
387	33201
388	33372
389	33545
390	33725
391	33905
392	34086
393	34262
394	34438
395	34615
396	34792
397	34971
398	35149
399	35329
400	35506
401	35685
402	35858
403	36039
404	36221
405	36403
406	36589
407	36769
408	36952
409	37134
410	37315
411	37499
412	37683
413	37878
414	38063
415	38259
416	38445
417	38645
418	38866
419	39065
420	39250
421	39438
422	39634
423	39822
424	40014
425	40214
426	40412
427	40612
428	40806
429	41001
430	41195
431	41389
432	41586
433	41780
434	41975
435	42179
436	42384
437	42588
438	42794
439	43001
440	43203
441	43399
442	43601
443	43796
444	43999
445	44196
446	44402
447	44614
448	44820
449	45027
450	45234
451	45439
452	45645
453	45850
454	46061
455	46267
456	46475
457	46683
458	46889
459	47100
460	47308
461	47517
462	47729
463	47944
464	48198
465	48416
466	48643
467	48881
468	49096
469	49314
470	49539
471	49758
472	49979
473	50196
474	50408
475	50630
476	50854
477	51097
478	51331
479	51547
480	51758
481	51986
482	52206
483	52421
484	52644
485	52874
486	53106
487	53337
488	53564
489	53782
490	54004
491	54234
492	54457
493	54681
494	54919
495	55145
496	55368
497	55607
498	55842
499	56070
500	56296
501	56532
502	56772
503	57016
504	57258
505	57501
506	57744
507	57983
508	58240
509	58473
510	58720
511	58970
512	59203
513	59442
514	59691
515	59945
516	60195
517	60478
518	60739
519	60986
520	61235
521	61479
522	61718
523	61959
524	62195
525	62453
526	62692
527	62936
528	63183
529	63426
530	63672
531	63915
532	64161
533	64412
534	64664
535	64918
536	65167
537	65418
538	65676
539	65915
540	66166
541	66409
542	66657
543	66921
544	67202
545	67629
546	67888
547	68153
548	68435
549	68732
550	69004
551	69263
552	69524
553	69802
554	70072
555	70343
556	70613
557	70871
558	71132
559	71401
560	71823
561	72086
562	72391
563	72668
564	72951
565	73219
566	73477
567	73740
568	74007
569	74274
570	74548
571	74824
572	75094
573	75369
574	75639
575	75905
576	76186
577	76469
578	76741
579	77005
580	77275
581	77553
582	77832
583	78116
584	78418
585	78730
586	79016
587	79287
588	79568
589	79855
590	80132
591	80401
592	80673
593	80949
594	81222
595	81509
596	81792
597	82075
598	82355
599	82643
600	82938
601	83227
602	83516
603	83809
604	84104
605	84400
606	84685
607	84973
608	85253
609	85537
610	85830
611	86119
612	86402
613	86692
614	86978
615	87279
616	87576
617	87883
618	88191
619	88502
620	88822
621	89116
622	89405
623	89708
624	90009
625	90297
626	90589
627	90887
628	91188
629	91479
630	91781
631	92091
632	92385
633	92681
634	92975
635	93304
636	93603
637	93915
638	94214
639	94522
640	94813
641	95111
642	95414
643	95717
644	96020
645	96329
646	96631
647	96938
648	97240
649	97542
650	97857
651	98189
652	98517
653	98848
654	99158
655	99477
656	99793
657	100096
658	100427
659	100753
660	101072
661	101374
662	101686
663	102008
664	102333
665	102657
666	102979
667	103302
668	103631
669	103958
670	104285
671	104613
672	104924
673	105235
674	105560
675	105882
676	106199
677	106516
678	106849
679	107182
680	107507
681	107832
682	108180
683	108519
684	108896
685	109233
686	109574
687	109900
688	110221
689	110535
690	110857
691	111195
692	111527
693	111863
694	112205
695	112550
696	112889
697	113224
698	113558
699	113896
700	114227
701	114562
702	114913
703	115254
704	115618
705	115976
706	116310
707	116654
708	117002
709	117338
710	117682
711	118031
712	118383
713	118743
714	119095
715	119445
716	119797
717	120158
718	120505
719	120860
720	121200
721	121548
722	121904
723	122354
724	122703
725	123063
726	123428
727	123787
728	124148
729	124505
730	124856
731	125201
732	125566
733	125934
734	126287
735	126657
736	127016
737	127374
738	127747
739	128099
740	128470
741	128856
742	129227
743	129591
744	129960
745	130326
746	130734
747	131113
748	131480
749	131835
750	132198
751	132559
752	132929
753	133310
754	133689
755	134068
756	134442
757	134821
758	135204
759	135570
760	135953
761	136323
762	136702
763	137072
764	137440
765	137810
766	138200
767	138599
768	138995
769	139380
770	139766
771	140151
772	140524
773	140886
774	141266
775	141659
776	142050
777	142424
778	142800
779	143179
780	143555
781	143935
782	144311
783	144689
784	145072
785	145458
786	145852
787	146242
788	146633
789	147034
790	147436
791	147824
792	148228
793	148652
794	149038
795	149419
796	149808
797	150192
798	150586
799	150967
800	151362
801	151748
802	152153
803	152561
804	152965
805	153360
806	153771
807	154178
808	154588
809	154993
810	155374
811	155789
812	156203
813	156616
814	157024
815	157426
816	157825
817	158228
818	158737
819	159160
820	159562
821	159982
822	160511
823	160913
824	161317
825	161735
826	162150
827	162548
828	162956
829	163366
830	163893
831	164425
832	164863
833	165310
834	165752
835	166187
836	166604
837	167076
838	167547
839	168165
840	168703
841	169170
842	169588
843	170104
844	170631
845	171170
846	171712
847	172166
848	172628
849	173159
850	173684
851	174106
852	174537
853	175145
854	175737
855	176238
856	176901
857	177412
858	177831
859	178475
860	179105
861	179542
862	180017
863	180700
864	181272
865	181705
866	182127
867	182548
868	182995
869	183437
870	183871
871	184322
872	184769
873	185229
874	185670
875	186098
876	186523
877	186952
878	187394
879	187829
880	188288
881	188803
882	189250
883	189690
884	190121
885	190576
886	191015
887	191446
888	191889
889	192319
890	192759
891	193194
892	193627
893	194062
894	194503
895	194948
896	195389
897	195824
898	196265
899	196702
900	197145
901	197596
902	198040
903	198489
904	198962
905	199420
906	199860
907	200305
908	200779
909	201249
910	201694
911	202152
912	202603
913	203054
914	203513
915	203962
916	204415
917	204868
918	205314
919	205771
920	206240
921	206689
922	207152
923	207605
924	208082
925	208548
926	209065
927	209538
928	210002
929	210469
930	210921
931	211391
932	211853
933	212314
934	212783
935	213280
936	213752
937	214227
938	214700
939	215171
940	215632
941	216105
942	216571
943	217044
944	217513
945	217984
946	218502
947	218966
948	219432
949	219905
950	220390
951	220853
952	221316
953	221793
954	222262
955	222733
956	223206
957	223688
958	224163
959	224634
960	225105
961	225592
962	226081
963	226556
964	227046
965	227521
966	228014
967	228578
968	229067
969	229547
970	230022
971	230507
972	231008
973	231499
974	231973
975	232458
976	232937
977	233432
978	233924
979	234417
980	234905
981	235397
982	235883
983	236372
984	236858
985	237347
986	237847
987	238356
988	238859
989	239350
990	239838
991	240335
992	240825
993	241314
994	241804
995	242299
996	242794
997	243285
998	243793
999	244300
1000	244798
1001	245288
1002	245785
1003	246290
1004	246789
1005	247305
1006	247815
1007	248349
1008	248876
1009	249387
1010	249905
1011	250439
1012	250953
1013	251462
1014	251965
1015	252469
1016	252992
1017	253500
1018	254002
1019	254514
1020	255025
1021	255544
1022	256070
1023	256608
1024	257144
1025	257658
1026	258182
1027	258754
1028	259260
1029	259772
1030	260288
1031	260799
1032	261307
1033	261822
1034	262332
1035	262831
1036	263343
1037	263855
1038	264380
1039	264899
1040	265418
1041	265940
1042	266478
1043	267009
1044	267527
1045	268061
1046	268617
1047	269153
1048	269940
1049	270512
1050	271037
1051	271556
1052	272080
1053	272609
1054	273540
1055	274099
1056	274851
1057	275555
1058	276098
1059	276682
1060	277224
1061	277796
1062	278439
1063	278979
1064	279577
1065	280119
1066	280661
1067	281188
1068	281711
1069	282232
1070	282777
1071	283575
1072	284126
1073	284673
1074	285224
1075	285763
1076	286319
1077	286866
1078	287424
1079	288024
1080	288592
1081	289161
1082	289702
1083	290236
1084	290781
1085	291345
1086	291911
1087	292483
1088	293044
1089	293597
1090	294147
1091	294699
1092	295275
1093	295845
1094	296406
1095	296969
1096	297532
1097	298107
1098	298671
1099	299255
1100	299800
1101	300383
1102	300947
1103	301533
1104	302110
1105	302672
1106	303241
1107	303801
1108	304364
1109	304938
1110	305503
1111	306077
1112	306641
1113	307205
1114	307784
1115	308373
1116	308945
1117	309522
1118	310100
1119	310666
1120	311236
1121	311815
1122	312373
1123	312945
1124	313535
1125	314109
1126	314687
1127	315273
1128	315852
1129	316431
1130	317016
1131	317602
1132	318209
1133	318798
1134	319394
1135	319978
1136	320561
1137	321121
1138	321696
1139	322273
1140	322848
1141	323430
1142	324007
1143	324586
1144	325169
1145	325748
1146	326326
1147	326923
1148	327515
1149	328116
1150	328741
1151	329366
1152	329948
1153	330556
1154	331169
1155	331748
1156	332333
1157	332919
1158	333502
1159	334097
1160	334694
1161	335280
1162	335884
1163	336470
1164	337073
1165	337677
1166	338299
1167	338915
1168	339534
1169	340179
1170	340766
1171	341405
1172	342005
1173	342620
1174	343238
1175	343870
1176	344479
1177	345107
1178	345717
1179	346332
1180	346934
1181	347526
1182	348170
1183	348765
1184	349375
1185	349998
1186	350614
1187	351216
1188	351822
1189	352421
1190	353021
1191	353627
1192	354232
1193	354858
1194	355457
1195	356065
1196	356690
1197	357294
1198	357911
1199	358539
1200	359158
1201	359768
1202	360369
1203	360985
1204	361599
1205	362213
1206	362841
1207	363464
1208	364068
1209	364692
1210	365303
1211	365927
1212	366544
1213	367156
1214	367810
1215	368457
1216	369066
1217	369704
1218	370349
1219	370966
1220	371582
1221	372210
1222	372833
1223	373460
1224	374101
1225	374755
1226	375406
1227	376039
1228	376685
1229	377330
1230	377986
1231	378653
1232	379305
1233	379937
1234	380565
1235	381190
1236	381843
1237	382496
1238	383138
1239	383802
1240	384459
1241	385110
1242	385760
1243	386389
1244	387039
1245	387707
1246	388363
1247	389017
1248	389674
1249	390316
1250	390959
1251	391609
1252	392262
1253	392925
1254	393595
1255	394229
1256	394888
1257	395535
1258	396185
1259	396848
1260	397505
1261	398180
1262	398863
1263	399500
1264	400142
1265	400798
1266	401472
1267	402124
1268	402796
1269	403471
1270	404102
1271	404770
1272	405441
1273	406114
1274	406786
1275	407464
1276	408159
1277	408828
1278	409495
1279	410173
1280	410820
1281	411481
1282	412134
1283	412797
1284	413460
1285	414122
1286	414799
1287	415461
1288	416129
1289	416789
1290	417459
1291	418166
1292	418882
1293	419541
1294	420217
1295	420906
1296	421577
1297	422242
1298	422924
1299	423846
1300	424532
1301	425213
1302	425888
1303	426946
1304	427666
1305	428873
1306	429615
1307	430335
1308	431033
1309	431706
1310	432394
1311	433095
1312	433781
1313	434471
1314	435161
1315	435849
1316	436548
1317	437217
1318	437942
1319	438644
1320	439330
1321	440021
1322	440702
1323	441373
1324	442063
1325	442760
1326	443440
1327	444135
1328	444832
1329	445519
1330	446235
1331	446932
1332	447625
1333	448344
1334	449041
1335	449727
1336	450412
1337	451126
1338	451844
1339	452530
1340	453232
1341	453938
1342	454641
1343	455345
1344	456035
1345	456748
1346	457465
1347	458219
1348	458937
1349	459654
1350	460334
1351	461031
1352	461727
1353	462428
1354	463139
1355	463847
1356	464555
1357	465257
1358	465968
1359	466679
1360	467405
1361	468129
1362	468844
1363	469548
1364	470261
1365	470968
1366	471682
1367	472385
1368	473094
1369	473806
1370	474568
1371	475353
1372	476127
1373	476851
1374	477571
1375	478302
1376	479011
1377	479712
1378	480446
1379	481164
1380	481895
1381	482608
1382	483348
1383	484091
1384	484827
1385	485543
1386	486260
1387	486991
1388	487733
1389	488476
1390	489205
1391	489920
1392	490640
1393	491384
1394	492102
1395	492836
1396	493564
1397	494311
1398	495052
1399	495776
1400	496519
1401	497256
1402	498038
1403	498797
1404	499536
1405	500276
1406	501030
1407	501789
1408	502549
1409	503297
1410	504025
1411	504989
1412	505710
1413	506463
1414	507233
1415	508004
1416	508741
1417	509454
1418	510185
1419	510921
1420	511645
1421	512370
1422	513097
1423	513822
1424	514548
1425	515277
1426	516005
1427	516749
1428	517498
1429	518246
1430	518971
1431	519705
1432	520437
1433	521186
1434	521904
1435	522630
1436	523353
1437	524108
1438	524840
1439	525568
1440	526307
1441	527040
1442	527823
1443	528597
1444	529336
1445	530079
1446	531012
1447	531998
1448	532818
1449	533963
1450	534804
1451	535632
1452	536569
1453	537459
1454	538750
1455	540225
1456	541092
1457	541935
1458	542905
1459	543975
1460	544743
1461	545516
1462	546305
1463	547087
1464	547950
1465	548838
1466	549702
1467	550664
1468	551519
1469	552528
1470	553382
1471	554225
1472	555279
1473	556194
1474	557075
1475	557910
1476	558789
1477	559715
1478	560618
1479	561454
1480	562317
1481	563096
1482	563890
1483	564663
1484	565521
1485	566302
1486	567154
1487	568026
1488	568863
1489	569659
1490	570462
1491	571389
1492	572277
1493	573232
1494	574020
1495	574813
1496	575699
1497	576595
1498	577396
1499	578228
1500	579051
1501	579868
1502	580640
1503	581481
1504	582301
1505	583084
1506	583930
1507	584746
1508	585542
1509	586311
1510	587086
1511	587954
1512	588722
1513	589495
1514	590262
1515	591031
1516	591807
1517	592575
1518	593383
1519	594167
1520	595533
1521	596876
1522	597686
1523	598876
1524	600073
1525	600839
1526	601643
1527	602423
1528	603205
1529	603991
1530	604771
1531	605555
1532	606358
1533	607187
1534	608040
1535	608827
1536	609685
1537	610524
1538	611326
1539	612139
1540	612956
1541	613858
1542	614725
1543	615558
1544	616580
1545	617732
1546	618851
1547	620336
1548	621319
1549	622401
1550	623345
1551	624800
1552	626070
1553	626875
1554	627729
1555	628668
1556	629528
1557	630363
1558	631183
1559	631973
1560	632764
1561	633560
1562	634403
1563	635227
1564	636047
1565	636888
1566	637771
1567	638892
1568	640022
1569	641096
1570	642330
1571	643167
1572	644410
1573	645251
1574	646097
1575	646946
1576	647805
1577	648609
1578	649464
1579	650310
1580	651147
1581	651998
1582	652842
1583	653675
1584	654495
1585	655298
1586	656129
1587	656972
1588	657866
1589	658702
1590	659519
1591	660374
1592	661586
1593	662399
1594	663224
1595	664047
1596	664871
1597	665690
1598	666516
1599	667385
1600	668255
1601	669078
1602	669905
1603	670728
1604	671579
1605	672406
1606	673231
1607	674063
1608	674888
1609	675745
1610	676630
1611	677610
1612	678872
1613	679946
1614	680803
1615	681623
1616	682471
1617	683287
1618	684119
1619	684981
1620	685837
1621	686974
1622	687870
1623	688746
1624	689966
1625	690990
1626	692335
1627	693204
1628	694123
1629	695048
1630	695949
1631	696855
1632	697766
1633	698645
1634	699539
1635	700423
1636	701294
1637	702202
1638	703114
1639	704010
1640	704907
1641	705794
1642	706671
1643	707581
1644	708493
1645	709369
1646	710240
1647	711116
1648	712001
1649	712870
1650	713739
1651	714615
1652	715516
1653	716404
1654	717345
1655	718231
1656	719108
1657	720002
1658	720879
1659	721760
1660	722637
1661	723549
1662	724438
1663	725354
1664	726244
1665	727157
1666	728102
1667	728998
1668	729887
1669	730795
1670	731720
1671	732615
1672	733527
1673	734428
1674	735324
1675	736226
1676	737143
1677	738065
1678	738979
1679	739867
1680	740762
1681	741688
1682	742627
1683	743540
1684	744456
1685	745362
1686	746283
1687	747237
1688	748157
1689	749065
1690	749975
1691	750897
1692	751826
1693	752785
1694	753736
1695	754656
1696	755569
1697	756504
1698	757473
1699	758406
1700	759354
1701	760304
1702	761233
1703	762133
1704	763045
1705	763993
1706	764892
1707	765818
1708	766743
1709	767711
1710	768635
1711	769570
1712	770485
1713	771408
1714	772333
1715	773285
1716	774251
1717	775176
1718	776121
1719	777070
1720	778021
1721	778942
1722	779897
1723	780821
1724	781742
1725	782661
1726	783605
1727	784554
1728	785513
1729	786620
1730	787597
1731	788522
1732	789452
1733	790589
1734	791513
1735	792471
1736	793399
1737	794335
1738	795299
1739	796262
1740	797237
1741	798415
1742	799668
1743	800654
1744	801620
1745	802568
1746	803937
1747	805229
1748	806248
1749	807224
1750	808226
1751	809198
1752	810157
1753	811092
1754	812031
1755	812980
1756	813938
1757	814913
1758	815858
1759	816824
1760	817803
1761	818797
1762	819737
1763	820673
1764	821612
1765	822558
1766	823528
1767	824526
1768	825511
1769	826468
1770	827488
1771	828510
1772	829490
1773	830464
1774	831420
1775	832377
1776	833365
1777	834329
1778	835289
1779	836280
1780	837317
1781	838286
1782	839235
1783	840204
1784	841164
1785	842119
1786	843085
1787	844039
1788	845002
1789	845994
1790	847005
1791	848020
1792	849008
1793	849977
1794	850951
1795	851913
1796	852877
1797	853887
1798	854866
1799	855853
1800	856853
1801	857886
1802	858884
1803	859869
1804	860872
1805	861857
1806	862823
1807	863840
1808	864860
1809	865840
1810	866820
1811	867822
1812	868809
1813	869799
1814	870831
1815	871824
1816	872800
1817	873786
1818	874791
1819	875808
1820	876797
1821	877821
1822	878828
1823	879841
1824	880829
1825	882250
1826	883414
1827	884913
1828	885917
1829	886957
1830	888109
1831	889175
1832	890157
1833	891174
1834	892186
1835	893191
1836	894177
1837	895166
1838	896168
1839	897230
1840	898231
1841	899220
1842	900203
1843	901452
1844	902439
1845	903452
1846	904476
1847	905692
1848	906763
1849	907789
1850	908794
1851	909786
1852	910795
1853	911788
1854	912830
1855	913842
1856	914868
1857	915882
1858	916920
1859	917951
1860	918975
1861	920005
1862	921023
1863	922032
1864	923046
1865	924054
1866	925094
1867	926113
1868	927205
1869	928220
1870	929234
1871	930271
1872	931298
1873	932333
1874	933367
1875	934413
1876	935452
1877	936492
1878	937550
1879	938578
1880	939600
1881	940629
1882	941669
1883	942701
1884	943754
1885	944779
1886	945807
1887	946872
1888	947919
1889	948975
1890	950009
1891	951047
1892	952101
1893	953133
1894	954187
1895	955230
1896	956282
1897	957357
1898	958438
1899	959488
1900	960539
1901	961576
1902	962654
1903	963686
1904	964713
1905	965757
1906	966863
1907	967917
1908	968972
1909	970013
1910	971050
1911	972080
1912	973148
1913	974203
1914	975250
1915	976353
1916	977455
1917	978514
1918	979575
1919	980622
1920	981670
1921	982727
1922	983765
1923	984810
1924	985936
1925	987042
1926	988103
1927	989375
1928	990457
1929	991538
1930	992802
1931	993892
1932	994946
1933	996006
1934	997132
1935	998205
1936	999287
1937	1000361
1938	1001412
1939	1002498
1940	1003583
1941	1004670
1942	1005756
1943	1006887
1944	1008026
1945	1009171
1946	1010249
1947	1011330
1948	1012463
1949	1013598
1950	1014699
1951	1015848
1952	1017043
1953	1018213
1954	1019332
1955	1020438
1956	1021523
1957	1022630
1958	1023784
1959	1024879
1960	1025969
1961	1027126
1962	1028273
1963	1029381
1964	1030483
1965	1031590
1966	1032691
1967	1033770
1968	1034871
1969	1036003
1970	1037144
1971	1038269
1972	1039371
1973	1040495
1974	1041634
1975	1043105
1976	1044239
1977	1045335
1978	1046942
1979	1048644
1980	1049992
1981	1051475
1982	1052546
1983	1053619
1984	1054721
1985	1055886
1986	1057114
1987	1058181
1988	1059248
1989	1060322
1990	1061777
1991	1062907
1992	1063992
1993	1065068
1994	1066629
1995	1068005
1996	1069238
1997	1070475
1998	1071681
1999	1072892
2000	1074107


==> sub_final/encsa.tex <==
n	millisec
1	0
2	1
3	1
4	2
5	3
6	5
7	6
8	7
9	9
10	11
11	13
12	16
13	19
14	22
15	25
16	28
17	31
18	35
19	39
20	43
21	49
22	55
23	61
24	67
25	73
26	78
27	84
28	90
29	96
30	103
31	109
32	117
33	125
34	132
35	140
36	147
37	155
38	164
39	173
40	183
41	193
42	202
43	211
44	220
45	228
46	238
47	252
48	262
49	274
50	284
51	295
52	307
53	319
54	330
55	342
56	353
57	368
58	384
59	396
60	408
61	421
62	433
63	451
64	469
65	483
66	498
67	515
68	530
69	546
70	562
71	584
72	613
73	638
74	656
75	714
76	746
77	801
78	848
79	903
80	930
81	947
82	964
83	981
84	997
85	1014
86	1031
87	1048
88	1066
89	1083
90	1101
91	1119
92	1138
93	1157
94	1175
95	1194
96	1213
97	1233
98	1252
99	1273
100	1299
101	1321
102	1345
103	1368
104	1389
105	1414
106	1438
107	1459
108	1481
109	1503
110	1526
111	1548
112	1572
113	1595
114	1618
115	1642
116	1666
117	1691
118	1717
119	1742
120	1770
121	1795
122	1821
123	1846
124	1877
125	1905
126	1930
127	1955
128	1980
129	2005
130	2030
131	2058
132	2085
133	2122
134	2151
135	2182
136	2210
137	2238
138	2266
139	2294
140	2328
141	2361
142	2392
143	2431
144	2461
145	2490
146	2520
147	2550
148	2579
149	2615
150	2646
151	2678
152	2708
153	2740
154	2773
155	2804
156	2836
157	2871
158	2905
159	2937
160	2970
161	3003
162	3036
163	3070
164	3102
165	3135
166	3173
167	3207
168	3242
169	3276
170	3310
171	3344
172	3379
173	3415
174	3452
175	3491
176	3527
177	3566
178	3602
179	3639
180	3676
181	3713
182	3752
183	3790
184	3829
185	3872
186	3912
187	3950
188	3989
189	4027
190	4066
191	4105
192	4145
193	4185
194	4224
195	4264
196	4304
197	4345
198	4387
199	4426
200	4466
201	4508
202	4549
203	4591
204	4633
205	4674
206	4716
207	4758
208	4800
209	4842
210	4890
211	4933
212	4977
213	5020
214	5064
215	5107
216	5151
217	5195
218	5240
219	5284
220	5329
221	5374
222	5419
223	5462
224	5507
225	5553
226	5598
227	5643
228	5688
229	5786
230	5888
231	6038
232	6091
233	6177
234	6227
235	6277
236	6330
237	6381
238	6431
239	6485
240	6534
241	6587
242	6637
243	6689
244	6738
245	6791
246	6843
247	6900
248	6953
249	7007
250	7063
251	7117
252	7173
253	7227
254	7284
255	7342
256	7402
257	7460
258	7518
259	7577
260	7635
261	7694
262	7751
263	7810
264	7869
265	7925
266	7984
267	8044
268	8104
269	8166
270	8225
271	8283
272	8341
273	8403
274	8464
275	8522
276	8581
277	8638
278	8701
279	8763
280	8826
281	8889
282	8948
283	9012
284	9076
285	9141
286	9205
287	9273
288	9338
289	9406
290	9472
291	9534
292	9598
293	9663
294	9727
295	9794
296	9860
297	9923
298	9989
299	10055
300	10118
301	10189
302	10259
303	10324
304	10393
305	10461
306	10529
307	10600
308	10670
309	10737
310	10807
311	10878
312	10945
313	11017
314	11088
315	11162
316	11233
317	11302
318	11370
319	11435
320	11505
321	11584
322	11673
323	11750
324	11840
325	11920
326	11996
327	12070
328	12142
329	12212
330	12287
331	12375
332	12466
333	12539
334	12613
335	12687
336	12763
337	12839
338	12918
339	12997
340	13078
341	13154
342	13232
343	13309
344	13391
345	13475
346	13550
347	13630
348	13715
349	13798
350	13875
351	13958
352	14042
353	14129
354	14216
355	14309
356	14400
357	14492
358	14579
359	14660
360	14739
361	14819
362	14899
363	14979
364	15055
365	15136
366	15217
367	15299
368	15386
369	15471
370	15551
371	15634
372	15716
373	15802
374	15888
375	15973
376	16060
377	16144
378	16228
379	16310
380	16396
381	16480
382	16561
383	16646
384	16732
385	16824
386	16913
387	17004
388	17094
389	17186
390	17272
391	17365
392	17454
393	17547
394	17634
395	17721
396	17808
397	17894
398	17979
399	18066
400	18155
401	18242
402	18331
403	18424
404	18517
405	18606
406	18695
407	18780
408	18870
409	18959
410	19048
411	19139
412	19232
413	19328
414	19424
415	19522
416	19613
417	19705
418	19794
419	19886
420	19979
421	20072
422	20165
423	20257
424	20350
425	20450
426	20545
427	20637
428	20730
429	20825
430	20919
431	21014
432	21108
433	21198
434	21294
435	21389
436	21485
437	21586
438	21706
439	21818
440	21921
441	22020
442	22117
443	22228
444	22338
445	22437
446	22537
447	22633
448	22733
449	22833
450	22932
451	23031
452	23132
453	23235
454	23343
455	23445
456	23546
457	23646
458	23747
459	23852
460	23951
461	24053
462	24154
463	24257
464	24359
465	24473
466	24580
467	24691
468	24797
469	24903
470	25013
471	25127
472	25239
473	25349
474	25455
475	25557
476	25662
477	25767
478	25873
479	25977
480	26083
481	26190
482	26299
483	26411
484	26526
485	26641
486	26755
487	26870
488	26977
489	27083
490	27194
491	27301
492	27409
493	27518
494	27627
495	27733
496	27848
497	27958
498	28070
499	28189
500	28298
501	28410
502	28522
503	28633
504	28748
505	28861
506	28974
507	29088
508	29203
509	29316
510	29430
511	29543
512	29659
513	29775
514	29893
515	30008
516	30121
517	30239
518	30364
519	30482
520	30596
521	30712
522	30831
523	30953
524	31076
525	31191
526	31306
527	31423
528	31548
529	31706
530	31835
531	31951
532	32077
533	32205
534	32344
535	32473
536	32595
537	32721
538	32844
539	32966
540	33088
541	33208
542	33331
543	33453
544	33576
545	33700
546	33824
547	33946
548	34071
549	34194
550	34320
551	34443
552	34566
553	34698
554	34827
555	34958
556	35084
557	35212
558	35336
559	35461
560	35588
561	35712
562	35839
563	35967
564	36100
565	36235
566	36371
567	36510
568	36642
569	36769
570	36903
571	37030
572	37158
573	37285
574	37416
575	37547
576	37676
577	37806
578	37940
579	38072
580	38205
581	38338
582	38469
583	38602
584	38734
585	38868
586	39003
587	39139
588	39271
589	39408
590	39544
591	39680
592	39826
593	39966
594	40101
595	40241
596	40375
597	40515
598	40651
599	40785
600	40921
601	41057
602	41192
603	41331
604	41479
605	41621
606	41809
607	41954
608	42094
609	42231
610	42399
611	42539
612	42677
613	42815
614	42961
615	43099
616	43239
617	43381
618	43520
619	43665
620	43806
621	43952
622	44093
623	44246
624	44394
625	44536
626	44681
627	44821
628	44968
629	45113
630	45267
631	45415
632	45572
633	45724
634	45874
635	46017
636	46163
637	46307
638	46450
639	46597
640	46743
641	46893
642	47040
643	47192
644	47337
645	47489
646	47631
647	47781
648	47933
649	48085
650	48233
651	48381
652	48533
653	48690
654	48850
655	49011
656	49173
657	49323
658	49475
659	49623
660	49775
661	49931
662	50096
663	50254
664	50417
665	50580
666	50730
667	50889
668	51044
669	51201
670	51357
671	51523
672	51700
673	51883
674	52041
675	52212
676	52397
677	52555
678	52717
679	52882
680	53037
681	53197
682	53374
683	53533
684	53692
685	53855
686	54013
687	54170
688	54332
689	54491
690	54652
691	54814
692	54972
693	55141
694	55308
695	55466
696	55625
697	55789
698	55955
699	56117
700	56279
701	56443
702	56606
703	56770
704	56934
705	57170
706	57356
707	57558
708	57749
709	57940
710	58145
711	58363
712	58560
713	58758
714	58958
715	59170
716	59367
717	59548
718	59740
719	59918
720	60098
721	60283
722	60483
723	60667
724	60863
725	61066
726	61254
727	61453
728	61688
729	61959
730	62148
731	62334
732	62552
733	62842
734	63076
735	63268
736	63451
737	63631
738	63804
739	63981
740	64149
741	64322
742	64496
743	64671
744	64846
745	65041
746	65224
747	65398
748	65570
749	65753
750	65928
751	66107
752	66282
753	66470
754	66664
755	66843
756	67026
757	67211
758	67388
759	67568
760	67747
761	67929
762	68125
763	68308
764	68484
765	68669
766	68855
767	69049
768	69231
769	69414
770	69597
771	69784
772	69989
773	70205
774	70407
775	70597
776	70807
777	70990
778	71173
779	71358
780	71547
781	71730
782	71914
783	72103
784	72294
785	72480
786	72665
787	72854
788	73044
789	73227
790	73417
791	73607
792	73792
793	73980
794	74166
795	74353
796	74544
797	74729
798	74918
799	75115
800	75315
801	75508
802	75702
803	75894
804	76090
805	76283
806	76469
807	76653
808	76837
809	77028
810	77220
811	77425
812	77621
813	77812
814	78009
815	78207
816	78406
817	78608
818	78804
819	79009
820	79205
821	79408
822	79603
823	79798
824	79995
825	80210
826	80410
827	80632
828	80836
829	81029
830	81225
831	81418
832	81614
833	81816
834	82012
835	82214
836	82411
837	82612
838	82824
839	83031
840	83232
841	83431
842	83627
843	83826
844	84026
845	84226
846	84428
847	84629
848	84837
849	85041
850	85246
851	85450
852	85649
853	85853
854	86056
855	86261
856	86464
857	86671
858	86874
859	87080
860	87284
861	87491
862	87697
863	87909
864	88113
865	88318
866	88526
867	88731
868	88939
869	89150
870	89354
871	89560
872	89766
873	89974
874	90198
875	90404
876	90629
877	90858
878	91077
879	91291
880	91502
881	91711
882	91923
883	92128
884	92342
885	92549
886	92761
887	92988
888	93212
889	93429
890	93648
891	93870
892	94081
893	94476
894	94701
895	94917
896	95138
897	95366
898	95587
899	95801
900	96019
901	96243
902	96462
903	96678
904	96894
905	97112
906	97336
907	97565
908	97793
909	98010
910	98228
911	98449
912	98820
913	99042
914	99299
915	99519
916	99742
917	99965
918	100204
919	100423
920	100653
921	100883
922	101101
923	101319
924	101544
925	101786
926	102005
927	102228
928	102453
929	102680
930	102914
931	103143
932	103362
933	103586
934	103817
935	104048
936	104275
937	104496
938	104722
939	104948
940	105175
941	105403
942	105633
943	105860
944	106086
945	106316
946	106545
947	106776
948	107003
949	107233
950	107466
951	107706
952	107946
953	108182
954	108405
955	108634
956	108863
957	109093
958	109322
959	109557
960	109787
961	110022
962	110272
963	110519
964	110774
965	111017
966	111260
967	111499
968	111739
969	111982
970	112220
971	112458
972	112684
973	112914
974	113151
975	113384
976	113614
977	113852
978	114086
979	114319
980	114549
981	114791
982	115037
983	115280
984	115524
985	115768
986	116010
987	116259
988	116498
989	116737
990	116990
991	117242
992	117488
993	117739
994	117988
995	118229
996	118468
997	118706
998	118942
999	119187
1000	119429
1001	119667
1002	119907
1003	120180
1004	120440
1005	120697
1006	120955
1007	121206
1008	121445
1009	121692
1010	121944
1011	122188
1012	122430
1013	122681
1014	122930
1015	123192
1016	123443
1017	123703
1018	123950
1019	124197
1020	124451
1021	124710
1022	124967
1023	125226
1024	125481
1025	125734
1026	125987
1027	126231
1028	126481
1029	126742
1030	126997
1031	127245
1032	127495
1033	127741
1034	127996
1035	128254
1036	128500
1037	128765
1038	129019
1039	129267
1040	129513
1041	129760
1042	130037
1043	130320
1044	130605
1045	130908
1046	131187
1047	131474
1048	131739
1049	131997
1050	132255
1051	132505
1052	132755
1053	133020
1054	133286
1055	133552
1056	133820
1057	134088
1058	134338
1059	134598
1060	134850
1061	135107
1062	135363
1063	135621
1064	135882
1065	136152
1066	136418
1067	136684
1068	136954
1069	137212
1070	137478
1071	137751
1072	138015
1073	138277
1074	138536
1075	138796
1076	139069
1077	139345
1078	139623
1079	139886
1080	140179
1081	140471
1082	140743
1083	141005
1084	141264
1085	141525
1086	141785
1087	142050
1088	142310
1089	142574
1090	142854
1091	143125
1092	143403
1093	143683
1094	143961
1095	144226
1096	144497
1097	144771
1098	145052
1099	145331
1100	145596
1101	145869
1102	146143
1103	146413
1104	146679
1105	146946
1106	147215
1107	147484
1108	147753
1109	148034
1110	148302
1111	148568
1112	148837
1113	149103
1114	149373
1115	149643
1116	149923
1117	150213
1118	150502
1119	150777
1120	151066
1121	151353
1122	151632
1123	151910
1124	152187
1125	152470
1126	152755
1127	153034
1128	153306
1129	153594
1130	153873
1131	154148
1132	154418
1133	154691
1134	154971
1135	155248
1136	155540
1137	155831
1138	156114
1139	156396
1140	156690
1141	156977
1142	157263
1143	157559
1144	157862
1145	158153
1146	158434
1147	158724
1148	159028
1149	159317
1150	159605
1151	159903
1152	160196
1153	160491
1154	160793
1155	161076
1156	161368
1157	161670
1158	161963
1159	162257
1160	162564
1161	162849
1162	163140
1163	163446
1164	163740
1165	164031
1166	164317
1167	164606
1168	164894
1169	165186
1170	165472
1171	165762
1172	166054
1173	166344
1174	166635
1175	166944
1176	167246
1177	167539
1178	167833
1179	168131
1180	168429
1181	168720
1182	169022
1183	169326
1184	169636
1185	169952
1186	170245
1187	170583
1188	170901
1189	171207
1190	171512
1191	171819
1192	172106
1193	172391
1194	172684
1195	172978
1196	173281
1197	173594
1198	173906
1199	174209
1200	174500
1201	174792
1202	175101
1203	175409
1204	175701
1205	175998
1206	176303
1207	176606
1208	176902
1209	177217
1210	177522
1211	177834
1212	178146
1213	178457
1214	178755
1215	179065
1216	179369
1217	179680
1218	180003
1219	180315
1220	180655
1221	180960
1222	181265
1223	181577
1224	181889
1225	182187
1226	182481
1227	182781
1228	183092
1229	183392
1230	183700
1231	184001
1232	184299
1233	184604
1234	184909
1235	185208
1236	185511
1237	185816
1238	186125
1239	186431
1240	186738
1241	187055
1242	187376
1243	187695
1244	188016
1245	188339
1246	188654
1247	188979
1248	189306
1249	189636
1250	189969
1251	190299
1252	190662
1253	190977
1254	191279
1255	191602
1256	191920
1257	192231
1258	192541
1259	192848
1260	193160
1261	193472
1262	193777
1263	194102
1264	194424
1265	194749
1266	195061
1267	195375
1268	195703
1269	196037
1270	196385
1271	196730
1272	197049
1273	197364
1274	197680
1275	197998
1276	198309
1277	198626
1278	198940
1279	199263
1280	199580
1281	199927
1282	200262
1283	200607
1284	200941
1285	201258
1286	201586
1287	201903
1288	202232
1289	202554
1290	202876
1291	203203
1292	203523
1293	203846
1294	204174
1295	204494
1296	204826
1297	205157
1298	205481
1299	205820
1300	206157
1301	206483
1302	206810
1303	207129
1304	207450
1305	207780
1306	208102
1307	208435
1308	208763
1309	209116
1310	209442
1311	209773
1312	210121
1313	210487
1314	210843
1315	211206
1316	211538
1317	211879
1318	212212
1319	212545
1320	212884
1321	213226
1322	213558
1323	213888
1324	214222
1325	214563
1326	214903
1327	215242
1328	215575
1329	215914
1330	216256
1331	216596
1332	216932
1333	217272
1334	217616
1335	217951
1336	218287
1337	218629
1338	218962
1339	219317
1340	219666
1341	220031
1342	220391
1343	220735
1344	221073
1345	221412
1346	221752
1347	222095
1348	222438
1349	222775
1350	223114
1351	223457
1352	223806
1353	224145
1354	224480
1355	224824
1356	225158
1357	225497
1358	225840
1359	226179
1360	226522
1361	226878
1362	227224
1363	227582
1364	227924
1365	228265
1366	228601
1367	228944
1368	229288
1369	229636
1370	230000
1371	230349
1372	230709
1373	231054
1374	231410
1375	231790
1376	232135
1377	232484
1378	232832
1379	233183
1380	233526
1381	233873
1382	234224
1383	234586
1384	234941
1385	235303
1386	235670
1387	236031
1388	236377
1389	236728
1390	237074
1391	237426
1392	237772
1393	238143
1394	238514
1395	238859
1396	239218
1397	239571
1398	239945
1399	240297
1400	240702
1401	241053
1402	241402
1403	241788
1404	242153
1405	242519
1406	242875
1407	243231
1408	243588
1409	243943
1410	244305
1411	244671
1412	245026
1413	245388
1414	245747
1415	246105
1416	246461
1417	246832
1418	247193
1419	247554
1420	247924
1421	248287
1422	248649
1423	249015
1424	249379
1425	249753
1426	250146
1427	250527
1428	250885
1429	251244
1430	251608
1431	251968
1432	252324
1433	252695
1434	253056
1435	253425
1436	253788
1437	254149
1438	254512
1439	254877
1440	255245
1441	255613
1442	255971
1443	256333
1444	256692
1445	257059
1446	257426
1447	257787
1448	258155
1449	258525
1450	258893
1451	259260
1452	259620
1453	260004
1454	260388
1455	260766
1456	261134
1457	261504
1458	261868
1459	262245
1460	262613
1461	262982
1462	263350
1463	263734
1464	264115
1465	264488
1466	264861
1467	265236
1468	265604
1469	265981
1470	266349
1471	266728
1472	267087
1473	267448
1474	267804
1475	268168
1476	268523
1477	268885
1478	269249
1479	269614
1480	270007
1481	270401
1482	270799
1483	271188
1484	271573
1485	271950
1486	272324
1487	272700
1488	273084
1489	273455
1490	273823
1491	274205
1492	274593
1493	274969
1494	275347
1495	275725
1496	276100
1497	276478
1498	276850
1499	277229
1500	277603
1501	277991
1502	278376
1503	278760
1504	279135
1505	279509
1506	279909
1507	280297
1508	280698
1509	281092
1510	281473
1511	281871
1512	282265
1513	282658
1514	283046
1515	283445
1516	283840
1517	284227
1518	284609
1519	285001
1520	285377
1521	285753
1522	286133
1523	286518
1524	286902
1525	287289
1526	287686
1527	288086
1528	288488
1529	288884
1530	289272
1531	289661
1532	290071
1533	290479
1534	290884
1535	291272
1536	291659
1537	292047
1538	292430
1539	292836
1540	293222
1541	293609
1542	294005
1543	294399
1544	294797
1545	295196
1546	295594
1547	295987
1548	296384
1549	296791
1550	297206
1551	297616
1552	298013
1553	298423
1554	298817
1555	299210
1556	299619
1557	300065
1558	300483
1559	300904
1560	301300
1561	301700
1562	302116
1563	302542
1564	302973
1565	303395
1566	303798
1567	304195
1568	304590
1569	305001
1570	305406
1571	305818
1572	306222
1573	306639
1574	307052
1575	307481
1576	307885
1577	308291
1578	308703
1579	309112
1580	309531
1581	309964
1582	310397
1583	310810
1584	311226
1585	311639
1586	312044
1587	312451
1588	312858
1589	313274
1590	313697
1591	314115
1592	314507
1593	314923
1594	315322
1595	315733
1596	316153
1597	316577
1598	316999
1599	317414
1600	317824
1601	318244
1602	318662
1603	319065
1604	319470
1605	319894
1606	320352
1607	320764
1608	321179
1609	321597
1610	322010
1611	322441
1612	322865
1613	323273
1614	323683
1615	324087
1616	324491
1617	324922
1618	325347
1619	325756
1620	326177
1621	326608
1622	327025
1623	327460
1624	327882
1625	328301
1626	328716
1627	329128
1628	329541
1629	329990
1630	330439
1631	330878
1632	331290
1633	331724
1634	332167
1635	332585
1636	333001
1637	333427
1638	333845
1639	334280
1640	334693
1641	335114
1642	335533
1643	335968
1644	336388
1645	336810
1646	337243
1647	337683
1648	338118
1649	338554
1650	338987
1651	339418
1652	339867
1653	340309
1654	340752
1655	341190
1656	341608
1657	342037
1658	342456
1659	342878
1660	343307
1661	343743
1662	344166
1663	344596
1664	345030
1665	345472
1666	345917
1667	346365
1668	346806
1669	347249
1670	347691
1671	348136
1672	348570
1673	349006
1674	349438
1675	349894
1676	350337
1677	350807
1678	351242
1679	351702
1680	352131
1681	352578
1682	353028
1683	353459
1684	353881
1685	354303
1686	354736
1687	355165
1688	355611
1689	356052
1690	356502
1691	356953
1692	357401
1693	357834
1694	358267
1695	358704
1696	359136
1697	359577
1698	360040
1699	360536
1700	360964
1701	361407
1702	361842
1703	362276
1704	362707
1705	363156
1706	363596
1707	364035
1708	364490
1709	364959
1710	365416
1711	365864
1712	366309
1713	366765
1714	367203
1715	367647
1716	368090
1717	368529
1718	368987
1719	369443
1720	369957
1721	370417
1722	370894
1723	371341
1724	371783
1725	372226
1726	372675
1727	373122
1728	373570
1729	374015
1730	374455
1731	374906
1732	375357
1733	375795
1734	376241
1735	376695
1736	377135
1737	377582
1738	378031
1739	378484
1740	378943
1741	379401
1742	379935
1743	380407
1744	380852
1745	381315
1746	381765
1747	382229
1748	382702
1749	383259
1750	383984
1751	384657
1752	385130
1753	385607
1754	386291
1755	386884
1756	387341
1757	387810
1758	388423
1759	388903
1760	389375
1761	389861
1762	390354
1763	390841
1764	391300
1765	391773
1766	392231
1767	392704
1768	393435
1769	393918
1770	394385
1771	394847
1772	395296
1773	395776
1774	396223
1775	396710
1776	397456
1777	398196
1778	398672
1779	399121
1780	399847
1781	400496
1782	401011
1783	401503
1784	402095
1785	402558
1786	403063
1787	403523
1788	403967
1789	404423
1790	404869
1791	405395
1792	406115
1793	406710
1794	407154
1795	407616
1796	408480
1797	409059
1798	409523
1799	410038
1800	410536
1801	411000
1802	411469
1803	411928
1804	412383
1805	412845
1806	413303
1807	413791
1808	414272
1809	414759
1810	415336
1811	416257
1812	416964
1813	417560
1814	418142
1815	418784
1816	419486
1817	420141
1818	420877
1819	421622
1820	422140
1821	422631
1822	423221
1823	423816
1824	424287
1825	424893
1826	425468
1827	425972
1828	426468
1829	426932
1830	427500
1831	427973
1832	428435
1833	429123
1834	429619
1835	430222
1836	430690
1837	431184
1838	431651
1839	432365
1840	432830
1841	433308
1842	433777
1843	434271
1844	434949
1845	435442
1846	435949
1847	436602
1848	437095
1849	437599
1850	438082
1851	438674
1852	439283
1853	440007
1854	440613
1855	441114
1856	441618
1857	442203
1858	442925
1859	443582
1860	444210
1861	444710
1862	445260
1863	445803
1864	446294
1865	446768
1866	447422
1867	447931
1868	448446
1869	449115
1870	449667
1871	450196
1872	450681
1873	451289
1874	451854
1875	452432
1876	453065
1877	453704
1878	454216
1879	454718
1880	455224
1881	455732
1882	456350
1883	456965
1884	457462
1885	457946
1886	458430
1887	458920
1888	459459
1889	459988
1890	460507
1891	461025
1892	461515
1893	462000
1894	462484
1895	462965
1896	463482
1897	463984
1898	464465
1899	464949
1900	465436
1901	465917
1902	466395
1903	466884
1904	467375
1905	467865
1906	468348
1907	468858
1908	469354
1909	469868
1910	470403
1911	470906
1912	471394
1913	471885
1914	472379
1915	472868
1916	473361
1917	473859
1918	474348
1919	474842
1920	475334
1921	475827
1922	476323
1923	476818
1924	477316
1925	477810
1926	478303
1927	478793
1928	479298
1929	479804
1930	480381
1931	480897
1932	481390
1933	481904
1934	482404
1935	482904
1936	483400
1937	483891
1938	484377
1939	484871
1940	485363
1941	485857
1942	486357
1943	486875
1944	487395
1945	487905
1946	488397
1947	488894
1948	489419
1949	489953
1950	490468
1951	490984
1952	491515
1953	492042
1954	492540
1955	493060
1956	493559
1957	494066
1958	494569
1959	495074
1960	495580
1961	496086
1962	496585
1963	497108
1964	497612
1965	498121
1966	498627
1967	499143
1968	499677
1969	500210
1970	500709
1971	501224
1972	501731
1973	502254
1974	502773
1975	503285
1976	503790
1977	504301
1978	504803
1979	505318
1980	505823
1981	506349
1982	506866
1983	507395
1984	507922
1985	508435
1986	508943
1987	509487
1988	510051
1989	510569
1990	511083
1991	511601
1992	512117
1993	512659
1994	513184
1995	513694
1996	514211
1997	514721
1998	515232
1999	515741
2000	516277


==> sub_final/encta.tex <==
n	millisec
1	0
2	1
3	3
4	4
5	6
6	8
7	9
8	11
9	13
10	15
11	16
12	18
13	20
14	23
15	26
16	29
17	32
18	36
19	39
20	43
21	46
22	49
23	52
24	56
25	60
26	63
27	67
28	71
29	75
30	78
31	82
32	87
33	92
34	97
35	102
36	109
37	116
38	121
39	127
40	133
41	142
42	148
43	154
44	160
45	166
46	172
47	178
48	184
49	191
50	198
51	204
52	211
53	217
54	226
55	232
56	239
57	248
58	258
59	268
60	275
61	283
62	292
63	299
64	307
65	315
66	324
67	333
68	343
69	352
70	360
71	369
72	377
73	389
74	398
75	406
76	415
77	424
78	434
79	444
80	453
81	463
82	476
83	486
84	497
85	508
86	518
87	528
88	538
89	548
90	558
91	570
92	582
93	592
94	604
95	620
96	633
97	649
98	660
99	672
100	688
101	700
102	712
103	723
104	735
105	748
106	763
107	776
108	789
109	801
110	819
111	835
112	849
113	862
114	876
115	893
116	907
117	920
118	934
119	947
120	960
121	974
122	994
123	1010
124	1024
125	1039
126	1053
127	1069
128	1083
129	1104
130	1119
131	1134
132	1149
133	1164
134	1180
135	1195
136	1210
137	1225
138	1247
139	1263
140	1278
141	1293
142	1308
143	1327
144	1344
145	1360
146	1376
147	1392
148	1414
149	1430
150	1447
151	1463
152	1479
153	1498
154	1523
155	1540
156	1562
157	1580
158	1597
159	1615
160	1634
161	1651
162	1677
163	1695
164	1714
165	1734
166	1754
167	1773
168	1801
169	1821
170	1840
171	1871
172	1891
173	1912
174	1934
175	1954
176	1973
177	1994
178	2015
179	2036
180	2057
181	2077
182	2097
183	2117
184	2141
185	2170
186	2195
187	2215
188	2235
189	2255
190	2280
191	2301
192	2323
193	2343
194	2363
195	2385
196	2408
197	2428
198	2449
199	2472
200	2501
201	2521
202	2543
203	2569
204	2597
205	2622
206	2648
207	2670
208	2695
209	2717
210	2739
211	2763
212	2786
213	2809
214	2831
215	2855
216	2879
217	2901
218	2924
219	2947
220	2986
221	3021
222	3064
223	3089
224	3113
225	3135
226	3169
227	3194
228	3219
229	3245
230	3281
231	3310
232	3346
233	3372
234	3404
235	3432
236	3458
237	3506
238	3541
239	3567
240	3595
241	3629
242	3656
243	3684
244	3720
245	3759
246	3803
247	3845
248	3902
249	3944
250	3994
251	4041
252	4090
253	4143
254	4184
255	4216
256	4248
257	4280
258	4310
259	4347
260	4379
261	4409
262	4441
263	4475
264	4511
265	4541
266	4573
267	4618
268	4651
269	4683
270	4714
271	4745
272	4770
273	4796
274	4823
275	4850
276	4881
277	4908
278	4934
279	4960
280	4985
281	5011
282	5036
283	5065
284	5092
285	5117
286	5142
287	5168
288	5196
289	5235
290	5261
291	5287
292	5313
293	5339
294	5373
295	5405
296	5442
297	5474
298	5501
299	5527
300	5554
301	5581
302	5614
303	5650
304	5677
305	5705
306	5733
307	5762
308	5789
309	5821
310	5848
311	5876
312	5908
313	5937
314	5966
315	5995
316	6023
317	6053
318	6081
319	6109
320	6139
321	6170
322	6199
323	6230
324	6261
325	6288
326	6317
327	6346
328	6374
329	6405
330	6432
331	6460
332	6489
333	6516
334	6544
335	6574
336	6604
337	6641
338	6669
339	6703
340	6743
341	6781
342	6822
343	6866
344	6906
345	6955
346	6992
347	7032
348	7070
349	7106
350	7153
351	7189
352	7224
353	7261
354	7297
355	7337
356	7370
357	7403
358	7442
359	7480
360	7516
361	7565
362	7618
363	7653
364	7692
365	7735
366	7765
367	7796
368	7829
369	7859
370	7889
371	7924
372	7959
373	7994
374	8033
375	8062
376	8092
377	8123
378	8155
379	8185
380	8222
381	8254
382	8285
383	8317
384	8349
385	8380
386	8410
387	8441
388	8473
389	8504
390	8535
391	8568
392	8605
393	8637
394	8668
395	8711
396	8742
397	8773
398	8807
399	8839
400	8884
401	8915
402	8962
403	8994
404	9026
405	9063
406	9095
407	9129
408	9162
409	9193
410	9227
411	9259
412	9291
413	9324
414	9357
415	9394
416	9426
417	9462
418	9495
419	9527
420	9560
421	9597
422	9630
423	9662
424	9694
425	9730
426	9768
427	9803
428	9841
429	9879
430	9911
431	9944
432	9986
433	10019
434	10052
435	10086
436	10120
437	10157
438	10190
439	10223
440	10257
441	10290
442	10323
443	10356
444	10389
445	10422
446	10454
447	10488
448	10521
449	10568
450	10608
451	10642
452	10675
453	10708
454	10745
455	10779
456	10813
457	10850
458	10884
459	10917
460	10951
461	10984
462	11019
463	11054
464	11088
465	11129
466	11164
467	11197
468	11241
469	11275
470	11308
471	11358
472	11394
473	11434
474	11469
475	11505
476	11540
477	11576
478	11617
479	11654
480	11691
481	11726
482	11762
483	11802
484	11837
485	11873
486	11916
487	11951
488	11987
489	12022
490	12060
491	12095
492	12130
493	12166
494	12204
495	12242
496	12276
497	12316
498	12356
499	12391
500	12426
501	12461
502	12507
503	12548
504	12586
505	12628
506	12667
507	12706
508	12756
509	12823
510	12863
511	12901
512	12940
513	12982
514	13023
515	13063
516	13099
517	13139
518	13177
519	13218
520	13257
521	13295
522	13343
523	13381
524	13427
525	13466
526	13508
527	13556
528	13607
529	13647
530	13685
531	13728
532	13764
533	13808
534	13850
535	13887
536	13924
537	13962
538	14000
539	14049
540	14086
541	14123
542	14164
543	14204
544	14245
545	14283
546	14320
547	14358
548	14396
549	14434
550	14482
551	14529
552	14568
553	14610
554	14655
555	14693
556	14737
557	14777
558	14819
559	14857
560	14896
561	14936
562	14976
563	15018
564	15057
565	15100
566	15139
567	15179
568	15219
569	15260
570	15300
571	15339
572	15384
573	15424
574	15463
575	15506
576	15546
577	15590
578	15637
579	15693
580	15733
581	15773
582	15813
583	15853
584	15892
585	15932
586	15979
587	16019
588	16062
589	16107
590	16147
591	16187
592	16227
593	16279
594	16319
595	16359
596	16398
597	16439
598	16479
599	16520
600	16561
601	16606
602	16647
603	16686
604	16733
605	16773
606	16817
607	16857
608	16911
609	16952
610	16995
611	17037
612	17085
613	17126
614	17169
615	17210
616	17250
617	17292
618	17333
619	17374
620	17415
621	17456
622	17498
623	17542
624	17589
625	17643
626	17686
627	17731
628	17775
629	17820
630	17863
631	17910
632	17954
633	18000
634	18044
635	18090
636	18135
637	18176
638	18220
639	18263
640	18304
641	18346
642	18387
643	18428
644	18469
645	18511
646	18553
647	18597
648	18644
649	18686
650	18728
651	18769
652	18810
653	18855
654	18896
655	18938
656	18979
657	19020
658	19062
659	19103
660	19148
661	19189
662	19231
663	19272
664	19313
665	19354
666	19396
667	19437
668	19478
669	19520
670	19561
671	19605
672	19646
673	19689
674	19730
675	19774
676	19820
677	19863
678	19908
679	19953
680	20004
681	20051
682	20093
683	20138
684	20180
685	20222
686	20267
687	20308
688	20349
689	20390
690	20433
691	20475
692	20518
693	20559
694	20606
695	20647
696	20690
697	20750
698	20794
699	20840
700	20883
701	20928
702	20971
703	21014
704	21057
705	21111
706	21154
707	21197
708	21243
709	21286
710	21328
711	21370
712	21415
713	21457
714	21500
715	21545
716	21595
717	21641
718	21687
719	21734
720	21779
721	21825
722	21870
723	21930
724	21976
725	22024
726	22069
727	22114
728	22160
729	22210
730	22264
731	22314
732	22361
733	22407
734	22454
735	22499
736	22546
737	22594
738	22640
739	22684
740	22731
741	22780
742	22829
743	22873
744	22942
745	22990
746	23036
747	23082
748	23126
749	23175
750	23220
751	23265
752	23311
753	23358
754	23407
755	23455
756	23515
757	23565
758	23614
759	23659
760	23702
761	23759
762	23803
763	23855
764	23901
765	23945
766	23988
767	24032
768	24076
769	24119
770	24165
771	24208
772	24258
773	24308
774	24363
775	24408
776	24474
777	24548
778	24595
779	24642
780	24689
781	24734
782	24780
783	24829
784	24878
785	24934
786	24983
787	25053
788	25102
789	25151
790	25204
791	25257
792	25310
793	25358
794	25409
795	25459
796	25509
797	25562
798	25609
799	25655
800	25701
801	25746
802	25792
803	25842
804	25892
805	25938
806	25988
807	26033
808	26080
809	26132
810	26185
811	26231
812	26278
813	26325
814	26378
815	26430
816	26477
817	26530
818	26581
819	26627
820	26675
821	26722
822	26768
823	26814
824	26860
825	26909
826	26956
827	27008
828	27054
829	27101
830	27150
831	27206
832	27253
833	27300
834	27347
835	27394
836	27440
837	27491
838	27542
839	27590
840	27637
841	27705
842	27753
843	27800
844	27850
845	27897
846	27944
847	27992
848	28047
849	28094
850	28142
851	28190
852	28238
853	28293
854	28341
855	28389
856	28436
857	28484
858	28545
859	28592
860	28641
861	28689
862	28737
863	28788
864	28841
865	28892
866	28944
867	28996
868	29045
869	29097
870	29153
871	29205
872	29256
873	29308
874	29360
875	29410
876	29471
877	29527
878	29577
879	29626
880	29696
881	29746
882	29795
883	29845
884	29895
885	29944
886	29994
887	30043
888	30094
889	30143
890	30193
891	30242
892	30291
893	30344
894	30394
895	30446
896	30498
897	30555
898	30607
899	30660
900	30717
901	30771
902	30820
903	30875
904	30924
905	30973
906	31030
907	31080
908	31129
909	31179
910	31228
911	31278
912	31329
913	31379
914	31430
915	31484
916	31552
917	31607
918	31680
919	31752
920	31805
921	31861
922	31912
923	31969
924	32021
925	32077
926	32128
927	32180
928	32233
929	32284
930	32335
931	32421
932	32472
933	32529
934	32579
935	32629
936	32681
937	32753
938	32809
939	32862
940	32913
941	32966
942	33021
943	33076
944	33135
945	33194
946	33257
947	33316
948	33376
949	33428
950	33480
951	33549
952	33639
953	33725
954	33812
955	33907
956	34013
957	34116
958	34205
959	34323
960	34416
961	34520
962	34584
963	34685
964	34820
965	34873
966	34931
967	34989
968	35048
969	35105
970	35192
971	35277
972	35362
973	35467
974	35565
975	35660
976	35736
977	35812
978	35909
979	35991
980	36075
981	36138
982	36192
983	36243
984	36295
985	36345
986	36411
987	36470
988	36525
989	36581
990	36635
991	36687
992	36761
993	36814
994	36869
995	36935
996	36989
997	37044
998	37115
999	37203
1000	37337
1001	37429
1002	37523
1003	37615
1004	37710
1005	37803
1006	37892
1007	38020
1008	38100
1009	38159
1010	38214
1011	38270
1012	38324
1013	38383
1014	38443
1015	38505
1016	38610
1017	38751
1018	38882
1019	38940
1020	39025
1021	39081
1022	39139
1023	39198
1024	39279
1025	39342
1026	39402
1027	39459
1028	39517
1029	39573
1030	39634
1031	39690
1032	39750
1033	39808
1034	39863
1035	39920
1036	39976
1037	40033
1038	40116
1039	40171
1040	40228
1041	40286
1042	40344
1043	40404
1044	40467
1045	40525
1046	40583
1047	40641
1048	40700
1049	40756
1050	40814
1051	40870
1052	40928
1053	40984
1054	41042
1055	41099
1056	41154
1057	41214
1058	41272
1059	41334
1060	41392
1061	41453
1062	41512
1063	41569
1064	41628
1065	41683
1066	41751
1067	41810
1068	41866
1069	41930
1070	42005
1071	42067
1072	42130
1073	42192
1074	42257
1075	42316
1076	42373
1077	42437
1078	42499
1079	42559
1080	42626
1081	42690
1082	42755
1083	42820
1084	42879
1085	42939
1086	43001
1087	43088
1088	43150
1089	43226
1090	43297
1091	43361
1092	43425
1093	43486
1094	43553
1095	43618
1096	43678
1097	43739
1098	43803
1099	43863
1100	43923
1101	43986
1102	44046
1103	44113
1104	44173
1105	44237
1106	44299
1107	44361
1108	44421
1109	44485
1110	44545
1111	44607
1112	44667
1113	44728
1114	44792
1115	44853
1116	44916
1117	44974
1118	45043
1119	45112
1120	45194
1121	45259
1122	45334
1123	45415
1124	45477
1125	45540
1126	45604
1127	45666
1128	45731
1129	45819
1130	45877
1131	45943
1132	46012
1133	46074
1134	46138
1135	46202
1136	46263
1137	46325
1138	46383
1139	46449
1140	46513
1141	46571
1142	46634
1143	46692
1144	46756
1145	46817
1146	46877
1147	46939
1148	46998
1149	47090
1150	47152
1151	47222
1152	47282
1153	47344
1154	47405
1155	47469
1156	47532
1157	47591
1158	47655
1159	47722
1160	47782
1161	47853
1162	47917
1163	47978
1164	48041
1165	48102
1166	48164
1167	48230
1168	48301
1169	48366
1170	48434
1171	48500
1172	48564
1173	48632
1174	48697
1175	48760
1176	48822
1177	48884
1178	48950
1179	49012
1180	49098
1181	49165
1182	49235
1183	49321
1184	49388
1185	49456
1186	49520
1187	49582
1188	49664
1189	49731
1190	49794
1191	49861
1192	49927
1193	49989
1194	50054
1195	50119
1196	50180
1197	50253
1198	50320
1199	50384
1200	50454
1201	50521
1202	50587
1203	50652
1204	50727
1205	50792
1206	50857
1207	50924
1208	50986
1209	51052
1210	51117
1211	51180
1212	51248
1213	51317
1214	51381
1215	51449
1216	51521
1217	51585
1218	51651
1219	51718
1220	51782
1221	51849
1222	51940
1223	52012
1224	52077
1225	52144
1226	52206
1227	52274
1228	52343
1229	52415
1230	52509
1231	52581
1232	52656
1233	52731
1234	52805
1235	52883
1236	52954
1237	53030
1238	53098
1239	53170
1240	53256
1241	53335
1242	53421
1243	53489
1244	53562
1245	53633
1246	53702
1247	53770
1248	53837
1249	53902
1250	53969
1251	54035
1252	54099
1253	54164
1254	54239
1255	54312
1256	54383
1257	54457
1258	54524
1259	54589
1260	54655
1261	54738
1262	54805
1263	54874
1264	54945
1265	55012
1266	55079
1267	55150
1268	55221
1269	55286
1270	55354
1271	55426
1272	55495
1273	55568
1274	55643
1275	55713
1276	55793
1277	55865
1278	55938
1279	56005
1280	56079
1281	56153
1282	56226
1283	56298
1284	56369
1285	56445
1286	56517
1287	56589
1288	56660
1289	56730
1290	56796
1291	56886
1292	56957
1293	57031
1294	57104
1295	57178
1296	57254
1297	57328
1298	57405
1299	57477
1300	57552
1301	57626
1302	57695
1303	57764
1304	57832
1305	57899
1306	57967
1307	58035
1308	58102
1309	58175
1310	58244
1311	58311
1312	58386
1313	58461
1314	58547
1315	58619
1316	58692
1317	58764
1318	58838
1319	58909
1320	58981
1321	59051
1322	59150
1323	59224
1324	59298
1325	59376
1326	59456
1327	59531
1328	59602
1329	59678
1330	59750
1331	59823
1332	59897
1333	59994
1334	60066
1335	60145
1336	60213
1337	60285
1338	60358
1339	60433
1340	60503
1341	60576
1342	60670
1343	60745
1344	60814
1345	60884
1346	60953
1347	61023
1348	61093
1349	61163
1350	61234
1351	61335
1352	61405
1353	61479
1354	61584
1355	61658
1356	61733
1357	61809
1358	61887
1359	61961
1360	62051
1361	62148
1362	62220
1363	62294
1364	62375
1365	62490
1366	62572
1367	62653
1368	62733
1369	62807
1370	62883
1371	62959
1372	63033
1373	63109
1374	63202
1375	63294
1376	63375
1377	63456
1378	63533
1379	63606
1380	63682
1381	63756
1382	63828
1383	63898
1384	63975
1385	64051
1386	64125
1387	64239
1388	64315
1389	64392
1390	64466
1391	64572
1392	64646
1393	64719
1394	64801
1395	64875
1396	64951
1397	65030
1398	65106
1399	65182
1400	65257
1401	65331
1402	65404
1403	65478
1404	65551
1405	65625
1406	65699
1407	65776
1408	65853
1409	65925
1410	66003
1411	66082
1412	66162
1413	66242
1414	66321
1415	66400
1416	66480
1417	66572
1418	66652
1419	66749
1420	66821
1421	66915
1422	66992
1423	67069
1424	67143
1425	67218
1426	67294
1427	67375
1428	67455
1429	67536
1430	67611
1431	67694
1432	67770
1433	67849
1434	67936
1435	68019
1436	68101
1437	68179
1438	68260
1439	68343
1440	68423
1441	68503
1442	68583
1443	68662
1444	68738
1445	68812
1446	68889
1447	68966
1448	69044
1449	69122
1450	69200
1451	69280
1452	69357
1453	69437
1454	69511
1455	69594
1456	69678
1457	69757
1458	69858
1459	69930
1460	70007
1461	70083
1462	70161
1463	70233
1464	70312
1465	70390
1466	70468
1467	70544
1468	70630
1469	70707
1470	70785
1471	70861
1472	70939
1473	71018
1474	71099
1475	71182
1476	71270
1477	71350
1478	71433
1479	71509
1480	71588
1481	71668
1482	71747
1483	71820
1484	71896
1485	71975
1486	72052
1487	72126
1488	72204
1489	72286
1490	72377
1491	72456
1492	72564
1493	72645
1494	72724
1495	72830
1496	72907
1497	72989
1498	73065
1499	73148
1500	73268
1501	73403
1502	73487
1503	73593
1504	73685
1505	73787
1506	73870
1507	73963
1508	74174
1509	74350
1510	74444
1511	74534
1512	74616
1513	74699
1514	74784
1515	74864
1516	74943
1517	75023
1518	75104
1519	75183
1520	75270
1521	75357
1522	75444
1523	75525
1524	75611
1525	75692
1526	75775
1527	75862
1528	75940
1529	76048
1530	76129
1531	76210
1532	76332
1533	76433
1534	76511
1535	76589
1536	76669
1537	76748
1538	76826
1539	76906
1540	76986
1541	77066
1542	77146
1543	77225
1544	77315
1545	77400
1546	77485
1547	77569
1548	77665
1549	77752
1550	77836
1551	77918
1552	78002
1553	78086
1554	78170
1555	78348
1556	78494
1557	78583
1558	78677
1559	78765
1560	78851
1561	78939
1562	79045
1563	79128
1564	79213
1565	79296
1566	79378
1567	79461
1568	79547
1569	79638
1570	79725
1571	79809
1572	79894
1573	79985
1574	80104
1575	80190
1576	80278
1577	80365
1578	80454
1579	80538
1580	80651
1581	80728
1582	80812
1583	80898
1584	80983
1585	81064
1586	81150
1587	81242
1588	81333
1589	81421
1590	81507
1591	81599
1592	81685
1593	81767
1594	81850
1595	81931
1596	82014
1597	82095
1598	82180
1599	82266
1600	82356
1601	82442
1602	82535
1603	82626
1604	82747
1605	82833
1606	82922
1607	83018
1608	83111
1609	83214
1610	83303
1611	83395
1612	83495
1613	83604
1614	83699
1615	83799
1616	83898
1617	83993
1618	84099
1619	84197
1620	84296
1621	84388
1622	84471
1623	84554
1624	84640
1625	84724
1626	84812
1627	84905
1628	85012
1629	85105
1630	85190
1631	85281
1632	85367
1633	85448
1634	85539
1635	85627
1636	85720
1637	85809
1638	85905
1639	85993
1640	86081
1641	86169
1642	86254
1643	86346
1644	86435
1645	86524
1646	86613
1647	86704
1648	86791
1649	86879
1650	86963
1651	87051
1652	87138
1653	87226
1654	87315
1655	87406
1656	87490
1657	87575
1658	87690
1659	87777
1660	87874
1661	87957
1662	88048
1663	88138
1664	88226
1665	88316
1666	88404
1667	88501
1668	88588
1669	88671
1670	88756
1671	88840
1672	88925
1673	89011
1674	89100
1675	89184
1676	89268
1677	89360
1678	89452
1679	89543
1680	89633
1681	89732
1682	89820
1683	89916
1684	90011
1685	90115
1686	90207
1687	90318
1688	90410
1689	90499
1690	90599
1691	90690
1692	90773
1693	90863
1694	90951
1695	91040
1696	91129
1697	91222
1698	91316
1699	91408
1700	91493
1701	91580
1702	91667
1703	91760
1704	91847
1705	91936
1706	92030
1707	92119
1708	92213
1709	92301
1710	92391
1711	92486
1712	92594
1713	92688
1714	92777
1715	92866
1716	92955
1717	93065
1718	93184
1719	93309
1720	93402
1721	93492
1722	93580
1723	93671
1724	93762
1725	93858
1726	93947
1727	94038
1728	94131
1729	94226
1730	94323
1731	94415
1732	94507
1733	94593
1734	94680
1735	94769
1736	94866
1737	94956
1738	95042
1739	95128
1740	95215
1741	95301
1742	95390
1743	95486
1744	95576
1745	95664
1746	95758
1747	95850
1748	95942
1749	96031
1750	96121
1751	96207
1752	96296
1753	96384
1754	96475
1755	96562
1756	96649
1757	96737
1758	96823
1759	96908
1760	97003
1761	97095
1762	97187
1763	97280
1764	97375
1765	97471
1766	97560
1767	97648
1768	97739
1769	97829
1770	97915
1771	98008
1772	98104
1773	98230
1774	98325
1775	98416
1776	98506
1777	98597
1778	98685
1779	98812
1780	98900
1781	98988
1782	99076
1783	99165
1784	99260
1785	99349
1786	99445
1787	99539
1788	99630
1789	99722
1790	99812
1791	99899
1792	99992
1793	100092
1794	100194
1795	100283
1796	100373
1797	100467
1798	100591
1799	100707
1800	100797
1801	100887
1802	100979
1803	101072
1804	101162
1805	101251
1806	101341
1807	101440
1808	101528
1809	101617
1810	101706
1811	101799
1812	101895
1813	101990
1814	102084
1815	102177
1816	102271
1817	102362
1818	102463
1819	102577
1820	102684
1821	102779
1822	102873
1823	102966
1824	103071
1825	103177
1826	103277
1827	103371
1828	103465
1829	103554
1830	103640
1831	103751
1832	103841
1833	103934
1834	104023
1835	104115
1836	104210
1837	104303
1838	104396
1839	104490
1840	104579
1841	104669
1842	104761
1843	104851
1844	104947
1845	105043
1846	105137
1847	105267
1848	105405
1849	105500
1850	105598
1851	105693
1852	105785
1853	105890
1854	105984
1855	106080
1856	106174
1857	106272
1858	106367
1859	106470
1860	106571
1861	106660
1862	106753
1863	106842
1864	106933
1865	107024
1866	107117
1867	107210
1868	107308
1869	107407
1870	107502
1871	107597
1872	107691
1873	107787
1874	107888
1875	107986
1876	108081
1877	108178
1878	108273
1879	108370
1880	108465
1881	108561
1882	108659
1883	108756
1884	108853
1885	108948
1886	109042
1887	109133
1888	109227
1889	109324
1890	109423
1891	109519
1892	109616
1893	109715
1894	109812
1895	109901
1896	109997
1897	110092
1898	110185
1899	110273
1900	110390
1901	110492
1902	110588
1903	110676
1904	110769
1905	110862
1906	110954
1907	111048
1908	111139
1909	111234
1910	111327
1911	111423
1912	111520
1913	111617
1914	111708
1915	111800
1916	111890
1917	111980
1918	112071
1919	112165
1920	112257
1921	112348
1922	112445
1923	112569
1924	112677
1925	112773
1926	112869
1927	112967
1928	113074
1929	113191
1930	113290
1931	113406
1932	113505
1933	113597
1934	113690
1935	113782
1936	113874
1937	113967
1938	114093
1939	114187
1940	114281
1941	114389
1942	114485
1943	114579
1944	114671
1945	114763
1946	114853
1947	114946
1948	115040
1949	115139
1950	115234
1951	115326
1952	115420
1953	115517
1954	115618
1955	115715
1956	115816
1957	115915
1958	116012
1959	116144
1960	116245
1961	116342
1962	116441
1963	116538
1964	116637
1965	116733
1966	116827
1967	116921
1968	117014
1969	117112
1970	117239
1971	117335
1972	117430
1973	117553
1974	117651
1975	117761
1976	117860
1977	117974
1978	118078
1979	118178
1980	118295
1981	118396
1982	118497
1983	118599
1984	118694
1985	118788
1986	118885
1987	118983
1988	119078
1989	119180
1990	119277
1991	119371
1992	119467
1993	119562
1994	119657
1995	119752
1996	119851
1997	119950
1998	120052
1999	120145
2000	120242


==> sub_final/enctrie.tex <==
n	millisec
1	1
2	2
3	2
4	3
5	3
6	3
7	3
8	4
9	4
10	4
11	5
12	5
13	6
14	6
15	7
16	7
17	8
18	9
19	9
20	10
21	10
22	11
23	11
24	12
25	13
26	14
27	15
28	16
29	16
30	17
31	18
32	19
33	20
34	22
35	23
36	24
37	25
38	27
39	28
40	29
41	31
42	33
43	35
44	36
45	38
46	39
47	41
48	43
49	44
50	45
51	46
52	48
53	50
54	52
55	53
56	55
57	57
58	58
59	60
60	62
61	64
62	65
63	68
64	70
65	72
66	74
67	76
68	78
69	82
70	84
71	86
72	88
73	90
74	92
75	94
76	97
77	99
78	101
79	105
80	107
81	110
82	112
83	114
84	116
85	118
86	121
87	124
88	126
89	129
90	131
91	133
92	136
93	139
94	141
95	143
96	146
97	149
98	152
99	155
100	159
101	162
102	165
103	168
104	171
105	175
106	180
107	183
108	187
109	190
110	194
111	197
112	201
113	204
114	208
115	213
116	217
117	220
118	224
119	228
120	232
121	235
122	239
123	243
124	248
125	252
126	256
127	259
128	263
129	269
130	273
131	278
132	283
133	287
134	291
135	295
136	299
137	304
138	308
139	311
140	315
141	321
142	324
143	328
144	332
145	338
146	343
147	346
148	350
149	356
150	360
151	364
152	368
153	373
154	379
155	384
156	389
157	395
158	400
159	404
160	410
161	414
162	419
163	423
164	429
165	433
166	438
167	443
168	447
169	452
170	456
171	462
172	468
173	473
174	480
175	485
176	490
177	495
178	501
179	506
180	511
181	518
182	523
183	528
184	534
185	539
186	544
187	549
188	555
189	560
190	565
191	571
192	578
193	584
194	591
195	596
196	600
197	607
198	612
199	617
200	623
201	630
202	635
203	641
204	646
205	652
206	657
207	664
208	669
209	675
210	683
211	688
212	694
213	699
214	705
215	710
216	716
217	721
218	727
219	732
220	738
221	744
222	750
223	756
224	761
225	766
226	772
227	780
228	786
229	792
230	797
231	803
232	809
233	815
234	820
235	826
236	832
237	838
238	844
239	850
240	856
241	862
242	868
243	874
244	884
245	890
246	896
247	902
248	908
249	914
250	920
251	926
252	932
253	938
254	944
255	950
256	956
257	962
258	968
259	975
260	982
261	989
262	994
263	1000
264	1006
265	1012
266	1018
267	1025
268	1030
269	1038
270	1044
271	1050
272	1058
273	1064
274	1070
275	1077
276	1085
277	1092
278	1098
279	1105
280	1111
281	1117
282	1124
283	1130
284	1136
285	1142
286	1149
287	1155
288	1161
289	1167
290	1175
291	1184
292	1190
293	1196
294	1203
295	1209
296	1215
297	1222
298	1229
299	1236
300	1243
301	1249
302	1256
303	1262
304	1269
305	1278
306	1287
307	1294
308	1300
309	1307
310	1314
311	1321
312	1328
313	1334
314	1341
315	1347
316	1354
317	1361
318	1368
319	1376
320	1386
321	1393
322	1400
323	1407
324	1414
325	1421
326	1428
327	1435
328	1441
329	1448
330	1455
331	1461
332	1468
333	1475
334	1485
335	1492
336	1499
337	1506
338	1513
339	1520
340	1527
341	1534
342	1540
343	1547
344	1554
345	1561
346	1567
347	1576
348	1586
349	1592
350	1599
351	1607
352	1614
353	1621
354	1628
355	1636
356	1642
357	1649
358	1656
359	1664
360	1671
361	1679
362	1688
363	1695
364	1702
365	1709
366	1716
367	1724
368	1731
369	1740
370	1747
371	1755
372	1762
373	1770
374	1778
375	1787
376	1794
377	1802
378	1809
379	1817
380	1824
381	1832
382	1840
383	1848
384	1855
385	1863
386	1871
387	1879
388	1888
389	1896
390	1903
391	1910
392	1919
393	1928
394	1935
395	1943
396	1950
397	1958
398	1966
399	1974
400	1984
401	1991
402	1999
403	2007
404	2015
405	2022
406	2030
407	2038
408	2046
409	2053
410	2061
411	2069
412	2076
413	2087
414	2096
415	2105
416	2114
417	2122
418	2130
419	2138
420	2146
421	2154
422	2163
423	2171
424	2180
425	2192
426	2200
427	2209
428	2217
429	2227
430	2235
431	2245
432	2253
433	2261
434	2270
435	2279
436	2287
437	2297
438	2305
439	2315
440	2323
441	2333
442	2341
443	2349
444	2358
445	2366
446	2374
447	2382
448	2390
449	2398
450	2407
451	2414
452	2423
453	2431
454	2439
455	2447
456	2456
457	2464
458	2472
459	2481
460	2488
461	2498
462	2506
463	2515
464	2525
465	2534
466	2542
467	2552
468	2562
469	2575
470	2583
471	2592
472	2599
473	2608
474	2616
475	2625
476	2633
477	2642
478	2650
479	2660
480	2668
481	2678
482	2687
483	2696
484	2705
485	2714
486	2722
487	2733
488	2743
489	2757
490	2768
491	2777
492	2787
493	2796
494	2806
495	2815
496	2824
497	2839
498	2849
499	2860
500	2870
501	2878
502	2891
503	2899
504	2910
505	2919
506	2929
507	2937
508	2946
509	2954
510	2965
511	2974
512	2985
513	2995
514	3003
515	3013
516	3022
517	3033
518	3041
519	3051
520	3060
521	3069
522	3078
523	3091
524	3099
525	3108
526	3116
527	3125
528	3134
529	3142
530	3150
531	3159
532	3169
533	3177
534	3189
535	3199
536	3208
537	3217
538	3226
539	3234
540	3243
541	3252
542	3261
543	3269
544	3278
545	3290
546	3299
547	3308
548	3317
549	3325
550	3334
551	3343
552	3351
553	3360
554	3369
555	3378
556	3390
557	3400
558	3409
559	3418
560	3428
561	3437
562	3447
563	3456
564	3466
565	3475
566	3488
567	3497
568	3507
569	3517
570	3527
571	3536
572	3545
573	3554
574	3563
575	3573
576	3583
577	3594
578	3604
579	3614
580	3625
581	3635
582	3646
583	3655
584	3665
585	3674
586	3686
587	3697
588	3705
589	3715
590	3724
591	3735
592	3745
593	3761
594	3776
595	3791
596	3807
597	3818
598	3829
599	3840
600	3855
601	3865
602	3875
603	3885
604	3897
605	3906
606	3916
607	3926
608	3935
609	3945
610	3954
611	3964
612	3974
613	3984
614	3995
615	4005
616	4015
617	4025
618	4034
619	4044
620	4053
621	4062
622	4072
623	4082
624	4094
625	4103
626	4112
627	4122
628	4132
629	4142
630	4151
631	4161
632	4171
633	4180
634	4192
635	4202
636	4212
637	4222
638	4231
639	4241
640	4251
641	4260
642	4270
643	4280
644	4291
645	4302
646	4311
647	4321
648	4331
649	4341
650	4351
651	4360
652	4371
653	4380
654	4391
655	4402
656	4412
657	4422
658	4432
659	4442
660	4451
661	4461
662	4470
663	4480
664	4493
665	4504
666	4515
667	4525
668	4537
669	4547
670	4557
671	4568
672	4578
673	4590
674	4602
675	4612
676	4622
677	4632
678	4642
679	4652
680	4662
681	4671
682	4681
683	4694
684	4704
685	4715
686	4725
687	4735
688	4745
689	4754
690	4765
691	4775
692	4786
693	4799
694	4808
695	4818
696	4827
697	4837
698	4847
699	4857
700	4869
701	4879
702	4889
703	4901
704	4912
705	4923
706	4933
707	4945
708	4955
709	4966
710	4976
711	4987
712	4999
713	5009
714	5021
715	5032
716	5042
717	5053
718	5062
719	5074
720	5085
721	5095
722	5108
723	5119
724	5131
725	5141
726	5151
727	5161
728	5173
729	5187
730	5201
731	5212
732	5221
733	5233
734	5242
735	5254
736	5264
737	5274
738	5286
739	5296
740	5309
741	5320
742	5330
743	5342
744	5351
745	5361
746	5372
747	5384
748	5395
749	5406
750	5417
751	5427
752	5438
753	5448
754	5458
755	5467
756	5477
757	5488
758	5499
759	5509
760	5520
761	5530
762	5539
763	5549
764	5559
765	5571
766	5581
767	5591
768	5604
769	5615
770	5625
771	5635
772	5645
773	5655
774	5665
775	5675
776	5686
777	5697
778	5709
779	5721
780	5731
781	5741
782	5752
783	5763
784	5775
785	5786
786	5797
787	5809
788	5820
789	5831
790	5841
791	5851
792	5862
793	5873
794	5884
795	5896
796	5909
797	5920
798	5930
799	5941
800	5951
801	5962
802	5973
803	5984
804	5994
805	6008
806	6019
807	6031
808	6043
809	6054
810	6065
811	6075
812	6088
813	6099
814	6112
815	6125
816	6137
817	6148
818	6161
819	6173
820	6184
821	6196
822	6211
823	6223
824	6235
825	6247
826	6257
827	6270
828	6282
829	6293
830	6307
831	6319
832	6332
833	6343
834	6356
835	6368
836	6379
837	6393
838	6407
839	6418
840	6430
841	6442
842	6454
843	6466
844	6477
845	6488
846	6501
847	6515
848	6526
849	6538
850	6550
851	6561
852	6574
853	6586
854	6597
855	6611
856	6624
857	6636
858	6648
859	6659
860	6670
861	6682
862	6695
863	6708
864	6721
865	6733
866	6744
867	6757
868	6770
869	6784
870	6795
871	6810
872	6823
873	6834
874	6846
875	6857
876	6869
877	6882
878	6894
879	6907
880	6921
881	6934
882	6945
883	6957
884	6969
885	6981
886	6994
887	7008
888	7021
889	7033
890	7044
891	7058
892	7069
893	7082
894	7095
895	7106
896	7122
897	7134
898	7146
899	7158
900	7171
901	7183
902	7194
903	7206
904	7219
905	7231
906	7245
907	7258
908	7270
909	7282
910	7296
911	7310
912	7322
913	7335
914	7349
915	7361
916	7374
917	7386
918	7399
919	7414
920	7425
921	7438
922	7450
923	7462
924	7475
925	7487
926	7499
927	7513
928	7525
929	7537
930	7549
931	7560
932	7573
933	7584
934	7596
935	7609
936	7622
937	7634
938	7646
939	7657
940	7669
941	7682
942	7694
943	7707
944	7720
945	7732
946	7743
947	7755
948	7768
949	7780
950	7792
951	7805
952	7818
953	7830
954	7842
955	7854
956	7865
957	7877
958	7889
959	7901
960	7915
961	7927
962	7939
963	7951
964	7963
965	7975
966	7988
967	8000
968	8015
969	8027
970	8040
971	8053
972	8064
973	8077
974	8090
975	8103
976	8117
977	8131
978	8143
979	8155
980	8167
981	8180
982	8193
983	8206
984	8222
985	8235
986	8248
987	8260
988	8273
989	8286
990	8298
991	8315
992	8327
993	8340
994	8352
995	8365
996	8379
997	8392
998	8405
999	8421
1000	8435
1001	8448
1002	8459
1003	8473
1004	8486
1005	8499
1006	8513
1007	8527
1008	8541
1009	8556
1010	8570
1011	8583
1012	8597
1013	8612
1014	8629
1015	8643
1016	8655
1017	8670
1018	8683
1019	8695
1020	8708
1021	8723
1022	8736
1023	8749
1024	8761
1025	8774
1026	8788
1027	8801
1028	8814
1029	8828
1030	8840
1031	8854
1032	8867
1033	8881
1034	8893
1035	8905
1036	8921
1037	8935
1038	8946
1039	8960
1040	8974
1041	8988
1042	9000
1043	9014
1044	9030
1045	9044
1046	9058
1047	9070
1048	9083
1049	9097
1050	9111
1051	9126
1052	9140
1053	9155
1054	9169
1055	9182
1056	9196
1057	9211
1058	9226
1059	9239
1060	9252
1061	9264
1062	9279
1063	9292
1064	9305
1065	9321
1066	9335
1067	9348
1068	9361
1069	9374
1070	9389
1071	9403
1072	9415
1073	9430
1074	9443
1075	9457
1076	9470
1077	9484
1078	9497
1079	9512
1080	9527
1081	9540
1082	9554
1083	9568
1084	9582
1085	9594
1086	9608
1087	9623
1088	9637
1089	9649
1090	9662
1091	9676
1092	9690
1093	9704
1094	9718
1095	9733
1096	9747
1097	9760
1098	9773
1099	9788
1100	9803
1101	9816
1102	9830
1103	9843
1104	9857
1105	9871
1106	9885
1107	9899
1108	9912
1109	9929
1110	9942
1111	9955
1112	9968
1113	9983
1114	9996
1115	10009
1116	10025
1117	10039
1118	10054
1119	10068
1120	10080
1121	10095
1122	10109
1123	10124
1124	10139
1125	10153
1126	10166
1127	10180
1128	10192
1129	10206
1130	10220
1131	10235
1132	10248
1133	10261
1134	10275
1135	10288
1136	10302
1137	10315
1138	10331
1139	10344
1140	10359
1141	10372
1142	10386
1143	10400
1144	10413
1145	10430
1146	10444
1147	10457
1148	10470
1149	10484
1150	10497
1151	10511
1152	10524
1153	10539
1154	10552
1155	10565
1156	10578
1157	10592
1158	10605
1159	10619
1160	10634
1161	10647
1162	10660
1163	10673
1164	10687
1165	10701
1166	10715
1167	10730
1168	10742
1169	10756
1170	10770
1171	10785
1172	10799
1173	10812
1174	10826
1175	10841
1176	10856
1177	10869
1178	10883
1179	10898
1180	10912
1181	10926
1182	10941
1183	10955
1184	10970
1185	10984
1186	10998
1187	11011
1188	11026
1189	11042
1190	11055
1191	11069
1192	11084
1193	11098
1194	11112
1195	11126
1196	11142
1197	11155
1198	11169
1199	11183
1200	11197
1201	11211
1202	11225
1203	11240
1204	11254
1205	11276
1206	11300
1207	11315
1208	11332
1209	11347
1210	11360
1211	11375
1212	11389
1213	11404
1214	11418
1215	11435
1216	11449
1217	11464
1218	11477
1219	11492
1220	11507
1221	11522
1222	11537
1223	11551
1224	11565
1225	11580
1226	11593
1227	11608
1228	11622
1229	11637
1230	11651
1231	11665
1232	11679
1233	11693
1234	11707
1235	11722
1236	11737
1237	11752
1238	11767
1239	11781
1240	11796
1241	11811
1242	11825
1243	11841
1244	11856
1245	11870
1246	11885
1247	11900
1248	11914
1249	11930
1250	11946
1251	11961
1252	11976
1253	11991
1254	12005
1255	12020
1256	12035
1257	12050
1258	12064
1259	12078
1260	12093
1261	12108
1262	12123
1263	12142
1264	12158
1265	12174
1266	12189
1267	12203
1268	12218
1269	12234
1270	12251
1271	12268
1272	12284
1273	12299
1274	12315
1275	12330
1276	12346
1277	12362
1278	12378
1279	12394
1280	12409
1281	12424
1282	12438
1283	12454
1284	12470
1285	12485
1286	12500
1287	12514
1288	12528
1289	12543
1290	12558
1291	12573
1292	12588
1293	12604
1294	12618
1295	12633
1296	12649
1297	12664
1298	12680
1299	12695
1300	12709
1301	12724
1302	12739
1303	12757
1304	12774
1305	12792
1306	12809
1307	12824
1308	12843
1309	12859
1310	12879
1311	12896
1312	12911
1313	12926
1314	12943
1315	12958
1316	12974
1317	12989
1318	13005
1319	13020
1320	13035
1321	13052
1322	13067
1323	13083
1324	13098
1325	13114
1326	13129
1327	13147
1328	13161
1329	13176
1330	13191
1331	13207
1332	13222
1333	13238
1334	13256
1335	13273
1336	13289
1337	13305
1338	13320
1339	13334
1340	13352
1341	13367
1342	13382
1343	13397
1344	13412
1345	13427
1346	13444
1347	13460
1348	13475
1349	13491
1350	13506
1351	13522
1352	13538
1353	13555
1354	13569
1355	13585
1356	13601
1357	13616
1358	13631
1359	13648
1360	13663
1361	13678
1362	13694
1363	13709
1364	13725
1365	13741
1366	13759
1367	13775
1368	13791
1369	13809
1370	13825
1371	13842
1372	13859
1373	13878
1374	13896
1375	13913
1376	13930
1377	13949
1378	13964
1379	13981
1380	13998
1381	14016
1382	14032
1383	14050
1384	14066
1385	14083
1386	14098
1387	14115
1388	14133
1389	14151
1390	14167
1391	14184
1392	14202
1393	14220
1394	14237
1395	14255
1396	14272
1397	14288
1398	14305
1399	14322
1400	14337
1401	14355
1402	14370
1403	14387
1404	14404
1405	14421
1406	14438
1407	14456
1408	14472
1409	14489
1410	14505
1411	14522
1412	14538
1413	14556
1414	14573
1415	14590
1416	14607
1417	14624
1418	14639
1419	14657
1420	14674
1421	14690
1422	14706
1423	14722
1424	14740
1425	14758
1426	14774
1427	14792
1428	14809
1429	14826
1430	14843
1431	14863
1432	14880
1433	14896
1434	14911
1435	14929
1436	14945
1437	14964
1438	14982
1439	14999
1440	15015
1441	15033
1442	15051
1443	15068
1444	15084
1445	15101
1446	15119
1447	15136
1448	15155
1449	15171
1450	15188
1451	15205
1452	15222
1453	15239
1454	15257
1455	15274
1456	15291
1457	15308
1458	15326
1459	15343
1460	15360
1461	15377
1462	15393
1463	15411
1464	15429
1465	15445
1466	15465
1467	15481
1468	15497
1469	15516
1470	15533
1471	15549
1472	15567
1473	15585
1474	15602
1475	15619
1476	15637
1477	15655
1478	15672
1479	15689
1480	15706
1481	15722
1482	15739
1483	15759
1484	15776
1485	15793
1486	15812
1487	15829
1488	15846
1489	15865
1490	15883
1491	15900
1492	15916
1493	15931
1494	15949
1495	15968
1496	15985
1497	16002
1498	16017
1499	16034
1500	16051
1501	16069
1502	16085
1503	16101
1504	16117
1505	16133
1506	16149
1507	16169
1508	16187
1509	16205
1510	16223
1511	16241
1512	16261
1513	16278
1514	16294
1515	16312
1516	16330
1517	16347
1518	16369
1519	16386
1520	16403
1521	16419
1522	16436
1523	16452
1524	16470
1525	16485
1526	16502
1527	16518
1528	16535
1529	16550
1530	16569
1531	16586
1532	16602
1533	16618
1534	16635
1535	16650
1536	16670
1537	16686
1538	16702
1539	16718
1540	16735
1541	16751
1542	16769
1543	16786
1544	16802
1545	16818
1546	16835
1547	16851
1548	16869
1549	16886
1550	16903
1551	16919
1552	16937
1553	16953
1554	16972
1555	16989
1556	17006
1557	17022
1558	17039
1559	17055
1560	17074
1561	17091
1562	17109
1563	17126
1564	17144
1565	17164
1566	17185
1567	17203
1568	17221
1569	17240
1570	17270
1571	17320
1572	17338
1573	17356
1574	17380
1575	17401
1576	17428
1577	17454
1578	17477
1579	17496
1580	17514
1581	17533
1582	17553
1583	17573
1584	17593
1585	17611
1586	17630
1587	17648
1588	17670
1589	17689
1590	17708
1591	17727
1592	17745
1593	17768
1594	17788
1595	17812
1596	17833
1597	17853
1598	17876
1599	17899
1600	17917
1601	17937
1602	17954
1603	17975
1604	17992
1605	18009
1606	18031
1607	18059
1608	18089
1609	18111
1610	18130
1611	18149
1612	18172
1613	18190
1614	18209
1615	18227
1616	18247
1617	18274
1618	18294
1619	18313
1620	18333
1621	18352
1622	18375
1623	18395
1624	18415
1625	18436
1626	18458
1627	18477
1628	18496
1629	18518
1630	18537
1631	18559
1632	18582
1633	18602
1634	18624
1635	18645
1636	18666
1637	18686
1638	18706
1639	18726
1640	18745
1641	18769
1642	18790
1643	18809
1644	18830
1645	18850
1646	18873
1647	18893
1648	18913
1649	18933
1650	18957
1651	18977
1652	18997
1653	19016
1654	19036
1655	19060
1656	19078
1657	19097
1658	19114
1659	19132
1660	19158
1661	19180
1662	19201
1663	19222
1664	19244
1665	19264
1666	19289
1667	19309
1668	19328
1669	19347
1670	19370
1671	19391
1672	19410
1673	19429
1674	19448
1675	19469
1676	19487
1677	19505
1678	19523
1679	19540
1680	19561
1681	19579
1682	19597
1683	19615
1684	19633
1685	19654
1686	19671
1687	19692
1688	19712
1689	19730
1690	19754
1691	19775
1692	19795
1693	19813
1694	19832
1695	19855
1696	19874
1697	19892
1698	19911
1699	19930
1700	19953
1701	19973
1702	19992
1703	20010
1704	20029
1705	20052
1706	20070
1707	20089
1708	20107
1709	20126
1710	20145
1711	20168
1712	20185
1713	20204
1714	20222
1715	20240
1716	20262
1717	20281
1718	20299
1719	20317
1720	20336
1721	20358
1722	20379
1723	20397
1724	20415
1725	20434
1726	20458
1727	20477
1728	20496
1729	20516
1730	20535
1731	20558
1732	20578
1733	20598
1734	20618
1735	20638
1736	20660
1737	20679
1738	20699
1739	20718
1740	20737
1741	20759
1742	20780
1743	20799
1744	20818
1745	20837
1746	20859
1747	20878
1748	20896
1749	20915
1750	20934
1751	20955
1752	20974
1753	20992
1754	21010
1755	21028
1756	21051
1757	21069
1758	21088
1759	21106
1760	21125
1761	21149
1762	21169
1763	21189
1764	21209
1765	21229
1766	21252
1767	21273
1768	21292
1769	21312
1770	21332
1771	21355
1772	21375
1773	21393
1774	21412
1775	21431
1776	21454
1777	21473
1778	21492
1779	21511
1780	21532
1781	21555
1782	21576
1783	21594
1784	21612
1785	21631
1786	21654
1787	21674
1788	21693
1789	21713
1790	21731
1791	21753
1792	21774
1793	21796
1794	21817
1795	21849
1796	21871
1797	21894
1798	21916
1799	21944
1800	21971
1801	21996
1802	22022
1803	22052
1804	22081
1805	22101
1806	22124
1807	22150
1808	22205
1809	22228
1810	22255
1811	22276
1812	22296
1813	22316
1814	22337
1815	22358
1816	22380
1817	22404
1818	22433
1819	22458
1820	22479
1821	22501
1822	22526
1823	22554
1824	22582
1825	22610
1826	22637
1827	22665
1828	22693
1829	22721
1830	22750
1831	22777
1832	22806
1833	22836
1834	22871
1835	22892
1836	22910
1837	22929
1838	22947
1839	22964
1840	22984
1841	23003
1842	23021
1843	23041
1844	23060
1845	23079
1846	23101
1847	23119
1848	23138
1849	23158
1850	23177
1851	23199
1852	23218
1853	23237
1854	23256
1855	23274
1856	23295
1857	23314
1858	23333
1859	23351
1860	23371
1861	23394
1862	23412
1863	23431
1864	23449
1865	23467
1866	23486
1867	23507
1868	23527
1869	23546
1870	23565
1871	23584
1872	23604
1873	23623
1874	23643
1875	23662
1876	23681
1877	23703
1878	23722
1879	23741
1880	23762
1881	23780
1882	23800
1883	23819
1884	23838
1885	23857
1886	23877
1887	23898
1888	23918
1889	23938
1890	23956
1891	23974
1892	23996
1893	24016
1894	24035
1895	24055
1896	24074
1897	24094
1898	24114
1899	24133
1900	24152
1901	24170
1902	24190
1903	24212
1904	24233
1905	24252
1906	24271
1907	24293
1908	24312
1909	24331
1910	24349
1911	24370
1912	24388
1913	24411
1914	24430
1915	24450
1916	24470
1917	24490
1918	24510
1919	24530
1920	24549
1921	24570
1922	24590
1923	24612
1924	24631
1925	24651
1926	24670
1927	24689
1928	24709
1929	24730
1930	24749
1931	24769
1932	24788
1933	24808
1934	24827
1935	24846
1936	24864
1937	24882
1938	24903
1939	24922
1940	24941
1941	24959
1942	24977
1943	24998
1944	25018
1945	25037
1946	25057
1947	25076
1948	25097
1949	25117
1950	25136
1951	25155
1952	25174
1953	25193
1954	25213
1955	25233
1956	25251
1957	25270
1958	25290
1959	25311
1960	25330
1961	25348
1962	25367
1963	25386
1964	25409
1965	25429
1966	25448
1967	25467
1968	25485
1969	25508
1970	25527
1971	25546
1972	25565
1973	25584
1974	25607
1975	25625
1976	25645
1977	25663
1978	25682
1979	25705
1980	25724
1981	25743
1982	25762
1983	25781
1984	25803
1985	25823
1986	25842
1987	25861
1988	25880
1989	25903
1990	25922
1991	25942
1992	25963
1993	25982
1994	26006
1995	26027
1996	26046
1997	26068
1998	26088
1999	26110
2000	26129


==> sub_final/enctrienaive.tex <==
n	millisec
1	1
2	1
3	2
4	2
5	2
6	3
7	3
8	4
9	4
10	4
11	5
12	6
13	9
14	11
15	13
16	14
17	18
18	21
19	24
20	29
21	31
22	32
23	33
24	35
25	36
26	37
27	39
28	43
29	44
30	46
31	48
32	50
33	52
34	54
35	56
36	58
37	61
38	63
39	65
40	67
41	70
42	73
43	75
44	77
45	80
46	82
47	84
48	87
49	89
50	92
51	96
52	98
53	101
54	104
55	108
56	111
57	114
58	119
59	122
60	126
61	129
62	132
63	136
64	139
65	143
66	146
67	150
68	153
69	157
70	161
71	164
72	168
73	172
74	176
75	180
76	184
77	188
78	193
79	198
80	202
81	206
82	210
83	215
84	221
85	226
86	230
87	235
88	240
89	245
90	250
91	255
92	259
93	264
94	269
95	274
96	279
97	284
98	290
99	296
100	302
101	308
102	313
103	321
104	326
105	332
106	338
107	345
108	351
109	357
110	364
111	370
112	377
113	383
114	390
115	397
116	404
117	411
118	420
119	427
120	434
121	441
122	448
123	455
124	463
125	470
126	477
127	485
128	492
129	499
130	507
131	514
132	523
133	530
134	537
135	545
136	552
137	560
138	567
139	574
140	582
141	589
142	597
143	604
144	612
145	621
146	629
147	637
148	645
149	653
150	661
151	670
152	678
153	686
154	694
155	703
156	711
157	721
158	731
159	739
160	748
161	757
162	765
163	774
164	784
165	793
166	801
167	810
168	820
169	830
170	839
171	849
172	858
173	868
174	877
175	887
176	897
177	906
178	918
179	929
180	938
181	947
182	957
183	965
184	975
185	984
186	994
187	1004
188	1015
189	1027
190	1037
191	1048
192	1059
193	1069
194	1080
195	1090
196	1101
197	1112
198	1124
199	1136
200	1147
201	1159
202	1170
203	1181
204	1193
205	1205
206	1217
207	1232
208	1243
209	1255
210	1266
211	1278
212	1290
213	1301
214	1313
215	1326
216	1337
217	1350
218	1360
219	1372
220	1383
221	1394
222	1407
223	1421
224	1432
225	1442
226	1455
227	1466
228	1477
229	1489
230	1500
231	1513
232	1527
233	1539
234	1551
235	1563
236	1576
237	1588
238	1601
239	1613
240	1626
241	1639
242	1652
243	1665
244	1676
245	1688
246	1700
247	1712
248	1725
249	1737
250	1749
251	1761
252	1774
253	1785
254	1798
255	1810
256	1823
257	1836
258	1848
259	1860
260	1872
261	1885
262	1897
263	1909
264	1923
265	1935
266	1947
267	1959
268	1971
269	1983
270	1995
271	2007
272	2021
273	2033
274	2044
275	2056
276	2067
277	2080
278	2093
279	2105
280	2122
281	2134
282	2147
283	2159
284	2172
285	2185
286	2196
287	2208
288	2222
289	2235
290	2248
291	2260
292	2272
293	2284
294	2297
295	2309
296	2323
297	2337
298	2352
299	2366
300	2379
301	2392
302	2408
303	2422
304	2437
305	2450
306	2464
307	2478
308	2492
309	2505
310	2521
311	2536
312	2550
313	2565
314	2577
315	2591
316	2605
317	2621
318	2634
319	2648
320	2662
321	2674
322	2688
323	2701
324	2714
325	2729
326	2741
327	2754
328	2767
329	2779
330	2793
331	2806
332	2821
333	2834
334	2848
335	2861
336	2874
337	2887
338	2901
339	2915
340	2931
341	2944
342	2957
343	2971
344	2984
345	2998
346	3013
347	3030
348	3044
349	3058
350	3070
351	3085
352	3099
353	3113
354	3128
355	3141
356	3154
357	3168
358	3181
359	3194
360	3208
361	3224
362	3238
363	3252
364	3265
365	3279
366	3294
367	3307
368	3325
369	3339
370	3353
371	3367
372	3381
373	3394
374	3408
375	3425
376	3440
377	3454
378	3468
379	3482
380	3497
381	3511
382	3527
383	3542
384	3557
385	3571
386	3585
387	3600
388	3614
389	3630
390	3645
391	3659
392	3673
393	3687
394	3702
395	3717
396	3732
397	3747
398	3761
399	3776
400	3791
401	3805
402	3822
403	3837
404	3852
405	3867
406	3882
407	3897
408	3911
409	3928
410	3943
411	3959
412	3974
413	3989
414	4005
415	4022
416	4036
417	4051
418	4066
419	4083
420	4099
421	4114
422	4131
423	4146
424	4162
425	4177
426	4193
427	4207
428	4226
429	4241
430	4257
431	4272
432	4286
433	4303
434	4320
435	4335
436	4351
437	4367
438	4382
439	4398
440	4414
441	4431
442	4450
443	4469
444	4485
445	4501
446	4518
447	4534
448	4550
449	4565
450	4582
451	4598
452	4616
453	4634
454	4649
455	4665
456	4680
457	4695
458	4711
459	4730
460	4746
461	4763
462	4779
463	4794
464	4810
465	4830
466	4846
467	4864
468	4879
469	4895
470	4912
471	4929
472	4943
473	4959
474	4975
475	4992
476	5008
477	5026
478	5042
479	5057
480	5074
481	5097
482	5120
483	5137
484	5155
485	5172
486	5189
487	5208
488	5226
489	5244
490	5261
491	5280
492	5299
493	5316
494	5334
495	5352
496	5367
497	5384
498	5402
499	5419
500	5437
501	5457
502	5475
503	5492
504	5511
505	5531
506	5550
507	5567
508	5586
509	5602
510	5618
511	5635
512	5655
513	5679
514	5702
515	5722
516	5743
517	5771
518	5792
519	5809
520	5829
521	5848
522	5866
523	5883
524	5900
525	5921
526	5938
527	5956
528	5972
529	5989
530	6006
531	6025
532	6043
533	6061
534	6079
535	6097
536	6119
537	6137
538	6155
539	6171
540	6189
541	6206
542	6226
543	6243
544	6260
545	6278
546	6296
547	6314
548	6333
549	6350
550	6367
551	6385
552	6402
553	6424
554	6442
555	6461
556	6481
557	6500
558	6520
559	6540
560	6560
561	6579
562	6599
563	6617
564	6638
565	6657
566	6677
567	6696
568	6715
569	6737
570	6757
571	6777
572	6795
573	6813
574	6835
575	6855
576	6874
577	6892
578	6912
579	6934
580	6954
581	6973
582	6994
583	7013
584	7033
585	7051
586	7068
587	7087
588	7105
589	7125
590	7143
591	7161
592	7180
593	7197
594	7216
595	7237
596	7255
597	7276
598	7296
599	7316
600	7337
601	7356
602	7377
603	7396
604	7416
605	7438
606	7458
607	7477
608	7496
609	7517
610	7538
611	7557
612	7576
613	7595
614	7613
615	7635
616	7654
617	7674
618	7693
619	7712
620	7734
621	7753
622	7772
623	7791
624	7810
625	7832
626	7854
627	7873
628	7893
629	7912
630	7933
631	7952
632	7972
633	7991
634	8010
635	8030
636	8049
637	8069
638	8087
639	8106
640	8128
641	8149
642	8168
643	8188
644	8209
645	8232
646	8251
647	8270
648	8289
649	8308
650	8329
651	8348
652	8370
653	8391
654	8412
655	8433
656	8452
657	8471
658	8490
659	8509
660	8529
661	8548
662	8567
663	8586
664	8605
665	8627
666	8645
667	8664
668	8683
669	8702
670	8723
671	8742
672	8762
673	8780
674	8800
675	8822
676	8841
677	8860
678	8879
679	8897
680	8918
681	8938
682	8958
683	8978
684	8997
685	9019
686	9038
687	9058
688	9078
689	9099
690	9120
691	9140
692	9162
693	9182
694	9201
695	9224
696	9243
697	9263
698	9284
699	9302
700	9325
701	9343
702	9362
703	9382
704	9401
705	9423
706	9443
707	9462
708	9481
709	9501
710	9525
711	9546
712	9567
713	9587
714	9607
715	9629
716	9649
717	9669
718	9688
719	9707
720	9729
721	9748
722	9768
723	9787
724	9807
725	9830
726	9849
727	9870
728	9890
729	9913
730	9932
731	9952
732	9971
733	9990
734	10012
735	10031
736	10052
737	10071
738	10090
739	10113
740	10132
741	10153
742	10173
743	10193
744	10215
745	10235
746	10254
747	10274
748	10294
749	10314
750	10334
751	10354
752	10374
753	10393
754	10416
755	10435
756	10456
757	10475
758	10494
759	10514
760	10534
761	10554
762	10574
763	10593
764	10615
765	10636
766	10656
767	10676
768	10696
769	10718
770	10737
771	10758
772	10777
773	10797
774	10821
775	10841
776	10861
777	10881
778	10903
779	10925
780	10945
781	10966
782	10986
783	11009
784	11030
785	11050
786	11071
787	11092
788	11116
789	11137
790	11157
791	11178
792	11198
793	11223
794	11244
795	11266
796	11288
797	11312
798	11333
799	11354
800	11374
801	11395
802	11418
803	11438
804	11460
805	11481
806	11502
807	11524
808	11547
809	11567
810	11588
811	11612
812	11633
813	11655
814	11677
815	11699
816	11722
817	11744
818	11765
819	11787
820	11811
821	11833
822	11854
823	11875
824	11900
825	11921
826	11945
827	11966
828	11987
829	12011
830	12032
831	12053
832	12075
833	12098
834	12120
835	12142
836	12166
837	12190
838	12214
839	12237
840	12259
841	12280
842	12307
843	12329
844	12351
845	12373
846	12396
847	12419
848	12440
849	12462
850	12483
851	12510
852	12531
853	12553
854	12576
855	12601
856	12623
857	12644
858	12665
859	12688
860	12713
861	12735
862	12758
863	12780
864	12805
865	12826
866	12849
867	12871
868	12894
869	12921
870	12942
871	12964
872	12986
873	13010
874	13031
875	13054
876	13076
877	13100
878	13125
879	13148
880	13171
881	13195
882	13221
883	13243
884	13268
885	13292
886	13320
887	13343
888	13366
889	13391
890	13418
891	13441
892	13463
893	13486
894	13512
895	13535
896	13557
897	13580
898	13607
899	13630
900	13652
901	13674
902	13696
903	13720
904	13743
905	13764
906	13787
907	13813
908	13836
909	13858
910	13880
911	13907
912	13932
913	13962
914	13987
915	14018
916	14049
917	14117
918	14154
919	14236
920	14309
921	14349
922	14373
923	14398
924	14425
925	14449
926	14473
927	14498
928	14523
929	14547
930	14570
931	14593
932	14618
933	14640
934	14664
935	14687
936	14714
937	14737
938	14762
939	14787
940	14812
941	14838
942	14861
943	14885
944	14911
945	14934
946	14959
947	14984
948	15013
949	15043
950	15073
951	15102
952	15130
953	15154
954	15180
955	15204
956	15228
957	15252
958	15276
959	15299
960	15324
961	15348
962	15370
963	15393
964	15416
965	15440
966	15465
967	15489
968	15512
969	15537
970	15561
971	15585
972	15608
973	15633
974	15659
975	15690
976	15719
977	15744
978	15772
979	15798
980	15825
981	15849
982	15872
983	15896
984	15922
985	15946
986	15969
987	15993
988	16019
989	16042
990	16068
991	16094
992	16118
993	16144
994	16169
995	16195
996	16224
997	16249
998	16275
999	16299
1000	16328
1001	16354
1002	16380
1003	16406
1004	16434
1005	16457
1006	16481
1007	16508
1008	16535
1009	16562
1010	16588
1011	16618
1012	16643
1013	16668
1014	16693
1015	16721
1016	16747
1017	16777
1018	16804
1019	16833
1020	16857
1021	16884
1022	16910
1023	16936
1024	16962
1025	16987
1026	17015
1027	17039
1028	17065
1029	17090
1030	17117
1031	17142
1032	17165
1033	17190
1034	17213
1035	17240
1036	17264
1037	17290
1038	17316
1039	17341
1040	17363
1041	17388
1042	17413
1043	17439
1044	17462
1045	17487
1046	17513
1047	17537
1048	17563
1049	17587
1050	17617
1051	17643
1052	17667
1053	17693
1054	17721
1055	17746
1056	17771
1057	17796
1058	17822
1059	17845
1060	17870
1061	17894
1062	17923
1063	17950
1064	17976
1065	18001
1066	18028
1067	18055
1068	18082
1069	18108
1070	18135
1071	18160
1072	18187
1073	18211
1074	18239
1075	18263
1076	18299
1077	18342
1078	18384
1079	18425
1080	18475
1081	18522
1082	18558
1083	18584
1084	18611
1085	18638
1086	18663
1087	18690
1088	18717
1089	18743
1090	18768
1091	18795
1092	18822
1093	18846
1094	18871
1095	18894
1096	18921
1097	18945
1098	18969
1099	18993
1100	19036
1101	19070
1102	19126
1103	19161
1104	19200
1105	19235
1106	19300
1107	19347
1108	19392
1109	19445
1110	19513
1111	19560
1112	19619
1113	19665
1114	19711
1115	19749
1116	19794
1117	19841
1118	19897
1119	19945
1120	19999
1121	20032
1122	20057
1123	20081
1124	20107
1125	20134
1126	20159
1127	20185
1128	20210
1129	20238
1130	20264
1131	20290
1132	20317
1133	20343
1134	20368
1135	20393
1136	20419
1137	20445
1138	20471
1139	20497
1140	20524
1141	20550
1142	20576
1143	20601
1144	20629
1145	20655
1146	20681
1147	20707
1148	20735
1149	20763
1150	20789
1151	20816
1152	20842
1153	20869
1154	20894
1155	20922
1156	20947
1157	20973
1158	20998
1159	21036
1160	21069
1161	21123
1162	21173
1163	21234
1164	21290
1165	21338
1166	21391
1167	21444
1168	21491
1169	21546
1170	21594
1171	21642
1172	21692
1173	21728
1174	21780
1175	21819
1176	21871
1177	21913
1178	21952
1179	22000
1180	22032
1181	22060
1182	22088
1183	22116
1184	22143
1185	22169
1186	22196
1187	22224
1188	22251
1189	22278
1190	22305
1191	22334
1192	22362
1193	22388
1194	22417
1195	22450
1196	22477
1197	22507
1198	22535
1199	22563
1200	22592
1201	22620
1202	22647
1203	22674
1204	22701
1205	22730
1206	22758
1207	22786
1208	22815
1209	22843
1210	22870
1211	22898
1212	22929
1213	22956
1214	22984
1215	23019
1216	23045
1217	23071
1218	23098
1219	23126
1220	23154
1221	23181
1222	23208
1223	23235
1224	23263
1225	23290
1226	23320
1227	23349
1228	23376
1229	23403
1230	23432
1231	23459
1232	23487
1233	23516
1234	23544
1235	23571
1236	23599
1237	23630
1238	23660
1239	23689
1240	23723
1241	23751
1242	23778
1243	23806
1244	23835
1245	23862
1246	23891
1247	23920
1248	23948
1249	23976
1250	24008
1251	24035
1252	24063
1253	24091
1254	24120
1255	24147
1256	24176
1257	24205
1258	24237
1259	24266
1260	24295
1261	24324
1262	24353
1263	24380
1264	24409
1265	24436
1266	24463
1267	24490
1268	24520
1269	24548
1270	24576
1271	24605
1272	24636
1273	24665
1274	24693
1275	24726
1276	24754
1277	24785
1278	24817
1279	24845
1280	24872
1281	24901
1282	24931
1283	24960
1284	24990
1285	25022
1286	25058
1287	25086
1288	25117
1289	25149
1290	25184
1291	25217
1292	25245
1293	25276
1294	25305
1295	25337
1296	25366
1297	25394
1298	25422
1299	25451
1300	25478
1301	25508
1302	25541
1303	25571
1304	25600
1305	25636
1306	25672
1307	25703
1308	25741
1309	25772
1310	25802
1311	25841
1312	25868
1313	25897
1314	25926
1315	25955
1316	25983
1317	26015
1318	26046
1319	26074
1320	26102
1321	26134
1322	26161
1323	26190
1324	26221
1325	26250
1326	26280
1327	26308
1328	26341
1329	26372
1330	26405
1331	26437
1332	26468
1333	26498
1334	26529
1335	26558
1336	26589
1337	26624
1338	26655
1339	26684
1340	26714
1341	26754
1342	26783
1343	26812
1344	26846
1345	26875
1346	26903
1347	26934
1348	26963
1349	26992
1350	27022
1351	27052
1352	27082
1353	27111
1354	27141
1355	27171
1356	27200
1357	27231
1358	27259
1359	27290
1360	27319
1361	27351
1362	27380
1363	27408
1364	27439
1365	27469
1366	27498
1367	27531
1368	27561
1369	27592
1370	27622
1371	27653
1372	27685
1373	27717
1374	27749
1375	27778
1376	27808
1377	27842
1378	27872
1379	27904
1380	27941
1381	27971
1382	28003
1383	28036
1384	28069
1385	28102
1386	28135
1387	28167
1388	28199
1389	28234
1390	28265
1391	28297
1392	28331
1393	28361
1394	28394
1395	28427
1396	28459
1397	28490
1398	28520
1399	28554
1400	28586
1401	28617
1402	28651
1403	28683
1404	28715
1405	28750
1406	28783
1407	28817
1408	28850
1409	28881
1410	28914
1411	28949
1412	28981
1413	29014
1414	29047
1415	29078
1416	29109
1417	29142
1418	29171
1419	29201
1420	29233
1421	29266
1422	29297
1423	29327
1424	29359
1425	29390
1426	29422
1427	29455
1428	29485
1429	29516
1430	29549
1431	29579
1432	29609
1433	29642
1434	29673
1435	29703
1436	29737
1437	29768
1438	29799
1439	29828
1440	29860
1441	29891
1442	29921
1443	29955
1444	29986
1445	30020
1446	30055
1447	30088
1448	30121
1449	30154
1450	30187
1451	30217
1452	30251
1453	30285
1454	30317
1455	30351
1456	30384
1457	30417
1458	30453
1459	30487
1460	30520
1461	30555
1462	30587
1463	30621
1464	30655
1465	30687
1466	30718
1467	30752
1468	30782
1469	30814
1470	30849
1471	30880
1472	30909
1473	30944
1474	30976
1475	31008
1476	31038
1477	31072
1478	31103
1479	31135
1480	31169
1481	31201
1482	31233
1483	31268
1484	31300
1485	31332
1486	31368
1487	31401
1488	31435
1489	31468
1490	31502
1491	31536
1492	31572
1493	31606
1494	31639
1495	31673
1496	31707
1497	31742
1498	31775
1499	31809
1500	31841
1501	31877
1502	31911
1503	31945
1504	31981
1505	32015
1506	32047
1507	32083
1508	32115
1509	32152
1510	32186
1511	32219
1512	32256
1513	32289
1514	32322
1515	32357
1516	32391
1517	32422
1518	32458
1519	32492
1520	32525
1521	32561
1522	32593
1523	32626
1524	32659
1525	32694
1526	32731
1527	32767
1528	32798
1529	32830
1530	32864
1531	32897
1532	32930
1533	32962
1534	32994
1535	33024
1536	33056
1537	33088
1538	33118
1539	33150
1540	33186
1541	33220
1542	33253
1543	33289
1544	33323
1545	33360
1546	33395
1547	33428
1548	33465
1549	33500
1550	33533
1551	33568
1552	33603
1553	33637
1554	33673
1555	33707
1556	33742
1557	33778
1558	33810
1559	33845
1560	33878
1561	33909
1562	33940
1563	33974
1564	34008
1565	34040
1566	34074
1567	34106
1568	34141
1569	34176
1570	34210
1571	34245
1572	34282
1573	34313
1574	34346
1575	34383
1576	34416
1577	34449
1578	34485
1579	34518
1580	34551
1581	34585
1582	34618
1583	34650
1584	34685
1585	34719
1586	34753
1587	34790
1588	34824
1589	34863
1590	34897
1591	34932
1592	34971
1593	35026
1594	35083
1595	35132
1596	35165
1597	35198
1598	35233
1599	35267
1600	35300
1601	35332
1602	35365
1603	35402
1604	35440
1605	35474
1606	35510
1607	35545
1608	35579
1609	35613
1610	35649
1611	35683
1612	35726
1613	35759
1614	35799
1615	35837
1616	35878
1617	35912
1618	35946
1619	35985
1620	36018
1621	36053
1622	36088
1623	36124
1624	36158
1625	36196
1626	36230
1627	36263
1628	36299
1629	36332
1630	36367
1631	36400
1632	36433
1633	36469
1634	36503
1635	36537
1636	36572
1637	36604
1638	36637
1639	36673
1640	36708
1641	36743
1642	36778
1643	36811
1644	36848
1645	36882
1646	36916
1647	36947
1648	36983
1649	37018
1650	37054
1651	37090
1652	37126
1653	37162
1654	37199
1655	37235
1656	37271
1657	37310
1658	37355
1659	37401
1660	37436
1661	37472
1662	37507
1663	37541
1664	37579
1665	37610
1666	37644
1667	37679
1668	37714
1669	37751
1670	37788
1671	37823
1672	37859
1673	37896
1674	37930
1675	37963
1676	38002
1677	38048
1678	38085
1679	38119
1680	38153
1681	38187
1682	38221
1683	38254
1684	38289
1685	38322
1686	38358
1687	38394
1688	38430
1689	38467
1690	38501
1691	38536
1692	38573
1693	38610
1694	38645
1695	38681
1696	38716
1697	38750
1698	38787
1699	38823
1700	38858
1701	38894
1702	38928
1703	38961
1704	38998
1705	39032
1706	39067
1707	39105
1708	39139
1709	39173
1710	39208
1711	39243
1712	39275
1713	39311
1714	39344
1715	39379
1716	39413
1717	39449
1718	39494
1719	39528
1720	39562
1721	39598
1722	39637
1723	39674
1724	39716
1725	39757
1726	39806
1727	39848
1728	39891
1729	39934
1730	39972
1731	40010
1732	40044
1733	40079
1734	40119
1735	40156
1736	40194
1737	40229
1738	40268
1739	40307
1740	40350
1741	40387
1742	40427
1743	40462
1744	40498
1745	40536
1746	40573
1747	40612
1748	40655
1749	40703
1750	40751
1751	40800
1752	40838
1753	40875
1754	40912
1755	40948
1756	40985
1757	41024
1758	41061
1759	41100
1760	41135
1761	41173
1762	41212
1763	41249
1764	41286
1765	41323
1766	41361
1767	41399
1768	41435
1769	41470
1770	41504
1771	41538
1772	41573
1773	41608
1774	41644
1775	41682
1776	41719
1777	41757
1778	41794
1779	41834
1780	41870
1781	41908
1782	41946
1783	41984
1784	42020
1785	42057
1786	42093
1787	42132
1788	42169
1789	42208
1790	42247
1791	42284
1792	42322
1793	42359
1794	42394
1795	42431
1796	42469
1797	42506
1798	42544
1799	42580
1800	42619
1801	42656
1802	42694
1803	42733
1804	42774
1805	42811
1806	42847
1807	42882
1808	42917
1809	42953
1810	42988
1811	43027
1812	43062
1813	43097
1814	43138
1815	43173
1816	43208
1817	43244
1818	43280
1819	43316
1820	43352
1821	43385
1822	43422
1823	43459
1824	43494
1825	43531
1826	43565
1827	43599
1828	43636
1829	43672
1830	43711
1831	43749
1832	43783
1833	43822
1834	43860
1835	43897
1836	43937
1837	43974
1838	44014
1839	44050
1840	44085
1841	44124
1842	44160
1843	44195
1844	44231
1845	44267
1846	44305
1847	44341
1848	44376
1849	44414
1850	44453
1851	44489
1852	44531
1853	44568
1854	44608
1855	44644
1856	44680
1857	44720
1858	44757
1859	44791
1860	44828
1861	44865
1862	44903
1863	44938
1864	44975
1865	45019
1866	45057
1867	45093
1868	45135
1869	45174
1870	45212
1871	45249
1872	45285
1873	45327
1874	45364
1875	45400
1876	45436
1877	45472
1878	45509
1879	45555
1880	45592
1881	45633
1882	45669
1883	45706
1884	45742
1885	45777
1886	45815
1887	45850
1888	45886
1889	45923
1890	45956
1891	45991
1892	46028
1893	46063
1894	46097
1895	46135
1896	46167
1897	46200
1898	46236
1899	46271
1900	46306
1901	46341
1902	46377
1903	46416
1904	46452
1905	46488
1906	46527
1907	46563
1908	46600
1909	46636
1910	46686
1911	46727
1912	46764
1913	46801
1914	46843
1915	46880
1916	46919
1917	46958
1918	46996
1919	47036
1920	47072
1921	47109
1922	47149
1923	47186
1924	47224
1925	47260
1926	47296
1927	47334
1928	47370
1929	47404
1930	47442
1931	47479
1932	47515
1933	47552
1934	47588
1935	47625
1936	47660
1937	47696
1938	47733
1939	47769
1940	47804
1941	47841
1942	47877
1943	47913
1944	47952
1945	47988
1946	48026
1947	48062
1948	48099
1949	48138
1950	48175
1951	48211
1952	48251
1953	48290
1954	48331
1955	48369
1956	48407
1957	48446
1958	48483
1959	48519
1960	48554
1961	48589
1962	48628
1963	48666
1964	48705
1965	48744
1966	48780
1967	48816
1968	48855
1969	48890
1970	48929
1971	48967
1972	49004
1973	49041
1974	49078
1975	49113
1976	49151
1977	49187
1978	49224
1979	49261
1980	49296
1981	49336
1982	49373
1983	49409
1984	49450
1985	49488
1986	49527
1987	49564
1988	49602
1989	49645
1990	49689
1991	49735
1992	49775
1993	49813
1994	49857
1995	49911
1996	49949
1997	49986
1998	50024
1999	50065
2000	50101


==> sub_final/introduction.tex <==
%===============================================================================
\section{Introduction}
\label{sec:intro}
%===============================================================================

\emph{Hyperproperties}~\cite{journals/jcs/ClarksonS10} are widely studied in (but not limited to) the context of secure information-flow control. They generalize trace properties in that they not only check the correctness of \emph{individual} computation traces in isolation, but relate \emph{multiple} computation traces to each other.
%Hyperproperties are widely studied in the context of information-flow control.
%Information-flow policies cannot be monitored with standard runtime verification tools
Examples include information-flow policies, such as observational determinism~\cite{journals/jcs/McLean92,conf/sp/Roscoe95,conf/csfw/ZdancewicM03}, (quantitative) noninterference~\cite{journals/jcs/McLean92,conf/fossacs/Smith09,conf/esorics/YasuokaT10} as well as symmetry~\cite{conf/cav/FinkbeinerRS15} and spurious dependencies in hardware designs~\cite{conf/tacas/FinkbeinerHST18}, error correcting codes~\cite{conf/cav/FinkbeinerRS15}, and anti-doping of automotive software~\cite{conf/esop/DArgenioBBFH17}.
%The application of hyperproperties 

In this article, we present the monitoring approach implemented in the latest version of $\tool$, an automata-based monitoring tool for hyperproperties~\cite{journals/fmsd/FinkbeinerH19}.
In dynamic verification of hyperproperties, efficient and light-weight monitoring techniques are instrumented in systems, which are usually far beyond the scope of static verification approaches. By doing so, countermeasures are enacted before, for example, irreparable information leaks happen.
%
A runtime verification tool for hyperproperties is in particular useful if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
$\tool$ also supports the verification workflow by providing a method to test and develop specifications: Specifications can be checked on sample traces without the need for a complete model.
Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning.

%However, standard runtime verification tools~\todo{cite} that only consider computations in isolation, can, in general, not monitor such properties.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The input of $\tool$ is given in the temporal logic $\hyperltl$~\cite{conf/post/ClarksonFKMRS14}, which expresses temporal hyperproperties by extending linear-time temporal logic with \emph{explicit} trace quantification (see~\cite{conf/lics/CoenenFHH19} for a recent study of hyperlogics).
HyperLTL has been used extensively to specify hyperproperties of practical interest (e.g~\cite{conf/cav/FinkbeinerRS15,journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18,conf/cav/FinkbeinerHT18,conf/cav/FinkbeinerHLST18,conf/esop/DArgenioBBFH17}).
For example, observational determinism is expressed as the following formula:
$$
\forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
$$
stating that every trace pair $\pi,\pi'$ has to agree on the output as long as it agrees on the inputs as well.
%$\hyperltl$ has been used to specify a variety of information-flow and security properties~\todo{cite}.
When detecting a violation, $\tool$ outputs a counter example, which is a set of traces that does not satisfy the input formula.
%Examples include classical properties like non-interference and observational determinism, as well as quantitative information-flow properties, symmetries in hardware designs, and formally verified error correcting codes~\cite{conf/cav/FinkbeinerRS15}.

Efficient model checking, synthesis and satisfiability checking tools for HyperLTL already exist~\cite{conf/cav/FinkbeinerRS15,conf/cav/FinkbeinerHT18,conf/concur/FinkbeinerH16,conf/atva/FinkbeinerHH18,conf/cav/FinkbeinerHS17,conf/cav/FinkbeinerHLST18,conf/cav/CoenenFST19}. Implementing an efficient runtime verification tool for HyperLTL specifications is, despite recent theoretical progress~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17,conf/csfw/BonakdarpourF18,conf/isola/BonakdarpourSS18,conf/tacas/HahnST19,journals/fmsd/FinkbeinerH19,DBLP:conf/fm/StuckiSSB19,DBLP:conf/rv/Hahn19} difficult:
%
%This is because monitoring hyperproperties is difficult:
In principle, the monitor not only needs to process every observed trace, but must also \emph{store} every trace observed so far, so that future traces can be compared with the traces seen so far.
%On the other hand, a runtime verification tool for hyperproperties is certainly useful, in particular if the implementation of a security critical system is not available. Even without access to the source code, monitoring the observable execution traces still detects insecure information flow.
%Furthermore, monitoring hyperproperties can be used to simulation plays a significant role in designing specifications and, for example, hardware.

%In this paper, we present $\tool$, a runtime verification tool for monitoring temporal hyperproperties.
The previous version of $\tool$ tackles this challenging problem by implementing two optimizations~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}: a \emph{specification analysis} to detect exploitable properties of a hyperproperty, such as \emph{symmetry} and a \emph{trace analysis}, which detects all redundant traces that can be omitted during the monitoring process. A limitation of the trace analysis, which is based on a language inclusion check, is that only \emph{entire} traces can be analyzed and pruned.
For example, consider the traces $t_1 = \{a\}\{a\}\{\}$ and $t_2 = \{a\}\{\}\{a\}$ of length $3$ and the HyperLTL formula $\forall \pi. \forall \pi'. \G ( a_\pi \rightarrow \neg b_{\pi'} )$. Neither $t_1$ nor $t_2$ is dominated by the other trace, in the sense of the trace analysis, i.e., that one of the traces poses strictly less requirements on future traces~\cite{journals/fmsd/FinkbeinerH19}.
The traces, however, are equal on the first position.
% storage optimization technique that arranges the traces in a tree-like structure.
%This leaves room for optimization, which we address in this article.
This provides an opportunity for optimization, which our new approach exploits.
We introduce a novel trace storage technique (that also has massive impact on the running time), such that $\tool$ can also handle \emph{partially equal} traces by storing them in a tree structure.

We evaluate $\tool$ on existing benchmarks such as classical information-flow security by checking for violations of noninterference or monitoring error-resistant encoder. $\hyperltl$ is, however, not limited to security policies. As an example of such an application beyond security, we show how $\tool$ can be used to detect spurious dependencies in hardware designs.

\paragraph{Structure of this Article.}

The remainder of this article is structured as follows.
We begin by giving preliminaries on $\hyperltl$, its finite trace semantics and notation in Section~\ref{sec:prelims}. In Section~\ref{sec:rvhyper}, we present automata-based monitoring approach implemented in $\tool$, before discussing optimizations in Section~\ref{sec:opt} that make the monitoring feasible in practice. In Section~\ref{sec:eval}, we evaluate $\tool$ with a focus on the novel storage optimization technique using our tree data structure.%: we show $\tool$s performance on a benchmark

This is a revised and extended version of a paper that appeared at TACAS~2018~\cite{conf/tacas/FinkbeinerHST18}.
Our contribution and extension compared to~\cite{conf/tacas/FinkbeinerHST18} is the inclusion of a new trace storage optimization technique presented in Sec.~\ref{sec:trie} and an extended evaluation in Sec.~\ref{sec:eval}.

\paragraph{Related Work.}

The temporal logic $\hyperltl$ was introduced to model check security properties of reactive systems~\cite{conf/post/ClarksonFKMRS14,conf/cav/FinkbeinerRS15}.
For one of its predecessors, $\secltl$~\cite{conf/vmcai/DimitrovaFKRS12}, there has been a proposal for a white-box monitoring approach~\cite{conf/isola/DimitrovaFR12} based on alternating automata.
%The problem of monitoring $\hyperltl$ has been considered before~\cite{conf/csfw/AgrawalB16,conf/tacas/BrettSB17}.
A recent survey on algorithms for monitoring hyperproperties is given in~\cite{DBLP:conf/rv/Hahn19}.
Agrawal and Bonakdarpour~\cite{conf/csfw/AgrawalB16} were the first to study the monitoring problem of HyperLTL for the sequential model. They give a syntactic characterization of monitorable $\hyperltl$ formulas. They present a first monitoring algorithm based on a progression logic expressing trace interdependencies and the composition of an LTL$_3$ monitor.
A first constraint-based approach has been outlined in~\cite{conf/tacas/BrettSB17}, which works for a subclass of HyperLTL specifications. The idea is to identify a set of propositions of interest and store corresponding constraints.
A constraint-based algorithm for the complete fragment of $\forall^2$ HyperLTL formulas has been proposed in~\cite{conf/tacas/HahnST19}. The algorithms rewrites a HyperLTL formula and an incoming event into a constraint composed of a plain LTL requirement as well as a HyperLTL requirement.
An constraint system is built incrementally: the HyperLTL part is encoded with variables, which will be incrementally defined with more incoming events of a trace.
Like with our monitoring algorithm, they do not have access to the implementation (black box), but in contrast to our work, they do not provide witnessing traces as a monitor verdict.

In~\cite{conf/csfw/BonakdarpourF18}, the authors study the complexity of monitoring hyperproperties. They show that the form and size of the input, as well as the formula have a significant impact on the feasibility of the monitoring process. They differentiate between several input forms and study their complexity: a set of linear traces, tree-shaped Kripke structures, and acyclic Kripke structures. For acyclic structures and alternation-free HyperLTL formulas, the problems complexity gets as low as NC.
In~\cite{conf/isola/BonakdarpourSS18,DBLP:conf/fm/StuckiSSB19}, the authors study where static analysis can be combined with runtime verification techniques to monitor HyperLTL formulas beyond the alternation-free fragment.%They discuss the challenges in monitoring formulas beyond this fragment and lay the foundations towards a general method.

For certain information flow policies, like non-interference and some extensions, dynamic enforcement mechanisms have been proposed.
Techniques for the enforcement of information flow policies include tracking dependencies at the hardware level~\cite{conf/asplos/SuhLZD04}, language-based monitors~\cite{journals/jsac/SabelfeldM03,conf/csfw/AskarovS09,conf/pldi/AustinF10,conf/csfw/VanhoefGDPR14,conf/post/BichhawatRGH14}, and abstraction-based dependency tracking~\cite{conf/asian/GuernicBJS06,conf/essos/KovacsS12,conf/csfw/ChudnovKN14}.
Secure multi-execution~\cite{conf/sp/DevrieseP10} is a technique that can enforce non-interference by executing a program multiple times in different security levels.
% and by using special rules for I/O operations.
To enforce non-interference, the inputs are replaced by default values whenever a program tries to read from a higher security level.
%In this article, we are concerned with the monitorability of hyperproperties expressed in $\hyperltl$, which is able to formalize security properties beyond non-interference.

==> sub_final/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> sub_final/mux30both.tex <==
0	995
1	1592
2	2593
3	3529
4	4194
5	6767
10	8701
100	43284
500	33717
1000	21278
1500	17417
2000	16069
3000	14591
5000	14893


==> sub_final/mux30naive.tex <==
0	272634
1	250936
2	252866
3	249152
4	244802
5	264751
10	228081
100	87208
500	24133
1000	16094
1500	13114
2000	12179
3000	11353
5000	12125


==> sub_final/mux30sa.tex <==
0	133530
1	121290
2	127720
3	125107
4	123211
5	126681
10	116338
100	44565
500	11987
1000	7848
1500	6533
2000	6065
3000	5657
5000	5787


==> sub_final/mux30ta.tex <==
0	1560
1	2468
2	4873
3	6519
4	7433
5	10895
10	15576
100	62777
500	46887
1000	29793
1500	24004
2000	22718
3000	20398
5000	20907


==> sub_final/mux30trie.tex <==
0	127
1	162
2	250
3	324
4	390
5	485
10	656
100	851
500	625
1000	647
1500	597
2000	583
3000	649
5000	622


==> sub_final/mux30trienaive.tex <==
0	121
1	191
2	351
3	511
4	638
5	806
10	1195
100	1580
500	1327
1000	1382
1500	1315
2000	1324
3000	1287
5000	1390


==> sub_final/preliminaries.tex <==
%===============================================================================
\section{Preliminaries}
%===============================================================================
\label{sec:prelims}
Let $\mathit{AP}$ be a finite set of \emph{atomic propositions} and let $\Sigma = 2^\mathit{AP}$ be the corresponding \emph{alphabet}.
An infinite \emph{trace} $t \in  \Sigma^\omega$ is an infinite sequence over the alphabet.
A subset $T \subseteq \Sigma^\omega$ is called a \emph{trace property}. A \emph{hyperproperty} $H \subseteq 2^{(\Sigma^\omega)}$ is a generalization of a trace property.
A finite trace $t \in \Sigma^+$ is a finite sequence over $\Sigma$.
In the case of finite traces, $|t|$ denotes the length of a trace.
%Depending on the context, we refer to either $(2^\mathit{AP})^\omega$ or $(2^\mathit{AP})^+$ as the alphabet $\Sigma^\omega$ or $\Sigma^+$.
We use the following notation to access and manipulate traces:
Let $t$ be a trace and $i$ be a natural number.
$t[i]$ denotes the $i$-th element of $t$.
Therefore, $t[0]$ represents the first element of the trace.
Let $j$ be natural number. If $j \geq i$ and $i\leq|t|$, then
$t[i,j]$ denotes the sequence $t[i] t[i+1] \cdots t[min(j,|t|-1)]$. Otherwise it denotes the empty trace $\epsilon$.
$t[i\rangle$ denotes the suffix of $t$ starting at position $i$.
For two finite traces $s$ and $t$, we denote their concatenation by $s \cdot t$.

%\subsection{LTL}
%\paragraph{Syntax.} Linear-time Temporal Logic (LTL)~\cite{} combines the usual Boolean connectives with temporal modalities.
%\begin{alignat*}{3}
%\varphi \coloneqq ~ a ~ | ~ \neg \varphi ~ | ~ \varphi \vee \varphi ~ | ~ \LTLnext \varphi ~ | ~ \varphi \LTLuntil \varphi
%\end{alignat*}
%where $a \in \mathit{AP}$ is an atomic proposition. We use the standard derived operators \emph{eventually} $\LTLdiamond \varphi \equiv \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \equiv \neg \LTLdiamond \neg \varphi$, \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \equiv (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \varphi_1 \LTLweakuntil (\varphi_1 \wedge \varphi_2)$.
%\paragraph{Semantics.} Let $a \in \mathit{AP}$ and $t \in \Sigma^\omega$. The semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\vDash_{LTL} a \quad &&\text{iff } a \in t[0] \\
%t &\vDash_{LTL} \psi_1 \vee \psi_2 \quad &&\text{iff } t \vDash \psi_1 \vee t \models_{LTL} \psi_2\\
%t &\vDash_{LTL} \neg \psi \quad &&\text{iff } t \not \models_{LTL} \psi\\
%t &\models_{LTL} \LTLnext \psi \quad &&\text{iff } t[1\rangle \models_{LTL} \psi\\
%t &\vDash_{LTL} \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; t[i\rangle \models_{LTL} \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \models_{LTL}\psi_1
%\end{alignat*}
%\paragraph{Finite trace Semantics.} Let $a \in \mathit{AP}$ and let $t \in \Sigma^+$ be a finite trace. The finite trace semantics of an LTL is defined by the following satisfaction relation.
%\begin{alignat*}{2}
%t &\modelsltlfin a \quad &&\text{iff } a \in t[0] \\
%t &\modelsltlfin \psi_1 \lor \psi_2 \quad &&\text{iff } t \modelsltlfin \psi_1 \text{ or } t \modelsltlfin \psi_2\\
%t &\modelsltlfin \neg \psi \quad &&\text{iff } t \not \modelsltlfin \psi\\
%t &\modelsltlfin \LTLnext \psi \quad &&\text{iff } |t| > 1 \text{ and } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \LTLweaknext \psi \quad &&\text{iff } |t| = 1 \text{ or } t[1\rangle \modelsltlfin \psi\\
%t &\modelsltlfin \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } t[j\rangle \modelsltlfin \psi_1\\
%t &\modelsltlfin \psi_1 \LTLrelease \psi_2 \quad &&\text{iff } \text{there exists } 0 \leq i < |t|: \; t[i\rangle \modelsltlfin \psi_1\\
%& &&\text{ and for all } 0 \leq j \leq i \text{ we have } t[j\rangle \modelsltlfin \psi_2\\
%& &&\text{ or for all } 0 \leq i < |t| \text{ we have } t[i\rangle \modelsltlfin \psi_2\\
%\end{alignat*}~\todo{finite trace semantics bauen die wir brauchen}


%-------------------------------------------------------------------------------
%\subsection{HyperLTL}
%-------------------------------------------------------------------------------

\paragraph{HyperLTL Syntax.}\label{thltl:syntax}
HyperLTL~\cite{conf/post/ClarksonFKMRS14} extends LTL with trace variables and trace quantifiers.
Let $\mathcal{V}$ be a finite set of trace variables.
The syntax of HyperLTL is given by the grammar
%\begin{figure}[h!]
\begin{alignat*}{3}
  \varphi  &{}\coloneqq ~ \forall \pi . \; \varphi \mid \exists \pi . \; \varphi \mid \psi  \\
  \psi &{}\coloneqq ~ a_{\pi} \mid \psi \wedge \psi \mid \neg \psi \mid \LTLnext \psi  \mid \psi \; \LTLuntil \;  \psi \enspace ,
\end{alignat*}
where $a \in \mathit{AP}$ is an atomic proposition and $\pi \in \mathcal{V}$ is a trace variable.
Atomic propositions are indexed by trace variables. The explicit trace quantification enables us to express properties like ``on all traces $\varphi$ must hold'', expressed by $\forall \pi \ldot \varphi$. Dually, we can express ``there exists a trace such that $\varphi$ holds'', expressed by $\exists \pi \ldot \varphi$.
We use the standard derived operators \emph{release} $\varphi \LTLrelease \psi \coloneqq \neg(\neg \varphi \LTLuntil \neg\psi)$, \emph{eventually} $\LTLdiamond \varphi \coloneqq \mathit{true} \LTLuntil \varphi$, \emph{globally} $\LTLsquare \varphi \coloneqq \neg \LTLdiamond \neg \varphi$, and \emph{weak until} $\varphi_1 \LTLweakuntil \varphi_2 \coloneqq (\varphi_1 \LTLuntil \varphi_2) \vee \LTLsquare \varphi_1$.
As we use the finite trace semantics, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to false.
To enable duality in the finite trace setting, we additionally use the \emph{weak} next operator $\LTLweaknext \varphi$ which evaluates to true if a trace ends before the satisfaction of $\varphi$ can be determined and is defined as $\LTLweaknext \varphi \coloneqq \neg \LTLnext \neg \varphi$.
%$\LTLuntil$ denotes the \emph{until}-operator, $\LTLrelease$ the \emph{release}-operator, and we distinguish between a weak and a strong next operator, where $\LTLweaknext \varphi$ denotes the \emph{weak} version, i.e., if a trace ends before the satisfaction of $\varphi$ can be determined, the satisfaction relation, defined below, evaluates to true. In contrast, $\LTLnext \varphi$ denotes the \emph{strong} version of the next operator.
%$\LTLdiamond$ means that $\varphi$ holds eventually in the future, $\LTLsquare$ means that $\varphi$ holds globally, and $\LTLweakuntil$ is the \emph{weak} version of the \emph{until} operator.
%We call a HyperLTL formula alternation-free, if either all trace variables are universally quantified or all trace variables are existentially quantified.
%, and \emph{release} $\varphi_1 \LTLrelease \varphi_2 \equiv \neg (\neg\varphi_1 \LTLuntil \neg \varphi_2)$.
We call $\psi$ of a HyperLTL formula $\vec{Q}. \psi$, with an arbitrary quantifier prefix $\vec{Q}$, the \emph{body} of the formula. A HyperLTL formula $\vec{Q}. \psi$ is in the \emph{alternation-free fragment} if either $\vec{Q}$ consists solely of universal quantifiers or solely of existential quantifiers.
%We also call the $\forall^n$ fragment and $\exists^n$ fragment, with $n$ being a natural number, as the respective alternation-free fragments.
We also denote the respective alternation-free fragments as the $\forall^n$ fragment and the $\exists^n$ fragment, with $n$ being the number of quantifiers in the prefix.

%\paragraph{Semantics}\label{thltl:sem}
%%Similar to \HLTL{}, \THLTL{} defines the semantics over a set $T$ of traces.
%A HyperLTL formula can express hyperproperties.
%A trace set $T$ satisfies the hyperproperty $H$ if $T \in H$.
%The semantics of HyperLTL is formally defined over a trace assignment, which is a partial mapping $\Pi: \mathcal{V} \to T$ from trace variables to  traces.
%We write $\Pi[\pi \mapsto t]$ for the updated trace assignment, where $\pi \text{ is mapped to } t$.
%$\Pi[i\rangle$ denotes the trace assignment that is equal to $\Pi(\pi)[i\rangle$ for all $\pi \in \dom(\Pi)$.
%We write the trace set $T$ as subscript since the satisfaction depends on the trace mapping.
%%For the sake of decidability, we assume that $x < y$.
%The satisfaction of a HyperLTL formula $\varphi$ over a trace assignment $\Pi$ and a set of traces $T$, denoted by $\Pi \models_T \varphi$, is defined as follows:
%\begin{alignat*}{2}
%\Pi &\vDash_T a_{\pi} \quad &&\text{iff } a \in \Pi(\pi)[0] \\
%\Pi &\vDash_T \psi_1 \wedge \psi_2 \quad &&\text{iff } \Pi \vDash_T \psi_1 \wedge \Pi \vDash_T \psi_2\\
%\Pi &\vDash_T \neg \psi \quad &&\text{iff } \Pi \nvDash_T \psi\\
%\Pi &\vDash_T \forall \pi. \; \psi \quad &&\text{iff } \forall t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\vDash_T \exists \pi. \; \psi \quad &&\text{iff } \exists t \in T: \Pi[\pi \mapsto t] \vDash_T \psi\\
%\Pi &\models_T \LTLnext \psi \quad &&\text{iff } \Pi[1\rangle \models_T \psi\\
%\Pi &\vDash_T \psi_1 \LTLuntil \psi_2 \quad &&\text{iff } \text{there exists } i \geq 0: \; \Pi[i\rangle \models_T \psi_2\\
%& &&\text{ and for all } 0 \leq j < i \text{ we have } \Pi[j\rangle \models_T \psi_1
%\end{alignat*}
%We say a trace set T satisfies a HyperLTL formula $\varphi$ if $\emptyset \models_T \varphi$.
%If unambiguously deducible from the context, we omit $T$ and just write $\models$ instead of $\models_T$.

\paragraph{Finite Trace Semantics.}
We recap the finite trace semantics for HyperLTL~\cite{conf/tacas/BrettSB17}, which is itself based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029}.
% and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%We define a finite trace semantics for $\hyperltl$ based on the finite trace semantics of $\ltl$~\cite{books/daglib/0080029} and the idea that temporal operators can only be satisfied if the finite traces are not yet terminated.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a HyperLTL formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
%Since we are in a finite trace setting, $t[i\rangle$ denotes the subsequence from position $i$ to position $|t|-1$.
Let $\pathassignfin : \pathvars \rightarrow \Sigma^+$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
$\pathassignfin[i\rangle$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i\rangle$ for all $\pi \in \dom(\pathassignfin)$.
By slight abuse of notation, we write $t \in \pathassignfin$ to access traces $t$ in the image of $\pathassignfin$.
%
The satisfaction of a HyperLTL formula $\varphi$ over a finite trace assignment $\pathassignfin$ and a set of finite traces $T$, denoted by $\pathassignfin \models_T \varphi$, is defined as follows:%~\todo{define min t in Pi fin}:
\begin{equation*}
\begin{array}{ll}
    \pathassignfin \models_T a_\pi         \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
    \pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
    \pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
    \pathassignfin \models_T \LTLnext \varphi          & \text{if } \forall t \in \pathassignfin \ldot |t|>1 \text{ and } \pathassignfin[1\rangle \models_T \varphi \\
%    \pathassignfin \models_T \LTLweaknext \varphi      & \text{if } \pathassignfin \models_T \LTLnext \varphi \\
%    & \text{or } \exists t \in \pathassignfin \text{ with } |t| \leq 1 \\
    \pathassignfin \models_T \varphi\LTLuntil\psi      & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \psi \\
    &~\hspace{1ex} \land \forall j < i \ldot \pathassignfin[j\rangle \models_T \varphi \\
%    \pathassignfin \models_T \varphi\LTLrelease\psi    & \text{if } \exists i < \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[i\rangle \models_T \varphi \land \forall j \leq i \ldot \pathassignfin[j\rangle \models_T \psi \\
%   & \text{or } \forall j \leq \min\nolimits_{t \in \pathassignfin} |t| \ldot \pathassignfin[j\rangle \models_T \varphi\\
    \pathassignfin \models_T \exists \pi \ldot \varphi & \text{if } \exists t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi \\
    \pathassignfin \models_T \forall \pi \ldot \varphi & \text{if } \forall t \in T \text{ holds that } \pathassignfin[\pi \mapsto t] \models_T \varphi
\end{array}
\end{equation*}
%\subsection{$\forall^2 \hyperltl$}
%As our constraint based monitoring approach will only be concerned with $\forall^2 \hyperltl$ formulas, we introduce special notation, which will help us down the road.
%\begin{definition}
%
The hyperproperty represented by a $\hyperltl$ formula $\varphi$, denoted by $\hlang(\varphi)$, is the set $\set{ T \subseteq \Sigma^\omega \mid T \models \varphi }$.
%Due to duality of $\LTLuntil$/$\LTLrelease$, $\LTLnext$/$\LTLweaknext$, $\exists$/$\forall$, and the standard Boolean operators, every HyperLTL formula $\varphi$ can be transformed into negation normal form~(NNF), i.e., for every $\varphi$ there is some $\psi$ in negation normal form such that for all $\pathassignfin$ and $T$ it holds that $\pathassignfin \models_T \varphi$ if, and only if, $\pathassignfin \models_T \psi$.
%
%The standard LTL semantic, written $t \modelsltlfin \varphi$, for some LTL formula $\varphi$ is equal to $\set{ \pi \mapsto t }_\mathit{fin} \models_\emptyset \varphi'$, where $\varphi'$ is derived from $\varphi$ by replacing every proposition $p \in \mathit{AP}$ by $p_\pi$.


==> sub_final/runtime-verification.tex <==
%===============================================================================
\section{Runtime Verification of Hyperproperties with $\tool$}
%===============================================================================
\label{sec:rvhyper}
%Since Hyperproperties relate multiple system executions to each other, $\tool$ necessarily processes (and stores) multiple runs of a system.
%For example, previous recorded sessions in a dating app or recorded daily behavior of a smart home.
%Monitoring a system against hyperproperties, such as information-flow policies, is essential if a user suspects that private information might be inferred from notwithstanding behavior of a single system run. For example, \emph{observational determinism} is a general information-flow policy that can be monitored with $\tool$. It states that low-security outputs may not depend on high-security inputs.
In this section, we present an overview over $\tool$, before describing the implementation setup, present the monitoring algorithm, and discuss our optimization techniques.

The input of $\tool$ is given as a universally quantified HyperLTL formula and, in addition, the observed behavior of the system under consideration.
The observed behavior is represented as a trace set $T$, where each $t \in T$ represents a previously observed execution of the system to monitor.
%
$\tool$ can therefore detect violations of every monitorable $k$-safety hyperproperty (see~\cite{journals/fmsd/FinkbeinerH19} for an extensive study of monitorability of hyperproperties).
If $\tool$ detects that the system violates the hyperproperty, it outputs a counter example, i.e, a $k$-ary tuple of traces, where $k$ is the number of quantifiers in the HyperLTL formula.
%that make the monitoring of hyperproperties (despite its theoretical unbounded memory consumption) feasible in practice.
%\subsection{Specification}
%The input specification of $\tool$ is given in $\hyperltl$, which is a temporal logic for specifying hyperproperties.
%It extends $\ltl$ by quantification over trace variables $\pi$ and a method to link atomic propositions to specific traces.
%The set of trace variables is $\pathvars$.
%Formulas in $\hyperltl$ are given by the grammar
%\begin{align*}
%\varphi &{}\Coloneqq \forall\pi\ldot\varphi \mid \exists\pi\ldot\varphi \mid \psi \enspace, \text{ and}\\
%\psi &{}\Coloneqq a_\pi \mid \neg\psi \mid \psi\lor\psi \mid \X\psi \mid \psi\U\psi \enspace,
%\end{align*}
%where $a \in \ap$ and $\pi \in \pathvars$.
%%
%%The formal semantics is given in Appendix~\ref{appendix:hyperltl}.
%The finite trace semantics for $\hyperltl$ is based on the finite trace semantics of LTL.
%In the following, when using $\lang(\varphi)$ we refer to the finite trace semantics of a $\hyperltl$ formula $\varphi$.
%Let $t$ be a finite trace, $\epsilon$ denotes the empty trace, and $|t|$ denotes the length of a trace. Since we are in a finite trace setting, $t[i,\ldots]$ denotes the subsequence from position $i$ to position $|t|-1$.
%Let $\pathassignfin : \pathvars \rightarrow \Sigma^*$ be a partial function mapping trace variables to finite traces. We define $\epsilon[0]$ as the empty set.
%$\pathassignfin[i, \ldots]$ denotes the trace assignment that is equal to $\pathassignfin(\pi)[i,\ldots]$ for all $\pi$. We define a subsequence of $t$ as follows.
%\[
%t[i,j] = \begin{cases}
%\epsilon & \text{if } i \geq |t|\\
%t[i,\textit{min}(j,|t|-1)], & \text{otherwise}
%\end{cases}
%\]
%\begin{equation*}
%\begin{array}{ll}
%\pathassignfin \models_T a_\pi         \qquad \qquad & \text{if } a \in \pathassignfin(\pi)[0] \\
%\pathassignfin \models_T \neg \varphi              & \text{if } \pathassignfin \nmodels_T \varphi \\
%\pathassignfin \models_T \varphi \lor \psi         & \text{if } \pathassignfin \models_T \varphi \text{ or } \pathassignfin \models_T \psi \\
%\pathassignfin \models_T \X \varphi                & \text{if } \pathassignfin[1,\ldots] \models_T \varphi \\
%%F \models_P \tilde{\X} \varphi                & \text{if } F[1,\ldots] \models_P \varphi \\
%\pathassignfin \models_T \varphi\U\psi             & \text{if } \exists i \geq 0 \ldot \pathassignfin[i,\ldots] \models_T \psi \land \forall 0 \leq j < i \ldot \pathassignfin[j,\ldots] \models_T \varphi \\
%\pathassignfin \models_T \exists \pi \ldot \varphi & \text{if there is some } t \in T \text{ such that } \pathassignfin[\pi \mapsto t] \models_T \varphi
%\end{array}
%\end{equation*}
%For example, above mentioned observational determinism can be formalized as the HyperLTL formula
%$\forall \pi \ldot \forall \pi' \ldot (O_\pi = O_{\pi'}) \WUntil (I_\pi \not = I_{\pi'})$, where $\WUntil$ is the weak version of $\Until$.
%
%While earlier work on $\hyperltl$~\cite{conf/cav/FinkbeinerRS15} has focused on model checking, recently runtime verification methods have been proposed as a complementation~\cite{conf/csfw/AgrawalB16,conf/rv/FinkbeinerHST17}.
%$\tool$ also supports the verification workflow by providing a method to test and develop $\hyperltl$ specifications: Specifications can be checked on sample traces without the need for a complete model.
%Based on the feedback of $\tool$, the specification can be refined until it matches the intended meaning~\todo{passt hier nicht?}.

\subsection{Implementation Details}
$\tool$\footnote{The implementation is available at \url{https://react.uni-saarland.de/tools/rvhyper/}.} is written in C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{++}}}.
We use \emph{spot}~\cite{conf/atva/Duret-LutzLFMRX16} for building the deterministic monitor automata and the \emph{Buddy} BDD library for handling symbolic constraints.
We use the $\hyperltl$ satisfiability solver $\eahyper$~\cite{conf/cav/FinkbeinerHS17,conf/concur/FinkbeinerH16} to determine whether the input formula is reflexive, symmetric, or transitive.
Depending on those results, we omit redundant tuples in the monitoring algorithm.

%-------------------------------------------------------------------------------
\subsection{Online Monitoring Algorithm}
%-------------------------------------------------------------------------------

For the online algorithm, we use standard techniques for building LTL monitoring automata and use this to instantiate this monitor by the traces as specified by the $\hyperltl$ formula.
Let $\ap$ be a set of atomic propositions and $\pathvars = \{\pi_1, \ldots, \pi_n\}$ a set of trace variables. 
A deterministic monitor template $\monitor = (\Sigma, Q, \delta, q_0, F)$ is a tuple of
a finite alphabet $\Sigma = 2^{(\ap \times \pathvars)}$,
a non-empty set of states $Q$,
a partial transition function $\delta: Q \times \Sigma \hookrightarrow Q$,
a designated initial state $q_0 \in Q$, and
a set of accepting states $F \subseteq Q$.
The instantiated automaton runs in parallel over traces in $(2^\ap)^*$, thus we define a run with respect to a $n$-ary tuple $N \in ((2^\ap)^*)^n$ of finite traces.
A run of $N$ is a sequence of states $q_0 q_1 \cdots q_m \in Q^*$, where $m$ is the length of the smallest trace in $N$, starting in the initial state $q_0$ such that for all $i$ with $0 \leq i < m$ it holds that 
\begin{equation*}
\delta\left(q_i, \bigcup_{j=1}^n \bigcup_{a \in N(j)(i)} \set{(a,\pi_j)} \right) = q_{i+1} \enspace.
\end{equation*}
A tuple $N$ is accepted if there is a run on $\monitor$ that ends in an accepting state.
For LTL, such a deterministic monitor can be constructed in doubly-exponential time in the size of the formula~\cite{conf/cav/dAmorimR05,journals/fmsd/TabakovRV12}.
%To simplify notation, we identify a path assignment $\pathassign$ over trace variables $\pathvars = \set{\pi_1,\dots,\pi_n}$ by a $n$-ary tuple.

\begin{example}  \label{ex:obsdet-monitor}
  As an example formula, consider again the observational determinism formula introduced in the introduction:
  \begin{equation*}
    \forall \pi. \forall \pi'. (o_\pi = o_{\pi'}) \LTLweakuntil (i_\pi \neq i_{\pi'})\enspace ,
  \end{equation*}
  The corresponding monitor template is depicted in Fig.~\ref{fig:monitor-template}.
\end{example}
\begin{figure}[t]
	\centering
 \begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.9]
 \node[state,initial,initial text=,accepting] (init) {$q_0$};
 \node[state,below left=1.3 and 1.5 of init,accepting] (accepting) {$q_\top$};
 \node[state,black!50,below right=1.3 and 1.5 of init] (rejecting) {$q_\bot$};
 
 \draw (init) edge[loop right] node[swap] {$o_\pi = o_{\pi'} \land i_\pi = i_{\pi'}$} ()
       (init) edge node {$i_\pi \neq i_{\pi'}$} (accepting)
       (init) edge[black!50] node[near end] {$o_\pi \neq o_{\pi'} \land i_\pi = i_{\pi'}$} (rejecting)
       (accepting) edge[loop right] node {$\top$} (accepting)
       (rejecting) edge[loop right,black!50] node {$\top$} (rejecting)
 ;
 \end{tikzpicture}
	\caption{Visualization of a monitor template corresponding to the formula given in Example~\ref{ex:obsdet-monitor}. We use a symbolic representation of the transition function $\delta$. We depict a sink rejecting state $q_\bot$.}
	\label{fig:monitor-template}
\end{figure}

%\paragraph{Online Algorithm.}~\todo{adept arbitarily formulas}
The algorithm for monitoring $\hyperltl$ formulas when traces are given sequentially to the monitor is presented as Algorithm~\ref{alg:algorithms-sequential}.
%The \emph{offline} algorithm takes a $\hyperltl$ formula $\varphi$ and a set of traces $T$ as input.
After building the deterministic monitoring automaton $\monitor_\varphi$, the algorithm accepts new traces and afterwards proceeds with the pace of the incoming stream.
We have a variable $S$ that maps tuples of traces to states of the deterministic monitor.
Whenever the current trace $t$ progresses, we progress every tuple $(t_1,\ldots,t_n)$ that contains $t$ with one of the following outcomes:
\begin{enumerate}
  \item One of the traces $t_1,\ldots,t_n$ may have ended, thus, we check if the monitor is in an accepting state and report a violation if this is not the case.
  \item There is a successor state in the monitor, thus we update $S$.
  \item There is no successor state, hence, we report a violation.
\end{enumerate}
When a new trace $t$ starts, only new tuples are considered for $S$, that are tuples $\vec{t} \in (T \cup \set{t})^n$ containing the new trace $t$.%~\todo{explain notion of instantiation?}
			\begin{algorithm*}[t]
				\SetKwInOut{Input}{input}
				\SetKwInOut{Output}{output}
				\SetAlgoLined
				%\KwResult{Write here the result }
				\Input{$\forall^n$ HyperLTL formula $\varphi$}
				\Output{satisfied or $n$-ary tuple witnessing violation}
				\BlankLine
				$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
				$T \gets \emptyset$\;
				$S: T^n \rightarrow Q$ \quad // initially empty\;
				$t$  \quad // container for the subsequently incoming event traces
				\BlankLine
				\While{there is a new event trace}{
                  $t \gets \epsilon$ \quad // initialize empty trace\;
                  \For(init $S$ for every new tuple $\vec{t}$){$\vec{t} \in ((T \cup \set{t})^n \setminus T^n)$}{
    				$S(\vec{t}) \gets q_0$\;
    			  }
                  \While{$p \in \Sigma$ is a new input event}{
						$t' \gets t~p$ \quad // append $p$ to $t$\;
                        \For(// progress every state in $S$) {$( (t_1,\ldots,t_n), q) \in S$ where $t \in \{t_1,\ldots,t_n\}$}{
                            \uIf(// some trace ended){$\exists t^* \in \{t_1,\ldots,t_n\} \ldot \card{t^*} < \card{t}$}{
                             \eIf {$q \in F$} {
                              remove $(t_1,\ldots,t_n)$ from $S$\;
                              \textbf{continue}\;
                             } { \Return violation and witnessing tuple $(t_1,\ldots,t_n)$\;}
                          }
                          $\vec{t} \gets (t_1,\ldots,t_n)$, where $t_i$ is replaced with $t'$, for each $t_i = t$\;
                          \uIf {$\delta(q, \bigcup_{i=1}^n \bigcup_{a \in \vec{t}(i)[\card{t'}-1]} \set{ (a, \pi_i) }) = q'$} {
        				     $S(\vec{t}) \gets q'$\;
        				  }
        				  \Else{
        				    \Return violation and witnessing tuple $\vec{t}$\;
        				  }
        				}
						$t \gets t'$ \quad // re-assign $t$\;
				  } 
				  $T \gets T \cup \set{t}$\; \quad //add $t$ to already seen traces
				}
				\Return satisfied\;
				\BlankLine
	\caption{Online monitoring algorithm for $\forall^n \hyperltl$: The algorithm subsequently reads event traces and monitors them against already seen traces. Already seen traces are stored in $T$ before continuing with a new event trace.}
	\label{alg:algorithms-sequential}
			\end{algorithm*}

\begin{example} \label{ex:obsdet-algorithm}
  We continue \autoref{ex:obsdet-monitor} by showing how the algorithm progresses on the given formula.
  Assume for the sake of readability that we have a single input proposition $i$ and a single output proposition $o$.
  Furthermore, assume that we have already seen the trace $t_0 = \set{i}\set{i,o}\set{o}$, that is, $T = \set{t_0}$ and $S(t_0,t_0) = q_0$.
  We now show how the algorithm continues with a fresh trace $t_1$.
  In lines 6--8 we add the pairs $(t_0,t_1)$, $(t_0,t_1)$, and $(t_1,t_1)$ with the initial state $q_0$ to $S$.
  Let $p = \set{i}$ be the first input proposition, thus, $t_1 = \set{i}$.
  Since $t_0[0] = t_1[0]$, the monitor remains in $q_0$ for every tuple.
  Let $p = \set{i}$ be the next input proposition, thus, $t_1 = \set{i}\set{i}$.
  Consider the tuple $(t_0,t_1)$.
  As $t_0[1]$ and $t_1[1]$ are equal with respect to $i$ but differ in $o$, the monitor progresses to the rejecting state $q_\bot$ and the algorithm terminates by reporting the violation.
  If, the previous input proposition is $p = \set{}$, both tuples, $(t_0,t_1)$ and $(t_1,t_0)$ would progress to the accepting sink state $q_\top$ as the input proposition is different to $t_0[1]$.
  Assume two more inputs, e.g., $t_1 = \set{i}\set{i}\set{}\set{}$, then the pairs $(t_0,t_0)$, $(t_0,t_1)$, and $(t_1,t_0)$ are removed from $S$ as $t_1$ is strict longer than $t_0$.
\end{example}


\section{Optimizations}
\label{sec:opt}
\vspace{-1ex}
In this section, we present three optimizations implemented in $\tool$, which, as we will see in the evaluation section, are necessary to make the automata-based monitoring approach feasible in practice. We begin by explaining a \emph{specification analysis}, which is a preprocessing step that exploits properties of the specification to reduce the algorithmic workload. In the subsequent section, we show how $\tool$ tackles the problem of potentially unbounded memory consumption: We recap the \emph{trace analysis}, which was so far the only storage optimization implemented in $\tool$. We then provide a novel storage optimization technique based on prefix-trees, so-called \emph{tries}, to exploit partial equality of the given traces.
%, which the trace analysis neglected so far.
\vspace{-1ex}
%-------------------------------------------------------------------------------
\subsection{Specification Analysis}
%-------------------------------------------------------------------------------
\vspace{-1ex}
In the example execution in \autoref{ex:obsdet-algorithm} we have seen that the algorithm had to do more work than necessary to monitor observational determinism.
For example, a tuple $(t,t)$ for some trace $t$ cannot violate observational determinism as the traces are equal.
Further, from the pairs $(t,t')$ and $(t',t)$ for some traces $t$ and $t'$, we only need to check one of them as a violation in one of them implies the violation in the other pair.
We can automatically check for such conditions and, thus, omit unnecessary work.

$\tool$ implements the specification analysis with the HyperLTL satisfiability solver EAHyper~\cite{conf/concur/FinkbeinerH16,conf/cav/FinkbeinerHS17}. The \emph{specification analysis} is a preprocessing step that analyzes the HyperLTL formula under consideration.
EAHyper can detect whether a formula is (1) \emph{symmetric}, i.e., we halve the number of instantiated monitors, (2) \emph{transitive}, i.e, we reduce the number of instantiated monitors to two, or (3) \emph{reflexive}, i.e., we can omit the self comparison of traces.

\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:symmetry}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	%Given a $\hyperltl$ formula $\varphi = \forall \pi_1 \dots \forall \pi_n \ldot \psi$, where $\psi$ is an $\ltl$ formula over trace variables $\{\pi_1, \dots, \pi_n\}$.
	%For an assignment $\pathassign$ and an permutation $\sigma : \Pi \to \Pi$, we define $\pathassign \circ \sigma$, such that $(\pathassign \circ \sigma)(\pi) = \pathassign(\sigma(\pi))$ for every $\pi \in \Pi$.
	We say $\varphi$ is invariant under trace variable permutation $\sigma : \pathvars \to \pathvars$, if for any set of traces $T \subseteq \Sigma^{\omega}$ and any assignment $\pathassign : \pathvars \to T$, $(\emptyset, \pathassign, 0) \models \psi \Leftrightarrow (\emptyset, \pathassign \circ \sigma, 0) \models \psi$.
	We say $\varphi$ is symmetric, if it is invariant under every trace variable permutation in $\pathvars$.
\end{definition}
Symmetry is particularly interesting since many information flow policies satisfy this property. Consider, for example, observational determinism: 
$
\forall \pi\ldot \forall \pi'\ldot (o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'}).
$ %\todo{different notation than in \autoref{ex:obsdet-algorithm} and intro.}
$\tool$ detects symmetry by translating this formula to a formula that is unsatisfiable if there exists no set of traces for which every trace pair violates the symmetry condition:
$
\exists \pi\ldot \exists \pi'\ldot \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big) \nleftrightarrow \big((o_\pi = o_{\pi'}) \W (i_\pi \neq i_{\pi'})\big)
$.
If the resulting formula turns out to be unsatisfiable, $\tool$ omits the symmetric instantiations of the monitor automaton.
%, which turns out to be, especially in combination with $\tool$s \emph{trace analysis}, a major optimization in practice~\cite{conf/rv/FinkbeinerHST17}.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:transitivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\set{\pi_1, \pi_2}$.
	Let $T = \set{t_1, t_2, t_3} \in \Sigma^{\omega}$ be a three-elemented set of traces.
	We define the assignment $\pathassign_{i,j} : \pathvars \to \Sigma^{\omega}$ by $\pathassign_{i,j} \coloneqq \{\pi_1 \mapsto t_i, \pi_2 \mapsto t_j\}$.
	We say $\varphi$ is transitive, if for all three-elemented sets $T$ it holds that $(\emptyset, \pathassign_{1,2}, 0) \models \psi \wedge (\emptyset, \pathassign_{2,3}, 0) \models \psi \rightarrow (\emptyset, \pathassign_{1,3}, 0) \models \psi$.
\end{definition}
While symmetric HyperLTL formulas allow us to prune half of the monitor instances, transitivity of a HyperLTL formula has an even larger impact on the required memory. Equality, i.e, $\forall \pi. \forall \pi' \ldot \G (a_\pi \leftrightarrow a_{\pi'})$, for example, is transitive and symmetric and allows us to reduce the number of monitor instances to one, since we can check equality against any reference trace.
\begin{definition}\cite{journals/fmsd/FinkbeinerH19} \label{def:reflexivity}
	Let $\psi$ be the quantifier-free part of some $\hyperltl$ formula $\varphi$ over trace variables $\pathvars$.
	We say $\varphi$ is reflexive, if for any trace $t \in \Sigma^{\omega}$ and the corresponding assignment $\pathassign : \pathvars \to \{t\}$, $(\emptyset, \pathassign, 0) \models \psi$.
\end{definition}
Lastly, if a formula is reflexive, $\tool$ omits the composition of a trace with itself during the monitoring process.
%Both $\hyperltl$ formulas considered in this section, $\mathit{ObsDet}$ and $\mathit{EQ}$, are reflexive.
For example, equality and observational determinism have reflexive HyperLTL formulas.

\begin{example}
  Consider again the observational determinism formula from \autoref{ex:obsdet-monitor}.
  We have seen that this formula is both, reflexive and symmetric, thus, we can omit those instances in the algorithm.  
\end{example}


%-------------------------------------------------------------------------------
\subsection{Optimizing Trace Storage}
\label{sec:trie}
%-------------------------------------------------------------------------------

The main obstacle in monitoring hyperproperties is the potentially unbounded space consumption.
Previously, RVHyper employed a \emph{trace analysis} technique to detect redundant traces, with respect to a given HyperLTL formula, i.e., traces that can be safely discarded without losing any information and without losing the ability to return a counter example.

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given a HyperLTL formula $\varphi$, a trace set $T$ and an arbitrary $t \in \traces$, we say that $t$ is $(T,\varphi)$-redundant if $T$ is a model of $\varphi$ if and only if $T \cup \set{t}$ is a model of $\varphi$ as well, formally
	\begin{equation*}
	\forall T' \supseteq T \ldot T' \in \hlang(\varphi) \Leftrightarrow T' \cup \{t\} \in \hlang(\varphi) \enspace.
	\end{equation*}
\end{definition}

\begin{definition}~\cite{journals/fmsd/FinkbeinerH19}
	Given $t,t' \in \Sigma^\omega$, we say $t$ \emph{dominates} $t'$ with respect to $\varphi$ (or simply $t$ \emph{dominates} $t'$ if it is clear from the context) if $t'$ is ($\{t\},\varphi$)-redundant.
\end{definition}

\begin{example}
  For observational determinism, a trace $t$ is dominated by a trace $t'$ if $\card{t} < \card{t'}$ and both traces agree on the input propositions.
\end{example}


This is efficiently implemented in $\tool$ (cf. Algorithm~\ref{alg:traceopti}) and is guaranteed to catch all redundant traces.
In our experiments~\cite{journals/fmsd/FinkbeinerH19,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.

The trace analysis, as it is based on a language inclusion check of the entire traces, cannot handle \emph{partial redundancy}, for example, in the case that traces have redundant prefix requirements.
This leaves room for optimization, which we address by implementing a \emph{trie} data structure for managing the storage of incoming traces.

\begin{algorithm}
	%\label{alg_minimization}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\SetAlgoLined
	%\KwResult{Write here the result }
	\Input{$\hyperltl$ formula $\varphi$, redundancy free trace set $T$, fresh trace $t$}
	\Output{redundancy free set of traces $T_\mathit{min} \subseteq T \cup \set{t}$}
	%\BlankLine
	$\monitor_\varphi =$ \texttt{build\_template($\varphi$)}
	\BlankLine
	\ForEach{$t' \in T$}{
		\If{ $t'$ dominates $t$ }
		{
			\Return $T$\;
		}
	}
	\ForEach{$t' \in T$}{
		\If{$t$ dominates $t'$}
		{
			$T \coloneqq T \setminus \set{t'}$\;
		}
	}
	\Return $T \cup \set{t}$\;
	%\BlankLine
	\caption{Trace analysis algorithm to minimize trace storage.}
	\label{alg:traceopti}
\end{algorithm}



%In our experiments~\cite{conf/rv/FinkbeinerHST17,conf/tacas/FinkbeinerHST18}, we made the observation that traces often share the same prefixes, leading to a lot of redundant monitor automaton instantiations, repetitive computations and duplicated information when those traces get stored.
%Ideally one wants to avoid this overhead when monitoring a trace that shares some prefixes with already seen traces.
%We implemented this idea with a so-called \emph{trie} data structure.
Tries, also known as prefix trees are a tree data structure, which can represent a set of words over an alphabet in a compact manner.
The root of a trie is identified with the empty word $\epsilon$, additionally each node can have several child nodes, each of which corresponds to a unique letter getting appended to the representing word of the parent node. So the set of words of a trie is identified with the set of words the leaf nodes represent.

\begin{definition}
A trie is a four tuple $(\Sigma, \Tau, \longrightarrow, \tau_0)$ consisting of
\begin{itemize}
    \item a finite alphabet $\Sigma$,
    \item a non-empty set of states $\Tau$,
    \item a transition function $\longrightarrow: \Tau \times \Sigma \rightarrow \Tau$,
    \item and a designated initial state $\tau_0 \in \Tau$ called the root.
    \end{itemize}
\end{definition}
Instead of $((\tau,a),\tau') \in \longrightarrow$ we will write $\tau \overset{a}{\longrightarrow} \tau'$ in the following.
For a trie to be of valid form we restrict $\longrightarrow$ such that, $\forall \tau,\tau' \in \Tau. |\{\tau \overset{a}{\longrightarrow} \tau'| a \in \Sigma\}| \leq 1$.

%Additionally to our analysis phases it would be helpful if we could use some insights from trace analysis 


%As mentioned before, storing the incoming traces succinctly is a major concern in monitoring hyperproperties.
In our case the alphabet would be the set of propositions used in the specification, and the word built by the trie represents the traces. %build from it are what we call traces.
%Tries provide a 
Instead of storing each trace individually, we store all of them in one trie structure, branching only in case of deviation. This means equal prefixes only have to be stored once.
Besides the obvious benefits for memory, we also can make use of the maintained trie data structure to improve the runtime of our monitoring algorithms. As traces with same prefixes end up corresponding to the same path in the trie, we only have to instantiate the monitor automaton as much as the trie contains branches.
%O(size branches) times.
\begin{example}
	Consider the following traces of length $6$ over the alphabet $2^{\{i,o\}}$:
	\begin{itemize}
		\item
		$t_1: \{\set{i},\set{i,o},\set{i},\set{i},\set{i},\set{i,o} \}$
		\item
		$t_2: \{\set{i}, \set{i,o}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_3: \{\set{i}, \set{i}, \set{i}, \set{i} , \set{i}, \set{i}\}$
		\item
		$t_4: \{\set{i}, \set{i}, \set{}, \set{} , \set{}, \set{}\}$
	\end{itemize}
After processing the traces sequentially, the resulting trie looks as follows:

\vspace{1ex}

\begin{tikzpicture}[sibling distance=7em, level distance = 30pt,
every node/.style = {shape=circle,
	draw, align=center, minimum size = 0.9cm, inner sep = 0pt},
level 1/.style = {sibling distance = 10em},
level 2/.style = {sibling distance = 5em},
level 5/.style = {sibling distance = 5em}]
\node {$\{i\}$}
child { node {$\{i\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} } } } } 
	child { node {$\{ \}$}  
		child { node {$\{ \}$} 
			child { node {$\{ \}$}
				child { node {$\{ \}$} } } } } }
child { node {$\{i,o\}$}
	child { node {$\{i\}$}
		child { node {$\{i\}$}
			child { node {$\{i\}$}
				child { node {$\{i\}$} }
				child { node {$\{i,o\}$} } } } } };
\end{tikzpicture}
\end{example}

\subsection{Trie-based Monitoring Algorithm}

We depict a trie-based offline monitoring algorithm in Fig.~\ref{alg:trie-offline}.
For the sake of readability, we assume that there are as many traces as universal quantifiers, that we progress through all traces in parallel, and that all traces have the same length.
This is merely a simplification in the presentation, one can build the trie in a sequential fashion for online monitoring by a slight modification of the presented algorithm.

Without using tries, our monitoring algorithm was based on instantiating the deterministic monitor template $\monitor_\varphi$ with tuples of traces. Now we instantiate $\monitor_\varphi$ with tuples of tries. Initially we only have to create the single instance having the the root of our trie.

\begin{comment}
	\begin{algorithm*}
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\;
		$S: \Tau^n \rightarrow Q$, \quad $E: \Tau^n \rightarrow \Sigma$\;
		$\tau_0 \coloneqq $\texttt{ new\_trie()}\;
		%$\mathbf{i} \coloneqq \underbrace{(\tau_0,\ldots,\tau_0)}{n \text{times}}$\;
		%$I \coloneqq \{\mathbf{i}\}$\;
		\BlankLine
		$i_0 \in \{ \tau_0 \}^n$\;
		$S(i_0) = q_0$\;
		\While{there is a new trace}{
			$I \leftarrow \{i_0\}$\;
			$\tau \leftarrow \tau_0$\;
			\While{$p \in \Sigma$ is a new event}{
				$\tau' \leftarrow$ \texttt{add\_child($\tau,p$)} //\texttt{assert($E(\tau')==p$)}\;
				$I_n \leftarrow \emptyset$\;
				\ForEach{$i \in I$}{
					$I' \leftarrow \{i' \mid i(j) \rightarrow i'(j), a \in \Sigma, 1 \leq j \leq n\}$\;
					$I' \leftarrow \{i' \in I' \mid \exists k. i'(k) = \tau'\}$\;
					\ForEach{$i' \in I'$}{
						\uIf{$\delta(S(i), \cup_{j=1}^n \cup_{a\in E(i'(j))} \{(a,\pi_j)\}) = q$}{
							$S(i') = q$\;
						}
						\Else{
							\Return(\texttt{rooted\_seq($i'(1)$)}, \ldots, \texttt{rooted\_seq($i'(n)$)})\;
						}
					}
				}
			}
		}
		%\While{$\mathbf{p} \leftarrow$ new elements (in a forward fashion)}{
		%	\For{$1 \leq j \leq n$}{
		%		$\mathbf{i}(j) \leftarrow $\texttt{add\_value($\mathbf{i}(j)$, $j$, $\mathbf{p}(j)$)}\;
		%	}
		%	$I \leftarrow \bigcup_{\mathbf{i} \in I} \{(i'_1,\ldots, i'_n)| \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n\}$\;
		%	\ForEach{$\mathbf{i} \in I$}{
		%		%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
		%		progress every state in $S$ according to $\delta$\;
		%		\If{violation in $M_\varphi$}{
		%			$t \coloneqq ($\texttt{rooted\_sequence($i(1)$)}$,\ldots,$\texttt{rooted\_sequence($i(n)$)}$)$\;
		%			\Return witnessing tuple $t^n$\;
		%		}
		%	}
		%}
		%\Return satisfied\;
		%\BlankLine
	\caption{Online algorithm using trie data structure.}
	\label{alg:trie-online-parallel}
	\end{algorithm*}
\end{comment}
	\begin{algorithm*}[t]
		\SetKwInOut{Input}{input}
		\SetKwInOut{Output}{output}
		\SetAlgoLined
		%\KwResult{Write here the result }
		\Input{$\forall^n$ HyperLTL formula $\varphi$}
		\Output{satisfied or $n$-ary tuple witnessing violation}
		\BlankLine
		$\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F) =$ \texttt{build\_template($\varphi$)}\\
		$S: \Tau^n \rightarrow Q$\\
		$\tau_0 \coloneqq $\texttt{new\_trie()}\\
		$\mathbf{i} \coloneqq (\tau_0,\ldots,\tau_0) \in \Tau^n$\\
		$I \coloneqq \{\mathbf{i}\}$  \quad // set of not-yet terminated branches\\
		\BlankLine
		\While{$\mathbf{p} \leftarrow$ new event (in $\Sigma^n$)}{
			\For{$1 \leq j \leq n$}{
				$\mathbf{i}(j) \leftarrow $\texttt{add\_child($\mathbf{i}(j)$, $\mathbf{p}(j)$)} \quad // add child with value $\vec{p}(j)$ to $\vec{i}(j)$ if needed \\
			}
			// update set of active branches\\
			$I \leftarrow \bigcup_{\mathbf{i} \in I} \set{ (i'_1,\ldots, i'_n) \mid \mathbf{i}(j) \overset{a}{\longrightarrow} i'_j, a \in \Sigma, 1 \leq j \leq n }$\\
			\ForEach{$\mathbf{i} \in I$}{
				%$t \coloneqq (\nu(\mathbf{i}(1)),\ldots,\nu(\mathbf{i}(n)))$\;
				progress every state in $S$ according to $\delta$\;
				\If{violation in $\monitor_\varphi$}{
				    // return sequence from root to $\vec{i}$\\
					$t \gets ($\texttt{rooted\_sequence($\vec{i}(1)$)}$,\ldots,$\texttt{rooted\_sequence($\vec{i}(n)$)}$)$\\
					\Return witnessing tuple $t^n$\\
				}
			}
		}
		\Return satisfied if $\forall \vec{i} \in I \ldots S(\vec{i}) \in F$ else violation\\
		\BlankLine
	\caption{Offline algorithm using trie data structure.}
	\label{alg:trie-offline}
\end{algorithm*}

The trie-based algorithm has much in common with its previously discussed trace-based counterpart. Initially, we have to build the deterministic monitor automaton $\monitor_\varphi = (\Sigma_\pathvars, Q, q_0, \delta, F)$.
We instantiate the monitor with a fresh trie root $\tau_0$.
A mapping from trie instantiations to a state in $\monitor_\varphi$ $S: \Tau^n \rightarrow Q$, stores the current state of every active branch of the trie, stored in the set $I$.
For each of the incoming traces, we provide an entry in a tuple of tries $\mathbf{\tau}$, each entry gets initialized to $\tau_0$.
During the run of our algorithm these entries are updated such that they always correspond to the word built by the traces up to this point.
For as long as there are traces left, which have not yet ended, and we have not yet detected a violation, we will proceed updating the entries in $\vec{i}$ as follows.
Having entry $\tau$ and the correspond trace sequence proceeds with $a$, if $\exists \tau' \in \Tau. \tau \overset{a}{\longrightarrow} \tau'$, we update the entry to $\tau'$ otherwise we create such a child node of $\tau$ (\texttt{add\_child} in line 8).
Creating a new node in the trie always occurs when the prefix of the incoming trace starts to differ from already seen prefixes.
After having moved one step in our traces sequences, we have to reflect this step in our trie structure, in order for the trie-instantiated automata to correctly monitor the new propositions.
As a trie node can branch to multiple child nodes, each monitor instantiation are replaced by the set of instantiations, where all possible child combinations of the different assigned tries are existent (update of $I$ in line 11).
Afterwards, we update $S$ in the same way as in Algorithm~\ref{alg:traceopti}, thus, we omit algorithmic details here.
%This can be efficiently implemented as we essential fork the monitor instantiation for the different branches in the trie.
%After this preprocessing we are able to update our mapping $S$ according to $\delta$.
If a violation is detected here, that is there is no transition in the monitor corresponding to $\vec{i}$, we will return the corresponding counter example as a tuple of traces, as those can get reconstructed by stepping upwards in the tries of $\vec{i}$.
%Note that the sequential algorithm is derived from the parallel one by progressing one trace at a time and additionally when forking the monitor instantiations, only those new instantiation have to be kept, which contain the (single) trie in $\mathbf{\tau}$ at least once. 
If the traces end, we check if every open branch $\vec{i} \in I$ is in an accepting state.

%\subsection{Tries and Trace Analysis in Combination}
%\todo{TODO}


==> sub_final/tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> sub_final/tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}

==> tikz/monitor_conference_example.tex <==
\begin{tikzpicture}[auto,->,>=stealth',shorten >=1pt,thick,transform shape, scale=0.8]
  \node[state,initial,initial text=] (init) {$q_0$};
  \node[state,below=of init,accepting] (accept) {$q_2$};
  \node[state,below left=1 and 2 of init] (wait-for-submit) {$q_1$};
  \node[state,below right=1 and 2 of init,accepting] (pc-equal) {$q_3$};
  \node[state,left=of wait-for-submit,accepting] (submitted) {$q_4$};
  
  \draw (init) edge node[swap] {$\neg pc_\pi \land pc_{\pi'}$} (wait-for-submit)
        (wait-for-submit) edge[loop right] node {$\neg s_\pi$} ()
        (wait-for-submit) edge[bend left] node {$s_\pi$} (submitted)
        (submitted) edge[bend left] node {$v_{\pi'} \land \neg s_\pi$} (wait-for-submit)
        (submitted) edge[loop left] node {$v_{\pi'} \land s_\pi$} ()
        (init) edge node {$\neg pc_{\pi'}$} (accept)
        (accept) edge[loop right] node {$\top$} ()
        (init) edge node {$pc_\pi \land pc_{\pi'}$} (pc-equal)
        (pc-equal) edge[loop right] node {$v_\pi \leftrightarrow v_{\pi'}$} ()
        ;
\end{tikzpicture}

==> tikz/mux.tex <==
\begin{tikzpicture}[auto,>=stealth',shorten >=1pt,thick,transform shape, scale=1]
  
  % cirucit
  \node[draw,minimum size=20pt] (mux) {\textsc{mux}};
  \node[draw,fill,below=0.5 and -0.3 of mux,minimum size=20pt] (bb) {};
  \node[draw,below=0.5 and -0.3 of bb,minimum size=20pt] (imux) {\textsc{imux}};
  
  % inputs
  \node[above left=0.5 and 0 of mux] (i) {$i$};
  \node[above right=0.5 and 0 of mux] (iPrime) {$i'$};
  \node[left=0.5 of i] (sel) {$\mathit{sel}$};
  
  % outputs
  \node[below left=0.5 and -0.1 of imux] (o) {$o$};
  \node[below right=0.5 and -0.1 of imux] (oPrime) {$o'$};  
  
  % lines
  \coordinate[xshift=-5pt] (muxi1) at (mux.north);
  \coordinate[xshift=5pt] (muxi2) at (mux.north);
  
  \coordinate[xshift=-5pt] (imuxo1) at (imux.south);
  \coordinate[xshift=5pt] (imuxo2) at (imux.south);
  
  \draw (i) -| (muxi1)
        (iPrime) -| (muxi2)
        (sel) |- (mux)
        (mux) -- (bb)
        (bb) -- (imux)
        (sel) |- (imux)
        (imuxo1) |- (o)
        (imuxo2) |- (oPrime)
        ;
  
  
\end{tikzpicture}
